Unified Theory of Characteristic Modes: Part II -- Tracking, Losses, and FEM Evaluation

This is the second component of a two-part paper dealing with a unification of characteristic mode decomposition. This second part addresses modal tracking and losses and presents several numerical examples for both surface- and volume-based method-of-moment formulations. A new tracking algorithm based on algebraic properties of the transition matrix is developed, achieving excellent precision and requiring a very low number of frequency samples as compared to procedures previously reported in the literature. The transition matrix is further utilized to show that characteristic mode decomposition of lossy objects fails to deliver orthogonal far fields and to demonstrate how characteristic modes can be evaluated using the finite element method.

==> pgflibrarypgfplots.colorbrewer.code.tex <==
\usetikzlibrary{colorbrewer}
\pgfplotscreateplotcyclelist{YlGn-3}{%
  YlGn-3-1\\%
  YlGn-3-2\\%
  YlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGn-4}{%
  YlGn-4-1\\%
  YlGn-4-2\\%
  YlGn-4-3\\%
  YlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGn-5}{%
  YlGn-5-1\\%
  YlGn-5-2\\%
  YlGn-5-3\\%
  YlGn-5-4\\%
  YlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGn-6}{%
  YlGn-6-1\\%
  YlGn-6-2\\%
  YlGn-6-3\\%
  YlGn-6-4\\%
  YlGn-6-5\\%
  YlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGn-7}{%
  YlGn-7-1\\%
  YlGn-7-2\\%
  YlGn-7-3\\%
  YlGn-7-4\\%
  YlGn-7-5\\%
  YlGn-7-6\\%
  YlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGn-8}{%
  YlGn-8-1\\%
  YlGn-8-2\\%
  YlGn-8-3\\%
  YlGn-8-4\\%
  YlGn-8-5\\%
  YlGn-8-6\\%
  YlGn-8-7\\%
  YlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGn-9}{%
  YlGn-9-1\\%
  YlGn-9-2\\%
  YlGn-9-3\\%
  YlGn-9-4\\%
  YlGn-9-5\\%
  YlGn-9-6\\%
  YlGn-9-7\\%
  YlGn-9-8\\%
  YlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-3}{%
  YlGnBu-3-1\\%
  YlGnBu-3-2\\%
  YlGnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-4}{%
  YlGnBu-4-1\\%
  YlGnBu-4-2\\%
  YlGnBu-4-3\\%
  YlGnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-5}{%
  YlGnBu-5-1\\%
  YlGnBu-5-2\\%
  YlGnBu-5-3\\%
  YlGnBu-5-4\\%
  YlGnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-6}{%
  YlGnBu-6-1\\%
  YlGnBu-6-2\\%
  YlGnBu-6-3\\%
  YlGnBu-6-4\\%
  YlGnBu-6-5\\%
  YlGnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-7}{%
  YlGnBu-7-1\\%
  YlGnBu-7-2\\%
  YlGnBu-7-3\\%
  YlGnBu-7-4\\%
  YlGnBu-7-5\\%
  YlGnBu-7-6\\%
  YlGnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-8}{%
  YlGnBu-8-1\\%
  YlGnBu-8-2\\%
  YlGnBu-8-3\\%
  YlGnBu-8-4\\%
  YlGnBu-8-5\\%
  YlGnBu-8-6\\%
  YlGnBu-8-7\\%
  YlGnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-9}{%
  YlGnBu-9-1\\%
  YlGnBu-9-2\\%
  YlGnBu-9-3\\%
  YlGnBu-9-4\\%
  YlGnBu-9-5\\%
  YlGnBu-9-6\\%
  YlGnBu-9-7\\%
  YlGnBu-9-8\\%
  YlGnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{GnBu-3}{%
  GnBu-3-1\\%
  GnBu-3-2\\%
  GnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{GnBu-4}{%
  GnBu-4-1\\%
  GnBu-4-2\\%
  GnBu-4-3\\%
  GnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{GnBu-5}{%
  GnBu-5-1\\%
  GnBu-5-2\\%
  GnBu-5-3\\%
  GnBu-5-4\\%
  GnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{GnBu-6}{%
  GnBu-6-1\\%
  GnBu-6-2\\%
  GnBu-6-3\\%
  GnBu-6-4\\%
  GnBu-6-5\\%
  GnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{GnBu-7}{%
  GnBu-7-1\\%
  GnBu-7-2\\%
  GnBu-7-3\\%
  GnBu-7-4\\%
  GnBu-7-5\\%
  GnBu-7-6\\%
  GnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{GnBu-8}{%
  GnBu-8-1\\%
  GnBu-8-2\\%
  GnBu-8-3\\%
  GnBu-8-4\\%
  GnBu-8-5\\%
  GnBu-8-6\\%
  GnBu-8-7\\%
  GnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{GnBu-9}{%
  GnBu-9-1\\%
  GnBu-9-2\\%
  GnBu-9-3\\%
  GnBu-9-4\\%
  GnBu-9-5\\%
  GnBu-9-6\\%
  GnBu-9-7\\%
  GnBu-9-8\\%
  GnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuGn-3}{%
  BuGn-3-1\\%
  BuGn-3-2\\%
  BuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{BuGn-4}{%
  BuGn-4-1\\%
  BuGn-4-2\\%
  BuGn-4-3\\%
  BuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{BuGn-5}{%
  BuGn-5-1\\%
  BuGn-5-2\\%
  BuGn-5-3\\%
  BuGn-5-4\\%
  BuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{BuGn-6}{%
  BuGn-6-1\\%
  BuGn-6-2\\%
  BuGn-6-3\\%
  BuGn-6-4\\%
  BuGn-6-5\\%
  BuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{BuGn-7}{%
  BuGn-7-1\\%
  BuGn-7-2\\%
  BuGn-7-3\\%
  BuGn-7-4\\%
  BuGn-7-5\\%
  BuGn-7-6\\%
  BuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{BuGn-8}{%
  BuGn-8-1\\%
  BuGn-8-2\\%
  BuGn-8-3\\%
  BuGn-8-4\\%
  BuGn-8-5\\%
  BuGn-8-6\\%
  BuGn-8-7\\%
  BuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{BuGn-9}{%
  BuGn-9-1\\%
  BuGn-9-2\\%
  BuGn-9-3\\%
  BuGn-9-4\\%
  BuGn-9-5\\%
  BuGn-9-6\\%
  BuGn-9-7\\%
  BuGn-9-8\\%
  BuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-3}{%
  PuBuGn-3-1\\%
  PuBuGn-3-2\\%
  PuBuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-4}{%
  PuBuGn-4-1\\%
  PuBuGn-4-2\\%
  PuBuGn-4-3\\%
  PuBuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-5}{%
  PuBuGn-5-1\\%
  PuBuGn-5-2\\%
  PuBuGn-5-3\\%
  PuBuGn-5-4\\%
  PuBuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-6}{%
  PuBuGn-6-1\\%
  PuBuGn-6-2\\%
  PuBuGn-6-3\\%
  PuBuGn-6-4\\%
  PuBuGn-6-5\\%
  PuBuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-7}{%
  PuBuGn-7-1\\%
  PuBuGn-7-2\\%
  PuBuGn-7-3\\%
  PuBuGn-7-4\\%
  PuBuGn-7-5\\%
  PuBuGn-7-6\\%
  PuBuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-8}{%
  PuBuGn-8-1\\%
  PuBuGn-8-2\\%
  PuBuGn-8-3\\%
  PuBuGn-8-4\\%
  PuBuGn-8-5\\%
  PuBuGn-8-6\\%
  PuBuGn-8-7\\%
  PuBuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-9}{%
  PuBuGn-9-1\\%
  PuBuGn-9-2\\%
  PuBuGn-9-3\\%
  PuBuGn-9-4\\%
  PuBuGn-9-5\\%
  PuBuGn-9-6\\%
  PuBuGn-9-7\\%
  PuBuGn-9-8\\%
  PuBuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBu-3}{%
  PuBu-3-1\\%
  PuBu-3-2\\%
  PuBu-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBu-4}{%
  PuBu-4-1\\%
  PuBu-4-2\\%
  PuBu-4-3\\%
  PuBu-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBu-5}{%
  PuBu-5-1\\%
  PuBu-5-2\\%
  PuBu-5-3\\%
  PuBu-5-4\\%
  PuBu-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBu-6}{%
  PuBu-6-1\\%
  PuBu-6-2\\%
  PuBu-6-3\\%
  PuBu-6-4\\%
  PuBu-6-5\\%
  PuBu-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBu-7}{%
  PuBu-7-1\\%
  PuBu-7-2\\%
  PuBu-7-3\\%
  PuBu-7-4\\%
  PuBu-7-5\\%
  PuBu-7-6\\%
  PuBu-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBu-8}{%
  PuBu-8-1\\%
  PuBu-8-2\\%
  PuBu-8-3\\%
  PuBu-8-4\\%
  PuBu-8-5\\%
  PuBu-8-6\\%
  PuBu-8-7\\%
  PuBu-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBu-9}{%
  PuBu-9-1\\%
  PuBu-9-2\\%
  PuBu-9-3\\%
  PuBu-9-4\\%
  PuBu-9-5\\%
  PuBu-9-6\\%
  PuBu-9-7\\%
  PuBu-9-8\\%
  PuBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuPu-3}{%
  BuPu-3-1\\%
  BuPu-3-2\\%
  BuPu-3-3\\%
}
\pgfplotscreateplotcyclelist{BuPu-4}{%
  BuPu-4-1\\%
  BuPu-4-2\\%
  BuPu-4-3\\%
  BuPu-4-4\\%
}
\pgfplotscreateplotcyclelist{BuPu-5}{%
  BuPu-5-1\\%
  BuPu-5-2\\%
  BuPu-5-3\\%
  BuPu-5-4\\%
  BuPu-5-5\\%
}
\pgfplotscreateplotcyclelist{BuPu-6}{%
  BuPu-6-1\\%
  BuPu-6-2\\%
  BuPu-6-3\\%
  BuPu-6-4\\%
  BuPu-6-5\\%
  BuPu-6-6\\%
}
\pgfplotscreateplotcyclelist{BuPu-7}{%
  BuPu-7-1\\%
  BuPu-7-2\\%
  BuPu-7-3\\%
  BuPu-7-4\\%
  BuPu-7-5\\%
  BuPu-7-6\\%
  BuPu-7-7\\%
}
\pgfplotscreateplotcyclelist{BuPu-8}{%
  BuPu-8-1\\%
  BuPu-8-2\\%
  BuPu-8-3\\%
  BuPu-8-4\\%
  BuPu-8-5\\%
  BuPu-8-6\\%
  BuPu-8-7\\%
  BuPu-8-8\\%
}
\pgfplotscreateplotcyclelist{BuPu-9}{%
  BuPu-9-1\\%
  BuPu-9-2\\%
  BuPu-9-3\\%
  BuPu-9-4\\%
  BuPu-9-5\\%
  BuPu-9-6\\%
  BuPu-9-7\\%
  BuPu-9-8\\%
  BuPu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdPu-3}{%
  RdPu-3-1\\%
  RdPu-3-2\\%
  RdPu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdPu-4}{%
  RdPu-4-1\\%
  RdPu-4-2\\%
  RdPu-4-3\\%
  RdPu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdPu-5}{%
  RdPu-5-1\\%
  RdPu-5-2\\%
  RdPu-5-3\\%
  RdPu-5-4\\%
  RdPu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdPu-6}{%
  RdPu-6-1\\%
  RdPu-6-2\\%
  RdPu-6-3\\%
  RdPu-6-4\\%
  RdPu-6-5\\%
  RdPu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdPu-7}{%
  RdPu-7-1\\%
  RdPu-7-2\\%
  RdPu-7-3\\%
  RdPu-7-4\\%
  RdPu-7-5\\%
  RdPu-7-6\\%
  RdPu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdPu-8}{%
  RdPu-8-1\\%
  RdPu-8-2\\%
  RdPu-8-3\\%
  RdPu-8-4\\%
  RdPu-8-5\\%
  RdPu-8-6\\%
  RdPu-8-7\\%
  RdPu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdPu-9}{%
  RdPu-9-1\\%
  RdPu-9-2\\%
  RdPu-9-3\\%
  RdPu-9-4\\%
  RdPu-9-5\\%
  RdPu-9-6\\%
  RdPu-9-7\\%
  RdPu-9-8\\%
  RdPu-9-9\\%
}
\pgfplotscreateplotcyclelist{PuRd-3}{%
  PuRd-3-1\\%
  PuRd-3-2\\%
  PuRd-3-3\\%
}
\pgfplotscreateplotcyclelist{PuRd-4}{%
  PuRd-4-1\\%
  PuRd-4-2\\%
  PuRd-4-3\\%
  PuRd-4-4\\%
}
\pgfplotscreateplotcyclelist{PuRd-5}{%
  PuRd-5-1\\%
  PuRd-5-2\\%
  PuRd-5-3\\%
  PuRd-5-4\\%
  PuRd-5-5\\%
}
\pgfplotscreateplotcyclelist{PuRd-6}{%
  PuRd-6-1\\%
  PuRd-6-2\\%
  PuRd-6-3\\%
  PuRd-6-4\\%
  PuRd-6-5\\%
  PuRd-6-6\\%
}
\pgfplotscreateplotcyclelist{PuRd-7}{%
  PuRd-7-1\\%
  PuRd-7-2\\%
  PuRd-7-3\\%
  PuRd-7-4\\%
  PuRd-7-5\\%
  PuRd-7-6\\%
  PuRd-7-7\\%
}
\pgfplotscreateplotcyclelist{PuRd-8}{%
  PuRd-8-1\\%
  PuRd-8-2\\%
  PuRd-8-3\\%
  PuRd-8-4\\%
  PuRd-8-5\\%
  PuRd-8-6\\%
  PuRd-8-7\\%
  PuRd-8-8\\%
}
\pgfplotscreateplotcyclelist{PuRd-9}{%
  PuRd-9-1\\%
  PuRd-9-2\\%
  PuRd-9-3\\%
  PuRd-9-4\\%
  PuRd-9-5\\%
  PuRd-9-6\\%
  PuRd-9-7\\%
  PuRd-9-8\\%
  PuRd-9-9\\%
}
\pgfplotscreateplotcyclelist{OrRd-3}{%
  OrRd-3-1\\%
  OrRd-3-2\\%
  OrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{OrRd-4}{%
  OrRd-4-1\\%
  OrRd-4-2\\%
  OrRd-4-3\\%
  OrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{OrRd-5}{%
  OrRd-5-1\\%
  OrRd-5-2\\%
  OrRd-5-3\\%
  OrRd-5-4\\%
  OrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{OrRd-6}{%
  OrRd-6-1\\%
  OrRd-6-2\\%
  OrRd-6-3\\%
  OrRd-6-4\\%
  OrRd-6-5\\%
  OrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{OrRd-7}{%
  OrRd-7-1\\%
  OrRd-7-2\\%
  OrRd-7-3\\%
  OrRd-7-4\\%
  OrRd-7-5\\%
  OrRd-7-6\\%
  OrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{OrRd-8}{%
  OrRd-8-1\\%
  OrRd-8-2\\%
  OrRd-8-3\\%
  OrRd-8-4\\%
  OrRd-8-5\\%
  OrRd-8-6\\%
  OrRd-8-7\\%
  OrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{OrRd-9}{%
  OrRd-9-1\\%
  OrRd-9-2\\%
  OrRd-9-3\\%
  OrRd-9-4\\%
  OrRd-9-5\\%
  OrRd-9-6\\%
  OrRd-9-7\\%
  OrRd-9-8\\%
  OrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-3}{%
  YlOrRd-3-1\\%
  YlOrRd-3-2\\%
  YlOrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-4}{%
  YlOrRd-4-1\\%
  YlOrRd-4-2\\%
  YlOrRd-4-3\\%
  YlOrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-5}{%
  YlOrRd-5-1\\%
  YlOrRd-5-2\\%
  YlOrRd-5-3\\%
  YlOrRd-5-4\\%
  YlOrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-6}{%
  YlOrRd-6-1\\%
  YlOrRd-6-2\\%
  YlOrRd-6-3\\%
  YlOrRd-6-4\\%
  YlOrRd-6-5\\%
  YlOrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-7}{%
  YlOrRd-7-1\\%
  YlOrRd-7-2\\%
  YlOrRd-7-3\\%
  YlOrRd-7-4\\%
  YlOrRd-7-5\\%
  YlOrRd-7-6\\%
  YlOrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-8}{%
  YlOrRd-8-1\\%
  YlOrRd-8-2\\%
  YlOrRd-8-3\\%
  YlOrRd-8-4\\%
  YlOrRd-8-5\\%
  YlOrRd-8-6\\%
  YlOrRd-8-7\\%
  YlOrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-9}{%
  YlOrRd-9-1\\%
  YlOrRd-9-2\\%
  YlOrRd-9-3\\%
  YlOrRd-9-4\\%
  YlOrRd-9-5\\%
  YlOrRd-9-6\\%
  YlOrRd-9-7\\%
  YlOrRd-9-8\\%
  YlOrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-3}{%
  YlOrBr-3-1\\%
  YlOrBr-3-2\\%
  YlOrBr-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-4}{%
  YlOrBr-4-1\\%
  YlOrBr-4-2\\%
  YlOrBr-4-3\\%
  YlOrBr-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-5}{%
  YlOrBr-5-1\\%
  YlOrBr-5-2\\%
  YlOrBr-5-3\\%
  YlOrBr-5-4\\%
  YlOrBr-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-6}{%
  YlOrBr-6-1\\%
  YlOrBr-6-2\\%
  YlOrBr-6-3\\%
  YlOrBr-6-4\\%
  YlOrBr-6-5\\%
  YlOrBr-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-7}{%
  YlOrBr-7-1\\%
  YlOrBr-7-2\\%
  YlOrBr-7-3\\%
  YlOrBr-7-4\\%
  YlOrBr-7-5\\%
  YlOrBr-7-6\\%
  YlOrBr-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-8}{%
  YlOrBr-8-1\\%
  YlOrBr-8-2\\%
  YlOrBr-8-3\\%
  YlOrBr-8-4\\%
  YlOrBr-8-5\\%
  YlOrBr-8-6\\%
  YlOrBr-8-7\\%
  YlOrBr-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-9}{%
  YlOrBr-9-1\\%
  YlOrBr-9-2\\%
  YlOrBr-9-3\\%
  YlOrBr-9-4\\%
  YlOrBr-9-5\\%
  YlOrBr-9-6\\%
  YlOrBr-9-7\\%
  YlOrBr-9-8\\%
  YlOrBr-9-9\\%
}
\pgfplotscreateplotcyclelist{Purples-3}{%
  Purples-3-1\\%
  Purples-3-2\\%
  Purples-3-3\\%
}
\pgfplotscreateplotcyclelist{Purples-4}{%
  Purples-4-1\\%
  Purples-4-2\\%
  Purples-4-3\\%
  Purples-4-4\\%
}
\pgfplotscreateplotcyclelist{Purples-5}{%
  Purples-5-1\\%
  Purples-5-2\\%
  Purples-5-3\\%
  Purples-5-4\\%
  Purples-5-5\\%
}
\pgfplotscreateplotcyclelist{Purples-6}{%
  Purples-6-1\\%
  Purples-6-2\\%
  Purples-6-3\\%
  Purples-6-4\\%
  Purples-6-5\\%
  Purples-6-6\\%
}
\pgfplotscreateplotcyclelist{Purples-7}{%
  Purples-7-1\\%
  Purples-7-2\\%
  Purples-7-3\\%
  Purples-7-4\\%
  Purples-7-5\\%
  Purples-7-6\\%
  Purples-7-7\\%
}
\pgfplotscreateplotcyclelist{Purples-8}{%
  Purples-8-1\\%
  Purples-8-2\\%
  Purples-8-3\\%
  Purples-8-4\\%
  Purples-8-5\\%
  Purples-8-6\\%
  Purples-8-7\\%
  Purples-8-8\\%
}
\pgfplotscreateplotcyclelist{Purples-9}{%
  Purples-9-1\\%
  Purples-9-2\\%
  Purples-9-3\\%
  Purples-9-4\\%
  Purples-9-5\\%
  Purples-9-6\\%
  Purples-9-7\\%
  Purples-9-8\\%
  Purples-9-9\\%
}
\pgfplotscreateplotcyclelist{Blues-3}{%
  Blues-3-1\\%
  Blues-3-2\\%
  Blues-3-3\\%
}
\pgfplotscreateplotcyclelist{Blues-4}{%
  Blues-4-1\\%
  Blues-4-2\\%
  Blues-4-3\\%
  Blues-4-4\\%
}
\pgfplotscreateplotcyclelist{Blues-5}{%
  Blues-5-1\\%
  Blues-5-2\\%
  Blues-5-3\\%
  Blues-5-4\\%
  Blues-5-5\\%
}
\pgfplotscreateplotcyclelist{Blues-6}{%
  Blues-6-1\\%
  Blues-6-2\\%
  Blues-6-3\\%
  Blues-6-4\\%
  Blues-6-5\\%
  Blues-6-6\\%
}
\pgfplotscreateplotcyclelist{Blues-7}{%
  Blues-7-1\\%
  Blues-7-2\\%
  Blues-7-3\\%
  Blues-7-4\\%
  Blues-7-5\\%
  Blues-7-6\\%
  Blues-7-7\\%
}
\pgfplotscreateplotcyclelist{Blues-8}{%
  Blues-8-1\\%
  Blues-8-2\\%
  Blues-8-3\\%
  Blues-8-4\\%
  Blues-8-5\\%
  Blues-8-6\\%
  Blues-8-7\\%
  Blues-8-8\\%
}
\pgfplotscreateplotcyclelist{Blues-9}{%
  Blues-9-1\\%
  Blues-9-2\\%
  Blues-9-3\\%
  Blues-9-4\\%
  Blues-9-5\\%
  Blues-9-6\\%
  Blues-9-7\\%
  Blues-9-8\\%
  Blues-9-9\\%
}
\pgfplotscreateplotcyclelist{Greens-3}{%
  Greens-3-1\\%
  Greens-3-2\\%
  Greens-3-3\\%
}
\pgfplotscreateplotcyclelist{Greens-4}{%
  Greens-4-1\\%
  Greens-4-2\\%
  Greens-4-3\\%
  Greens-4-4\\%
}
\pgfplotscreateplotcyclelist{Greens-5}{%
  Greens-5-1\\%
  Greens-5-2\\%
  Greens-5-3\\%
  Greens-5-4\\%
  Greens-5-5\\%
}
\pgfplotscreateplotcyclelist{Greens-6}{%
  Greens-6-1\\%
  Greens-6-2\\%
  Greens-6-3\\%
  Greens-6-4\\%
  Greens-6-5\\%
  Greens-6-6\\%
}
\pgfplotscreateplotcyclelist{Greens-7}{%
  Greens-7-1\\%
  Greens-7-2\\%
  Greens-7-3\\%
  Greens-7-4\\%
  Greens-7-5\\%
  Greens-7-6\\%
  Greens-7-7\\%
}
\pgfplotscreateplotcyclelist{Greens-8}{%
  Greens-8-1\\%
  Greens-8-2\\%
  Greens-8-3\\%
  Greens-8-4\\%
  Greens-8-5\\%
  Greens-8-6\\%
  Greens-8-7\\%
  Greens-8-8\\%
}
\pgfplotscreateplotcyclelist{Greens-9}{%
  Greens-9-1\\%
  Greens-9-2\\%
  Greens-9-3\\%
  Greens-9-4\\%
  Greens-9-5\\%
  Greens-9-6\\%
  Greens-9-7\\%
  Greens-9-8\\%
  Greens-9-9\\%
}
\pgfplotscreateplotcyclelist{Oranges-3}{%
  Oranges-3-1\\%
  Oranges-3-2\\%
  Oranges-3-3\\%
}
\pgfplotscreateplotcyclelist{Oranges-4}{%
  Oranges-4-1\\%
  Oranges-4-2\\%
  Oranges-4-3\\%
  Oranges-4-4\\%
}
\pgfplotscreateplotcyclelist{Oranges-5}{%
  Oranges-5-1\\%
  Oranges-5-2\\%
  Oranges-5-3\\%
  Oranges-5-4\\%
  Oranges-5-5\\%
}
\pgfplotscreateplotcyclelist{Oranges-6}{%
  Oranges-6-1\\%
  Oranges-6-2\\%
  Oranges-6-3\\%
  Oranges-6-4\\%
  Oranges-6-5\\%
  Oranges-6-6\\%
}
\pgfplotscreateplotcyclelist{Oranges-7}{%
  Oranges-7-1\\%
  Oranges-7-2\\%
  Oranges-7-3\\%
  Oranges-7-4\\%
  Oranges-7-5\\%
  Oranges-7-6\\%
  Oranges-7-7\\%
}
\pgfplotscreateplotcyclelist{Oranges-8}{%
  Oranges-8-1\\%
  Oranges-8-2\\%
  Oranges-8-3\\%
  Oranges-8-4\\%
  Oranges-8-5\\%
  Oranges-8-6\\%
  Oranges-8-7\\%
  Oranges-8-8\\%
}
\pgfplotscreateplotcyclelist{Oranges-9}{%
  Oranges-9-1\\%
  Oranges-9-2\\%
  Oranges-9-3\\%
  Oranges-9-4\\%
  Oranges-9-5\\%
  Oranges-9-6\\%
  Oranges-9-7\\%
  Oranges-9-8\\%
  Oranges-9-9\\%
}
\pgfplotscreateplotcyclelist{Reds-3}{%
  Reds-3-1\\%
  Reds-3-2\\%
  Reds-3-3\\%
}
\pgfplotscreateplotcyclelist{Reds-4}{%
  Reds-4-1\\%
  Reds-4-2\\%
  Reds-4-3\\%
  Reds-4-4\\%
}
\pgfplotscreateplotcyclelist{Reds-5}{%
  Reds-5-1\\%
  Reds-5-2\\%
  Reds-5-3\\%
  Reds-5-4\\%
  Reds-5-5\\%
}
\pgfplotscreateplotcyclelist{Reds-6}{%
  Reds-6-1\\%
  Reds-6-2\\%
  Reds-6-3\\%
  Reds-6-4\\%
  Reds-6-5\\%
  Reds-6-6\\%
}
\pgfplotscreateplotcyclelist{Reds-7}{%
  Reds-7-1\\%
  Reds-7-2\\%
  Reds-7-3\\%
  Reds-7-4\\%
  Reds-7-5\\%
  Reds-7-6\\%
  Reds-7-7\\%
}
\pgfplotscreateplotcyclelist{Reds-8}{%
  Reds-8-1\\%
  Reds-8-2\\%
  Reds-8-3\\%
  Reds-8-4\\%
  Reds-8-5\\%
  Reds-8-6\\%
  Reds-8-7\\%
  Reds-8-8\\%
}
\pgfplotscreateplotcyclelist{Reds-9}{%
  Reds-9-1\\%
  Reds-9-2\\%
  Reds-9-3\\%
  Reds-9-4\\%
  Reds-9-5\\%
  Reds-9-6\\%
  Reds-9-7\\%
  Reds-9-8\\%
  Reds-9-9\\%
}
\pgfplotscreateplotcyclelist{Greys-3}{%
  Greys-3-1\\%
  Greys-3-2\\%
  Greys-3-3\\%
}
\pgfplotscreateplotcyclelist{Greys-4}{%
  Greys-4-1\\%
  Greys-4-2\\%
  Greys-4-3\\%
  Greys-4-4\\%
}
\pgfplotscreateplotcyclelist{Greys-5}{%
  Greys-5-1\\%
  Greys-5-2\\%
  Greys-5-3\\%
  Greys-5-4\\%
  Greys-5-5\\%
}
\pgfplotscreateplotcyclelist{Greys-6}{%
  Greys-6-1\\%
  Greys-6-2\\%
  Greys-6-3\\%
  Greys-6-4\\%
  Greys-6-5\\%
  Greys-6-6\\%
}
\pgfplotscreateplotcyclelist{Greys-7}{%
  Greys-7-1\\%
  Greys-7-2\\%
  Greys-7-3\\%
  Greys-7-4\\%
  Greys-7-5\\%
  Greys-7-6\\%
  Greys-7-7\\%
}
\pgfplotscreateplotcyclelist{Greys-8}{%
  Greys-8-1\\%
  Greys-8-2\\%
  Greys-8-3\\%
  Greys-8-4\\%
  Greys-8-5\\%
  Greys-8-6\\%
  Greys-8-7\\%
  Greys-8-8\\%
}
\pgfplotscreateplotcyclelist{Greys-9}{%
  Greys-9-1\\%
  Greys-9-2\\%
  Greys-9-3\\%
  Greys-9-4\\%
  Greys-9-5\\%
  Greys-9-6\\%
  Greys-9-7\\%
  Greys-9-8\\%
  Greys-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-3}{%
  PuOr-3-1\\%
  PuOr-3-2\\%
  PuOr-3-3\\%
}
\pgfplotscreateplotcyclelist{PuOr-4}{%
  PuOr-4-1\\%
  PuOr-4-2\\%
  PuOr-4-3\\%
  PuOr-4-4\\%
}
\pgfplotscreateplotcyclelist{PuOr-5}{%
  PuOr-5-1\\%
  PuOr-5-2\\%
  PuOr-5-3\\%
  PuOr-5-4\\%
  PuOr-5-5\\%
}
\pgfplotscreateplotcyclelist{PuOr-6}{%
  PuOr-6-1\\%
  PuOr-6-2\\%
  PuOr-6-3\\%
  PuOr-6-4\\%
  PuOr-6-5\\%
  PuOr-6-6\\%
}
\pgfplotscreateplotcyclelist{PuOr-7}{%
  PuOr-7-1\\%
  PuOr-7-2\\%
  PuOr-7-3\\%
  PuOr-7-4\\%
  PuOr-7-5\\%
  PuOr-7-6\\%
  PuOr-7-7\\%
}
\pgfplotscreateplotcyclelist{PuOr-8}{%
  PuOr-8-1\\%
  PuOr-8-2\\%
  PuOr-8-3\\%
  PuOr-8-4\\%
  PuOr-8-5\\%
  PuOr-8-6\\%
  PuOr-8-7\\%
  PuOr-8-8\\%
}
\pgfplotscreateplotcyclelist{PuOr-9}{%
  PuOr-9-1\\%
  PuOr-9-2\\%
  PuOr-9-3\\%
  PuOr-9-4\\%
  PuOr-9-5\\%
  PuOr-9-6\\%
  PuOr-9-7\\%
  PuOr-9-8\\%
  PuOr-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-10}{%
  PuOr-10-1\\%
  PuOr-10-2\\%
  PuOr-10-3\\%
  PuOr-10-4\\%
  PuOr-10-5\\%
  PuOr-10-6\\%
  PuOr-10-7\\%
  PuOr-10-8\\%
  PuOr-10-9\\%
  PuOr-10-10\\%
}
\pgfplotscreateplotcyclelist{PuOr-11}{%
  PuOr-11-1\\%
  PuOr-11-2\\%
  PuOr-11-3\\%
  PuOr-11-4\\%
  PuOr-11-5\\%
  PuOr-11-6\\%
  PuOr-11-7\\%
  PuOr-11-8\\%
  PuOr-11-9\\%
  PuOr-11-10\\%
  PuOr-11-11\\%
}
\pgfplotscreateplotcyclelist{BrBG-3}{%
  BrBG-3-1\\%
  BrBG-3-2\\%
  BrBG-3-3\\%
}
\pgfplotscreateplotcyclelist{BrBG-4}{%
  BrBG-4-1\\%
  BrBG-4-2\\%
  BrBG-4-3\\%
  BrBG-4-4\\%
}
\pgfplotscreateplotcyclelist{BrBG-5}{%
  BrBG-5-1\\%
  BrBG-5-2\\%
  BrBG-5-3\\%
  BrBG-5-4\\%
  BrBG-5-5\\%
}
\pgfplotscreateplotcyclelist{BrBG-6}{%
  BrBG-6-1\\%
  BrBG-6-2\\%
  BrBG-6-3\\%
  BrBG-6-4\\%
  BrBG-6-5\\%
  BrBG-6-6\\%
}
\pgfplotscreateplotcyclelist{BrBG-7}{%
  BrBG-7-1\\%
  BrBG-7-2\\%
  BrBG-7-3\\%
  BrBG-7-4\\%
  BrBG-7-5\\%
  BrBG-7-6\\%
  BrBG-7-7\\%
}
\pgfplotscreateplotcyclelist{BrBG-8}{%
  BrBG-8-1\\%
  BrBG-8-2\\%
  BrBG-8-3\\%
  BrBG-8-4\\%
  BrBG-8-5\\%
  BrBG-8-6\\%
  BrBG-8-7\\%
  BrBG-8-8\\%
}
\pgfplotscreateplotcyclelist{BrBG-9}{%
  BrBG-9-1\\%
  BrBG-9-2\\%
  BrBG-9-3\\%
  BrBG-9-4\\%
  BrBG-9-5\\%
  BrBG-9-6\\%
  BrBG-9-7\\%
  BrBG-9-8\\%
  BrBG-9-9\\%
}
\pgfplotscreateplotcyclelist{BrBG-10}{%
  BrBG-10-1\\%
  BrBG-10-2\\%
  BrBG-10-3\\%
  BrBG-10-4\\%
  BrBG-10-5\\%
  BrBG-10-6\\%
  BrBG-10-7\\%
  BrBG-10-8\\%
  BrBG-10-9\\%
  BrBG-10-10\\%
}
\pgfplotscreateplotcyclelist{BrBG-11}{%
  BrBG-11-1\\%
  BrBG-11-2\\%
  BrBG-11-3\\%
  BrBG-11-4\\%
  BrBG-11-5\\%
  BrBG-11-6\\%
  BrBG-11-7\\%
  BrBG-11-8\\%
  BrBG-11-9\\%
  BrBG-11-10\\%
  BrBG-11-11\\%
}
\pgfplotscreateplotcyclelist{PRGn-3}{%
  PRGn-3-1\\%
  PRGn-3-2\\%
  PRGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PRGn-4}{%
  PRGn-4-1\\%
  PRGn-4-2\\%
  PRGn-4-3\\%
  PRGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PRGn-5}{%
  PRGn-5-1\\%
  PRGn-5-2\\%
  PRGn-5-3\\%
  PRGn-5-4\\%
  PRGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PRGn-6}{%
  PRGn-6-1\\%
  PRGn-6-2\\%
  PRGn-6-3\\%
  PRGn-6-4\\%
  PRGn-6-5\\%
  PRGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PRGn-7}{%
  PRGn-7-1\\%
  PRGn-7-2\\%
  PRGn-7-3\\%
  PRGn-7-4\\%
  PRGn-7-5\\%
  PRGn-7-6\\%
  PRGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PRGn-8}{%
  PRGn-8-1\\%
  PRGn-8-2\\%
  PRGn-8-3\\%
  PRGn-8-4\\%
  PRGn-8-5\\%
  PRGn-8-6\\%
  PRGn-8-7\\%
  PRGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PRGn-9}{%
  PRGn-9-1\\%
  PRGn-9-2\\%
  PRGn-9-3\\%
  PRGn-9-4\\%
  PRGn-9-5\\%
  PRGn-9-6\\%
  PRGn-9-7\\%
  PRGn-9-8\\%
  PRGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PRGn-10}{%
  PRGn-10-1\\%
  PRGn-10-2\\%
  PRGn-10-3\\%
  PRGn-10-4\\%
  PRGn-10-5\\%
  PRGn-10-6\\%
  PRGn-10-7\\%
  PRGn-10-8\\%
  PRGn-10-9\\%
  PRGn-10-10\\%
}
\pgfplotscreateplotcyclelist{PRGn-11}{%
  PRGn-11-1\\%
  PRGn-11-2\\%
  PRGn-11-3\\%
  PRGn-11-4\\%
  PRGn-11-5\\%
  PRGn-11-6\\%
  PRGn-11-7\\%
  PRGn-11-8\\%
  PRGn-11-9\\%
  PRGn-11-10\\%
  PRGn-11-11\\%
}
\pgfplotscreateplotcyclelist{PiYG-3}{%
  PiYG-3-1\\%
  PiYG-3-2\\%
  PiYG-3-3\\%
}
\pgfplotscreateplotcyclelist{PiYG-4}{%
  PiYG-4-1\\%
  PiYG-4-2\\%
  PiYG-4-3\\%
  PiYG-4-4\\%
}
\pgfplotscreateplotcyclelist{PiYG-5}{%
  PiYG-5-1\\%
  PiYG-5-2\\%
  PiYG-5-3\\%
  PiYG-5-4\\%
  PiYG-5-5\\%
}
\pgfplotscreateplotcyclelist{PiYG-6}{%
  PiYG-6-1\\%
  PiYG-6-2\\%
  PiYG-6-3\\%
  PiYG-6-4\\%
  PiYG-6-5\\%
  PiYG-6-6\\%
}
\pgfplotscreateplotcyclelist{PiYG-7}{%
  PiYG-7-1\\%
  PiYG-7-2\\%
  PiYG-7-3\\%
  PiYG-7-4\\%
  PiYG-7-5\\%
  PiYG-7-6\\%
  PiYG-7-7\\%
}
\pgfplotscreateplotcyclelist{PiYG-8}{%
  PiYG-8-1\\%
  PiYG-8-2\\%
  PiYG-8-3\\%
  PiYG-8-4\\%
  PiYG-8-5\\%
  PiYG-8-6\\%
  PiYG-8-7\\%
  PiYG-8-8\\%
}
\pgfplotscreateplotcyclelist{PiYG-9}{%
  PiYG-9-1\\%
  PiYG-9-2\\%
  PiYG-9-3\\%
  PiYG-9-4\\%
  PiYG-9-5\\%
  PiYG-9-6\\%
  PiYG-9-7\\%
  PiYG-9-8\\%
  PiYG-9-9\\%
}
\pgfplotscreateplotcyclelist{PiYG-10}{%
  PiYG-10-1\\%
  PiYG-10-2\\%
  PiYG-10-3\\%
  PiYG-10-4\\%
  PiYG-10-5\\%
  PiYG-10-6\\%
  PiYG-10-7\\%
  PiYG-10-8\\%
  PiYG-10-9\\%
  PiYG-10-10\\%
}
\pgfplotscreateplotcyclelist{PiYG-11}{%
  PiYG-11-1\\%
  PiYG-11-2\\%
  PiYG-11-3\\%
  PiYG-11-4\\%
  PiYG-11-5\\%
  PiYG-11-6\\%
  PiYG-11-7\\%
  PiYG-11-8\\%
  PiYG-11-9\\%
  PiYG-11-10\\%
  PiYG-11-11\\%
}
\pgfplotscreateplotcyclelist{RdBu-3}{%
  RdBu-3-1\\%
  RdBu-3-2\\%
  RdBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdBu-4}{%
  RdBu-4-1\\%
  RdBu-4-2\\%
  RdBu-4-3\\%
  RdBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdBu-5}{%
  RdBu-5-1\\%
  RdBu-5-2\\%
  RdBu-5-3\\%
  RdBu-5-4\\%
  RdBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdBu-6}{%
  RdBu-6-1\\%
  RdBu-6-2\\%
  RdBu-6-3\\%
  RdBu-6-4\\%
  RdBu-6-5\\%
  RdBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdBu-7}{%
  RdBu-7-1\\%
  RdBu-7-2\\%
  RdBu-7-3\\%
  RdBu-7-4\\%
  RdBu-7-5\\%
  RdBu-7-6\\%
  RdBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdBu-8}{%
  RdBu-8-1\\%
  RdBu-8-2\\%
  RdBu-8-3\\%
  RdBu-8-4\\%
  RdBu-8-5\\%
  RdBu-8-6\\%
  RdBu-8-7\\%
  RdBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdBu-9}{%
  RdBu-9-1\\%
  RdBu-9-2\\%
  RdBu-9-3\\%
  RdBu-9-4\\%
  RdBu-9-5\\%
  RdBu-9-6\\%
  RdBu-9-7\\%
  RdBu-9-8\\%
  RdBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdBu-10}{%
  RdBu-10-1\\%
  RdBu-10-2\\%
  RdBu-10-3\\%
  RdBu-10-4\\%
  RdBu-10-5\\%
  RdBu-10-6\\%
  RdBu-10-7\\%
  RdBu-10-8\\%
  RdBu-10-9\\%
  RdBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdBu-11}{%
  RdBu-11-1\\%
  RdBu-11-2\\%
  RdBu-11-3\\%
  RdBu-11-4\\%
  RdBu-11-5\\%
  RdBu-11-6\\%
  RdBu-11-7\\%
  RdBu-11-8\\%
  RdBu-11-9\\%
  RdBu-11-10\\%
  RdBu-11-11\\%
}
\pgfplotscreateplotcyclelist{RdGy-3}{%
  RdGy-3-1\\%
  RdGy-3-2\\%
  RdGy-3-3\\%
}
\pgfplotscreateplotcyclelist{RdGy-4}{%
  RdGy-4-1\\%
  RdGy-4-2\\%
  RdGy-4-3\\%
  RdGy-4-4\\%
}
\pgfplotscreateplotcyclelist{RdGy-5}{%
  RdGy-5-1\\%
  RdGy-5-2\\%
  RdGy-5-3\\%
  RdGy-5-4\\%
  RdGy-5-5\\%
}
\pgfplotscreateplotcyclelist{RdGy-6}{%
  RdGy-6-1\\%
  RdGy-6-2\\%
  RdGy-6-3\\%
  RdGy-6-4\\%
  RdGy-6-5\\%
  RdGy-6-6\\%
}
\pgfplotscreateplotcyclelist{RdGy-7}{%
  RdGy-7-1\\%
  RdGy-7-2\\%
  RdGy-7-3\\%
  RdGy-7-4\\%
  RdGy-7-5\\%
  RdGy-7-6\\%
  RdGy-7-7\\%
}
\pgfplotscreateplotcyclelist{RdGy-8}{%
  RdGy-8-1\\%
  RdGy-8-2\\%
  RdGy-8-3\\%
  RdGy-8-4\\%
  RdGy-8-5\\%
  RdGy-8-6\\%
  RdGy-8-7\\%
  RdGy-8-8\\%
}
\pgfplotscreateplotcyclelist{RdGy-9}{%
  RdGy-9-1\\%
  RdGy-9-2\\%
  RdGy-9-3\\%
  RdGy-9-4\\%
  RdGy-9-5\\%
  RdGy-9-6\\%
  RdGy-9-7\\%
  RdGy-9-8\\%
  RdGy-9-9\\%
}
\pgfplotscreateplotcyclelist{RdGy-10}{%
  RdGy-10-1\\%
  RdGy-10-2\\%
  RdGy-10-3\\%
  RdGy-10-4\\%
  RdGy-10-5\\%
  RdGy-10-6\\%
  RdGy-10-7\\%
  RdGy-10-8\\%
  RdGy-10-9\\%
  RdGy-10-10\\%
}
\pgfplotscreateplotcyclelist{RdGy-11}{%
  RdGy-11-1\\%
  RdGy-11-2\\%
  RdGy-11-3\\%
  RdGy-11-4\\%
  RdGy-11-5\\%
  RdGy-11-6\\%
  RdGy-11-7\\%
  RdGy-11-8\\%
  RdGy-11-9\\%
  RdGy-11-10\\%
  RdGy-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-3}{%
  RdYlBu-3-1\\%
  RdYlBu-3-2\\%
  RdYlBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-4}{%
  RdYlBu-4-1\\%
  RdYlBu-4-2\\%
  RdYlBu-4-3\\%
  RdYlBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-5}{%
  RdYlBu-5-1\\%
  RdYlBu-5-2\\%
  RdYlBu-5-3\\%
  RdYlBu-5-4\\%
  RdYlBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-6}{%
  RdYlBu-6-1\\%
  RdYlBu-6-2\\%
  RdYlBu-6-3\\%
  RdYlBu-6-4\\%
  RdYlBu-6-5\\%
  RdYlBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-7}{%
  RdYlBu-7-1\\%
  RdYlBu-7-2\\%
  RdYlBu-7-3\\%
  RdYlBu-7-4\\%
  RdYlBu-7-5\\%
  RdYlBu-7-6\\%
  RdYlBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-8}{%
  RdYlBu-8-1\\%
  RdYlBu-8-2\\%
  RdYlBu-8-3\\%
  RdYlBu-8-4\\%
  RdYlBu-8-5\\%
  RdYlBu-8-6\\%
  RdYlBu-8-7\\%
  RdYlBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-9}{%
  RdYlBu-9-1\\%
  RdYlBu-9-2\\%
  RdYlBu-9-3\\%
  RdYlBu-9-4\\%
  RdYlBu-9-5\\%
  RdYlBu-9-6\\%
  RdYlBu-9-7\\%
  RdYlBu-9-8\\%
  RdYlBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-10}{%
  RdYlBu-10-1\\%
  RdYlBu-10-2\\%
  RdYlBu-10-3\\%
  RdYlBu-10-4\\%
  RdYlBu-10-5\\%
  RdYlBu-10-6\\%
  RdYlBu-10-7\\%
  RdYlBu-10-8\\%
  RdYlBu-10-9\\%
  RdYlBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-11}{%
  RdYlBu-11-1\\%
  RdYlBu-11-2\\%
  RdYlBu-11-3\\%
  RdYlBu-11-4\\%
  RdYlBu-11-5\\%
  RdYlBu-11-6\\%
  RdYlBu-11-7\\%
  RdYlBu-11-8\\%
  RdYlBu-11-9\\%
  RdYlBu-11-10\\%
  RdYlBu-11-11\\%
}
\pgfplotscreateplotcyclelist{Spectral-3}{%
  Spectral-3-1\\%
  Spectral-3-2\\%
  Spectral-3-3\\%
}
\pgfplotscreateplotcyclelist{Spectral-4}{%
  Spectral-4-1\\%
  Spectral-4-2\\%
  Spectral-4-3\\%
  Spectral-4-4\\%
}
\pgfplotscreateplotcyclelist{Spectral-5}{%
  Spectral-5-1\\%
  Spectral-5-2\\%
  Spectral-5-3\\%
  Spectral-5-4\\%
  Spectral-5-5\\%
}
\pgfplotscreateplotcyclelist{Spectral-6}{%
  Spectral-6-1\\%
  Spectral-6-2\\%
  Spectral-6-3\\%
  Spectral-6-4\\%
  Spectral-6-5\\%
  Spectral-6-6\\%
}
\pgfplotscreateplotcyclelist{Spectral-7}{%
  Spectral-7-1\\%
  Spectral-7-2\\%
  Spectral-7-3\\%
  Spectral-7-4\\%
  Spectral-7-5\\%
  Spectral-7-6\\%
  Spectral-7-7\\%
}
\pgfplotscreateplotcyclelist{Spectral-8}{%
  Spectral-8-1\\%
  Spectral-8-2\\%
  Spectral-8-3\\%
  Spectral-8-4\\%
  Spectral-8-5\\%
  Spectral-8-6\\%
  Spectral-8-7\\%
  Spectral-8-8\\%
}
\pgfplotscreateplotcyclelist{Spectral-9}{%
  Spectral-9-1\\%
  Spectral-9-2\\%
  Spectral-9-3\\%
  Spectral-9-4\\%
  Spectral-9-5\\%
  Spectral-9-6\\%
  Spectral-9-7\\%
  Spectral-9-8\\%
  Spectral-9-9\\%
}
\pgfplotscreateplotcyclelist{Spectral-10}{%
  Spectral-10-1\\%
  Spectral-10-2\\%
  Spectral-10-3\\%
  Spectral-10-4\\%
  Spectral-10-5\\%
  Spectral-10-6\\%
  Spectral-10-7\\%
  Spectral-10-8\\%
  Spectral-10-9\\%
  Spectral-10-10\\%
}
\pgfplotscreateplotcyclelist{Spectral-11}{%
  Spectral-11-1\\%
  Spectral-11-2\\%
  Spectral-11-3\\%
  Spectral-11-4\\%
  Spectral-11-5\\%
  Spectral-11-6\\%
  Spectral-11-7\\%
  Spectral-11-8\\%
  Spectral-11-9\\%
  Spectral-11-10\\%
  Spectral-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-3}{%
  RdYlGn-3-1\\%
  RdYlGn-3-2\\%
  RdYlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-4}{%
  RdYlGn-4-1\\%
  RdYlGn-4-2\\%
  RdYlGn-4-3\\%
  RdYlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-5}{%
  RdYlGn-5-1\\%
  RdYlGn-5-2\\%
  RdYlGn-5-3\\%
  RdYlGn-5-4\\%
  RdYlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-6}{%
  RdYlGn-6-1\\%
  RdYlGn-6-2\\%
  RdYlGn-6-3\\%
  RdYlGn-6-4\\%
  RdYlGn-6-5\\%
  RdYlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-7}{%
  RdYlGn-7-1\\%
  RdYlGn-7-2\\%
  RdYlGn-7-3\\%
  RdYlGn-7-4\\%
  RdYlGn-7-5\\%
  RdYlGn-7-6\\%
  RdYlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-8}{%
  RdYlGn-8-1\\%
  RdYlGn-8-2\\%
  RdYlGn-8-3\\%
  RdYlGn-8-4\\%
  RdYlGn-8-5\\%
  RdYlGn-8-6\\%
  RdYlGn-8-7\\%
  RdYlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-9}{%
  RdYlGn-9-1\\%
  RdYlGn-9-2\\%
  RdYlGn-9-3\\%
  RdYlGn-9-4\\%
  RdYlGn-9-5\\%
  RdYlGn-9-6\\%
  RdYlGn-9-7\\%
  RdYlGn-9-8\\%
  RdYlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-10}{%
  RdYlGn-10-1\\%
  RdYlGn-10-2\\%
  RdYlGn-10-3\\%
  RdYlGn-10-4\\%
  RdYlGn-10-5\\%
  RdYlGn-10-6\\%
  RdYlGn-10-7\\%
  RdYlGn-10-8\\%
  RdYlGn-10-9\\%
  RdYlGn-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-11}{%
  RdYlGn-11-1\\%
  RdYlGn-11-2\\%
  RdYlGn-11-3\\%
  RdYlGn-11-4\\%
  RdYlGn-11-5\\%
  RdYlGn-11-6\\%
  RdYlGn-11-7\\%
  RdYlGn-11-8\\%
  RdYlGn-11-9\\%
  RdYlGn-11-10\\%
  RdYlGn-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-3}{%
  Set3-3-1\\%
  Set3-3-2\\%
  Set3-3-3\\%
}
\pgfplotscreateplotcyclelist{Set3-4}{%
  Set3-4-1\\%
  Set3-4-2\\%
  Set3-4-3\\%
  Set3-4-4\\%
}
\pgfplotscreateplotcyclelist{Set3-5}{%
  Set3-5-1\\%
  Set3-5-2\\%
  Set3-5-3\\%
  Set3-5-4\\%
  Set3-5-5\\%
}
\pgfplotscreateplotcyclelist{Set3-6}{%
  Set3-6-1\\%
  Set3-6-2\\%
  Set3-6-3\\%
  Set3-6-4\\%
  Set3-6-5\\%
  Set3-6-6\\%
}
\pgfplotscreateplotcyclelist{Set3-7}{%
  Set3-7-1\\%
  Set3-7-2\\%
  Set3-7-3\\%
  Set3-7-4\\%
  Set3-7-5\\%
  Set3-7-6\\%
  Set3-7-7\\%
}
\pgfplotscreateplotcyclelist{Set3-8}{%
  Set3-8-1\\%
  Set3-8-2\\%
  Set3-8-3\\%
  Set3-8-4\\%
  Set3-8-5\\%
  Set3-8-6\\%
  Set3-8-7\\%
  Set3-8-8\\%
}
\pgfplotscreateplotcyclelist{Set3-9}{%
  Set3-9-1\\%
  Set3-9-2\\%
  Set3-9-3\\%
  Set3-9-4\\%
  Set3-9-5\\%
  Set3-9-6\\%
  Set3-9-7\\%
  Set3-9-8\\%
  Set3-9-9\\%
}
\pgfplotscreateplotcyclelist{Set3-10}{%
  Set3-10-1\\%
  Set3-10-2\\%
  Set3-10-3\\%
  Set3-10-4\\%
  Set3-10-5\\%
  Set3-10-6\\%
  Set3-10-7\\%
  Set3-10-8\\%
  Set3-10-9\\%
  Set3-10-10\\%
}
\pgfplotscreateplotcyclelist{Set3-11}{%
  Set3-11-1\\%
  Set3-11-2\\%
  Set3-11-3\\%
  Set3-11-4\\%
  Set3-11-5\\%
  Set3-11-6\\%
  Set3-11-7\\%
  Set3-11-8\\%
  Set3-11-9\\%
  Set3-11-10\\%
  Set3-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-12}{%
  Set3-12-1\\%
  Set3-12-2\\%
  Set3-12-3\\%
  Set3-12-4\\%
  Set3-12-5\\%
  Set3-12-6\\%
  Set3-12-7\\%
  Set3-12-8\\%
  Set3-12-9\\%
  Set3-12-10\\%
  Set3-12-11\\%
  Set3-12-12\\%
}
\pgfplotscreateplotcyclelist{Pastel1-3}{%
  Pastel1-3-1\\%
  Pastel1-3-2\\%
  Pastel1-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel1-4}{%
  Pastel1-4-1\\%
  Pastel1-4-2\\%
  Pastel1-4-3\\%
  Pastel1-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel1-5}{%
  Pastel1-5-1\\%
  Pastel1-5-2\\%
  Pastel1-5-3\\%
  Pastel1-5-4\\%
  Pastel1-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel1-6}{%
  Pastel1-6-1\\%
  Pastel1-6-2\\%
  Pastel1-6-3\\%
  Pastel1-6-4\\%
  Pastel1-6-5\\%
  Pastel1-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel1-7}{%
  Pastel1-7-1\\%
  Pastel1-7-2\\%
  Pastel1-7-3\\%
  Pastel1-7-4\\%
  Pastel1-7-5\\%
  Pastel1-7-6\\%
  Pastel1-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel1-8}{%
  Pastel1-8-1\\%
  Pastel1-8-2\\%
  Pastel1-8-3\\%
  Pastel1-8-4\\%
  Pastel1-8-5\\%
  Pastel1-8-6\\%
  Pastel1-8-7\\%
  Pastel1-8-8\\%
}
\pgfplotscreateplotcyclelist{Pastel1-9}{%
  Pastel1-9-1\\%
  Pastel1-9-2\\%
  Pastel1-9-3\\%
  Pastel1-9-4\\%
  Pastel1-9-5\\%
  Pastel1-9-6\\%
  Pastel1-9-7\\%
  Pastel1-9-8\\%
  Pastel1-9-9\\%
}
\pgfplotscreateplotcyclelist{Set1-3}{%
  Set1-3-1\\%
  Set1-3-2\\%
  Set1-3-3\\%
}
\pgfplotscreateplotcyclelist{Set1-4}{%
  Set1-4-1\\%
  Set1-4-2\\%
  Set1-4-3\\%
  Set1-4-4\\%
}
\pgfplotscreateplotcyclelist{Set1-5}{%
  Set1-5-1\\%
  Set1-5-2\\%
  Set1-5-3\\%
  Set1-5-4\\%
  Set1-5-5\\%
}
\pgfplotscreateplotcyclelist{Set1-6}{%
  Set1-6-1\\%
  Set1-6-2\\%
  Set1-6-3\\%
  Set1-6-4\\%
  Set1-6-5\\%
  Set1-6-6\\%
}
\pgfplotscreateplotcyclelist{Set1-7}{%
  Set1-7-1\\%
  Set1-7-2\\%
  Set1-7-3\\%
  Set1-7-4\\%
  Set1-7-5\\%
  Set1-7-6\\%
  Set1-7-7\\%
}
\pgfplotscreateplotcyclelist{Set1-8}{%
  Set1-8-1\\%
  Set1-8-2\\%
  Set1-8-3\\%
  Set1-8-4\\%
  Set1-8-5\\%
  Set1-8-6\\%
  Set1-8-7\\%
  Set1-8-8\\%
}
\pgfplotscreateplotcyclelist{Set1-9}{%
  Set1-9-1\\%
  Set1-9-2\\%
  Set1-9-3\\%
  Set1-9-4\\%
  Set1-9-5\\%
  Set1-9-6\\%
  Set1-9-7\\%
  Set1-9-8\\%
  Set1-9-9\\%
}
\pgfplotscreateplotcyclelist{Pastel2-3}{%
  Pastel2-3-1\\%
  Pastel2-3-2\\%
  Pastel2-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel2-4}{%
  Pastel2-4-1\\%
  Pastel2-4-2\\%
  Pastel2-4-3\\%
  Pastel2-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel2-5}{%
  Pastel2-5-1\\%
  Pastel2-5-2\\%
  Pastel2-5-3\\%
  Pastel2-5-4\\%
  Pastel2-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel2-6}{%
  Pastel2-6-1\\%
  Pastel2-6-2\\%
  Pastel2-6-3\\%
  Pastel2-6-4\\%
  Pastel2-6-5\\%
  Pastel2-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel2-7}{%
  Pastel2-7-1\\%
  Pastel2-7-2\\%
  Pastel2-7-3\\%
  Pastel2-7-4\\%
  Pastel2-7-5\\%
  Pastel2-7-6\\%
  Pastel2-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel2-8}{%
  Pastel2-8-1\\%
  Pastel2-8-2\\%
  Pastel2-8-3\\%
  Pastel2-8-4\\%
  Pastel2-8-5\\%
  Pastel2-8-6\\%
  Pastel2-8-7\\%
  Pastel2-8-8\\%
}
\pgfplotscreateplotcyclelist{Set2-3}{%
  Set2-3-1\\%
  Set2-3-2\\%
  Set2-3-3\\%
}
\pgfplotscreateplotcyclelist{Set2-4}{%
  Set2-4-1\\%
  Set2-4-2\\%
  Set2-4-3\\%
  Set2-4-4\\%
}
\pgfplotscreateplotcyclelist{Set2-5}{%
  Set2-5-1\\%
  Set2-5-2\\%
  Set2-5-3\\%
  Set2-5-4\\%
  Set2-5-5\\%
}
\pgfplotscreateplotcyclelist{Set2-6}{%
  Set2-6-1\\%
  Set2-6-2\\%
  Set2-6-3\\%
  Set2-6-4\\%
  Set2-6-5\\%
  Set2-6-6\\%
}
\pgfplotscreateplotcyclelist{Set2-7}{%
  Set2-7-1\\%
  Set2-7-2\\%
  Set2-7-3\\%
  Set2-7-4\\%
  Set2-7-5\\%
  Set2-7-6\\%
  Set2-7-7\\%
}
\pgfplotscreateplotcyclelist{Set2-8}{%
  Set2-8-1\\%
  Set2-8-2\\%
  Set2-8-3\\%
  Set2-8-4\\%
  Set2-8-5\\%
  Set2-8-6\\%
  Set2-8-7\\%
  Set2-8-8\\%
}
\pgfplotscreateplotcyclelist{Dark2-3}{%
  Dark2-3-1\\%
  Dark2-3-2\\%
  Dark2-3-3\\%
}
\pgfplotscreateplotcyclelist{Dark2-4}{%
  Dark2-4-1\\%
  Dark2-4-2\\%
  Dark2-4-3\\%
  Dark2-4-4\\%
}
\pgfplotscreateplotcyclelist{Dark2-5}{%
  Dark2-5-1\\%
  Dark2-5-2\\%
  Dark2-5-3\\%
  Dark2-5-4\\%
  Dark2-5-5\\%
}
\pgfplotscreateplotcyclelist{Dark2-6}{%
  Dark2-6-1\\%
  Dark2-6-2\\%
  Dark2-6-3\\%
  Dark2-6-4\\%
  Dark2-6-5\\%
  Dark2-6-6\\%
}
\pgfplotscreateplotcyclelist{Dark2-7}{%
  Dark2-7-1\\%
  Dark2-7-2\\%
  Dark2-7-3\\%
  Dark2-7-4\\%
  Dark2-7-5\\%
  Dark2-7-6\\%
  Dark2-7-7\\%
}
\pgfplotscreateplotcyclelist{Dark2-8}{%
  Dark2-8-1\\%
  Dark2-8-2\\%
  Dark2-8-3\\%
  Dark2-8-4\\%
  Dark2-8-5\\%
  Dark2-8-6\\%
  Dark2-8-7\\%
  Dark2-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-3}{%
  Paired-3-1\\%
  Paired-3-2\\%
  Paired-3-3\\%
}
\pgfplotscreateplotcyclelist{Paired-4}{%
  Paired-4-1\\%
  Paired-4-2\\%
  Paired-4-3\\%
  Paired-4-4\\%
}
\pgfplotscreateplotcyclelist{Paired-5}{%
  Paired-5-1\\%
  Paired-5-2\\%
  Paired-5-3\\%
  Paired-5-4\\%
  Paired-5-5\\%
}
\pgfplotscreateplotcyclelist{Paired-6}{%
  Paired-6-1\\%
  Paired-6-2\\%
  Paired-6-3\\%
  Paired-6-4\\%
  Paired-6-5\\%
  Paired-6-6\\%
}
\pgfplotscreateplotcyclelist{Paired-7}{%
  Paired-7-1\\%
  Paired-7-2\\%
  Paired-7-3\\%
  Paired-7-4\\%
  Paired-7-5\\%
  Paired-7-6\\%
  Paired-7-7\\%
}
\pgfplotscreateplotcyclelist{Paired-8}{%
  Paired-8-1\\%
  Paired-8-2\\%
  Paired-8-3\\%
  Paired-8-4\\%
  Paired-8-5\\%
  Paired-8-6\\%
  Paired-8-7\\%
  Paired-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-9}{%
  Paired-9-1\\%
  Paired-9-2\\%
  Paired-9-3\\%
  Paired-9-4\\%
  Paired-9-5\\%
  Paired-9-6\\%
  Paired-9-7\\%
  Paired-9-8\\%
  Paired-9-9\\%
}
\pgfplotscreateplotcyclelist{Paired-10}{%
  Paired-10-1\\%
  Paired-10-2\\%
  Paired-10-3\\%
  Paired-10-4\\%
  Paired-10-5\\%
  Paired-10-6\\%
  Paired-10-7\\%
  Paired-10-8\\%
  Paired-10-9\\%
  Paired-10-10\\%
}
\pgfplotscreateplotcyclelist{Paired-11}{%
  Paired-11-1\\%
  Paired-11-2\\%
  Paired-11-3\\%
  Paired-11-4\\%
  Paired-11-5\\%
  Paired-11-6\\%
  Paired-11-7\\%
  Paired-11-8\\%
  Paired-11-9\\%
  Paired-11-10\\%
  Paired-11-11\\%
}
\pgfplotscreateplotcyclelist{Paired-12}{%
  Paired-12-1\\%
  Paired-12-2\\%
  Paired-12-3\\%
  Paired-12-4\\%
  Paired-12-5\\%
  Paired-12-6\\%
  Paired-12-7\\%
  Paired-12-8\\%
  Paired-12-9\\%
  Paired-12-10\\%
  Paired-12-11\\%
  Paired-12-12\\%
}
\pgfplotscreateplotcyclelist{Accent-3}{%
  Accent-3-1\\%
  Accent-3-2\\%
  Accent-3-3\\%
}
\pgfplotscreateplotcyclelist{Accent-4}{%
  Accent-4-1\\%
  Accent-4-2\\%
  Accent-4-3\\%
  Accent-4-4\\%
}
\pgfplotscreateplotcyclelist{Accent-5}{%
  Accent-5-1\\%
  Accent-5-2\\%
  Accent-5-3\\%
  Accent-5-4\\%
  Accent-5-5\\%
}
\pgfplotscreateplotcyclelist{Accent-6}{%
  Accent-6-1\\%
  Accent-6-2\\%
  Accent-6-3\\%
  Accent-6-4\\%
  Accent-6-5\\%
  Accent-6-6\\%
}
\pgfplotscreateplotcyclelist{Accent-7}{%
  Accent-7-1\\%
  Accent-7-2\\%
  Accent-7-3\\%
  Accent-7-4\\%
  Accent-7-5\\%
  Accent-7-6\\%
  Accent-7-7\\%
}
\pgfplotscreateplotcyclelist{Accent-8}{%
  Accent-8-1\\%
  Accent-8-2\\%
  Accent-8-3\\%
  Accent-8-4\\%
  Accent-8-5\\%
  Accent-8-6\\%
  Accent-8-7\\%
  Accent-8-8\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-3}{%
 YlGn-3-1!70!black, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70!black, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70!black, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-4}{%
 YlGn-4-1!70!black, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70!black, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70!black, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70!black, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-5}{%
 YlGn-5-1!70!black, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70!black, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70!black, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70!black, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70!black, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-6}{%
 YlGn-6-1!70!black, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70!black, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70!black, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70!black, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70!black, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70!black, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-7}{%
 YlGn-7-1!70!black, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70!black, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70!black, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70!black, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70!black, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70!black, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70!black, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-8}{%
 YlGn-8-1!70!black, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70!black, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70!black, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70!black, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70!black, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70!black, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70!black, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70!black, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-9}{%
 YlGn-9-1!70!black, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70!black, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70!black, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70!black, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70!black, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70!black, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70!black, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70!black, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70!black, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-3}{%
 YlGnBu-3-1!70!black, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70!black, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70!black, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-4}{%
 YlGnBu-4-1!70!black, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70!black, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70!black, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70!black, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-5}{%
 YlGnBu-5-1!70!black, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70!black, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70!black, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70!black, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70!black, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-6}{%
 YlGnBu-6-1!70!black, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70!black, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70!black, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70!black, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70!black, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70!black, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-7}{%
 YlGnBu-7-1!70!black, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70!black, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70!black, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70!black, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70!black, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70!black, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70!black, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-8}{%
 YlGnBu-8-1!70!black, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70!black, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70!black, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70!black, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70!black, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70!black, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70!black, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70!black, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-9}{%
 YlGnBu-9-1!70!black, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70!black, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70!black, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70!black, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70!black, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70!black, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70!black, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70!black, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70!black, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-3}{%
 GnBu-3-1!70!black, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70!black, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70!black, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-4}{%
 GnBu-4-1!70!black, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70!black, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70!black, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70!black, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-5}{%
 GnBu-5-1!70!black, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70!black, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70!black, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70!black, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70!black, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-6}{%
 GnBu-6-1!70!black, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70!black, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70!black, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70!black, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70!black, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70!black, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-7}{%
 GnBu-7-1!70!black, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70!black, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70!black, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70!black, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70!black, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70!black, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70!black, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-8}{%
 GnBu-8-1!70!black, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70!black, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70!black, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70!black, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70!black, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70!black, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70!black, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70!black, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-9}{%
 GnBu-9-1!70!black, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70!black, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70!black, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70!black, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70!black, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70!black, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70!black, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70!black, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70!black, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-3}{%
 BuGn-3-1!70!black, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70!black, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70!black, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-4}{%
 BuGn-4-1!70!black, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70!black, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70!black, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70!black, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-5}{%
 BuGn-5-1!70!black, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70!black, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70!black, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70!black, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70!black, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-6}{%
 BuGn-6-1!70!black, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70!black, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70!black, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70!black, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70!black, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70!black, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-7}{%
 BuGn-7-1!70!black, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70!black, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70!black, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70!black, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70!black, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70!black, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70!black, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-8}{%
 BuGn-8-1!70!black, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70!black, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70!black, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70!black, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70!black, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70!black, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70!black, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70!black, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-9}{%
 BuGn-9-1!70!black, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70!black, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70!black, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70!black, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70!black, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70!black, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70!black, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70!black, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70!black, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-3}{%
 PuBuGn-3-1!70!black, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70!black, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70!black, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-4}{%
 PuBuGn-4-1!70!black, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70!black, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70!black, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70!black, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-5}{%
 PuBuGn-5-1!70!black, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70!black, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70!black, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70!black, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70!black, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-6}{%
 PuBuGn-6-1!70!black, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70!black, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70!black, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70!black, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70!black, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70!black, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-7}{%
 PuBuGn-7-1!70!black, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70!black, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70!black, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70!black, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70!black, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70!black, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70!black, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-8}{%
 PuBuGn-8-1!70!black, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70!black, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70!black, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70!black, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70!black, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70!black, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70!black, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70!black, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-9}{%
 PuBuGn-9-1!70!black, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70!black, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70!black, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70!black, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70!black, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70!black, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70!black, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70!black, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70!black, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-3}{%
 PuBu-3-1!70!black, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70!black, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70!black, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-4}{%
 PuBu-4-1!70!black, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70!black, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70!black, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70!black, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-5}{%
 PuBu-5-1!70!black, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70!black, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70!black, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70!black, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70!black, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-6}{%
 PuBu-6-1!70!black, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70!black, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70!black, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70!black, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70!black, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70!black, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-7}{%
 PuBu-7-1!70!black, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70!black, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70!black, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70!black, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70!black, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70!black, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70!black, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-8}{%
 PuBu-8-1!70!black, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70!black, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70!black, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70!black, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70!black, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70!black, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70!black, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70!black, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-9}{%
 PuBu-9-1!70!black, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70!black, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70!black, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70!black, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70!black, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70!black, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70!black, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70!black, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70!black, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-3}{%
 BuPu-3-1!70!black, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70!black, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70!black, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-4}{%
 BuPu-4-1!70!black, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70!black, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70!black, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70!black, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-5}{%
 BuPu-5-1!70!black, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70!black, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70!black, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70!black, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70!black, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-6}{%
 BuPu-6-1!70!black, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70!black, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70!black, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70!black, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70!black, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70!black, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-7}{%
 BuPu-7-1!70!black, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70!black, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70!black, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70!black, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70!black, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70!black, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70!black, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-8}{%
 BuPu-8-1!70!black, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70!black, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70!black, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70!black, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70!black, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70!black, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70!black, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70!black, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-9}{%
 BuPu-9-1!70!black, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70!black, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70!black, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70!black, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70!black, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70!black, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70!black, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70!black, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70!black, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-3}{%
 RdPu-3-1!70!black, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70!black, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70!black, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-4}{%
 RdPu-4-1!70!black, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70!black, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70!black, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70!black, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-5}{%
 RdPu-5-1!70!black, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70!black, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70!black, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70!black, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70!black, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-6}{%
 RdPu-6-1!70!black, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70!black, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70!black, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70!black, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70!black, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70!black, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-7}{%
 RdPu-7-1!70!black, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70!black, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70!black, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70!black, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70!black, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70!black, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70!black, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-8}{%
 RdPu-8-1!70!black, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70!black, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70!black, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70!black, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70!black, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70!black, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70!black, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70!black, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-9}{%
 RdPu-9-1!70!black, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70!black, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70!black, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70!black, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70!black, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70!black, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70!black, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70!black, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70!black, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-3}{%
 PuRd-3-1!70!black, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70!black, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70!black, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-4}{%
 PuRd-4-1!70!black, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70!black, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70!black, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70!black, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-5}{%
 PuRd-5-1!70!black, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70!black, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70!black, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70!black, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70!black, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-6}{%
 PuRd-6-1!70!black, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70!black, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70!black, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70!black, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70!black, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70!black, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-7}{%
 PuRd-7-1!70!black, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70!black, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70!black, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70!black, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70!black, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70!black, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70!black, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-8}{%
 PuRd-8-1!70!black, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70!black, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70!black, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70!black, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70!black, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70!black, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70!black, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70!black, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-9}{%
 PuRd-9-1!70!black, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70!black, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70!black, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70!black, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70!black, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70!black, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70!black, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70!black, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70!black, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-3}{%
 OrRd-3-1!70!black, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70!black, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70!black, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-4}{%
 OrRd-4-1!70!black, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70!black, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70!black, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70!black, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-5}{%
 OrRd-5-1!70!black, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70!black, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70!black, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70!black, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70!black, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-6}{%
 OrRd-6-1!70!black, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70!black, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70!black, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70!black, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70!black, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70!black, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-7}{%
 OrRd-7-1!70!black, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70!black, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70!black, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70!black, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70!black, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70!black, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70!black, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-8}{%
 OrRd-8-1!70!black, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70!black, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70!black, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70!black, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70!black, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70!black, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70!black, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70!black, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-9}{%
 OrRd-9-1!70!black, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70!black, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70!black, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70!black, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70!black, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70!black, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70!black, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70!black, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70!black, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-3}{%
 YlOrRd-3-1!70!black, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70!black, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70!black, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-4}{%
 YlOrRd-4-1!70!black, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70!black, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70!black, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70!black, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-5}{%
 YlOrRd-5-1!70!black, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70!black, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70!black, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70!black, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70!black, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-6}{%
 YlOrRd-6-1!70!black, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70!black, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70!black, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70!black, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70!black, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70!black, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-7}{%
 YlOrRd-7-1!70!black, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70!black, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70!black, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70!black, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70!black, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70!black, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70!black, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-8}{%
 YlOrRd-8-1!70!black, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70!black, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70!black, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70!black, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70!black, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70!black, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70!black, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70!black, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-9}{%
 YlOrRd-9-1!70!black, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70!black, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70!black, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70!black, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70!black, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70!black, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70!black, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70!black, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70!black, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-3}{%
 YlOrBr-3-1!70!black, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70!black, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70!black, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-4}{%
 YlOrBr-4-1!70!black, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70!black, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70!black, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70!black, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-5}{%
 YlOrBr-5-1!70!black, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70!black, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70!black, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70!black, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70!black, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-6}{%
 YlOrBr-6-1!70!black, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70!black, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70!black, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70!black, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70!black, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70!black, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-7}{%
 YlOrBr-7-1!70!black, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70!black, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70!black, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70!black, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70!black, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70!black, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70!black, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-8}{%
 YlOrBr-8-1!70!black, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70!black, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70!black, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70!black, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70!black, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70!black, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70!black, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70!black, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-9}{%
 YlOrBr-9-1!70!black, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70!black, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70!black, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70!black, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70!black, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70!black, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70!black, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70!black, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70!black, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-3}{%
 Purples-3-1!70!black, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70!black, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70!black, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-4}{%
 Purples-4-1!70!black, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70!black, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70!black, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70!black, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-5}{%
 Purples-5-1!70!black, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70!black, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70!black, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70!black, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70!black, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-6}{%
 Purples-6-1!70!black, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70!black, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70!black, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70!black, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70!black, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70!black, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-7}{%
 Purples-7-1!70!black, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70!black, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70!black, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70!black, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70!black, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70!black, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70!black, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-8}{%
 Purples-8-1!70!black, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70!black, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70!black, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70!black, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70!black, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70!black, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70!black, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70!black, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-9}{%
 Purples-9-1!70!black, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70!black, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70!black, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70!black, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70!black, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70!black, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70!black, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70!black, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70!black, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-3}{%
 Blues-3-1!70!black, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70!black, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70!black, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-4}{%
 Blues-4-1!70!black, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70!black, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70!black, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70!black, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-5}{%
 Blues-5-1!70!black, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70!black, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70!black, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70!black, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70!black, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-6}{%
 Blues-6-1!70!black, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70!black, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70!black, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70!black, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70!black, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70!black, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-7}{%
 Blues-7-1!70!black, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70!black, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70!black, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70!black, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70!black, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70!black, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70!black, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-8}{%
 Blues-8-1!70!black, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70!black, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70!black, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70!black, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70!black, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70!black, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70!black, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70!black, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-9}{%
 Blues-9-1!70!black, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70!black, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70!black, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70!black, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70!black, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70!black, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70!black, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70!black, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70!black, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-3}{%
 Greens-3-1!70!black, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70!black, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70!black, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-4}{%
 Greens-4-1!70!black, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70!black, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70!black, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70!black, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-5}{%
 Greens-5-1!70!black, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70!black, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70!black, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70!black, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70!black, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-6}{%
 Greens-6-1!70!black, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70!black, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70!black, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70!black, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70!black, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70!black, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-7}{%
 Greens-7-1!70!black, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70!black, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70!black, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70!black, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70!black, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70!black, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70!black, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-8}{%
 Greens-8-1!70!black, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70!black, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70!black, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70!black, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70!black, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70!black, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70!black, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70!black, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-9}{%
 Greens-9-1!70!black, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70!black, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70!black, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70!black, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70!black, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70!black, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70!black, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70!black, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70!black, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-3}{%
 Oranges-3-1!70!black, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70!black, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70!black, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-4}{%
 Oranges-4-1!70!black, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70!black, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70!black, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70!black, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-5}{%
 Oranges-5-1!70!black, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70!black, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70!black, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70!black, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70!black, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-6}{%
 Oranges-6-1!70!black, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70!black, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70!black, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70!black, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70!black, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70!black, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-7}{%
 Oranges-7-1!70!black, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70!black, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70!black, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70!black, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70!black, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70!black, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70!black, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-8}{%
 Oranges-8-1!70!black, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70!black, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70!black, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70!black, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70!black, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70!black, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70!black, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70!black, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-9}{%
 Oranges-9-1!70!black, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70!black, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70!black, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70!black, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70!black, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70!black, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70!black, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70!black, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70!black, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-3}{%
 Reds-3-1!70!black, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70!black, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70!black, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-4}{%
 Reds-4-1!70!black, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70!black, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70!black, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70!black, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-5}{%
 Reds-5-1!70!black, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70!black, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70!black, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70!black, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70!black, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-6}{%
 Reds-6-1!70!black, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70!black, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70!black, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70!black, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70!black, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70!black, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-7}{%
 Reds-7-1!70!black, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70!black, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70!black, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70!black, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70!black, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70!black, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70!black, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-8}{%
 Reds-8-1!70!black, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70!black, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70!black, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70!black, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70!black, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70!black, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70!black, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70!black, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-9}{%
 Reds-9-1!70!black, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70!black, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70!black, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70!black, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70!black, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70!black, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70!black, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70!black, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70!black, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-3}{%
 Greys-3-1!70!black, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70!black, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70!black, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-4}{%
 Greys-4-1!70!black, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70!black, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70!black, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70!black, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-5}{%
 Greys-5-1!70!black, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70!black, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70!black, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70!black, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70!black, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-6}{%
 Greys-6-1!70!black, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70!black, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70!black, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70!black, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70!black, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70!black, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-7}{%
 Greys-7-1!70!black, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70!black, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70!black, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70!black, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70!black, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70!black, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70!black, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-8}{%
 Greys-8-1!70!black, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70!black, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70!black, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70!black, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70!black, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70!black, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70!black, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70!black, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-9}{%
 Greys-9-1!70!black, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70!black, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70!black, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70!black, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70!black, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70!black, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70!black, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70!black, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70!black, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-3}{%
 PuOr-3-1!70!black, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70!black, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70!black, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-4}{%
 PuOr-4-1!70!black, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70!black, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70!black, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70!black, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-5}{%
 PuOr-5-1!70!black, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70!black, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70!black, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70!black, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70!black, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-6}{%
 PuOr-6-1!70!black, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70!black, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70!black, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70!black, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70!black, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70!black, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-7}{%
 PuOr-7-1!70!black, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70!black, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70!black, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70!black, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70!black, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70!black, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70!black, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-8}{%
 PuOr-8-1!70!black, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70!black, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70!black, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70!black, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70!black, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70!black, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70!black, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70!black, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-9}{%
 PuOr-9-1!70!black, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70!black, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70!black, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70!black, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70!black, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70!black, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70!black, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70!black, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70!black, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-10}{%
 PuOr-10-1!70!black, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70!black, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70!black, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70!black, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70!black, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70!black, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70!black, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70!black, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70!black, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70!black, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-11}{%
 PuOr-11-1!70!black, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70!black, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70!black, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70!black, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70!black, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70!black, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70!black, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70!black, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70!black, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70!black, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-3}{%
 BrBG-3-1!70!black, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70!black, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70!black, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-4}{%
 BrBG-4-1!70!black, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70!black, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70!black, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70!black, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-5}{%
 BrBG-5-1!70!black, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70!black, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70!black, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70!black, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70!black, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-6}{%
 BrBG-6-1!70!black, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70!black, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70!black, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70!black, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70!black, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70!black, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-7}{%
 BrBG-7-1!70!black, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70!black, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70!black, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70!black, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70!black, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70!black, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70!black, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-8}{%
 BrBG-8-1!70!black, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70!black, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70!black, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70!black, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70!black, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70!black, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70!black, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70!black, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-9}{%
 BrBG-9-1!70!black, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70!black, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70!black, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70!black, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70!black, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70!black, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70!black, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70!black, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70!black, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-10}{%
 BrBG-10-1!70!black, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70!black, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70!black, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70!black, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70!black, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70!black, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70!black, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70!black, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70!black, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70!black, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-11}{%
 BrBG-11-1!70!black, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70!black, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70!black, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70!black, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70!black, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70!black, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70!black, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70!black, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70!black, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70!black, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-3}{%
 PRGn-3-1!70!black, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70!black, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70!black, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-4}{%
 PRGn-4-1!70!black, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70!black, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70!black, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70!black, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-5}{%
 PRGn-5-1!70!black, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70!black, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70!black, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70!black, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70!black, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-6}{%
 PRGn-6-1!70!black, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70!black, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70!black, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70!black, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70!black, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70!black, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-7}{%
 PRGn-7-1!70!black, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70!black, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70!black, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70!black, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70!black, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70!black, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70!black, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-8}{%
 PRGn-8-1!70!black, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70!black, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70!black, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70!black, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70!black, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70!black, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70!black, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70!black, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-9}{%
 PRGn-9-1!70!black, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70!black, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70!black, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70!black, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70!black, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70!black, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70!black, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70!black, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70!black, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-10}{%
 PRGn-10-1!70!black, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70!black, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70!black, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70!black, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70!black, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70!black, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70!black, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70!black, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70!black, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70!black, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-11}{%
 PRGn-11-1!70!black, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70!black, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70!black, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70!black, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70!black, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70!black, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70!black, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70!black, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70!black, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70!black, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-3}{%
 PiYG-3-1!70!black, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70!black, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70!black, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-4}{%
 PiYG-4-1!70!black, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70!black, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70!black, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70!black, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-5}{%
 PiYG-5-1!70!black, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70!black, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70!black, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70!black, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70!black, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-6}{%
 PiYG-6-1!70!black, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70!black, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70!black, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70!black, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70!black, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70!black, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-7}{%
 PiYG-7-1!70!black, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70!black, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70!black, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70!black, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70!black, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70!black, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70!black, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-8}{%
 PiYG-8-1!70!black, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70!black, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70!black, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70!black, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70!black, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70!black, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70!black, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70!black, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-9}{%
 PiYG-9-1!70!black, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70!black, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70!black, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70!black, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70!black, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70!black, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70!black, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70!black, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70!black, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-10}{%
 PiYG-10-1!70!black, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70!black, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70!black, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70!black, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70!black, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70!black, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70!black, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70!black, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70!black, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70!black, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-11}{%
 PiYG-11-1!70!black, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70!black, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70!black, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70!black, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70!black, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70!black, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70!black, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70!black, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70!black, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70!black, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-3}{%
 RdBu-3-1!70!black, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70!black, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70!black, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-4}{%
 RdBu-4-1!70!black, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70!black, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70!black, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70!black, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-5}{%
 RdBu-5-1!70!black, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70!black, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70!black, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70!black, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70!black, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-6}{%
 RdBu-6-1!70!black, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70!black, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70!black, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70!black, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70!black, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70!black, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-7}{%
 RdBu-7-1!70!black, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70!black, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70!black, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70!black, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70!black, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70!black, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70!black, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-8}{%
 RdBu-8-1!70!black, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70!black, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70!black, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70!black, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70!black, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70!black, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70!black, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70!black, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-9}{%
 RdBu-9-1!70!black, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70!black, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70!black, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70!black, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70!black, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70!black, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70!black, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70!black, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70!black, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-10}{%
 RdBu-10-1!70!black, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70!black, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70!black, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70!black, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70!black, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70!black, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70!black, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70!black, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70!black, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70!black, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-11}{%
 RdBu-11-1!70!black, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70!black, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70!black, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70!black, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70!black, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70!black, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70!black, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70!black, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70!black, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70!black, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-3}{%
 RdGy-3-1!70!black, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70!black, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70!black, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-4}{%
 RdGy-4-1!70!black, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70!black, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70!black, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70!black, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-5}{%
 RdGy-5-1!70!black, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70!black, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70!black, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70!black, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70!black, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-6}{%
 RdGy-6-1!70!black, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70!black, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70!black, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70!black, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70!black, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70!black, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-7}{%
 RdGy-7-1!70!black, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70!black, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70!black, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70!black, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70!black, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70!black, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70!black, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-8}{%
 RdGy-8-1!70!black, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70!black, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70!black, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70!black, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70!black, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70!black, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70!black, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70!black, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-9}{%
 RdGy-9-1!70!black, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70!black, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70!black, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70!black, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70!black, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70!black, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70!black, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70!black, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70!black, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-10}{%
 RdGy-10-1!70!black, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70!black, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70!black, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70!black, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70!black, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70!black, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70!black, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70!black, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70!black, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70!black, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-11}{%
 RdGy-11-1!70!black, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70!black, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70!black, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70!black, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70!black, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70!black, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70!black, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70!black, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70!black, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70!black, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-3}{%
 RdYlBu-3-1!70!black, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70!black, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70!black, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-4}{%
 RdYlBu-4-1!70!black, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70!black, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70!black, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70!black, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-5}{%
 RdYlBu-5-1!70!black, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70!black, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70!black, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70!black, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70!black, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-6}{%
 RdYlBu-6-1!70!black, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70!black, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70!black, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70!black, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70!black, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70!black, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-7}{%
 RdYlBu-7-1!70!black, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70!black, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70!black, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70!black, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70!black, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70!black, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70!black, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-8}{%
 RdYlBu-8-1!70!black, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70!black, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70!black, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70!black, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70!black, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70!black, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70!black, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70!black, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-9}{%
 RdYlBu-9-1!70!black, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70!black, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70!black, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70!black, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70!black, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70!black, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70!black, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70!black, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70!black, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-10}{%
 RdYlBu-10-1!70!black, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70!black, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70!black, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70!black, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70!black, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70!black, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70!black, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70!black, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70!black, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70!black, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-11}{%
 RdYlBu-11-1!70!black, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70!black, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70!black, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70!black, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70!black, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70!black, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70!black, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70!black, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70!black, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70!black, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-3}{%
 Spectral-3-1!70!black, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70!black, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70!black, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-4}{%
 Spectral-4-1!70!black, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70!black, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70!black, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70!black, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-5}{%
 Spectral-5-1!70!black, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70!black, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70!black, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70!black, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70!black, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-6}{%
 Spectral-6-1!70!black, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70!black, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70!black, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70!black, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70!black, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70!black, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-7}{%
 Spectral-7-1!70!black, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70!black, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70!black, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70!black, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70!black, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70!black, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70!black, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-8}{%
 Spectral-8-1!70!black, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70!black, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70!black, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70!black, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70!black, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70!black, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70!black, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70!black, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-9}{%
 Spectral-9-1!70!black, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70!black, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70!black, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70!black, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70!black, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70!black, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70!black, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70!black, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70!black, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-10}{%
 Spectral-10-1!70!black, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70!black, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70!black, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70!black, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70!black, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70!black, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70!black, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70!black, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70!black, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70!black, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-11}{%
 Spectral-11-1!70!black, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70!black, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70!black, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70!black, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70!black, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70!black, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70!black, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70!black, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70!black, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70!black, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-3}{%
 RdYlGn-3-1!70!black, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70!black, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70!black, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-4}{%
 RdYlGn-4-1!70!black, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70!black, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70!black, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70!black, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-5}{%
 RdYlGn-5-1!70!black, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70!black, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70!black, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70!black, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70!black, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-6}{%
 RdYlGn-6-1!70!black, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70!black, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70!black, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70!black, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70!black, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70!black, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-7}{%
 RdYlGn-7-1!70!black, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70!black, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70!black, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70!black, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70!black, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70!black, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70!black, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-8}{%
 RdYlGn-8-1!70!black, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70!black, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70!black, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70!black, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70!black, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70!black, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70!black, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70!black, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-9}{%
 RdYlGn-9-1!70!black, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70!black, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70!black, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70!black, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70!black, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70!black, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70!black, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70!black, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70!black, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-10}{%
 RdYlGn-10-1!70!black, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70!black, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70!black, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70!black, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70!black, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70!black, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70!black, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70!black, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70!black, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70!black, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-11}{%
 RdYlGn-11-1!70!black, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70!black, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70!black, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70!black, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70!black, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70!black, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70!black, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70!black, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70!black, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70!black, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-3}{%
 Set3-3-1!70!black, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70!black, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70!black, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-4}{%
 Set3-4-1!70!black, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70!black, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70!black, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70!black, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-5}{%
 Set3-5-1!70!black, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70!black, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70!black, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70!black, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70!black, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-6}{%
 Set3-6-1!70!black, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70!black, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70!black, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70!black, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70!black, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70!black, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-7}{%
 Set3-7-1!70!black, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70!black, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70!black, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70!black, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70!black, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70!black, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70!black, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-8}{%
 Set3-8-1!70!black, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70!black, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70!black, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70!black, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70!black, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70!black, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70!black, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70!black, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-9}{%
 Set3-9-1!70!black, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70!black, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70!black, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70!black, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70!black, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70!black, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70!black, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70!black, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70!black, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-10}{%
 Set3-10-1!70!black, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70!black, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70!black, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70!black, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70!black, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70!black, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70!black, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70!black, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70!black, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70!black, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-11}{%
 Set3-11-1!70!black, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70!black, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70!black, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70!black, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70!black, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70!black, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70!black, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70!black, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70!black, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70!black, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-12}{%
 Set3-12-1!70!black, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70!black, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70!black, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70!black, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70!black, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70!black, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70!black, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70!black, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70!black, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70!black, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-3}{%
 Pastel1-3-1!70!black, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70!black, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70!black, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-4}{%
 Pastel1-4-1!70!black, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70!black, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70!black, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70!black, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-5}{%
 Pastel1-5-1!70!black, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70!black, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70!black, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70!black, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70!black, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-6}{%
 Pastel1-6-1!70!black, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70!black, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70!black, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70!black, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70!black, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70!black, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-7}{%
 Pastel1-7-1!70!black, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70!black, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70!black, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70!black, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70!black, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70!black, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70!black, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-8}{%
 Pastel1-8-1!70!black, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70!black, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70!black, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70!black, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70!black, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70!black, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70!black, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70!black, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-9}{%
 Pastel1-9-1!70!black, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70!black, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70!black, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70!black, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70!black, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70!black, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70!black, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70!black, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70!black, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-3}{%
 Set1-3-1!70!black, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70!black, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70!black, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-4}{%
 Set1-4-1!70!black, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70!black, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70!black, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70!black, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-5}{%
 Set1-5-1!70!black, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70!black, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70!black, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70!black, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70!black, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-6}{%
 Set1-6-1!70!black, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70!black, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70!black, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70!black, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70!black, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70!black, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-7}{%
 Set1-7-1!70!black, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70!black, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70!black, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70!black, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70!black, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70!black, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70!black, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-8}{%
 Set1-8-1!70!black, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70!black, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70!black, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70!black, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70!black, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70!black, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70!black, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70!black, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-9}{%
 Set1-9-1!70!black, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70!black, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70!black, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70!black, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70!black, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70!black, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70!black, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70!black, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70!black, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-3}{%
 Pastel2-3-1!70!black, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70!black, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70!black, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-4}{%
 Pastel2-4-1!70!black, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70!black, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70!black, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70!black, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-5}{%
 Pastel2-5-1!70!black, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70!black, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70!black, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70!black, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70!black, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-6}{%
 Pastel2-6-1!70!black, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70!black, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70!black, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70!black, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70!black, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70!black, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-7}{%
 Pastel2-7-1!70!black, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70!black, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70!black, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70!black, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70!black, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70!black, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70!black, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-8}{%
 Pastel2-8-1!70!black, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70!black, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70!black, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70!black, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70!black, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70!black, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70!black, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70!black, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-3}{%
 Set2-3-1!70!black, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70!black, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70!black, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-4}{%
 Set2-4-1!70!black, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70!black, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70!black, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70!black, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-5}{%
 Set2-5-1!70!black, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70!black, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70!black, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70!black, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70!black, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-6}{%
 Set2-6-1!70!black, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70!black, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70!black, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70!black, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70!black, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70!black, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-7}{%
 Set2-7-1!70!black, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70!black, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70!black, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70!black, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70!black, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70!black, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70!black, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-8}{%
 Set2-8-1!70!black, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70!black, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70!black, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70!black, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70!black, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70!black, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70!black, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70!black, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-3}{%
 Dark2-3-1!70!black, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70!black, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70!black, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-4}{%
 Dark2-4-1!70!black, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70!black, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70!black, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70!black, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-5}{%
 Dark2-5-1!70!black, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70!black, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70!black, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70!black, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70!black, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-6}{%
 Dark2-6-1!70!black, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70!black, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70!black, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70!black, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70!black, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70!black, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-7}{%
 Dark2-7-1!70!black, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70!black, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70!black, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70!black, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70!black, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70!black, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70!black, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-8}{%
 Dark2-8-1!70!black, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70!black, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70!black, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70!black, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70!black, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70!black, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70!black, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70!black, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-3}{%
 Paired-3-1!70!black, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70!black, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70!black, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-4}{%
 Paired-4-1!70!black, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70!black, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70!black, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70!black, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-5}{%
 Paired-5-1!70!black, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70!black, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70!black, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70!black, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70!black, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-6}{%
 Paired-6-1!70!black, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70!black, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70!black, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70!black, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70!black, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70!black, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-7}{%
 Paired-7-1!70!black, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70!black, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70!black, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70!black, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70!black, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70!black, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70!black, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-8}{%
 Paired-8-1!70!black, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70!black, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70!black, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70!black, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70!black, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70!black, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70!black, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70!black, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-9}{%
 Paired-9-1!70!black, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70!black, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70!black, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70!black, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70!black, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70!black, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70!black, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70!black, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70!black, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-10}{%
 Paired-10-1!70!black, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70!black, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70!black, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70!black, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70!black, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70!black, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70!black, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70!black, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70!black, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70!black, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-11}{%
 Paired-11-1!70!black, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70!black, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70!black, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70!black, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70!black, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70!black, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70!black, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70!black, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70!black, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70!black, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-12}{%
 Paired-12-1!70!black, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70!black, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70!black, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70!black, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70!black, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70!black, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70!black, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70!black, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70!black, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70!black, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-3}{%
 Accent-3-1!70!black, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70!black, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70!black, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-4}{%
 Accent-4-1!70!black, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70!black, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70!black, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70!black, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-5}{%
 Accent-5-1!70!black, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70!black, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70!black, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70!black, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70!black, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-6}{%
 Accent-6-1!70!black, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70!black, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70!black, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70!black, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70!black, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70!black, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-7}{%
 Accent-7-1!70!black, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70!black, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70!black, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70!black, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70!black, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70!black, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70!black, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-8}{%
 Accent-8-1!70!black, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70!black, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70!black, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70!black, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70!black, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70!black, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70!black, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70!black, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-3}{%
 YlGn-3-1!70, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-4}{%
 YlGn-4-1!70, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-5}{%
 YlGn-5-1!70, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-6}{%
 YlGn-6-1!70, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-7}{%
 YlGn-7-1!70, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-8}{%
 YlGn-8-1!70, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-9}{%
 YlGn-9-1!70, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-3}{%
 YlGnBu-3-1!70, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-4}{%
 YlGnBu-4-1!70, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-5}{%
 YlGnBu-5-1!70, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-6}{%
 YlGnBu-6-1!70, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-7}{%
 YlGnBu-7-1!70, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-8}{%
 YlGnBu-8-1!70, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-9}{%
 YlGnBu-9-1!70, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-3}{%
 GnBu-3-1!70, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-4}{%
 GnBu-4-1!70, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-5}{%
 GnBu-5-1!70, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-6}{%
 GnBu-6-1!70, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-7}{%
 GnBu-7-1!70, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-8}{%
 GnBu-8-1!70, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-9}{%
 GnBu-9-1!70, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-3}{%
 BuGn-3-1!70, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-4}{%
 BuGn-4-1!70, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-5}{%
 BuGn-5-1!70, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-6}{%
 BuGn-6-1!70, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-7}{%
 BuGn-7-1!70, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-8}{%
 BuGn-8-1!70, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-9}{%
 BuGn-9-1!70, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-3}{%
 PuBuGn-3-1!70, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-4}{%
 PuBuGn-4-1!70, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-5}{%
 PuBuGn-5-1!70, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-6}{%
 PuBuGn-6-1!70, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-7}{%
 PuBuGn-7-1!70, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-8}{%
 PuBuGn-8-1!70, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-9}{%
 PuBuGn-9-1!70, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-3}{%
 PuBu-3-1!70, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-4}{%
 PuBu-4-1!70, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-5}{%
 PuBu-5-1!70, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-6}{%
 PuBu-6-1!70, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-7}{%
 PuBu-7-1!70, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-8}{%
 PuBu-8-1!70, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-9}{%
 PuBu-9-1!70, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-3}{%
 BuPu-3-1!70, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-4}{%
 BuPu-4-1!70, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-5}{%
 BuPu-5-1!70, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-6}{%
 BuPu-6-1!70, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-7}{%
 BuPu-7-1!70, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-8}{%
 BuPu-8-1!70, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-9}{%
 BuPu-9-1!70, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-3}{%
 RdPu-3-1!70, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-4}{%
 RdPu-4-1!70, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-5}{%
 RdPu-5-1!70, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-6}{%
 RdPu-6-1!70, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-7}{%
 RdPu-7-1!70, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-8}{%
 RdPu-8-1!70, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-9}{%
 RdPu-9-1!70, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-3}{%
 PuRd-3-1!70, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-4}{%
 PuRd-4-1!70, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-5}{%
 PuRd-5-1!70, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-6}{%
 PuRd-6-1!70, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-7}{%
 PuRd-7-1!70, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-8}{%
 PuRd-8-1!70, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-9}{%
 PuRd-9-1!70, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-3}{%
 OrRd-3-1!70, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-4}{%
 OrRd-4-1!70, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-5}{%
 OrRd-5-1!70, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-6}{%
 OrRd-6-1!70, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-7}{%
 OrRd-7-1!70, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-8}{%
 OrRd-8-1!70, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-9}{%
 OrRd-9-1!70, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-3}{%
 YlOrRd-3-1!70, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-4}{%
 YlOrRd-4-1!70, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-5}{%
 YlOrRd-5-1!70, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-6}{%
 YlOrRd-6-1!70, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-7}{%
 YlOrRd-7-1!70, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-8}{%
 YlOrRd-8-1!70, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-9}{%
 YlOrRd-9-1!70, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-3}{%
 YlOrBr-3-1!70, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-4}{%
 YlOrBr-4-1!70, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-5}{%
 YlOrBr-5-1!70, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-6}{%
 YlOrBr-6-1!70, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-7}{%
 YlOrBr-7-1!70, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-8}{%
 YlOrBr-8-1!70, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-9}{%
 YlOrBr-9-1!70, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-3}{%
 Purples-3-1!70, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-4}{%
 Purples-4-1!70, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-5}{%
 Purples-5-1!70, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-6}{%
 Purples-6-1!70, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-7}{%
 Purples-7-1!70, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-8}{%
 Purples-8-1!70, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-9}{%
 Purples-9-1!70, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-3}{%
 Blues-3-1!70, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-4}{%
 Blues-4-1!70, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-5}{%
 Blues-5-1!70, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-6}{%
 Blues-6-1!70, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-7}{%
 Blues-7-1!70, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-8}{%
 Blues-8-1!70, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-9}{%
 Blues-9-1!70, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-3}{%
 Greens-3-1!70, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-4}{%
 Greens-4-1!70, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-5}{%
 Greens-5-1!70, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-6}{%
 Greens-6-1!70, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-7}{%
 Greens-7-1!70, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-8}{%
 Greens-8-1!70, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-9}{%
 Greens-9-1!70, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-3}{%
 Oranges-3-1!70, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-4}{%
 Oranges-4-1!70, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-5}{%
 Oranges-5-1!70, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-6}{%
 Oranges-6-1!70, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-7}{%
 Oranges-7-1!70, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-8}{%
 Oranges-8-1!70, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-9}{%
 Oranges-9-1!70, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-3}{%
 Reds-3-1!70, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-4}{%
 Reds-4-1!70, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-5}{%
 Reds-5-1!70, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-6}{%
 Reds-6-1!70, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-7}{%
 Reds-7-1!70, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-8}{%
 Reds-8-1!70, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-9}{%
 Reds-9-1!70, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-3}{%
 Greys-3-1!70, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-4}{%
 Greys-4-1!70, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-5}{%
 Greys-5-1!70, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-6}{%
 Greys-6-1!70, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-7}{%
 Greys-7-1!70, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-8}{%
 Greys-8-1!70, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-9}{%
 Greys-9-1!70, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-3}{%
 PuOr-3-1!70, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-4}{%
 PuOr-4-1!70, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-5}{%
 PuOr-5-1!70, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-6}{%
 PuOr-6-1!70, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-7}{%
 PuOr-7-1!70, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-8}{%
 PuOr-8-1!70, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-9}{%
 PuOr-9-1!70, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-10}{%
 PuOr-10-1!70, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-11}{%
 PuOr-11-1!70, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-3}{%
 BrBG-3-1!70, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-4}{%
 BrBG-4-1!70, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-5}{%
 BrBG-5-1!70, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-6}{%
 BrBG-6-1!70, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-7}{%
 BrBG-7-1!70, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-8}{%
 BrBG-8-1!70, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-9}{%
 BrBG-9-1!70, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-10}{%
 BrBG-10-1!70, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-11}{%
 BrBG-11-1!70, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-3}{%
 PRGn-3-1!70, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-4}{%
 PRGn-4-1!70, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-5}{%
 PRGn-5-1!70, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-6}{%
 PRGn-6-1!70, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-7}{%
 PRGn-7-1!70, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-8}{%
 PRGn-8-1!70, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-9}{%
 PRGn-9-1!70, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-10}{%
 PRGn-10-1!70, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-11}{%
 PRGn-11-1!70, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-3}{%
 PiYG-3-1!70, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-4}{%
 PiYG-4-1!70, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-5}{%
 PiYG-5-1!70, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-6}{%
 PiYG-6-1!70, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-7}{%
 PiYG-7-1!70, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-8}{%
 PiYG-8-1!70, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-9}{%
 PiYG-9-1!70, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-10}{%
 PiYG-10-1!70, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-11}{%
 PiYG-11-1!70, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-3}{%
 RdBu-3-1!70, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-4}{%
 RdBu-4-1!70, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-5}{%
 RdBu-5-1!70, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-6}{%
 RdBu-6-1!70, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-7}{%
 RdBu-7-1!70, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-8}{%
 RdBu-8-1!70, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-9}{%
 RdBu-9-1!70, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-10}{%
 RdBu-10-1!70, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-11}{%
 RdBu-11-1!70, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-3}{%
 RdGy-3-1!70, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-4}{%
 RdGy-4-1!70, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-5}{%
 RdGy-5-1!70, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-6}{%
 RdGy-6-1!70, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-7}{%
 RdGy-7-1!70, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-8}{%
 RdGy-8-1!70, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-9}{%
 RdGy-9-1!70, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-10}{%
 RdGy-10-1!70, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-11}{%
 RdGy-11-1!70, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-3}{%
 RdYlBu-3-1!70, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-4}{%
 RdYlBu-4-1!70, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-5}{%
 RdYlBu-5-1!70, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-6}{%
 RdYlBu-6-1!70, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-7}{%
 RdYlBu-7-1!70, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-8}{%
 RdYlBu-8-1!70, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-9}{%
 RdYlBu-9-1!70, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-10}{%
 RdYlBu-10-1!70, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-11}{%
 RdYlBu-11-1!70, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-3}{%
 Spectral-3-1!70, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-4}{%
 Spectral-4-1!70, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-5}{%
 Spectral-5-1!70, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-6}{%
 Spectral-6-1!70, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-7}{%
 Spectral-7-1!70, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-8}{%
 Spectral-8-1!70, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-9}{%
 Spectral-9-1!70, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-10}{%
 Spectral-10-1!70, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-11}{%
 Spectral-11-1!70, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-3}{%
 RdYlGn-3-1!70, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-4}{%
 RdYlGn-4-1!70, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-5}{%
 RdYlGn-5-1!70, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-6}{%
 RdYlGn-6-1!70, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-7}{%
 RdYlGn-7-1!70, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-8}{%
 RdYlGn-8-1!70, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-9}{%
 RdYlGn-9-1!70, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-10}{%
 RdYlGn-10-1!70, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-11}{%
 RdYlGn-11-1!70, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-3}{%
 Set3-3-1!70, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-4}{%
 Set3-4-1!70, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-5}{%
 Set3-5-1!70, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-6}{%
 Set3-6-1!70, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-7}{%
 Set3-7-1!70, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-8}{%
 Set3-8-1!70, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-9}{%
 Set3-9-1!70, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-10}{%
 Set3-10-1!70, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-11}{%
 Set3-11-1!70, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-12}{%
 Set3-12-1!70, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-3}{%
 Pastel1-3-1!70, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-4}{%
 Pastel1-4-1!70, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-5}{%
 Pastel1-5-1!70, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-6}{%
 Pastel1-6-1!70, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-7}{%
 Pastel1-7-1!70, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-8}{%
 Pastel1-8-1!70, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-9}{%
 Pastel1-9-1!70, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-3}{%
 Set1-3-1!70, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-4}{%
 Set1-4-1!70, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-5}{%
 Set1-5-1!70, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-6}{%
 Set1-6-1!70, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-7}{%
 Set1-7-1!70, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-8}{%
 Set1-8-1!70, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-9}{%
 Set1-9-1!70, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-3}{%
 Pastel2-3-1!70, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-4}{%
 Pastel2-4-1!70, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-5}{%
 Pastel2-5-1!70, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-6}{%
 Pastel2-6-1!70, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-7}{%
 Pastel2-7-1!70, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-8}{%
 Pastel2-8-1!70, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-3}{%
 Set2-3-1!70, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-4}{%
 Set2-4-1!70, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-5}{%
 Set2-5-1!70, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-6}{%
 Set2-6-1!70, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-7}{%
 Set2-7-1!70, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-8}{%
 Set2-8-1!70, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-3}{%
 Dark2-3-1!70, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-4}{%
 Dark2-4-1!70, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-5}{%
 Dark2-5-1!70, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-6}{%
 Dark2-6-1!70, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-7}{%
 Dark2-7-1!70, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-8}{%
 Dark2-8-1!70, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-3}{%
 Paired-3-1!70, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-4}{%
 Paired-4-1!70, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-5}{%
 Paired-5-1!70, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-6}{%
 Paired-6-1!70, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-7}{%
 Paired-7-1!70, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-8}{%
 Paired-8-1!70, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-9}{%
 Paired-9-1!70, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-10}{%
 Paired-10-1!70, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-11}{%
 Paired-11-1!70, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-12}{%
 Paired-12-1!70, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-3}{%
 Accent-3-1!70, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-4}{%
 Accent-4-1!70, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-5}{%
 Accent-5-1!70, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-6}{%
 Accent-6-1!70, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-7}{%
 Accent-7-1!70, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-8}{%
 Accent-8-1!70, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-3}{%
 YlGn-3-1,mark=x\\%
 YlGn-3-2,mark=+\\%
 YlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-4}{%
 YlGn-4-1,mark=x\\%
 YlGn-4-2,mark=+\\%
 YlGn-4-3,mark=-\\%
 YlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-5}{%
 YlGn-5-1,mark=x\\%
 YlGn-5-2,mark=+\\%
 YlGn-5-3,mark=-\\%
 YlGn-5-4,mark=|\\%
 YlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-6}{%
 YlGn-6-1,mark=x\\%
 YlGn-6-2,mark=+\\%
 YlGn-6-3,mark=-\\%
 YlGn-6-4,mark=|\\%
 YlGn-6-5,mark=asterisk\\%
 YlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-7}{%
 YlGn-7-1,mark=x\\%
 YlGn-7-2,mark=+\\%
 YlGn-7-3,mark=-\\%
 YlGn-7-4,mark=|\\%
 YlGn-7-5,mark=asterisk\\%
 YlGn-7-6,mark=star\\%
 YlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-8}{%
 YlGn-8-1,mark=x\\%
 YlGn-8-2,mark=+\\%
 YlGn-8-3,mark=-\\%
 YlGn-8-4,mark=|\\%
 YlGn-8-5,mark=asterisk\\%
 YlGn-8-6,mark=star\\%
 YlGn-8-7,mark=10-pointed star\\%
 YlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-9}{%
 YlGn-9-1,mark=x\\%
 YlGn-9-2,mark=+\\%
 YlGn-9-3,mark=-\\%
 YlGn-9-4,mark=|\\%
 YlGn-9-5,mark=asterisk\\%
 YlGn-9-6,mark=star\\%
 YlGn-9-7,mark=10-pointed star\\%
 YlGn-9-8,mark=Mercedes star\\%
 YlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-3}{%
 YlGnBu-3-1,mark=x\\%
 YlGnBu-3-2,mark=+\\%
 YlGnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-4}{%
 YlGnBu-4-1,mark=x\\%
 YlGnBu-4-2,mark=+\\%
 YlGnBu-4-3,mark=-\\%
 YlGnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-5}{%
 YlGnBu-5-1,mark=x\\%
 YlGnBu-5-2,mark=+\\%
 YlGnBu-5-3,mark=-\\%
 YlGnBu-5-4,mark=|\\%
 YlGnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-6}{%
 YlGnBu-6-1,mark=x\\%
 YlGnBu-6-2,mark=+\\%
 YlGnBu-6-3,mark=-\\%
 YlGnBu-6-4,mark=|\\%
 YlGnBu-6-5,mark=asterisk\\%
 YlGnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-7}{%
 YlGnBu-7-1,mark=x\\%
 YlGnBu-7-2,mark=+\\%
 YlGnBu-7-3,mark=-\\%
 YlGnBu-7-4,mark=|\\%
 YlGnBu-7-5,mark=asterisk\\%
 YlGnBu-7-6,mark=star\\%
 YlGnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-8}{%
 YlGnBu-8-1,mark=x\\%
 YlGnBu-8-2,mark=+\\%
 YlGnBu-8-3,mark=-\\%
 YlGnBu-8-4,mark=|\\%
 YlGnBu-8-5,mark=asterisk\\%
 YlGnBu-8-6,mark=star\\%
 YlGnBu-8-7,mark=10-pointed star\\%
 YlGnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-9}{%
 YlGnBu-9-1,mark=x\\%
 YlGnBu-9-2,mark=+\\%
 YlGnBu-9-3,mark=-\\%
 YlGnBu-9-4,mark=|\\%
 YlGnBu-9-5,mark=asterisk\\%
 YlGnBu-9-6,mark=star\\%
 YlGnBu-9-7,mark=10-pointed star\\%
 YlGnBu-9-8,mark=Mercedes star\\%
 YlGnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-3}{%
 GnBu-3-1,mark=x\\%
 GnBu-3-2,mark=+\\%
 GnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-4}{%
 GnBu-4-1,mark=x\\%
 GnBu-4-2,mark=+\\%
 GnBu-4-3,mark=-\\%
 GnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-5}{%
 GnBu-5-1,mark=x\\%
 GnBu-5-2,mark=+\\%
 GnBu-5-3,mark=-\\%
 GnBu-5-4,mark=|\\%
 GnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-6}{%
 GnBu-6-1,mark=x\\%
 GnBu-6-2,mark=+\\%
 GnBu-6-3,mark=-\\%
 GnBu-6-4,mark=|\\%
 GnBu-6-5,mark=asterisk\\%
 GnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-7}{%
 GnBu-7-1,mark=x\\%
 GnBu-7-2,mark=+\\%
 GnBu-7-3,mark=-\\%
 GnBu-7-4,mark=|\\%
 GnBu-7-5,mark=asterisk\\%
 GnBu-7-6,mark=star\\%
 GnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-8}{%
 GnBu-8-1,mark=x\\%
 GnBu-8-2,mark=+\\%
 GnBu-8-3,mark=-\\%
 GnBu-8-4,mark=|\\%
 GnBu-8-5,mark=asterisk\\%
 GnBu-8-6,mark=star\\%
 GnBu-8-7,mark=10-pointed star\\%
 GnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-9}{%
 GnBu-9-1,mark=x\\%
 GnBu-9-2,mark=+\\%
 GnBu-9-3,mark=-\\%
 GnBu-9-4,mark=|\\%
 GnBu-9-5,mark=asterisk\\%
 GnBu-9-6,mark=star\\%
 GnBu-9-7,mark=10-pointed star\\%
 GnBu-9-8,mark=Mercedes star\\%
 GnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-3}{%
 BuGn-3-1,mark=x\\%
 BuGn-3-2,mark=+\\%
 BuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-4}{%
 BuGn-4-1,mark=x\\%
 BuGn-4-2,mark=+\\%
 BuGn-4-3,mark=-\\%
 BuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-5}{%
 BuGn-5-1,mark=x\\%
 BuGn-5-2,mark=+\\%
 BuGn-5-3,mark=-\\%
 BuGn-5-4,mark=|\\%
 BuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-6}{%
 BuGn-6-1,mark=x\\%
 BuGn-6-2,mark=+\\%
 BuGn-6-3,mark=-\\%
 BuGn-6-4,mark=|\\%
 BuGn-6-5,mark=asterisk\\%
 BuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-7}{%
 BuGn-7-1,mark=x\\%
 BuGn-7-2,mark=+\\%
 BuGn-7-3,mark=-\\%
 BuGn-7-4,mark=|\\%
 BuGn-7-5,mark=asterisk\\%
 BuGn-7-6,mark=star\\%
 BuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-8}{%
 BuGn-8-1,mark=x\\%
 BuGn-8-2,mark=+\\%
 BuGn-8-3,mark=-\\%
 BuGn-8-4,mark=|\\%
 BuGn-8-5,mark=asterisk\\%
 BuGn-8-6,mark=star\\%
 BuGn-8-7,mark=10-pointed star\\%
 BuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-9}{%
 BuGn-9-1,mark=x\\%
 BuGn-9-2,mark=+\\%
 BuGn-9-3,mark=-\\%
 BuGn-9-4,mark=|\\%
 BuGn-9-5,mark=asterisk\\%
 BuGn-9-6,mark=star\\%
 BuGn-9-7,mark=10-pointed star\\%
 BuGn-9-8,mark=Mercedes star\\%
 BuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-3}{%
 PuBuGn-3-1,mark=x\\%
 PuBuGn-3-2,mark=+\\%
 PuBuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-4}{%
 PuBuGn-4-1,mark=x\\%
 PuBuGn-4-2,mark=+\\%
 PuBuGn-4-3,mark=-\\%
 PuBuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-5}{%
 PuBuGn-5-1,mark=x\\%
 PuBuGn-5-2,mark=+\\%
 PuBuGn-5-3,mark=-\\%
 PuBuGn-5-4,mark=|\\%
 PuBuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-6}{%
 PuBuGn-6-1,mark=x\\%
 PuBuGn-6-2,mark=+\\%
 PuBuGn-6-3,mark=-\\%
 PuBuGn-6-4,mark=|\\%
 PuBuGn-6-5,mark=asterisk\\%
 PuBuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-7}{%
 PuBuGn-7-1,mark=x\\%
 PuBuGn-7-2,mark=+\\%
 PuBuGn-7-3,mark=-\\%
 PuBuGn-7-4,mark=|\\%
 PuBuGn-7-5,mark=asterisk\\%
 PuBuGn-7-6,mark=star\\%
 PuBuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-8}{%
 PuBuGn-8-1,mark=x\\%
 PuBuGn-8-2,mark=+\\%
 PuBuGn-8-3,mark=-\\%
 PuBuGn-8-4,mark=|\\%
 PuBuGn-8-5,mark=asterisk\\%
 PuBuGn-8-6,mark=star\\%
 PuBuGn-8-7,mark=10-pointed star\\%
 PuBuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-9}{%
 PuBuGn-9-1,mark=x\\%
 PuBuGn-9-2,mark=+\\%
 PuBuGn-9-3,mark=-\\%
 PuBuGn-9-4,mark=|\\%
 PuBuGn-9-5,mark=asterisk\\%
 PuBuGn-9-6,mark=star\\%
 PuBuGn-9-7,mark=10-pointed star\\%
 PuBuGn-9-8,mark=Mercedes star\\%
 PuBuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-3}{%
 PuBu-3-1,mark=x\\%
 PuBu-3-2,mark=+\\%
 PuBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-4}{%
 PuBu-4-1,mark=x\\%
 PuBu-4-2,mark=+\\%
 PuBu-4-3,mark=-\\%
 PuBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-5}{%
 PuBu-5-1,mark=x\\%
 PuBu-5-2,mark=+\\%
 PuBu-5-3,mark=-\\%
 PuBu-5-4,mark=|\\%
 PuBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-6}{%
 PuBu-6-1,mark=x\\%
 PuBu-6-2,mark=+\\%
 PuBu-6-3,mark=-\\%
 PuBu-6-4,mark=|\\%
 PuBu-6-5,mark=asterisk\\%
 PuBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-7}{%
 PuBu-7-1,mark=x\\%
 PuBu-7-2,mark=+\\%
 PuBu-7-3,mark=-\\%
 PuBu-7-4,mark=|\\%
 PuBu-7-5,mark=asterisk\\%
 PuBu-7-6,mark=star\\%
 PuBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-8}{%
 PuBu-8-1,mark=x\\%
 PuBu-8-2,mark=+\\%
 PuBu-8-3,mark=-\\%
 PuBu-8-4,mark=|\\%
 PuBu-8-5,mark=asterisk\\%
 PuBu-8-6,mark=star\\%
 PuBu-8-7,mark=10-pointed star\\%
 PuBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-9}{%
 PuBu-9-1,mark=x\\%
 PuBu-9-2,mark=+\\%
 PuBu-9-3,mark=-\\%
 PuBu-9-4,mark=|\\%
 PuBu-9-5,mark=asterisk\\%
 PuBu-9-6,mark=star\\%
 PuBu-9-7,mark=10-pointed star\\%
 PuBu-9-8,mark=Mercedes star\\%
 PuBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-3}{%
 BuPu-3-1,mark=x\\%
 BuPu-3-2,mark=+\\%
 BuPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-4}{%
 BuPu-4-1,mark=x\\%
 BuPu-4-2,mark=+\\%
 BuPu-4-3,mark=-\\%
 BuPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-5}{%
 BuPu-5-1,mark=x\\%
 BuPu-5-2,mark=+\\%
 BuPu-5-3,mark=-\\%
 BuPu-5-4,mark=|\\%
 BuPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-6}{%
 BuPu-6-1,mark=x\\%
 BuPu-6-2,mark=+\\%
 BuPu-6-3,mark=-\\%
 BuPu-6-4,mark=|\\%
 BuPu-6-5,mark=asterisk\\%
 BuPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-7}{%
 BuPu-7-1,mark=x\\%
 BuPu-7-2,mark=+\\%
 BuPu-7-3,mark=-\\%
 BuPu-7-4,mark=|\\%
 BuPu-7-5,mark=asterisk\\%
 BuPu-7-6,mark=star\\%
 BuPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-8}{%
 BuPu-8-1,mark=x\\%
 BuPu-8-2,mark=+\\%
 BuPu-8-3,mark=-\\%
 BuPu-8-4,mark=|\\%
 BuPu-8-5,mark=asterisk\\%
 BuPu-8-6,mark=star\\%
 BuPu-8-7,mark=10-pointed star\\%
 BuPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-9}{%
 BuPu-9-1,mark=x\\%
 BuPu-9-2,mark=+\\%
 BuPu-9-3,mark=-\\%
 BuPu-9-4,mark=|\\%
 BuPu-9-5,mark=asterisk\\%
 BuPu-9-6,mark=star\\%
 BuPu-9-7,mark=10-pointed star\\%
 BuPu-9-8,mark=Mercedes star\\%
 BuPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-3}{%
 RdPu-3-1,mark=x\\%
 RdPu-3-2,mark=+\\%
 RdPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-4}{%
 RdPu-4-1,mark=x\\%
 RdPu-4-2,mark=+\\%
 RdPu-4-3,mark=-\\%
 RdPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-5}{%
 RdPu-5-1,mark=x\\%
 RdPu-5-2,mark=+\\%
 RdPu-5-3,mark=-\\%
 RdPu-5-4,mark=|\\%
 RdPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-6}{%
 RdPu-6-1,mark=x\\%
 RdPu-6-2,mark=+\\%
 RdPu-6-3,mark=-\\%
 RdPu-6-4,mark=|\\%
 RdPu-6-5,mark=asterisk\\%
 RdPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-7}{%
 RdPu-7-1,mark=x\\%
 RdPu-7-2,mark=+\\%
 RdPu-7-3,mark=-\\%
 RdPu-7-4,mark=|\\%
 RdPu-7-5,mark=asterisk\\%
 RdPu-7-6,mark=star\\%
 RdPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-8}{%
 RdPu-8-1,mark=x\\%
 RdPu-8-2,mark=+\\%
 RdPu-8-3,mark=-\\%
 RdPu-8-4,mark=|\\%
 RdPu-8-5,mark=asterisk\\%
 RdPu-8-6,mark=star\\%
 RdPu-8-7,mark=10-pointed star\\%
 RdPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-9}{%
 RdPu-9-1,mark=x\\%
 RdPu-9-2,mark=+\\%
 RdPu-9-3,mark=-\\%
 RdPu-9-4,mark=|\\%
 RdPu-9-5,mark=asterisk\\%
 RdPu-9-6,mark=star\\%
 RdPu-9-7,mark=10-pointed star\\%
 RdPu-9-8,mark=Mercedes star\\%
 RdPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-3}{%
 PuRd-3-1,mark=x\\%
 PuRd-3-2,mark=+\\%
 PuRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-4}{%
 PuRd-4-1,mark=x\\%
 PuRd-4-2,mark=+\\%
 PuRd-4-3,mark=-\\%
 PuRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-5}{%
 PuRd-5-1,mark=x\\%
 PuRd-5-2,mark=+\\%
 PuRd-5-3,mark=-\\%
 PuRd-5-4,mark=|\\%
 PuRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-6}{%
 PuRd-6-1,mark=x\\%
 PuRd-6-2,mark=+\\%
 PuRd-6-3,mark=-\\%
 PuRd-6-4,mark=|\\%
 PuRd-6-5,mark=asterisk\\%
 PuRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-7}{%
 PuRd-7-1,mark=x\\%
 PuRd-7-2,mark=+\\%
 PuRd-7-3,mark=-\\%
 PuRd-7-4,mark=|\\%
 PuRd-7-5,mark=asterisk\\%
 PuRd-7-6,mark=star\\%
 PuRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-8}{%
 PuRd-8-1,mark=x\\%
 PuRd-8-2,mark=+\\%
 PuRd-8-3,mark=-\\%
 PuRd-8-4,mark=|\\%
 PuRd-8-5,mark=asterisk\\%
 PuRd-8-6,mark=star\\%
 PuRd-8-7,mark=10-pointed star\\%
 PuRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-9}{%
 PuRd-9-1,mark=x\\%
 PuRd-9-2,mark=+\\%
 PuRd-9-3,mark=-\\%
 PuRd-9-4,mark=|\\%
 PuRd-9-5,mark=asterisk\\%
 PuRd-9-6,mark=star\\%
 PuRd-9-7,mark=10-pointed star\\%
 PuRd-9-8,mark=Mercedes star\\%
 PuRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-3}{%
 OrRd-3-1,mark=x\\%
 OrRd-3-2,mark=+\\%
 OrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-4}{%
 OrRd-4-1,mark=x\\%
 OrRd-4-2,mark=+\\%
 OrRd-4-3,mark=-\\%
 OrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-5}{%
 OrRd-5-1,mark=x\\%
 OrRd-5-2,mark=+\\%
 OrRd-5-3,mark=-\\%
 OrRd-5-4,mark=|\\%
 OrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-6}{%
 OrRd-6-1,mark=x\\%
 OrRd-6-2,mark=+\\%
 OrRd-6-3,mark=-\\%
 OrRd-6-4,mark=|\\%
 OrRd-6-5,mark=asterisk\\%
 OrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-7}{%
 OrRd-7-1,mark=x\\%
 OrRd-7-2,mark=+\\%
 OrRd-7-3,mark=-\\%
 OrRd-7-4,mark=|\\%
 OrRd-7-5,mark=asterisk\\%
 OrRd-7-6,mark=star\\%
 OrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-8}{%
 OrRd-8-1,mark=x\\%
 OrRd-8-2,mark=+\\%
 OrRd-8-3,mark=-\\%
 OrRd-8-4,mark=|\\%
 OrRd-8-5,mark=asterisk\\%
 OrRd-8-6,mark=star\\%
 OrRd-8-7,mark=10-pointed star\\%
 OrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-9}{%
 OrRd-9-1,mark=x\\%
 OrRd-9-2,mark=+\\%
 OrRd-9-3,mark=-\\%
 OrRd-9-4,mark=|\\%
 OrRd-9-5,mark=asterisk\\%
 OrRd-9-6,mark=star\\%
 OrRd-9-7,mark=10-pointed star\\%
 OrRd-9-8,mark=Mercedes star\\%
 OrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-3}{%
 YlOrRd-3-1,mark=x\\%
 YlOrRd-3-2,mark=+\\%
 YlOrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-4}{%
 YlOrRd-4-1,mark=x\\%
 YlOrRd-4-2,mark=+\\%
 YlOrRd-4-3,mark=-\\%
 YlOrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-5}{%
 YlOrRd-5-1,mark=x\\%
 YlOrRd-5-2,mark=+\\%
 YlOrRd-5-3,mark=-\\%
 YlOrRd-5-4,mark=|\\%
 YlOrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-6}{%
 YlOrRd-6-1,mark=x\\%
 YlOrRd-6-2,mark=+\\%
 YlOrRd-6-3,mark=-\\%
 YlOrRd-6-4,mark=|\\%
 YlOrRd-6-5,mark=asterisk\\%
 YlOrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-7}{%
 YlOrRd-7-1,mark=x\\%
 YlOrRd-7-2,mark=+\\%
 YlOrRd-7-3,mark=-\\%
 YlOrRd-7-4,mark=|\\%
 YlOrRd-7-5,mark=asterisk\\%
 YlOrRd-7-6,mark=star\\%
 YlOrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-8}{%
 YlOrRd-8-1,mark=x\\%
 YlOrRd-8-2,mark=+\\%
 YlOrRd-8-3,mark=-\\%
 YlOrRd-8-4,mark=|\\%
 YlOrRd-8-5,mark=asterisk\\%
 YlOrRd-8-6,mark=star\\%
 YlOrRd-8-7,mark=10-pointed star\\%
 YlOrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-9}{%
 YlOrRd-9-1,mark=x\\%
 YlOrRd-9-2,mark=+\\%
 YlOrRd-9-3,mark=-\\%
 YlOrRd-9-4,mark=|\\%
 YlOrRd-9-5,mark=asterisk\\%
 YlOrRd-9-6,mark=star\\%
 YlOrRd-9-7,mark=10-pointed star\\%
 YlOrRd-9-8,mark=Mercedes star\\%
 YlOrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-3}{%
 YlOrBr-3-1,mark=x\\%
 YlOrBr-3-2,mark=+\\%
 YlOrBr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-4}{%
 YlOrBr-4-1,mark=x\\%
 YlOrBr-4-2,mark=+\\%
 YlOrBr-4-3,mark=-\\%
 YlOrBr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-5}{%
 YlOrBr-5-1,mark=x\\%
 YlOrBr-5-2,mark=+\\%
 YlOrBr-5-3,mark=-\\%
 YlOrBr-5-4,mark=|\\%
 YlOrBr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-6}{%
 YlOrBr-6-1,mark=x\\%
 YlOrBr-6-2,mark=+\\%
 YlOrBr-6-3,mark=-\\%
 YlOrBr-6-4,mark=|\\%
 YlOrBr-6-5,mark=asterisk\\%
 YlOrBr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-7}{%
 YlOrBr-7-1,mark=x\\%
 YlOrBr-7-2,mark=+\\%
 YlOrBr-7-3,mark=-\\%
 YlOrBr-7-4,mark=|\\%
 YlOrBr-7-5,mark=asterisk\\%
 YlOrBr-7-6,mark=star\\%
 YlOrBr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-8}{%
 YlOrBr-8-1,mark=x\\%
 YlOrBr-8-2,mark=+\\%
 YlOrBr-8-3,mark=-\\%
 YlOrBr-8-4,mark=|\\%
 YlOrBr-8-5,mark=asterisk\\%
 YlOrBr-8-6,mark=star\\%
 YlOrBr-8-7,mark=10-pointed star\\%
 YlOrBr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-9}{%
 YlOrBr-9-1,mark=x\\%
 YlOrBr-9-2,mark=+\\%
 YlOrBr-9-3,mark=-\\%
 YlOrBr-9-4,mark=|\\%
 YlOrBr-9-5,mark=asterisk\\%
 YlOrBr-9-6,mark=star\\%
 YlOrBr-9-7,mark=10-pointed star\\%
 YlOrBr-9-8,mark=Mercedes star\\%
 YlOrBr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-3}{%
 Purples-3-1,mark=x\\%
 Purples-3-2,mark=+\\%
 Purples-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-4}{%
 Purples-4-1,mark=x\\%
 Purples-4-2,mark=+\\%
 Purples-4-3,mark=-\\%
 Purples-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-5}{%
 Purples-5-1,mark=x\\%
 Purples-5-2,mark=+\\%
 Purples-5-3,mark=-\\%
 Purples-5-4,mark=|\\%
 Purples-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-6}{%
 Purples-6-1,mark=x\\%
 Purples-6-2,mark=+\\%
 Purples-6-3,mark=-\\%
 Purples-6-4,mark=|\\%
 Purples-6-5,mark=asterisk\\%
 Purples-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-7}{%
 Purples-7-1,mark=x\\%
 Purples-7-2,mark=+\\%
 Purples-7-3,mark=-\\%
 Purples-7-4,mark=|\\%
 Purples-7-5,mark=asterisk\\%
 Purples-7-6,mark=star\\%
 Purples-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-8}{%
 Purples-8-1,mark=x\\%
 Purples-8-2,mark=+\\%
 Purples-8-3,mark=-\\%
 Purples-8-4,mark=|\\%
 Purples-8-5,mark=asterisk\\%
 Purples-8-6,mark=star\\%
 Purples-8-7,mark=10-pointed star\\%
 Purples-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-9}{%
 Purples-9-1,mark=x\\%
 Purples-9-2,mark=+\\%
 Purples-9-3,mark=-\\%
 Purples-9-4,mark=|\\%
 Purples-9-5,mark=asterisk\\%
 Purples-9-6,mark=star\\%
 Purples-9-7,mark=10-pointed star\\%
 Purples-9-8,mark=Mercedes star\\%
 Purples-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-3}{%
 Blues-3-1,mark=x\\%
 Blues-3-2,mark=+\\%
 Blues-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-4}{%
 Blues-4-1,mark=x\\%
 Blues-4-2,mark=+\\%
 Blues-4-3,mark=-\\%
 Blues-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-5}{%
 Blues-5-1,mark=x\\%
 Blues-5-2,mark=+\\%
 Blues-5-3,mark=-\\%
 Blues-5-4,mark=|\\%
 Blues-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-6}{%
 Blues-6-1,mark=x\\%
 Blues-6-2,mark=+\\%
 Blues-6-3,mark=-\\%
 Blues-6-4,mark=|\\%
 Blues-6-5,mark=asterisk\\%
 Blues-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-7}{%
 Blues-7-1,mark=x\\%
 Blues-7-2,mark=+\\%
 Blues-7-3,mark=-\\%
 Blues-7-4,mark=|\\%
 Blues-7-5,mark=asterisk\\%
 Blues-7-6,mark=star\\%
 Blues-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-8}{%
 Blues-8-1,mark=x\\%
 Blues-8-2,mark=+\\%
 Blues-8-3,mark=-\\%
 Blues-8-4,mark=|\\%
 Blues-8-5,mark=asterisk\\%
 Blues-8-6,mark=star\\%
 Blues-8-7,mark=10-pointed star\\%
 Blues-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-9}{%
 Blues-9-1,mark=x\\%
 Blues-9-2,mark=+\\%
 Blues-9-3,mark=-\\%
 Blues-9-4,mark=|\\%
 Blues-9-5,mark=asterisk\\%
 Blues-9-6,mark=star\\%
 Blues-9-7,mark=10-pointed star\\%
 Blues-9-8,mark=Mercedes star\\%
 Blues-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-3}{%
 Greens-3-1,mark=x\\%
 Greens-3-2,mark=+\\%
 Greens-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-4}{%
 Greens-4-1,mark=x\\%
 Greens-4-2,mark=+\\%
 Greens-4-3,mark=-\\%
 Greens-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-5}{%
 Greens-5-1,mark=x\\%
 Greens-5-2,mark=+\\%
 Greens-5-3,mark=-\\%
 Greens-5-4,mark=|\\%
 Greens-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-6}{%
 Greens-6-1,mark=x\\%
 Greens-6-2,mark=+\\%
 Greens-6-3,mark=-\\%
 Greens-6-4,mark=|\\%
 Greens-6-5,mark=asterisk\\%
 Greens-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-7}{%
 Greens-7-1,mark=x\\%
 Greens-7-2,mark=+\\%
 Greens-7-3,mark=-\\%
 Greens-7-4,mark=|\\%
 Greens-7-5,mark=asterisk\\%
 Greens-7-6,mark=star\\%
 Greens-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-8}{%
 Greens-8-1,mark=x\\%
 Greens-8-2,mark=+\\%
 Greens-8-3,mark=-\\%
 Greens-8-4,mark=|\\%
 Greens-8-5,mark=asterisk\\%
 Greens-8-6,mark=star\\%
 Greens-8-7,mark=10-pointed star\\%
 Greens-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-9}{%
 Greens-9-1,mark=x\\%
 Greens-9-2,mark=+\\%
 Greens-9-3,mark=-\\%
 Greens-9-4,mark=|\\%
 Greens-9-5,mark=asterisk\\%
 Greens-9-6,mark=star\\%
 Greens-9-7,mark=10-pointed star\\%
 Greens-9-8,mark=Mercedes star\\%
 Greens-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-3}{%
 Oranges-3-1,mark=x\\%
 Oranges-3-2,mark=+\\%
 Oranges-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-4}{%
 Oranges-4-1,mark=x\\%
 Oranges-4-2,mark=+\\%
 Oranges-4-3,mark=-\\%
 Oranges-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-5}{%
 Oranges-5-1,mark=x\\%
 Oranges-5-2,mark=+\\%
 Oranges-5-3,mark=-\\%
 Oranges-5-4,mark=|\\%
 Oranges-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-6}{%
 Oranges-6-1,mark=x\\%
 Oranges-6-2,mark=+\\%
 Oranges-6-3,mark=-\\%
 Oranges-6-4,mark=|\\%
 Oranges-6-5,mark=asterisk\\%
 Oranges-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-7}{%
 Oranges-7-1,mark=x\\%
 Oranges-7-2,mark=+\\%
 Oranges-7-3,mark=-\\%
 Oranges-7-4,mark=|\\%
 Oranges-7-5,mark=asterisk\\%
 Oranges-7-6,mark=star\\%
 Oranges-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-8}{%
 Oranges-8-1,mark=x\\%
 Oranges-8-2,mark=+\\%
 Oranges-8-3,mark=-\\%
 Oranges-8-4,mark=|\\%
 Oranges-8-5,mark=asterisk\\%
 Oranges-8-6,mark=star\\%
 Oranges-8-7,mark=10-pointed star\\%
 Oranges-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-9}{%
 Oranges-9-1,mark=x\\%
 Oranges-9-2,mark=+\\%
 Oranges-9-3,mark=-\\%
 Oranges-9-4,mark=|\\%
 Oranges-9-5,mark=asterisk\\%
 Oranges-9-6,mark=star\\%
 Oranges-9-7,mark=10-pointed star\\%
 Oranges-9-8,mark=Mercedes star\\%
 Oranges-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-3}{%
 Reds-3-1,mark=x\\%
 Reds-3-2,mark=+\\%
 Reds-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-4}{%
 Reds-4-1,mark=x\\%
 Reds-4-2,mark=+\\%
 Reds-4-3,mark=-\\%
 Reds-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-5}{%
 Reds-5-1,mark=x\\%
 Reds-5-2,mark=+\\%
 Reds-5-3,mark=-\\%
 Reds-5-4,mark=|\\%
 Reds-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-6}{%
 Reds-6-1,mark=x\\%
 Reds-6-2,mark=+\\%
 Reds-6-3,mark=-\\%
 Reds-6-4,mark=|\\%
 Reds-6-5,mark=asterisk\\%
 Reds-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-7}{%
 Reds-7-1,mark=x\\%
 Reds-7-2,mark=+\\%
 Reds-7-3,mark=-\\%
 Reds-7-4,mark=|\\%
 Reds-7-5,mark=asterisk\\%
 Reds-7-6,mark=star\\%
 Reds-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-8}{%
 Reds-8-1,mark=x\\%
 Reds-8-2,mark=+\\%
 Reds-8-3,mark=-\\%
 Reds-8-4,mark=|\\%
 Reds-8-5,mark=asterisk\\%
 Reds-8-6,mark=star\\%
 Reds-8-7,mark=10-pointed star\\%
 Reds-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-9}{%
 Reds-9-1,mark=x\\%
 Reds-9-2,mark=+\\%
 Reds-9-3,mark=-\\%
 Reds-9-4,mark=|\\%
 Reds-9-5,mark=asterisk\\%
 Reds-9-6,mark=star\\%
 Reds-9-7,mark=10-pointed star\\%
 Reds-9-8,mark=Mercedes star\\%
 Reds-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-3}{%
 Greys-3-1,mark=x\\%
 Greys-3-2,mark=+\\%
 Greys-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-4}{%
 Greys-4-1,mark=x\\%
 Greys-4-2,mark=+\\%
 Greys-4-3,mark=-\\%
 Greys-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-5}{%
 Greys-5-1,mark=x\\%
 Greys-5-2,mark=+\\%
 Greys-5-3,mark=-\\%
 Greys-5-4,mark=|\\%
 Greys-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-6}{%
 Greys-6-1,mark=x\\%
 Greys-6-2,mark=+\\%
 Greys-6-3,mark=-\\%
 Greys-6-4,mark=|\\%
 Greys-6-5,mark=asterisk\\%
 Greys-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-7}{%
 Greys-7-1,mark=x\\%
 Greys-7-2,mark=+\\%
 Greys-7-3,mark=-\\%
 Greys-7-4,mark=|\\%
 Greys-7-5,mark=asterisk\\%
 Greys-7-6,mark=star\\%
 Greys-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-8}{%
 Greys-8-1,mark=x\\%
 Greys-8-2,mark=+\\%
 Greys-8-3,mark=-\\%
 Greys-8-4,mark=|\\%
 Greys-8-5,mark=asterisk\\%
 Greys-8-6,mark=star\\%
 Greys-8-7,mark=10-pointed star\\%
 Greys-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-9}{%
 Greys-9-1,mark=x\\%
 Greys-9-2,mark=+\\%
 Greys-9-3,mark=-\\%
 Greys-9-4,mark=|\\%
 Greys-9-5,mark=asterisk\\%
 Greys-9-6,mark=star\\%
 Greys-9-7,mark=10-pointed star\\%
 Greys-9-8,mark=Mercedes star\\%
 Greys-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-3}{%
 PuOr-3-1,mark=x\\%
 PuOr-3-2,mark=+\\%
 PuOr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-4}{%
 PuOr-4-1,mark=x\\%
 PuOr-4-2,mark=+\\%
 PuOr-4-3,mark=-\\%
 PuOr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-5}{%
 PuOr-5-1,mark=x\\%
 PuOr-5-2,mark=+\\%
 PuOr-5-3,mark=-\\%
 PuOr-5-4,mark=|\\%
 PuOr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-6}{%
 PuOr-6-1,mark=x\\%
 PuOr-6-2,mark=+\\%
 PuOr-6-3,mark=-\\%
 PuOr-6-4,mark=|\\%
 PuOr-6-5,mark=asterisk\\%
 PuOr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-7}{%
 PuOr-7-1,mark=x\\%
 PuOr-7-2,mark=+\\%
 PuOr-7-3,mark=-\\%
 PuOr-7-4,mark=|\\%
 PuOr-7-5,mark=asterisk\\%
 PuOr-7-6,mark=star\\%
 PuOr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-8}{%
 PuOr-8-1,mark=x\\%
 PuOr-8-2,mark=+\\%
 PuOr-8-3,mark=-\\%
 PuOr-8-4,mark=|\\%
 PuOr-8-5,mark=asterisk\\%
 PuOr-8-6,mark=star\\%
 PuOr-8-7,mark=10-pointed star\\%
 PuOr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-9}{%
 PuOr-9-1,mark=x\\%
 PuOr-9-2,mark=+\\%
 PuOr-9-3,mark=-\\%
 PuOr-9-4,mark=|\\%
 PuOr-9-5,mark=asterisk\\%
 PuOr-9-6,mark=star\\%
 PuOr-9-7,mark=10-pointed star\\%
 PuOr-9-8,mark=Mercedes star\\%
 PuOr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-10}{%
 PuOr-10-1,mark=x\\%
 PuOr-10-2,mark=+\\%
 PuOr-10-3,mark=-\\%
 PuOr-10-4,mark=|\\%
 PuOr-10-5,mark=asterisk\\%
 PuOr-10-6,mark=star\\%
 PuOr-10-7,mark=10-pointed star\\%
 PuOr-10-8,mark=Mercedes star\\%
 PuOr-10-9,mark=Mercedes star flipped\\%
 PuOr-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-11}{%
 PuOr-11-1,mark=x\\%
 PuOr-11-2,mark=+\\%
 PuOr-11-3,mark=-\\%
 PuOr-11-4,mark=|\\%
 PuOr-11-5,mark=asterisk\\%
 PuOr-11-6,mark=star\\%
 PuOr-11-7,mark=10-pointed star\\%
 PuOr-11-8,mark=Mercedes star\\%
 PuOr-11-9,mark=Mercedes star flipped\\%
 PuOr-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-3}{%
 BrBG-3-1,mark=x\\%
 BrBG-3-2,mark=+\\%
 BrBG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-4}{%
 BrBG-4-1,mark=x\\%
 BrBG-4-2,mark=+\\%
 BrBG-4-3,mark=-\\%
 BrBG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-5}{%
 BrBG-5-1,mark=x\\%
 BrBG-5-2,mark=+\\%
 BrBG-5-3,mark=-\\%
 BrBG-5-4,mark=|\\%
 BrBG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-6}{%
 BrBG-6-1,mark=x\\%
 BrBG-6-2,mark=+\\%
 BrBG-6-3,mark=-\\%
 BrBG-6-4,mark=|\\%
 BrBG-6-5,mark=asterisk\\%
 BrBG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-7}{%
 BrBG-7-1,mark=x\\%
 BrBG-7-2,mark=+\\%
 BrBG-7-3,mark=-\\%
 BrBG-7-4,mark=|\\%
 BrBG-7-5,mark=asterisk\\%
 BrBG-7-6,mark=star\\%
 BrBG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-8}{%
 BrBG-8-1,mark=x\\%
 BrBG-8-2,mark=+\\%
 BrBG-8-3,mark=-\\%
 BrBG-8-4,mark=|\\%
 BrBG-8-5,mark=asterisk\\%
 BrBG-8-6,mark=star\\%
 BrBG-8-7,mark=10-pointed star\\%
 BrBG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-9}{%
 BrBG-9-1,mark=x\\%
 BrBG-9-2,mark=+\\%
 BrBG-9-3,mark=-\\%
 BrBG-9-4,mark=|\\%
 BrBG-9-5,mark=asterisk\\%
 BrBG-9-6,mark=star\\%
 BrBG-9-7,mark=10-pointed star\\%
 BrBG-9-8,mark=Mercedes star\\%
 BrBG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-10}{%
 BrBG-10-1,mark=x\\%
 BrBG-10-2,mark=+\\%
 BrBG-10-3,mark=-\\%
 BrBG-10-4,mark=|\\%
 BrBG-10-5,mark=asterisk\\%
 BrBG-10-6,mark=star\\%
 BrBG-10-7,mark=10-pointed star\\%
 BrBG-10-8,mark=Mercedes star\\%
 BrBG-10-9,mark=Mercedes star flipped\\%
 BrBG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-11}{%
 BrBG-11-1,mark=x\\%
 BrBG-11-2,mark=+\\%
 BrBG-11-3,mark=-\\%
 BrBG-11-4,mark=|\\%
 BrBG-11-5,mark=asterisk\\%
 BrBG-11-6,mark=star\\%
 BrBG-11-7,mark=10-pointed star\\%
 BrBG-11-8,mark=Mercedes star\\%
 BrBG-11-9,mark=Mercedes star flipped\\%
 BrBG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-3}{%
 PRGn-3-1,mark=x\\%
 PRGn-3-2,mark=+\\%
 PRGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-4}{%
 PRGn-4-1,mark=x\\%
 PRGn-4-2,mark=+\\%
 PRGn-4-3,mark=-\\%
 PRGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-5}{%
 PRGn-5-1,mark=x\\%
 PRGn-5-2,mark=+\\%
 PRGn-5-3,mark=-\\%
 PRGn-5-4,mark=|\\%
 PRGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-6}{%
 PRGn-6-1,mark=x\\%
 PRGn-6-2,mark=+\\%
 PRGn-6-3,mark=-\\%
 PRGn-6-4,mark=|\\%
 PRGn-6-5,mark=asterisk\\%
 PRGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-7}{%
 PRGn-7-1,mark=x\\%
 PRGn-7-2,mark=+\\%
 PRGn-7-3,mark=-\\%
 PRGn-7-4,mark=|\\%
 PRGn-7-5,mark=asterisk\\%
 PRGn-7-6,mark=star\\%
 PRGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-8}{%
 PRGn-8-1,mark=x\\%
 PRGn-8-2,mark=+\\%
 PRGn-8-3,mark=-\\%
 PRGn-8-4,mark=|\\%
 PRGn-8-5,mark=asterisk\\%
 PRGn-8-6,mark=star\\%
 PRGn-8-7,mark=10-pointed star\\%
 PRGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-9}{%
 PRGn-9-1,mark=x\\%
 PRGn-9-2,mark=+\\%
 PRGn-9-3,mark=-\\%
 PRGn-9-4,mark=|\\%
 PRGn-9-5,mark=asterisk\\%
 PRGn-9-6,mark=star\\%
 PRGn-9-7,mark=10-pointed star\\%
 PRGn-9-8,mark=Mercedes star\\%
 PRGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-10}{%
 PRGn-10-1,mark=x\\%
 PRGn-10-2,mark=+\\%
 PRGn-10-3,mark=-\\%
 PRGn-10-4,mark=|\\%
 PRGn-10-5,mark=asterisk\\%
 PRGn-10-6,mark=star\\%
 PRGn-10-7,mark=10-pointed star\\%
 PRGn-10-8,mark=Mercedes star\\%
 PRGn-10-9,mark=Mercedes star flipped\\%
 PRGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-11}{%
 PRGn-11-1,mark=x\\%
 PRGn-11-2,mark=+\\%
 PRGn-11-3,mark=-\\%
 PRGn-11-4,mark=|\\%
 PRGn-11-5,mark=asterisk\\%
 PRGn-11-6,mark=star\\%
 PRGn-11-7,mark=10-pointed star\\%
 PRGn-11-8,mark=Mercedes star\\%
 PRGn-11-9,mark=Mercedes star flipped\\%
 PRGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-3}{%
 PiYG-3-1,mark=x\\%
 PiYG-3-2,mark=+\\%
 PiYG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-4}{%
 PiYG-4-1,mark=x\\%
 PiYG-4-2,mark=+\\%
 PiYG-4-3,mark=-\\%
 PiYG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-5}{%
 PiYG-5-1,mark=x\\%
 PiYG-5-2,mark=+\\%
 PiYG-5-3,mark=-\\%
 PiYG-5-4,mark=|\\%
 PiYG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-6}{%
 PiYG-6-1,mark=x\\%
 PiYG-6-2,mark=+\\%
 PiYG-6-3,mark=-\\%
 PiYG-6-4,mark=|\\%
 PiYG-6-5,mark=asterisk\\%
 PiYG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-7}{%
 PiYG-7-1,mark=x\\%
 PiYG-7-2,mark=+\\%
 PiYG-7-3,mark=-\\%
 PiYG-7-4,mark=|\\%
 PiYG-7-5,mark=asterisk\\%
 PiYG-7-6,mark=star\\%
 PiYG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-8}{%
 PiYG-8-1,mark=x\\%
 PiYG-8-2,mark=+\\%
 PiYG-8-3,mark=-\\%
 PiYG-8-4,mark=|\\%
 PiYG-8-5,mark=asterisk\\%
 PiYG-8-6,mark=star\\%
 PiYG-8-7,mark=10-pointed star\\%
 PiYG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-9}{%
 PiYG-9-1,mark=x\\%
 PiYG-9-2,mark=+\\%
 PiYG-9-3,mark=-\\%
 PiYG-9-4,mark=|\\%
 PiYG-9-5,mark=asterisk\\%
 PiYG-9-6,mark=star\\%
 PiYG-9-7,mark=10-pointed star\\%
 PiYG-9-8,mark=Mercedes star\\%
 PiYG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-10}{%
 PiYG-10-1,mark=x\\%
 PiYG-10-2,mark=+\\%
 PiYG-10-3,mark=-\\%
 PiYG-10-4,mark=|\\%
 PiYG-10-5,mark=asterisk\\%
 PiYG-10-6,mark=star\\%
 PiYG-10-7,mark=10-pointed star\\%
 PiYG-10-8,mark=Mercedes star\\%
 PiYG-10-9,mark=Mercedes star flipped\\%
 PiYG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-11}{%
 PiYG-11-1,mark=x\\%
 PiYG-11-2,mark=+\\%
 PiYG-11-3,mark=-\\%
 PiYG-11-4,mark=|\\%
 PiYG-11-5,mark=asterisk\\%
 PiYG-11-6,mark=star\\%
 PiYG-11-7,mark=10-pointed star\\%
 PiYG-11-8,mark=Mercedes star\\%
 PiYG-11-9,mark=Mercedes star flipped\\%
 PiYG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-3}{%
 RdBu-3-1,mark=x\\%
 RdBu-3-2,mark=+\\%
 RdBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-4}{%
 RdBu-4-1,mark=x\\%
 RdBu-4-2,mark=+\\%
 RdBu-4-3,mark=-\\%
 RdBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-5}{%
 RdBu-5-1,mark=x\\%
 RdBu-5-2,mark=+\\%
 RdBu-5-3,mark=-\\%
 RdBu-5-4,mark=|\\%
 RdBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-6}{%
 RdBu-6-1,mark=x\\%
 RdBu-6-2,mark=+\\%
 RdBu-6-3,mark=-\\%
 RdBu-6-4,mark=|\\%
 RdBu-6-5,mark=asterisk\\%
 RdBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-7}{%
 RdBu-7-1,mark=x\\%
 RdBu-7-2,mark=+\\%
 RdBu-7-3,mark=-\\%
 RdBu-7-4,mark=|\\%
 RdBu-7-5,mark=asterisk\\%
 RdBu-7-6,mark=star\\%
 RdBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-8}{%
 RdBu-8-1,mark=x\\%
 RdBu-8-2,mark=+\\%
 RdBu-8-3,mark=-\\%
 RdBu-8-4,mark=|\\%
 RdBu-8-5,mark=asterisk\\%
 RdBu-8-6,mark=star\\%
 RdBu-8-7,mark=10-pointed star\\%
 RdBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-9}{%
 RdBu-9-1,mark=x\\%
 RdBu-9-2,mark=+\\%
 RdBu-9-3,mark=-\\%
 RdBu-9-4,mark=|\\%
 RdBu-9-5,mark=asterisk\\%
 RdBu-9-6,mark=star\\%
 RdBu-9-7,mark=10-pointed star\\%
 RdBu-9-8,mark=Mercedes star\\%
 RdBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-10}{%
 RdBu-10-1,mark=x\\%
 RdBu-10-2,mark=+\\%
 RdBu-10-3,mark=-\\%
 RdBu-10-4,mark=|\\%
 RdBu-10-5,mark=asterisk\\%
 RdBu-10-6,mark=star\\%
 RdBu-10-7,mark=10-pointed star\\%
 RdBu-10-8,mark=Mercedes star\\%
 RdBu-10-9,mark=Mercedes star flipped\\%
 RdBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-11}{%
 RdBu-11-1,mark=x\\%
 RdBu-11-2,mark=+\\%
 RdBu-11-3,mark=-\\%
 RdBu-11-4,mark=|\\%
 RdBu-11-5,mark=asterisk\\%
 RdBu-11-6,mark=star\\%
 RdBu-11-7,mark=10-pointed star\\%
 RdBu-11-8,mark=Mercedes star\\%
 RdBu-11-9,mark=Mercedes star flipped\\%
 RdBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-3}{%
 RdGy-3-1,mark=x\\%
 RdGy-3-2,mark=+\\%
 RdGy-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-4}{%
 RdGy-4-1,mark=x\\%
 RdGy-4-2,mark=+\\%
 RdGy-4-3,mark=-\\%
 RdGy-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-5}{%
 RdGy-5-1,mark=x\\%
 RdGy-5-2,mark=+\\%
 RdGy-5-3,mark=-\\%
 RdGy-5-4,mark=|\\%
 RdGy-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-6}{%
 RdGy-6-1,mark=x\\%
 RdGy-6-2,mark=+\\%
 RdGy-6-3,mark=-\\%
 RdGy-6-4,mark=|\\%
 RdGy-6-5,mark=asterisk\\%
 RdGy-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-7}{%
 RdGy-7-1,mark=x\\%
 RdGy-7-2,mark=+\\%
 RdGy-7-3,mark=-\\%
 RdGy-7-4,mark=|\\%
 RdGy-7-5,mark=asterisk\\%
 RdGy-7-6,mark=star\\%
 RdGy-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-8}{%
 RdGy-8-1,mark=x\\%
 RdGy-8-2,mark=+\\%
 RdGy-8-3,mark=-\\%
 RdGy-8-4,mark=|\\%
 RdGy-8-5,mark=asterisk\\%
 RdGy-8-6,mark=star\\%
 RdGy-8-7,mark=10-pointed star\\%
 RdGy-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-9}{%
 RdGy-9-1,mark=x\\%
 RdGy-9-2,mark=+\\%
 RdGy-9-3,mark=-\\%
 RdGy-9-4,mark=|\\%
 RdGy-9-5,mark=asterisk\\%
 RdGy-9-6,mark=star\\%
 RdGy-9-7,mark=10-pointed star\\%
 RdGy-9-8,mark=Mercedes star\\%
 RdGy-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-10}{%
 RdGy-10-1,mark=x\\%
 RdGy-10-2,mark=+\\%
 RdGy-10-3,mark=-\\%
 RdGy-10-4,mark=|\\%
 RdGy-10-5,mark=asterisk\\%
 RdGy-10-6,mark=star\\%
 RdGy-10-7,mark=10-pointed star\\%
 RdGy-10-8,mark=Mercedes star\\%
 RdGy-10-9,mark=Mercedes star flipped\\%
 RdGy-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-11}{%
 RdGy-11-1,mark=x\\%
 RdGy-11-2,mark=+\\%
 RdGy-11-3,mark=-\\%
 RdGy-11-4,mark=|\\%
 RdGy-11-5,mark=asterisk\\%
 RdGy-11-6,mark=star\\%
 RdGy-11-7,mark=10-pointed star\\%
 RdGy-11-8,mark=Mercedes star\\%
 RdGy-11-9,mark=Mercedes star flipped\\%
 RdGy-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-3}{%
 RdYlBu-3-1,mark=x\\%
 RdYlBu-3-2,mark=+\\%
 RdYlBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-4}{%
 RdYlBu-4-1,mark=x\\%
 RdYlBu-4-2,mark=+\\%
 RdYlBu-4-3,mark=-\\%
 RdYlBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-5}{%
 RdYlBu-5-1,mark=x\\%
 RdYlBu-5-2,mark=+\\%
 RdYlBu-5-3,mark=-\\%
 RdYlBu-5-4,mark=|\\%
 RdYlBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-6}{%
 RdYlBu-6-1,mark=x\\%
 RdYlBu-6-2,mark=+\\%
 RdYlBu-6-3,mark=-\\%
 RdYlBu-6-4,mark=|\\%
 RdYlBu-6-5,mark=asterisk\\%
 RdYlBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-7}{%
 RdYlBu-7-1,mark=x\\%
 RdYlBu-7-2,mark=+\\%
 RdYlBu-7-3,mark=-\\%
 RdYlBu-7-4,mark=|\\%
 RdYlBu-7-5,mark=asterisk\\%
 RdYlBu-7-6,mark=star\\%
 RdYlBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-8}{%
 RdYlBu-8-1,mark=x\\%
 RdYlBu-8-2,mark=+\\%
 RdYlBu-8-3,mark=-\\%
 RdYlBu-8-4,mark=|\\%
 RdYlBu-8-5,mark=asterisk\\%
 RdYlBu-8-6,mark=star\\%
 RdYlBu-8-7,mark=10-pointed star\\%
 RdYlBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-9}{%
 RdYlBu-9-1,mark=x\\%
 RdYlBu-9-2,mark=+\\%
 RdYlBu-9-3,mark=-\\%
 RdYlBu-9-4,mark=|\\%
 RdYlBu-9-5,mark=asterisk\\%
 RdYlBu-9-6,mark=star\\%
 RdYlBu-9-7,mark=10-pointed star\\%
 RdYlBu-9-8,mark=Mercedes star\\%
 RdYlBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-10}{%
 RdYlBu-10-1,mark=x\\%
 RdYlBu-10-2,mark=+\\%
 RdYlBu-10-3,mark=-\\%
 RdYlBu-10-4,mark=|\\%
 RdYlBu-10-5,mark=asterisk\\%
 RdYlBu-10-6,mark=star\\%
 RdYlBu-10-7,mark=10-pointed star\\%
 RdYlBu-10-8,mark=Mercedes star\\%
 RdYlBu-10-9,mark=Mercedes star flipped\\%
 RdYlBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-11}{%
 RdYlBu-11-1,mark=x\\%
 RdYlBu-11-2,mark=+\\%
 RdYlBu-11-3,mark=-\\%
 RdYlBu-11-4,mark=|\\%
 RdYlBu-11-5,mark=asterisk\\%
 RdYlBu-11-6,mark=star\\%
 RdYlBu-11-7,mark=10-pointed star\\%
 RdYlBu-11-8,mark=Mercedes star\\%
 RdYlBu-11-9,mark=Mercedes star flipped\\%
 RdYlBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-3}{%
 Spectral-3-1,mark=x\\%
 Spectral-3-2,mark=+\\%
 Spectral-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-4}{%
 Spectral-4-1,mark=x\\%
 Spectral-4-2,mark=+\\%
 Spectral-4-3,mark=-\\%
 Spectral-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-5}{%
 Spectral-5-1,mark=x\\%
 Spectral-5-2,mark=+\\%
 Spectral-5-3,mark=-\\%
 Spectral-5-4,mark=|\\%
 Spectral-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-6}{%
 Spectral-6-1,mark=x\\%
 Spectral-6-2,mark=+\\%
 Spectral-6-3,mark=-\\%
 Spectral-6-4,mark=|\\%
 Spectral-6-5,mark=asterisk\\%
 Spectral-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-7}{%
 Spectral-7-1,mark=x\\%
 Spectral-7-2,mark=+\\%
 Spectral-7-3,mark=-\\%
 Spectral-7-4,mark=|\\%
 Spectral-7-5,mark=asterisk\\%
 Spectral-7-6,mark=star\\%
 Spectral-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-8}{%
 Spectral-8-1,mark=x\\%
 Spectral-8-2,mark=+\\%
 Spectral-8-3,mark=-\\%
 Spectral-8-4,mark=|\\%
 Spectral-8-5,mark=asterisk\\%
 Spectral-8-6,mark=star\\%
 Spectral-8-7,mark=10-pointed star\\%
 Spectral-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-9}{%
 Spectral-9-1,mark=x\\%
 Spectral-9-2,mark=+\\%
 Spectral-9-3,mark=-\\%
 Spectral-9-4,mark=|\\%
 Spectral-9-5,mark=asterisk\\%
 Spectral-9-6,mark=star\\%
 Spectral-9-7,mark=10-pointed star\\%
 Spectral-9-8,mark=Mercedes star\\%
 Spectral-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-10}{%
 Spectral-10-1,mark=x\\%
 Spectral-10-2,mark=+\\%
 Spectral-10-3,mark=-\\%
 Spectral-10-4,mark=|\\%
 Spectral-10-5,mark=asterisk\\%
 Spectral-10-6,mark=star\\%
 Spectral-10-7,mark=10-pointed star\\%
 Spectral-10-8,mark=Mercedes star\\%
 Spectral-10-9,mark=Mercedes star flipped\\%
 Spectral-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-11}{%
 Spectral-11-1,mark=x\\%
 Spectral-11-2,mark=+\\%
 Spectral-11-3,mark=-\\%
 Spectral-11-4,mark=|\\%
 Spectral-11-5,mark=asterisk\\%
 Spectral-11-6,mark=star\\%
 Spectral-11-7,mark=10-pointed star\\%
 Spectral-11-8,mark=Mercedes star\\%
 Spectral-11-9,mark=Mercedes star flipped\\%
 Spectral-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-3}{%
 RdYlGn-3-1,mark=x\\%
 RdYlGn-3-2,mark=+\\%
 RdYlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-4}{%
 RdYlGn-4-1,mark=x\\%
 RdYlGn-4-2,mark=+\\%
 RdYlGn-4-3,mark=-\\%
 RdYlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-5}{%
 RdYlGn-5-1,mark=x\\%
 RdYlGn-5-2,mark=+\\%
 RdYlGn-5-3,mark=-\\%
 RdYlGn-5-4,mark=|\\%
 RdYlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-6}{%
 RdYlGn-6-1,mark=x\\%
 RdYlGn-6-2,mark=+\\%
 RdYlGn-6-3,mark=-\\%
 RdYlGn-6-4,mark=|\\%
 RdYlGn-6-5,mark=asterisk\\%
 RdYlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-7}{%
 RdYlGn-7-1,mark=x\\%
 RdYlGn-7-2,mark=+\\%
 RdYlGn-7-3,mark=-\\%
 RdYlGn-7-4,mark=|\\%
 RdYlGn-7-5,mark=asterisk\\%
 RdYlGn-7-6,mark=star\\%
 RdYlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-8}{%
 RdYlGn-8-1,mark=x\\%
 RdYlGn-8-2,mark=+\\%
 RdYlGn-8-3,mark=-\\%
 RdYlGn-8-4,mark=|\\%
 RdYlGn-8-5,mark=asterisk\\%
 RdYlGn-8-6,mark=star\\%
 RdYlGn-8-7,mark=10-pointed star\\%
 RdYlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-9}{%
 RdYlGn-9-1,mark=x\\%
 RdYlGn-9-2,mark=+\\%
 RdYlGn-9-3,mark=-\\%
 RdYlGn-9-4,mark=|\\%
 RdYlGn-9-5,mark=asterisk\\%
 RdYlGn-9-6,mark=star\\%
 RdYlGn-9-7,mark=10-pointed star\\%
 RdYlGn-9-8,mark=Mercedes star\\%
 RdYlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-10}{%
 RdYlGn-10-1,mark=x\\%
 RdYlGn-10-2,mark=+\\%
 RdYlGn-10-3,mark=-\\%
 RdYlGn-10-4,mark=|\\%
 RdYlGn-10-5,mark=asterisk\\%
 RdYlGn-10-6,mark=star\\%
 RdYlGn-10-7,mark=10-pointed star\\%
 RdYlGn-10-8,mark=Mercedes star\\%
 RdYlGn-10-9,mark=Mercedes star flipped\\%
 RdYlGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-11}{%
 RdYlGn-11-1,mark=x\\%
 RdYlGn-11-2,mark=+\\%
 RdYlGn-11-3,mark=-\\%
 RdYlGn-11-4,mark=|\\%
 RdYlGn-11-5,mark=asterisk\\%
 RdYlGn-11-6,mark=star\\%
 RdYlGn-11-7,mark=10-pointed star\\%
 RdYlGn-11-8,mark=Mercedes star\\%
 RdYlGn-11-9,mark=Mercedes star flipped\\%
 RdYlGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-3}{%
 Set3-3-1,mark=x\\%
 Set3-3-2,mark=+\\%
 Set3-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-4}{%
 Set3-4-1,mark=x\\%
 Set3-4-2,mark=+\\%
 Set3-4-3,mark=-\\%
 Set3-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-5}{%
 Set3-5-1,mark=x\\%
 Set3-5-2,mark=+\\%
 Set3-5-3,mark=-\\%
 Set3-5-4,mark=|\\%
 Set3-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-6}{%
 Set3-6-1,mark=x\\%
 Set3-6-2,mark=+\\%
 Set3-6-3,mark=-\\%
 Set3-6-4,mark=|\\%
 Set3-6-5,mark=asterisk\\%
 Set3-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-7}{%
 Set3-7-1,mark=x\\%
 Set3-7-2,mark=+\\%
 Set3-7-3,mark=-\\%
 Set3-7-4,mark=|\\%
 Set3-7-5,mark=asterisk\\%
 Set3-7-6,mark=star\\%
 Set3-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-8}{%
 Set3-8-1,mark=x\\%
 Set3-8-2,mark=+\\%
 Set3-8-3,mark=-\\%
 Set3-8-4,mark=|\\%
 Set3-8-5,mark=asterisk\\%
 Set3-8-6,mark=star\\%
 Set3-8-7,mark=10-pointed star\\%
 Set3-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-9}{%
 Set3-9-1,mark=x\\%
 Set3-9-2,mark=+\\%
 Set3-9-3,mark=-\\%
 Set3-9-4,mark=|\\%
 Set3-9-5,mark=asterisk\\%
 Set3-9-6,mark=star\\%
 Set3-9-7,mark=10-pointed star\\%
 Set3-9-8,mark=Mercedes star\\%
 Set3-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-10}{%
 Set3-10-1,mark=x\\%
 Set3-10-2,mark=+\\%
 Set3-10-3,mark=-\\%
 Set3-10-4,mark=|\\%
 Set3-10-5,mark=asterisk\\%
 Set3-10-6,mark=star\\%
 Set3-10-7,mark=10-pointed star\\%
 Set3-10-8,mark=Mercedes star\\%
 Set3-10-9,mark=Mercedes star flipped\\%
 Set3-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-11}{%
 Set3-11-1,mark=x\\%
 Set3-11-2,mark=+\\%
 Set3-11-3,mark=-\\%
 Set3-11-4,mark=|\\%
 Set3-11-5,mark=asterisk\\%
 Set3-11-6,mark=star\\%
 Set3-11-7,mark=10-pointed star\\%
 Set3-11-8,mark=Mercedes star\\%
 Set3-11-9,mark=Mercedes star flipped\\%
 Set3-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-12}{%
 Set3-12-1,mark=x\\%
 Set3-12-2,mark=+\\%
 Set3-12-3,mark=-\\%
 Set3-12-4,mark=|\\%
 Set3-12-5,mark=asterisk\\%
 Set3-12-6,mark=star\\%
 Set3-12-7,mark=10-pointed star\\%
 Set3-12-8,mark=Mercedes star\\%
 Set3-12-9,mark=Mercedes star flipped\\%
 Set3-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-3}{%
 Pastel1-3-1,mark=x\\%
 Pastel1-3-2,mark=+\\%
 Pastel1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-4}{%
 Pastel1-4-1,mark=x\\%
 Pastel1-4-2,mark=+\\%
 Pastel1-4-3,mark=-\\%
 Pastel1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-5}{%
 Pastel1-5-1,mark=x\\%
 Pastel1-5-2,mark=+\\%
 Pastel1-5-3,mark=-\\%
 Pastel1-5-4,mark=|\\%
 Pastel1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-6}{%
 Pastel1-6-1,mark=x\\%
 Pastel1-6-2,mark=+\\%
 Pastel1-6-3,mark=-\\%
 Pastel1-6-4,mark=|\\%
 Pastel1-6-5,mark=asterisk\\%
 Pastel1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-7}{%
 Pastel1-7-1,mark=x\\%
 Pastel1-7-2,mark=+\\%
 Pastel1-7-3,mark=-\\%
 Pastel1-7-4,mark=|\\%
 Pastel1-7-5,mark=asterisk\\%
 Pastel1-7-6,mark=star\\%
 Pastel1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-8}{%
 Pastel1-8-1,mark=x\\%
 Pastel1-8-2,mark=+\\%
 Pastel1-8-3,mark=-\\%
 Pastel1-8-4,mark=|\\%
 Pastel1-8-5,mark=asterisk\\%
 Pastel1-8-6,mark=star\\%
 Pastel1-8-7,mark=10-pointed star\\%
 Pastel1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-9}{%
 Pastel1-9-1,mark=x\\%
 Pastel1-9-2,mark=+\\%
 Pastel1-9-3,mark=-\\%
 Pastel1-9-4,mark=|\\%
 Pastel1-9-5,mark=asterisk\\%
 Pastel1-9-6,mark=star\\%
 Pastel1-9-7,mark=10-pointed star\\%
 Pastel1-9-8,mark=Mercedes star\\%
 Pastel1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-3}{%
 Set1-3-1,mark=x\\%
 Set1-3-2,mark=+\\%
 Set1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-4}{%
 Set1-4-1,mark=x\\%
 Set1-4-2,mark=+\\%
 Set1-4-3,mark=-\\%
 Set1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-5}{%
 Set1-5-1,mark=x\\%
 Set1-5-2,mark=+\\%
 Set1-5-3,mark=-\\%
 Set1-5-4,mark=|\\%
 Set1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-6}{%
 Set1-6-1,mark=x\\%
 Set1-6-2,mark=+\\%
 Set1-6-3,mark=-\\%
 Set1-6-4,mark=|\\%
 Set1-6-5,mark=asterisk\\%
 Set1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-7}{%
 Set1-7-1,mark=x\\%
 Set1-7-2,mark=+\\%
 Set1-7-3,mark=-\\%
 Set1-7-4,mark=|\\%
 Set1-7-5,mark=asterisk\\%
 Set1-7-6,mark=star\\%
 Set1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-8}{%
 Set1-8-1,mark=x\\%
 Set1-8-2,mark=+\\%
 Set1-8-3,mark=-\\%
 Set1-8-4,mark=|\\%
 Set1-8-5,mark=asterisk\\%
 Set1-8-6,mark=star\\%
 Set1-8-7,mark=10-pointed star\\%
 Set1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-9}{%
 Set1-9-1,mark=x\\%
 Set1-9-2,mark=+\\%
 Set1-9-3,mark=-\\%
 Set1-9-4,mark=|\\%
 Set1-9-5,mark=asterisk\\%
 Set1-9-6,mark=star\\%
 Set1-9-7,mark=10-pointed star\\%
 Set1-9-8,mark=Mercedes star\\%
 Set1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-3}{%
 Pastel2-3-1,mark=x\\%
 Pastel2-3-2,mark=+\\%
 Pastel2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-4}{%
 Pastel2-4-1,mark=x\\%
 Pastel2-4-2,mark=+\\%
 Pastel2-4-3,mark=-\\%
 Pastel2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-5}{%
 Pastel2-5-1,mark=x\\%
 Pastel2-5-2,mark=+\\%
 Pastel2-5-3,mark=-\\%
 Pastel2-5-4,mark=|\\%
 Pastel2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-6}{%
 Pastel2-6-1,mark=x\\%
 Pastel2-6-2,mark=+\\%
 Pastel2-6-3,mark=-\\%
 Pastel2-6-4,mark=|\\%
 Pastel2-6-5,mark=asterisk\\%
 Pastel2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-7}{%
 Pastel2-7-1,mark=x\\%
 Pastel2-7-2,mark=+\\%
 Pastel2-7-3,mark=-\\%
 Pastel2-7-4,mark=|\\%
 Pastel2-7-5,mark=asterisk\\%
 Pastel2-7-6,mark=star\\%
 Pastel2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-8}{%
 Pastel2-8-1,mark=x\\%
 Pastel2-8-2,mark=+\\%
 Pastel2-8-3,mark=-\\%
 Pastel2-8-4,mark=|\\%
 Pastel2-8-5,mark=asterisk\\%
 Pastel2-8-6,mark=star\\%
 Pastel2-8-7,mark=10-pointed star\\%
 Pastel2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-3}{%
 Set2-3-1,mark=x\\%
 Set2-3-2,mark=+\\%
 Set2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-4}{%
 Set2-4-1,mark=x\\%
 Set2-4-2,mark=+\\%
 Set2-4-3,mark=-\\%
 Set2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-5}{%
 Set2-5-1,mark=x\\%
 Set2-5-2,mark=+\\%
 Set2-5-3,mark=-\\%
 Set2-5-4,mark=|\\%
 Set2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-6}{%
 Set2-6-1,mark=x\\%
 Set2-6-2,mark=+\\%
 Set2-6-3,mark=-\\%
 Set2-6-4,mark=|\\%
 Set2-6-5,mark=asterisk\\%
 Set2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-7}{%
 Set2-7-1,mark=x\\%
 Set2-7-2,mark=+\\%
 Set2-7-3,mark=-\\%
 Set2-7-4,mark=|\\%
 Set2-7-5,mark=asterisk\\%
 Set2-7-6,mark=star\\%
 Set2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-8}{%
 Set2-8-1,mark=x\\%
 Set2-8-2,mark=+\\%
 Set2-8-3,mark=-\\%
 Set2-8-4,mark=|\\%
 Set2-8-5,mark=asterisk\\%
 Set2-8-6,mark=star\\%
 Set2-8-7,mark=10-pointed star\\%
 Set2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-3}{%
 Dark2-3-1,mark=x\\%
 Dark2-3-2,mark=+\\%
 Dark2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-4}{%
 Dark2-4-1,mark=x\\%
 Dark2-4-2,mark=+\\%
 Dark2-4-3,mark=-\\%
 Dark2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-5}{%
 Dark2-5-1,mark=x\\%
 Dark2-5-2,mark=+\\%
 Dark2-5-3,mark=-\\%
 Dark2-5-4,mark=|\\%
 Dark2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-6}{%
 Dark2-6-1,mark=x\\%
 Dark2-6-2,mark=+\\%
 Dark2-6-3,mark=-\\%
 Dark2-6-4,mark=|\\%
 Dark2-6-5,mark=asterisk\\%
 Dark2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-7}{%
 Dark2-7-1,mark=x\\%
 Dark2-7-2,mark=+\\%
 Dark2-7-3,mark=-\\%
 Dark2-7-4,mark=|\\%
 Dark2-7-5,mark=asterisk\\%
 Dark2-7-6,mark=star\\%
 Dark2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-8}{%
 Dark2-8-1,mark=x\\%
 Dark2-8-2,mark=+\\%
 Dark2-8-3,mark=-\\%
 Dark2-8-4,mark=|\\%
 Dark2-8-5,mark=asterisk\\%
 Dark2-8-6,mark=star\\%
 Dark2-8-7,mark=10-pointed star\\%
 Dark2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-3}{%
 Paired-3-1,mark=x\\%
 Paired-3-2,mark=+\\%
 Paired-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-4}{%
 Paired-4-1,mark=x\\%
 Paired-4-2,mark=+\\%
 Paired-4-3,mark=-\\%
 Paired-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-5}{%
 Paired-5-1,mark=x\\%
 Paired-5-2,mark=+\\%
 Paired-5-3,mark=-\\%
 Paired-5-4,mark=|\\%
 Paired-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-6}{%
 Paired-6-1,mark=x\\%
 Paired-6-2,mark=+\\%
 Paired-6-3,mark=-\\%
 Paired-6-4,mark=|\\%
 Paired-6-5,mark=asterisk\\%
 Paired-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-7}{%
 Paired-7-1,mark=x\\%
 Paired-7-2,mark=+\\%
 Paired-7-3,mark=-\\%
 Paired-7-4,mark=|\\%
 Paired-7-5,mark=asterisk\\%
 Paired-7-6,mark=star\\%
 Paired-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-8}{%
 Paired-8-1,mark=x\\%
 Paired-8-2,mark=+\\%
 Paired-8-3,mark=-\\%
 Paired-8-4,mark=|\\%
 Paired-8-5,mark=asterisk\\%
 Paired-8-6,mark=star\\%
 Paired-8-7,mark=10-pointed star\\%
 Paired-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-9}{%
 Paired-9-1,mark=x\\%
 Paired-9-2,mark=+\\%
 Paired-9-3,mark=-\\%
 Paired-9-4,mark=|\\%
 Paired-9-5,mark=asterisk\\%
 Paired-9-6,mark=star\\%
 Paired-9-7,mark=10-pointed star\\%
 Paired-9-8,mark=Mercedes star\\%
 Paired-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-10}{%
 Paired-10-1,mark=x\\%
 Paired-10-2,mark=+\\%
 Paired-10-3,mark=-\\%
 Paired-10-4,mark=|\\%
 Paired-10-5,mark=asterisk\\%
 Paired-10-6,mark=star\\%
 Paired-10-7,mark=10-pointed star\\%
 Paired-10-8,mark=Mercedes star\\%
 Paired-10-9,mark=Mercedes star flipped\\%
 Paired-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-11}{%
 Paired-11-1,mark=x\\%
 Paired-11-2,mark=+\\%
 Paired-11-3,mark=-\\%
 Paired-11-4,mark=|\\%
 Paired-11-5,mark=asterisk\\%
 Paired-11-6,mark=star\\%
 Paired-11-7,mark=10-pointed star\\%
 Paired-11-8,mark=Mercedes star\\%
 Paired-11-9,mark=Mercedes star flipped\\%
 Paired-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-12}{%
 Paired-12-1,mark=x\\%
 Paired-12-2,mark=+\\%
 Paired-12-3,mark=-\\%
 Paired-12-4,mark=|\\%
 Paired-12-5,mark=asterisk\\%
 Paired-12-6,mark=star\\%
 Paired-12-7,mark=10-pointed star\\%
 Paired-12-8,mark=Mercedes star\\%
 Paired-12-9,mark=Mercedes star flipped\\%
 Paired-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-3}{%
 Accent-3-1,mark=x\\%
 Accent-3-2,mark=+\\%
 Accent-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-4}{%
 Accent-4-1,mark=x\\%
 Accent-4-2,mark=+\\%
 Accent-4-3,mark=-\\%
 Accent-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-5}{%
 Accent-5-1,mark=x\\%
 Accent-5-2,mark=+\\%
 Accent-5-3,mark=-\\%
 Accent-5-4,mark=|\\%
 Accent-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-6}{%
 Accent-6-1,mark=x\\%
 Accent-6-2,mark=+\\%
 Accent-6-3,mark=-\\%
 Accent-6-4,mark=|\\%
 Accent-6-5,mark=asterisk\\%
 Accent-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-7}{%
 Accent-7-1,mark=x\\%
 Accent-7-2,mark=+\\%
 Accent-7-3,mark=-\\%
 Accent-7-4,mark=|\\%
 Accent-7-5,mark=asterisk\\%
 Accent-7-6,mark=star\\%
 Accent-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-8}{%
 Accent-8-1,mark=x\\%
 Accent-8-2,mark=+\\%
 Accent-8-3,mark=-\\%
 Accent-8-4,mark=|\\%
 Accent-8-5,mark=asterisk\\%
 Accent-8-6,mark=star\\%
 Accent-8-7,mark=10-pointed star\\%
 Accent-8-8,mark=Mercedes star\\%
}
\pgfplotsset{
colormap={YlGn-3}{
  color=(YlGn-3-1);
  color=(YlGn-3-2);
  color=(YlGn-3-3);
},
colormap={YlGn-4}{
  color=(YlGn-4-1);
  color=(YlGn-4-2);
  color=(YlGn-4-3);
  color=(YlGn-4-4);
},
colormap={YlGn-5}{
  color=(YlGn-5-1);
  color=(YlGn-5-2);
  color=(YlGn-5-3);
  color=(YlGn-5-4);
  color=(YlGn-5-5);
},
colormap={YlGn-6}{
  color=(YlGn-6-1);
  color=(YlGn-6-2);
  color=(YlGn-6-3);
  color=(YlGn-6-4);
  color=(YlGn-6-5);
  color=(YlGn-6-6);
},
colormap={YlGn-7}{
  color=(YlGn-7-1);
  color=(YlGn-7-2);
  color=(YlGn-7-3);
  color=(YlGn-7-4);
  color=(YlGn-7-5);
  color=(YlGn-7-6);
  color=(YlGn-7-7);
},
colormap={YlGn-8}{
  color=(YlGn-8-1);
  color=(YlGn-8-2);
  color=(YlGn-8-3);
  color=(YlGn-8-4);
  color=(YlGn-8-5);
  color=(YlGn-8-6);
  color=(YlGn-8-7);
  color=(YlGn-8-8);
},
colormap={YlGn-9}{
  color=(YlGn-9-1);
  color=(YlGn-9-2);
  color=(YlGn-9-3);
  color=(YlGn-9-4);
  color=(YlGn-9-5);
  color=(YlGn-9-6);
  color=(YlGn-9-7);
  color=(YlGn-9-8);
  color=(YlGn-9-9);
},
colormap={YlGnBu-3}{
  color=(YlGnBu-3-1);
  color=(YlGnBu-3-2);
  color=(YlGnBu-3-3);
},
colormap={YlGnBu-4}{
  color=(YlGnBu-4-1);
  color=(YlGnBu-4-2);
  color=(YlGnBu-4-3);
  color=(YlGnBu-4-4);
},
colormap={YlGnBu-5}{
  color=(YlGnBu-5-1);
  color=(YlGnBu-5-2);
  color=(YlGnBu-5-3);
  color=(YlGnBu-5-4);
  color=(YlGnBu-5-5);
},
colormap={YlGnBu-6}{
  color=(YlGnBu-6-1);
  color=(YlGnBu-6-2);
  color=(YlGnBu-6-3);
  color=(YlGnBu-6-4);
  color=(YlGnBu-6-5);
  color=(YlGnBu-6-6);
},
colormap={YlGnBu-7}{
  color=(YlGnBu-7-1);
  color=(YlGnBu-7-2);
  color=(YlGnBu-7-3);
  color=(YlGnBu-7-4);
  color=(YlGnBu-7-5);
  color=(YlGnBu-7-6);
  color=(YlGnBu-7-7);
},
colormap={YlGnBu-8}{
  color=(YlGnBu-8-1);
  color=(YlGnBu-8-2);
  color=(YlGnBu-8-3);
  color=(YlGnBu-8-4);
  color=(YlGnBu-8-5);
  color=(YlGnBu-8-6);
  color=(YlGnBu-8-7);
  color=(YlGnBu-8-8);
},
colormap={YlGnBu-9}{
  color=(YlGnBu-9-1);
  color=(YlGnBu-9-2);
  color=(YlGnBu-9-3);
  color=(YlGnBu-9-4);
  color=(YlGnBu-9-5);
  color=(YlGnBu-9-6);
  color=(YlGnBu-9-7);
  color=(YlGnBu-9-8);
  color=(YlGnBu-9-9);
},
colormap={GnBu-3}{
  color=(GnBu-3-1);
  color=(GnBu-3-2);
  color=(GnBu-3-3);
},
colormap={GnBu-4}{
  color=(GnBu-4-1);
  color=(GnBu-4-2);
  color=(GnBu-4-3);
  color=(GnBu-4-4);
},
colormap={GnBu-5}{
  color=(GnBu-5-1);
  color=(GnBu-5-2);
  color=(GnBu-5-3);
  color=(GnBu-5-4);
  color=(GnBu-5-5);
},
colormap={GnBu-6}{
  color=(GnBu-6-1);
  color=(GnBu-6-2);
  color=(GnBu-6-3);
  color=(GnBu-6-4);
  color=(GnBu-6-5);
  color=(GnBu-6-6);
},
colormap={GnBu-7}{
  color=(GnBu-7-1);
  color=(GnBu-7-2);
  color=(GnBu-7-3);
  color=(GnBu-7-4);
  color=(GnBu-7-5);
  color=(GnBu-7-6);
  color=(GnBu-7-7);
},
colormap={GnBu-8}{
  color=(GnBu-8-1);
  color=(GnBu-8-2);
  color=(GnBu-8-3);
  color=(GnBu-8-4);
  color=(GnBu-8-5);
  color=(GnBu-8-6);
  color=(GnBu-8-7);
  color=(GnBu-8-8);
},
colormap={GnBu-9}{
  color=(GnBu-9-1);
  color=(GnBu-9-2);
  color=(GnBu-9-3);
  color=(GnBu-9-4);
  color=(GnBu-9-5);
  color=(GnBu-9-6);
  color=(GnBu-9-7);
  color=(GnBu-9-8);
  color=(GnBu-9-9);
},
colormap={BuGn-3}{
  color=(BuGn-3-1);
  color=(BuGn-3-2);
  color=(BuGn-3-3);
},
colormap={BuGn-4}{
  color=(BuGn-4-1);
  color=(BuGn-4-2);
  color=(BuGn-4-3);
  color=(BuGn-4-4);
},
colormap={BuGn-5}{
  color=(BuGn-5-1);
  color=(BuGn-5-2);
  color=(BuGn-5-3);
  color=(BuGn-5-4);
  color=(BuGn-5-5);
},
colormap={BuGn-6}{
  color=(BuGn-6-1);
  color=(BuGn-6-2);
  color=(BuGn-6-3);
  color=(BuGn-6-4);
  color=(BuGn-6-5);
  color=(BuGn-6-6);
},
colormap={BuGn-7}{
  color=(BuGn-7-1);
  color=(BuGn-7-2);
  color=(BuGn-7-3);
  color=(BuGn-7-4);
  color=(BuGn-7-5);
  color=(BuGn-7-6);
  color=(BuGn-7-7);
},
colormap={BuGn-8}{
  color=(BuGn-8-1);
  color=(BuGn-8-2);
  color=(BuGn-8-3);
  color=(BuGn-8-4);
  color=(BuGn-8-5);
  color=(BuGn-8-6);
  color=(BuGn-8-7);
  color=(BuGn-8-8);
},
colormap={BuGn-9}{
  color=(BuGn-9-1);
  color=(BuGn-9-2);
  color=(BuGn-9-3);
  color=(BuGn-9-4);
  color=(BuGn-9-5);
  color=(BuGn-9-6);
  color=(BuGn-9-7);
  color=(BuGn-9-8);
  color=(BuGn-9-9);
},
colormap={PuBuGn-3}{
  color=(PuBuGn-3-1);
  color=(PuBuGn-3-2);
  color=(PuBuGn-3-3);
},
colormap={PuBuGn-4}{
  color=(PuBuGn-4-1);
  color=(PuBuGn-4-2);
  color=(PuBuGn-4-3);
  color=(PuBuGn-4-4);
},
colormap={PuBuGn-5}{
  color=(PuBuGn-5-1);
  color=(PuBuGn-5-2);
  color=(PuBuGn-5-3);
  color=(PuBuGn-5-4);
  color=(PuBuGn-5-5);
},
colormap={PuBuGn-6}{
  color=(PuBuGn-6-1);
  color=(PuBuGn-6-2);
  color=(PuBuGn-6-3);
  color=(PuBuGn-6-4);
  color=(PuBuGn-6-5);
  color=(PuBuGn-6-6);
},
colormap={PuBuGn-7}{
  color=(PuBuGn-7-1);
  color=(PuBuGn-7-2);
  color=(PuBuGn-7-3);
  color=(PuBuGn-7-4);
  color=(PuBuGn-7-5);
  color=(PuBuGn-7-6);
  color=(PuBuGn-7-7);
},
colormap={PuBuGn-8}{
  color=(PuBuGn-8-1);
  color=(PuBuGn-8-2);
  color=(PuBuGn-8-3);
  color=(PuBuGn-8-4);
  color=(PuBuGn-8-5);
  color=(PuBuGn-8-6);
  color=(PuBuGn-8-7);
  color=(PuBuGn-8-8);
},
colormap={PuBuGn-9}{
  color=(PuBuGn-9-1);
  color=(PuBuGn-9-2);
  color=(PuBuGn-9-3);
  color=(PuBuGn-9-4);
  color=(PuBuGn-9-5);
  color=(PuBuGn-9-6);
  color=(PuBuGn-9-7);
  color=(PuBuGn-9-8);
  color=(PuBuGn-9-9);
},
colormap={PuBu-3}{
  color=(PuBu-3-1);
  color=(PuBu-3-2);
  color=(PuBu-3-3);
},
colormap={PuBu-4}{
  color=(PuBu-4-1);
  color=(PuBu-4-2);
  color=(PuBu-4-3);
  color=(PuBu-4-4);
},
colormap={PuBu-5}{
  color=(PuBu-5-1);
  color=(PuBu-5-2);
  color=(PuBu-5-3);
  color=(PuBu-5-4);
  color=(PuBu-5-5);
},
colormap={PuBu-6}{
  color=(PuBu-6-1);
  color=(PuBu-6-2);
  color=(PuBu-6-3);
  color=(PuBu-6-4);
  color=(PuBu-6-5);
  color=(PuBu-6-6);
},
colormap={PuBu-7}{
  color=(PuBu-7-1);
  color=(PuBu-7-2);
  color=(PuBu-7-3);
  color=(PuBu-7-4);
  color=(PuBu-7-5);
  color=(PuBu-7-6);
  color=(PuBu-7-7);
},
colormap={PuBu-8}{
  color=(PuBu-8-1);
  color=(PuBu-8-2);
  color=(PuBu-8-3);
  color=(PuBu-8-4);
  color=(PuBu-8-5);
  color=(PuBu-8-6);
  color=(PuBu-8-7);
  color=(PuBu-8-8);
},
colormap={PuBu-9}{
  color=(PuBu-9-1);
  color=(PuBu-9-2);
  color=(PuBu-9-3);
  color=(PuBu-9-4);
  color=(PuBu-9-5);
  color=(PuBu-9-6);
  color=(PuBu-9-7);
  color=(PuBu-9-8);
  color=(PuBu-9-9);
},
colormap={BuPu-3}{
  color=(BuPu-3-1);
  color=(BuPu-3-2);
  color=(BuPu-3-3);
},
colormap={BuPu-4}{
  color=(BuPu-4-1);
  color=(BuPu-4-2);
  color=(BuPu-4-3);
  color=(BuPu-4-4);
},
colormap={BuPu-5}{
  color=(BuPu-5-1);
  color=(BuPu-5-2);
  color=(BuPu-5-3);
  color=(BuPu-5-4);
  color=(BuPu-5-5);
},
colormap={BuPu-6}{
  color=(BuPu-6-1);
  color=(BuPu-6-2);
  color=(BuPu-6-3);
  color=(BuPu-6-4);
  color=(BuPu-6-5);
  color=(BuPu-6-6);
},
colormap={BuPu-7}{
  color=(BuPu-7-1);
  color=(BuPu-7-2);
  color=(BuPu-7-3);
  color=(BuPu-7-4);
  color=(BuPu-7-5);
  color=(BuPu-7-6);
  color=(BuPu-7-7);
},
colormap={BuPu-8}{
  color=(BuPu-8-1);
  color=(BuPu-8-2);
  color=(BuPu-8-3);
  color=(BuPu-8-4);
  color=(BuPu-8-5);
  color=(BuPu-8-6);
  color=(BuPu-8-7);
  color=(BuPu-8-8);
},
colormap={BuPu-9}{
  color=(BuPu-9-1);
  color=(BuPu-9-2);
  color=(BuPu-9-3);
  color=(BuPu-9-4);
  color=(BuPu-9-5);
  color=(BuPu-9-6);
  color=(BuPu-9-7);
  color=(BuPu-9-8);
  color=(BuPu-9-9);
},
colormap={RdPu-3}{
  color=(RdPu-3-1);
  color=(RdPu-3-2);
  color=(RdPu-3-3);
},
colormap={RdPu-4}{
  color=(RdPu-4-1);
  color=(RdPu-4-2);
  color=(RdPu-4-3);
  color=(RdPu-4-4);
},
colormap={RdPu-5}{
  color=(RdPu-5-1);
  color=(RdPu-5-2);
  color=(RdPu-5-3);
  color=(RdPu-5-4);
  color=(RdPu-5-5);
},
colormap={RdPu-6}{
  color=(RdPu-6-1);
  color=(RdPu-6-2);
  color=(RdPu-6-3);
  color=(RdPu-6-4);
  color=(RdPu-6-5);
  color=(RdPu-6-6);
},
colormap={RdPu-7}{
  color=(RdPu-7-1);
  color=(RdPu-7-2);
  color=(RdPu-7-3);
  color=(RdPu-7-4);
  color=(RdPu-7-5);
  color=(RdPu-7-6);
  color=(RdPu-7-7);
},
colormap={RdPu-8}{
  color=(RdPu-8-1);
  color=(RdPu-8-2);
  color=(RdPu-8-3);
  color=(RdPu-8-4);
  color=(RdPu-8-5);
  color=(RdPu-8-6);
  color=(RdPu-8-7);
  color=(RdPu-8-8);
},
colormap={RdPu-9}{
  color=(RdPu-9-1);
  color=(RdPu-9-2);
  color=(RdPu-9-3);
  color=(RdPu-9-4);
  color=(RdPu-9-5);
  color=(RdPu-9-6);
  color=(RdPu-9-7);
  color=(RdPu-9-8);
  color=(RdPu-9-9);
},
colormap={PuRd-3}{
  color=(PuRd-3-1);
  color=(PuRd-3-2);
  color=(PuRd-3-3);
},
colormap={PuRd-4}{
  color=(PuRd-4-1);
  color=(PuRd-4-2);
  color=(PuRd-4-3);
  color=(PuRd-4-4);
},
colormap={PuRd-5}{
  color=(PuRd-5-1);
  color=(PuRd-5-2);
  color=(PuRd-5-3);
  color=(PuRd-5-4);
  color=(PuRd-5-5);
},
colormap={PuRd-6}{
  color=(PuRd-6-1);
  color=(PuRd-6-2);
  color=(PuRd-6-3);
  color=(PuRd-6-4);
  color=(PuRd-6-5);
  color=(PuRd-6-6);
},
colormap={PuRd-7}{
  color=(PuRd-7-1);
  color=(PuRd-7-2);
  color=(PuRd-7-3);
  color=(PuRd-7-4);
  color=(PuRd-7-5);
  color=(PuRd-7-6);
  color=(PuRd-7-7);
},
colormap={PuRd-8}{
  color=(PuRd-8-1);
  color=(PuRd-8-2);
  color=(PuRd-8-3);
  color=(PuRd-8-4);
  color=(PuRd-8-5);
  color=(PuRd-8-6);
  color=(PuRd-8-7);
  color=(PuRd-8-8);
},
colormap={PuRd-9}{
  color=(PuRd-9-1);
  color=(PuRd-9-2);
  color=(PuRd-9-3);
  color=(PuRd-9-4);
  color=(PuRd-9-5);
  color=(PuRd-9-6);
  color=(PuRd-9-7);
  color=(PuRd-9-8);
  color=(PuRd-9-9);
},
colormap={OrRd-3}{
  color=(OrRd-3-1);
  color=(OrRd-3-2);
  color=(OrRd-3-3);
},
colormap={OrRd-4}{
  color=(OrRd-4-1);
  color=(OrRd-4-2);
  color=(OrRd-4-3);
  color=(OrRd-4-4);
},
colormap={OrRd-5}{
  color=(OrRd-5-1);
  color=(OrRd-5-2);
  color=(OrRd-5-3);
  color=(OrRd-5-4);
  color=(OrRd-5-5);
},
colormap={OrRd-6}{
  color=(OrRd-6-1);
  color=(OrRd-6-2);
  color=(OrRd-6-3);
  color=(OrRd-6-4);
  color=(OrRd-6-5);
  color=(OrRd-6-6);
},
colormap={OrRd-7}{
  color=(OrRd-7-1);
  color=(OrRd-7-2);
  color=(OrRd-7-3);
  color=(OrRd-7-4);
  color=(OrRd-7-5);
  color=(OrRd-7-6);
  color=(OrRd-7-7);
},
colormap={OrRd-8}{
  color=(OrRd-8-1);
  color=(OrRd-8-2);
  color=(OrRd-8-3);
  color=(OrRd-8-4);
  color=(OrRd-8-5);
  color=(OrRd-8-6);
  color=(OrRd-8-7);
  color=(OrRd-8-8);
},
colormap={OrRd-9}{
  color=(OrRd-9-1);
  color=(OrRd-9-2);
  color=(OrRd-9-3);
  color=(OrRd-9-4);
  color=(OrRd-9-5);
  color=(OrRd-9-6);
  color=(OrRd-9-7);
  color=(OrRd-9-8);
  color=(OrRd-9-9);
},
colormap={YlOrRd-3}{
  color=(YlOrRd-3-1);
  color=(YlOrRd-3-2);
  color=(YlOrRd-3-3);
},
colormap={YlOrRd-4}{
  color=(YlOrRd-4-1);
  color=(YlOrRd-4-2);
  color=(YlOrRd-4-3);
  color=(YlOrRd-4-4);
},
colormap={YlOrRd-5}{
  color=(YlOrRd-5-1);
  color=(YlOrRd-5-2);
  color=(YlOrRd-5-3);
  color=(YlOrRd-5-4);
  color=(YlOrRd-5-5);
},
colormap={YlOrRd-6}{
  color=(YlOrRd-6-1);
  color=(YlOrRd-6-2);
  color=(YlOrRd-6-3);
  color=(YlOrRd-6-4);
  color=(YlOrRd-6-5);
  color=(YlOrRd-6-6);
},
colormap={YlOrRd-7}{
  color=(YlOrRd-7-1);
  color=(YlOrRd-7-2);
  color=(YlOrRd-7-3);
  color=(YlOrRd-7-4);
  color=(YlOrRd-7-5);
  color=(YlOrRd-7-6);
  color=(YlOrRd-7-7);
},
colormap={YlOrRd-8}{
  color=(YlOrRd-8-1);
  color=(YlOrRd-8-2);
  color=(YlOrRd-8-3);
  color=(YlOrRd-8-4);
  color=(YlOrRd-8-5);
  color=(YlOrRd-8-6);
  color=(YlOrRd-8-7);
  color=(YlOrRd-8-8);
},
colormap={YlOrRd-9}{
  color=(YlOrRd-9-1);
  color=(YlOrRd-9-2);
  color=(YlOrRd-9-3);
  color=(YlOrRd-9-4);
  color=(YlOrRd-9-5);
  color=(YlOrRd-9-6);
  color=(YlOrRd-9-7);
  color=(YlOrRd-9-8);
  color=(YlOrRd-9-9);
},
colormap={YlOrBr-3}{
  color=(YlOrBr-3-1);
  color=(YlOrBr-3-2);
  color=(YlOrBr-3-3);
},
colormap={YlOrBr-4}{
  color=(YlOrBr-4-1);
  color=(YlOrBr-4-2);
  color=(YlOrBr-4-3);
  color=(YlOrBr-4-4);
},
colormap={YlOrBr-5}{
  color=(YlOrBr-5-1);
  color=(YlOrBr-5-2);
  color=(YlOrBr-5-3);
  color=(YlOrBr-5-4);
  color=(YlOrBr-5-5);
},
colormap={YlOrBr-6}{
  color=(YlOrBr-6-1);
  color=(YlOrBr-6-2);
  color=(YlOrBr-6-3);
  color=(YlOrBr-6-4);
  color=(YlOrBr-6-5);
  color=(YlOrBr-6-6);
},
colormap={YlOrBr-7}{
  color=(YlOrBr-7-1);
  color=(YlOrBr-7-2);
  color=(YlOrBr-7-3);
  color=(YlOrBr-7-4);
  color=(YlOrBr-7-5);
  color=(YlOrBr-7-6);
  color=(YlOrBr-7-7);
},
colormap={YlOrBr-8}{
  color=(YlOrBr-8-1);
  color=(YlOrBr-8-2);
  color=(YlOrBr-8-3);
  color=(YlOrBr-8-4);
  color=(YlOrBr-8-5);
  color=(YlOrBr-8-6);
  color=(YlOrBr-8-7);
  color=(YlOrBr-8-8);
},
colormap={YlOrBr-9}{
  color=(YlOrBr-9-1);
  color=(YlOrBr-9-2);
  color=(YlOrBr-9-3);
  color=(YlOrBr-9-4);
  color=(YlOrBr-9-5);
  color=(YlOrBr-9-6);
  color=(YlOrBr-9-7);
  color=(YlOrBr-9-8);
  color=(YlOrBr-9-9);
},
colormap={Purples-3}{
  color=(Purples-3-1);
  color=(Purples-3-2);
  color=(Purples-3-3);
},
colormap={Purples-4}{
  color=(Purples-4-1);
  color=(Purples-4-2);
  color=(Purples-4-3);
  color=(Purples-4-4);
},
colormap={Purples-5}{
  color=(Purples-5-1);
  color=(Purples-5-2);
  color=(Purples-5-3);
  color=(Purples-5-4);
  color=(Purples-5-5);
},
colormap={Purples-6}{
  color=(Purples-6-1);
  color=(Purples-6-2);
  color=(Purples-6-3);
  color=(Purples-6-4);
  color=(Purples-6-5);
  color=(Purples-6-6);
},
colormap={Purples-7}{
  color=(Purples-7-1);
  color=(Purples-7-2);
  color=(Purples-7-3);
  color=(Purples-7-4);
  color=(Purples-7-5);
  color=(Purples-7-6);
  color=(Purples-7-7);
},
colormap={Purples-8}{
  color=(Purples-8-1);
  color=(Purples-8-2);
  color=(Purples-8-3);
  color=(Purples-8-4);
  color=(Purples-8-5);
  color=(Purples-8-6);
  color=(Purples-8-7);
  color=(Purples-8-8);
},
colormap={Purples-9}{
  color=(Purples-9-1);
  color=(Purples-9-2);
  color=(Purples-9-3);
  color=(Purples-9-4);
  color=(Purples-9-5);
  color=(Purples-9-6);
  color=(Purples-9-7);
  color=(Purples-9-8);
  color=(Purples-9-9);
},
colormap={Blues-3}{
  color=(Blues-3-1);
  color=(Blues-3-2);
  color=(Blues-3-3);
},
colormap={Blues-4}{
  color=(Blues-4-1);
  color=(Blues-4-2);
  color=(Blues-4-3);
  color=(Blues-4-4);
},
colormap={Blues-5}{
  color=(Blues-5-1);
  color=(Blues-5-2);
  color=(Blues-5-3);
  color=(Blues-5-4);
  color=(Blues-5-5);
},
colormap={Blues-6}{
  color=(Blues-6-1);
  color=(Blues-6-2);
  color=(Blues-6-3);
  color=(Blues-6-4);
  color=(Blues-6-5);
  color=(Blues-6-6);
},
colormap={Blues-7}{
  color=(Blues-7-1);
  color=(Blues-7-2);
  color=(Blues-7-3);
  color=(Blues-7-4);
  color=(Blues-7-5);
  color=(Blues-7-6);
  color=(Blues-7-7);
},
colormap={Blues-8}{
  color=(Blues-8-1);
  color=(Blues-8-2);
  color=(Blues-8-3);
  color=(Blues-8-4);
  color=(Blues-8-5);
  color=(Blues-8-6);
  color=(Blues-8-7);
  color=(Blues-8-8);
},
colormap={Blues-9}{
  color=(Blues-9-1);
  color=(Blues-9-2);
  color=(Blues-9-3);
  color=(Blues-9-4);
  color=(Blues-9-5);
  color=(Blues-9-6);
  color=(Blues-9-7);
  color=(Blues-9-8);
  color=(Blues-9-9);
},
colormap={Greens-3}{
  color=(Greens-3-1);
  color=(Greens-3-2);
  color=(Greens-3-3);
},
colormap={Greens-4}{
  color=(Greens-4-1);
  color=(Greens-4-2);
  color=(Greens-4-3);
  color=(Greens-4-4);
},
colormap={Greens-5}{
  color=(Greens-5-1);
  color=(Greens-5-2);
  color=(Greens-5-3);
  color=(Greens-5-4);
  color=(Greens-5-5);
},
colormap={Greens-6}{
  color=(Greens-6-1);
  color=(Greens-6-2);
  color=(Greens-6-3);
  color=(Greens-6-4);
  color=(Greens-6-5);
  color=(Greens-6-6);
},
colormap={Greens-7}{
  color=(Greens-7-1);
  color=(Greens-7-2);
  color=(Greens-7-3);
  color=(Greens-7-4);
  color=(Greens-7-5);
  color=(Greens-7-6);
  color=(Greens-7-7);
},
colormap={Greens-8}{
  color=(Greens-8-1);
  color=(Greens-8-2);
  color=(Greens-8-3);
  color=(Greens-8-4);
  color=(Greens-8-5);
  color=(Greens-8-6);
  color=(Greens-8-7);
  color=(Greens-8-8);
},
colormap={Greens-9}{
  color=(Greens-9-1);
  color=(Greens-9-2);
  color=(Greens-9-3);
  color=(Greens-9-4);
  color=(Greens-9-5);
  color=(Greens-9-6);
  color=(Greens-9-7);
  color=(Greens-9-8);
  color=(Greens-9-9);
},
colormap={Oranges-3}{
  color=(Oranges-3-1);
  color=(Oranges-3-2);
  color=(Oranges-3-3);
},
colormap={Oranges-4}{
  color=(Oranges-4-1);
  color=(Oranges-4-2);
  color=(Oranges-4-3);
  color=(Oranges-4-4);
},
colormap={Oranges-5}{
  color=(Oranges-5-1);
  color=(Oranges-5-2);
  color=(Oranges-5-3);
  color=(Oranges-5-4);
  color=(Oranges-5-5);
},
colormap={Oranges-6}{
  color=(Oranges-6-1);
  color=(Oranges-6-2);
  color=(Oranges-6-3);
  color=(Oranges-6-4);
  color=(Oranges-6-5);
  color=(Oranges-6-6);
},
colormap={Oranges-7}{
  color=(Oranges-7-1);
  color=(Oranges-7-2);
  color=(Oranges-7-3);
  color=(Oranges-7-4);
  color=(Oranges-7-5);
  color=(Oranges-7-6);
  color=(Oranges-7-7);
},
colormap={Oranges-8}{
  color=(Oranges-8-1);
  color=(Oranges-8-2);
  color=(Oranges-8-3);
  color=(Oranges-8-4);
  color=(Oranges-8-5);
  color=(Oranges-8-6);
  color=(Oranges-8-7);
  color=(Oranges-8-8);
},
colormap={Oranges-9}{
  color=(Oranges-9-1);
  color=(Oranges-9-2);
  color=(Oranges-9-3);
  color=(Oranges-9-4);
  color=(Oranges-9-5);
  color=(Oranges-9-6);
  color=(Oranges-9-7);
  color=(Oranges-9-8);
  color=(Oranges-9-9);
},
colormap={Reds-3}{
  color=(Reds-3-1);
  color=(Reds-3-2);
  color=(Reds-3-3);
},
colormap={Reds-4}{
  color=(Reds-4-1);
  color=(Reds-4-2);
  color=(Reds-4-3);
  color=(Reds-4-4);
},
colormap={Reds-5}{
  color=(Reds-5-1);
  color=(Reds-5-2);
  color=(Reds-5-3);
  color=(Reds-5-4);
  color=(Reds-5-5);
},
colormap={Reds-6}{
  color=(Reds-6-1);
  color=(Reds-6-2);
  color=(Reds-6-3);
  color=(Reds-6-4);
  color=(Reds-6-5);
  color=(Reds-6-6);
},
colormap={Reds-7}{
  color=(Reds-7-1);
  color=(Reds-7-2);
  color=(Reds-7-3);
  color=(Reds-7-4);
  color=(Reds-7-5);
  color=(Reds-7-6);
  color=(Reds-7-7);
},
colormap={Reds-8}{
  color=(Reds-8-1);
  color=(Reds-8-2);
  color=(Reds-8-3);
  color=(Reds-8-4);
  color=(Reds-8-5);
  color=(Reds-8-6);
  color=(Reds-8-7);
  color=(Reds-8-8);
},
colormap={Reds-9}{
  color=(Reds-9-1);
  color=(Reds-9-2);
  color=(Reds-9-3);
  color=(Reds-9-4);
  color=(Reds-9-5);
  color=(Reds-9-6);
  color=(Reds-9-7);
  color=(Reds-9-8);
  color=(Reds-9-9);
},
colormap={Greys-3}{
  color=(Greys-3-1);
  color=(Greys-3-2);
  color=(Greys-3-3);
},
colormap={Greys-4}{
  color=(Greys-4-1);
  color=(Greys-4-2);
  color=(Greys-4-3);
  color=(Greys-4-4);
},
colormap={Greys-5}{
  color=(Greys-5-1);
  color=(Greys-5-2);
  color=(Greys-5-3);
  color=(Greys-5-4);
  color=(Greys-5-5);
},
colormap={Greys-6}{
  color=(Greys-6-1);
  color=(Greys-6-2);
  color=(Greys-6-3);
  color=(Greys-6-4);
  color=(Greys-6-5);
  color=(Greys-6-6);
},
colormap={Greys-7}{
  color=(Greys-7-1);
  color=(Greys-7-2);
  color=(Greys-7-3);
  color=(Greys-7-4);
  color=(Greys-7-5);
  color=(Greys-7-6);
  color=(Greys-7-7);
},
colormap={Greys-8}{
  color=(Greys-8-1);
  color=(Greys-8-2);
  color=(Greys-8-3);
  color=(Greys-8-4);
  color=(Greys-8-5);
  color=(Greys-8-6);
  color=(Greys-8-7);
  color=(Greys-8-8);
},
colormap={Greys-9}{
  color=(Greys-9-1);
  color=(Greys-9-2);
  color=(Greys-9-3);
  color=(Greys-9-4);
  color=(Greys-9-5);
  color=(Greys-9-6);
  color=(Greys-9-7);
  color=(Greys-9-8);
  color=(Greys-9-9);
},
colormap={PuOr-3}{
  color=(PuOr-3-1);
  color=(PuOr-3-2);
  color=(PuOr-3-3);
},
colormap={PuOr-4}{
  color=(PuOr-4-1);
  color=(PuOr-4-2);
  color=(PuOr-4-3);
  color=(PuOr-4-4);
},
colormap={PuOr-5}{
  color=(PuOr-5-1);
  color=(PuOr-5-2);
  color=(PuOr-5-3);
  color=(PuOr-5-4);
  color=(PuOr-5-5);
},
colormap={PuOr-6}{
  color=(PuOr-6-1);
  color=(PuOr-6-2);
  color=(PuOr-6-3);
  color=(PuOr-6-4);
  color=(PuOr-6-5);
  color=(PuOr-6-6);
},
colormap={PuOr-7}{
  color=(PuOr-7-1);
  color=(PuOr-7-2);
  color=(PuOr-7-3);
  color=(PuOr-7-4);
  color=(PuOr-7-5);
  color=(PuOr-7-6);
  color=(PuOr-7-7);
},
colormap={PuOr-8}{
  color=(PuOr-8-1);
  color=(PuOr-8-2);
  color=(PuOr-8-3);
  color=(PuOr-8-4);
  color=(PuOr-8-5);
  color=(PuOr-8-6);
  color=(PuOr-8-7);
  color=(PuOr-8-8);
},
colormap={PuOr-9}{
  color=(PuOr-9-1);
  color=(PuOr-9-2);
  color=(PuOr-9-3);
  color=(PuOr-9-4);
  color=(PuOr-9-5);
  color=(PuOr-9-6);
  color=(PuOr-9-7);
  color=(PuOr-9-8);
  color=(PuOr-9-9);
},
colormap={PuOr-10}{
  color=(PuOr-10-1);
  color=(PuOr-10-2);
  color=(PuOr-10-3);
  color=(PuOr-10-4);
  color=(PuOr-10-5);
  color=(PuOr-10-6);
  color=(PuOr-10-7);
  color=(PuOr-10-8);
  color=(PuOr-10-9);
  color=(PuOr-10-10);
},
colormap={PuOr-11}{
  color=(PuOr-11-1);
  color=(PuOr-11-2);
  color=(PuOr-11-3);
  color=(PuOr-11-4);
  color=(PuOr-11-5);
  color=(PuOr-11-6);
  color=(PuOr-11-7);
  color=(PuOr-11-8);
  color=(PuOr-11-9);
  color=(PuOr-11-10);
  color=(PuOr-11-11);
},
colormap={BrBG-3}{
  color=(BrBG-3-1);
  color=(BrBG-3-2);
  color=(BrBG-3-3);
},
colormap={BrBG-4}{
  color=(BrBG-4-1);
  color=(BrBG-4-2);
  color=(BrBG-4-3);
  color=(BrBG-4-4);
},
colormap={BrBG-5}{
  color=(BrBG-5-1);
  color=(BrBG-5-2);
  color=(BrBG-5-3);
  color=(BrBG-5-4);
  color=(BrBG-5-5);
},
colormap={BrBG-6}{
  color=(BrBG-6-1);
  color=(BrBG-6-2);
  color=(BrBG-6-3);
  color=(BrBG-6-4);
  color=(BrBG-6-5);
  color=(BrBG-6-6);
},
colormap={BrBG-7}{
  color=(BrBG-7-1);
  color=(BrBG-7-2);
  color=(BrBG-7-3);
  color=(BrBG-7-4);
  color=(BrBG-7-5);
  color=(BrBG-7-6);
  color=(BrBG-7-7);
},
colormap={BrBG-8}{
  color=(BrBG-8-1);
  color=(BrBG-8-2);
  color=(BrBG-8-3);
  color=(BrBG-8-4);
  color=(BrBG-8-5);
  color=(BrBG-8-6);
  color=(BrBG-8-7);
  color=(BrBG-8-8);
},
colormap={BrBG-9}{
  color=(BrBG-9-1);
  color=(BrBG-9-2);
  color=(BrBG-9-3);
  color=(BrBG-9-4);
  color=(BrBG-9-5);
  color=(BrBG-9-6);
  color=(BrBG-9-7);
  color=(BrBG-9-8);
  color=(BrBG-9-9);
},
colormap={BrBG-10}{
  color=(BrBG-10-1);
  color=(BrBG-10-2);
  color=(BrBG-10-3);
  color=(BrBG-10-4);
  color=(BrBG-10-5);
  color=(BrBG-10-6);
  color=(BrBG-10-7);
  color=(BrBG-10-8);
  color=(BrBG-10-9);
  color=(BrBG-10-10);
},
colormap={BrBG-11}{
  color=(BrBG-11-1);
  color=(BrBG-11-2);
  color=(BrBG-11-3);
  color=(BrBG-11-4);
  color=(BrBG-11-5);
  color=(BrBG-11-6);
  color=(BrBG-11-7);
  color=(BrBG-11-8);
  color=(BrBG-11-9);
  color=(BrBG-11-10);
  color=(BrBG-11-11);
},
colormap={PRGn-3}{
  color=(PRGn-3-1);
  color=(PRGn-3-2);
  color=(PRGn-3-3);
},
colormap={PRGn-4}{
  color=(PRGn-4-1);
  color=(PRGn-4-2);
  color=(PRGn-4-3);
  color=(PRGn-4-4);
},
colormap={PRGn-5}{
  color=(PRGn-5-1);
  color=(PRGn-5-2);
  color=(PRGn-5-3);
  color=(PRGn-5-4);
  color=(PRGn-5-5);
},
colormap={PRGn-6}{
  color=(PRGn-6-1);
  color=(PRGn-6-2);
  color=(PRGn-6-3);
  color=(PRGn-6-4);
  color=(PRGn-6-5);
  color=(PRGn-6-6);
},
colormap={PRGn-7}{
  color=(PRGn-7-1);
  color=(PRGn-7-2);
  color=(PRGn-7-3);
  color=(PRGn-7-4);
  color=(PRGn-7-5);
  color=(PRGn-7-6);
  color=(PRGn-7-7);
},
colormap={PRGn-8}{
  color=(PRGn-8-1);
  color=(PRGn-8-2);
  color=(PRGn-8-3);
  color=(PRGn-8-4);
  color=(PRGn-8-5);
  color=(PRGn-8-6);
  color=(PRGn-8-7);
  color=(PRGn-8-8);
},
colormap={PRGn-9}{
  color=(PRGn-9-1);
  color=(PRGn-9-2);
  color=(PRGn-9-3);
  color=(PRGn-9-4);
  color=(PRGn-9-5);
  color=(PRGn-9-6);
  color=(PRGn-9-7);
  color=(PRGn-9-8);
  color=(PRGn-9-9);
},
colormap={PRGn-10}{
  color=(PRGn-10-1);
  color=(PRGn-10-2);
  color=(PRGn-10-3);
  color=(PRGn-10-4);
  color=(PRGn-10-5);
  color=(PRGn-10-6);
  color=(PRGn-10-7);
  color=(PRGn-10-8);
  color=(PRGn-10-9);
  color=(PRGn-10-10);
},
colormap={PRGn-11}{
  color=(PRGn-11-1);
  color=(PRGn-11-2);
  color=(PRGn-11-3);
  color=(PRGn-11-4);
  color=(PRGn-11-5);
  color=(PRGn-11-6);
  color=(PRGn-11-7);
  color=(PRGn-11-8);
  color=(PRGn-11-9);
  color=(PRGn-11-10);
  color=(PRGn-11-11);
},
colormap={PiYG-3}{
  color=(PiYG-3-1);
  color=(PiYG-3-2);
  color=(PiYG-3-3);
},
colormap={PiYG-4}{
  color=(PiYG-4-1);
  color=(PiYG-4-2);
  color=(PiYG-4-3);
  color=(PiYG-4-4);
},
colormap={PiYG-5}{
  color=(PiYG-5-1);
  color=(PiYG-5-2);
  color=(PiYG-5-3);
  color=(PiYG-5-4);
  color=(PiYG-5-5);
},
colormap={PiYG-6}{
  color=(PiYG-6-1);
  color=(PiYG-6-2);
  color=(PiYG-6-3);
  color=(PiYG-6-4);
  color=(PiYG-6-5);
  color=(PiYG-6-6);
},
colormap={PiYG-7}{
  color=(PiYG-7-1);
  color=(PiYG-7-2);
  color=(PiYG-7-3);
  color=(PiYG-7-4);
  color=(PiYG-7-5);
  color=(PiYG-7-6);
  color=(PiYG-7-7);
},
colormap={PiYG-8}{
  color=(PiYG-8-1);
  color=(PiYG-8-2);
  color=(PiYG-8-3);
  color=(PiYG-8-4);
  color=(PiYG-8-5);
  color=(PiYG-8-6);
  color=(PiYG-8-7);
  color=(PiYG-8-8);
},
colormap={PiYG-9}{
  color=(PiYG-9-1);
  color=(PiYG-9-2);
  color=(PiYG-9-3);
  color=(PiYG-9-4);
  color=(PiYG-9-5);
  color=(PiYG-9-6);
  color=(PiYG-9-7);
  color=(PiYG-9-8);
  color=(PiYG-9-9);
},
colormap={PiYG-10}{
  color=(PiYG-10-1);
  color=(PiYG-10-2);
  color=(PiYG-10-3);
  color=(PiYG-10-4);
  color=(PiYG-10-5);
  color=(PiYG-10-6);
  color=(PiYG-10-7);
  color=(PiYG-10-8);
  color=(PiYG-10-9);
  color=(PiYG-10-10);
},
colormap={PiYG-11}{
  color=(PiYG-11-1);
  color=(PiYG-11-2);
  color=(PiYG-11-3);
  color=(PiYG-11-4);
  color=(PiYG-11-5);
  color=(PiYG-11-6);
  color=(PiYG-11-7);
  color=(PiYG-11-8);
  color=(PiYG-11-9);
  color=(PiYG-11-10);
  color=(PiYG-11-11);
},
colormap={RdBu-3}{
  color=(RdBu-3-1);
  color=(RdBu-3-2);
  color=(RdBu-3-3);
},
colormap={RdBu-4}{
  color=(RdBu-4-1);
  color=(RdBu-4-2);
  color=(RdBu-4-3);
  color=(RdBu-4-4);
},
colormap={RdBu-5}{
  color=(RdBu-5-1);
  color=(RdBu-5-2);
  color=(RdBu-5-3);
  color=(RdBu-5-4);
  color=(RdBu-5-5);
},
colormap={RdBu-6}{
  color=(RdBu-6-1);
  color=(RdBu-6-2);
  color=(RdBu-6-3);
  color=(RdBu-6-4);
  color=(RdBu-6-5);
  color=(RdBu-6-6);
},
colormap={RdBu-7}{
  color=(RdBu-7-1);
  color=(RdBu-7-2);
  color=(RdBu-7-3);
  color=(RdBu-7-4);
  color=(RdBu-7-5);
  color=(RdBu-7-6);
  color=(RdBu-7-7);
},
colormap={RdBu-8}{
  color=(RdBu-8-1);
  color=(RdBu-8-2);
  color=(RdBu-8-3);
  color=(RdBu-8-4);
  color=(RdBu-8-5);
  color=(RdBu-8-6);
  color=(RdBu-8-7);
  color=(RdBu-8-8);
},
colormap={RdBu-9}{
  color=(RdBu-9-1);
  color=(RdBu-9-2);
  color=(RdBu-9-3);
  color=(RdBu-9-4);
  color=(RdBu-9-5);
  color=(RdBu-9-6);
  color=(RdBu-9-7);
  color=(RdBu-9-8);
  color=(RdBu-9-9);
},
colormap={RdBu-10}{
  color=(RdBu-10-1);
  color=(RdBu-10-2);
  color=(RdBu-10-3);
  color=(RdBu-10-4);
  color=(RdBu-10-5);
  color=(RdBu-10-6);
  color=(RdBu-10-7);
  color=(RdBu-10-8);
  color=(RdBu-10-9);
  color=(RdBu-10-10);
},
colormap={RdBu-11}{
  color=(RdBu-11-1);
  color=(RdBu-11-2);
  color=(RdBu-11-3);
  color=(RdBu-11-4);
  color=(RdBu-11-5);
  color=(RdBu-11-6);
  color=(RdBu-11-7);
  color=(RdBu-11-8);
  color=(RdBu-11-9);
  color=(RdBu-11-10);
  color=(RdBu-11-11);
},
colormap={RdGy-3}{
  color=(RdGy-3-1);
  color=(RdGy-3-2);
  color=(RdGy-3-3);
},
colormap={RdGy-4}{
  color=(RdGy-4-1);
  color=(RdGy-4-2);
  color=(RdGy-4-3);
  color=(RdGy-4-4);
},
colormap={RdGy-5}{
  color=(RdGy-5-1);
  color=(RdGy-5-2);
  color=(RdGy-5-3);
  color=(RdGy-5-4);
  color=(RdGy-5-5);
},
colormap={RdGy-6}{
  color=(RdGy-6-1);
  color=(RdGy-6-2);
  color=(RdGy-6-3);
  color=(RdGy-6-4);
  color=(RdGy-6-5);
  color=(RdGy-6-6);
},
colormap={RdGy-7}{
  color=(RdGy-7-1);
  color=(RdGy-7-2);
  color=(RdGy-7-3);
  color=(RdGy-7-4);
  color=(RdGy-7-5);
  color=(RdGy-7-6);
  color=(RdGy-7-7);
},
colormap={RdGy-8}{
  color=(RdGy-8-1);
  color=(RdGy-8-2);
  color=(RdGy-8-3);
  color=(RdGy-8-4);
  color=(RdGy-8-5);
  color=(RdGy-8-6);
  color=(RdGy-8-7);
  color=(RdGy-8-8);
},
colormap={RdGy-9}{
  color=(RdGy-9-1);
  color=(RdGy-9-2);
  color=(RdGy-9-3);
  color=(RdGy-9-4);
  color=(RdGy-9-5);
  color=(RdGy-9-6);
  color=(RdGy-9-7);
  color=(RdGy-9-8);
  color=(RdGy-9-9);
},
colormap={RdGy-10}{
  color=(RdGy-10-1);
  color=(RdGy-10-2);
  color=(RdGy-10-3);
  color=(RdGy-10-4);
  color=(RdGy-10-5);
  color=(RdGy-10-6);
  color=(RdGy-10-7);
  color=(RdGy-10-8);
  color=(RdGy-10-9);
  color=(RdGy-10-10);
},
colormap={RdGy-11}{
  color=(RdGy-11-1);
  color=(RdGy-11-2);
  color=(RdGy-11-3);
  color=(RdGy-11-4);
  color=(RdGy-11-5);
  color=(RdGy-11-6);
  color=(RdGy-11-7);
  color=(RdGy-11-8);
  color=(RdGy-11-9);
  color=(RdGy-11-10);
  color=(RdGy-11-11);
},
colormap={RdYlBu-3}{
  color=(RdYlBu-3-1);
  color=(RdYlBu-3-2);
  color=(RdYlBu-3-3);
},
colormap={RdYlBu-4}{
  color=(RdYlBu-4-1);
  color=(RdYlBu-4-2);
  color=(RdYlBu-4-3);
  color=(RdYlBu-4-4);
},
colormap={RdYlBu-5}{
  color=(RdYlBu-5-1);
  color=(RdYlBu-5-2);
  color=(RdYlBu-5-3);
  color=(RdYlBu-5-4);
  color=(RdYlBu-5-5);
},
colormap={RdYlBu-6}{
  color=(RdYlBu-6-1);
  color=(RdYlBu-6-2);
  color=(RdYlBu-6-3);
  color=(RdYlBu-6-4);
  color=(RdYlBu-6-5);
  color=(RdYlBu-6-6);
},
colormap={RdYlBu-7}{
  color=(RdYlBu-7-1);
  color=(RdYlBu-7-2);
  color=(RdYlBu-7-3);
  color=(RdYlBu-7-4);
  color=(RdYlBu-7-5);
  color=(RdYlBu-7-6);
  color=(RdYlBu-7-7);
},
colormap={RdYlBu-8}{
  color=(RdYlBu-8-1);
  color=(RdYlBu-8-2);
  color=(RdYlBu-8-3);
  color=(RdYlBu-8-4);
  color=(RdYlBu-8-5);
  color=(RdYlBu-8-6);
  color=(RdYlBu-8-7);
  color=(RdYlBu-8-8);
},
colormap={RdYlBu-9}{
  color=(RdYlBu-9-1);
  color=(RdYlBu-9-2);
  color=(RdYlBu-9-3);
  color=(RdYlBu-9-4);
  color=(RdYlBu-9-5);
  color=(RdYlBu-9-6);
  color=(RdYlBu-9-7);
  color=(RdYlBu-9-8);
  color=(RdYlBu-9-9);
},
colormap={RdYlBu-10}{
  color=(RdYlBu-10-1);
  color=(RdYlBu-10-2);
  color=(RdYlBu-10-3);
  color=(RdYlBu-10-4);
  color=(RdYlBu-10-5);
  color=(RdYlBu-10-6);
  color=(RdYlBu-10-7);
  color=(RdYlBu-10-8);
  color=(RdYlBu-10-9);
  color=(RdYlBu-10-10);
},
colormap={RdYlBu-11}{
  color=(RdYlBu-11-1);
  color=(RdYlBu-11-2);
  color=(RdYlBu-11-3);
  color=(RdYlBu-11-4);
  color=(RdYlBu-11-5);
  color=(RdYlBu-11-6);
  color=(RdYlBu-11-7);
  color=(RdYlBu-11-8);
  color=(RdYlBu-11-9);
  color=(RdYlBu-11-10);
  color=(RdYlBu-11-11);
},
colormap={Spectral-3}{
  color=(Spectral-3-1);
  color=(Spectral-3-2);
  color=(Spectral-3-3);
},
colormap={Spectral-4}{
  color=(Spectral-4-1);
  color=(Spectral-4-2);
  color=(Spectral-4-3);
  color=(Spectral-4-4);
},
colormap={Spectral-5}{
  color=(Spectral-5-1);
  color=(Spectral-5-2);
  color=(Spectral-5-3);
  color=(Spectral-5-4);
  color=(Spectral-5-5);
},
colormap={Spectral-6}{
  color=(Spectral-6-1);
  color=(Spectral-6-2);
  color=(Spectral-6-3);
  color=(Spectral-6-4);
  color=(Spectral-6-5);
  color=(Spectral-6-6);
},
colormap={Spectral-7}{
  color=(Spectral-7-1);
  color=(Spectral-7-2);
  color=(Spectral-7-3);
  color=(Spectral-7-4);
  color=(Spectral-7-5);
  color=(Spectral-7-6);
  color=(Spectral-7-7);
},
colormap={Spectral-8}{
  color=(Spectral-8-1);
  color=(Spectral-8-2);
  color=(Spectral-8-3);
  color=(Spectral-8-4);
  color=(Spectral-8-5);
  color=(Spectral-8-6);
  color=(Spectral-8-7);
  color=(Spectral-8-8);
},
colormap={Spectral-9}{
  color=(Spectral-9-1);
  color=(Spectral-9-2);
  color=(Spectral-9-3);
  color=(Spectral-9-4);
  color=(Spectral-9-5);
  color=(Spectral-9-6);
  color=(Spectral-9-7);
  color=(Spectral-9-8);
  color=(Spectral-9-9);
},
colormap={Spectral-10}{
  color=(Spectral-10-1);
  color=(Spectral-10-2);
  color=(Spectral-10-3);
  color=(Spectral-10-4);
  color=(Spectral-10-5);
  color=(Spectral-10-6);
  color=(Spectral-10-7);
  color=(Spectral-10-8);
  color=(Spectral-10-9);
  color=(Spectral-10-10);
},
colormap={Spectral-11}{
  color=(Spectral-11-1);
  color=(Spectral-11-2);
  color=(Spectral-11-3);
  color=(Spectral-11-4);
  color=(Spectral-11-5);
  color=(Spectral-11-6);
  color=(Spectral-11-7);
  color=(Spectral-11-8);
  color=(Spectral-11-9);
  color=(Spectral-11-10);
  color=(Spectral-11-11);
},
colormap={RdYlGn-3}{
  color=(RdYlGn-3-1);
  color=(RdYlGn-3-2);
  color=(RdYlGn-3-3);
},
colormap={RdYlGn-4}{
  color=(RdYlGn-4-1);
  color=(RdYlGn-4-2);
  color=(RdYlGn-4-3);
  color=(RdYlGn-4-4);
},
colormap={RdYlGn-5}{
  color=(RdYlGn-5-1);
  color=(RdYlGn-5-2);
  color=(RdYlGn-5-3);
  color=(RdYlGn-5-4);
  color=(RdYlGn-5-5);
},
colormap={RdYlGn-6}{
  color=(RdYlGn-6-1);
  color=(RdYlGn-6-2);
  color=(RdYlGn-6-3);
  color=(RdYlGn-6-4);
  color=(RdYlGn-6-5);
  color=(RdYlGn-6-6);
},
colormap={RdYlGn-7}{
  color=(RdYlGn-7-1);
  color=(RdYlGn-7-2);
  color=(RdYlGn-7-3);
  color=(RdYlGn-7-4);
  color=(RdYlGn-7-5);
  color=(RdYlGn-7-6);
  color=(RdYlGn-7-7);
},
colormap={RdYlGn-8}{
  color=(RdYlGn-8-1);
  color=(RdYlGn-8-2);
  color=(RdYlGn-8-3);
  color=(RdYlGn-8-4);
  color=(RdYlGn-8-5);
  color=(RdYlGn-8-6);
  color=(RdYlGn-8-7);
  color=(RdYlGn-8-8);
},
colormap={RdYlGn-9}{
  color=(RdYlGn-9-1);
  color=(RdYlGn-9-2);
  color=(RdYlGn-9-3);
  color=(RdYlGn-9-4);
  color=(RdYlGn-9-5);
  color=(RdYlGn-9-6);
  color=(RdYlGn-9-7);
  color=(RdYlGn-9-8);
  color=(RdYlGn-9-9);
},
colormap={RdYlGn-10}{
  color=(RdYlGn-10-1);
  color=(RdYlGn-10-2);
  color=(RdYlGn-10-3);
  color=(RdYlGn-10-4);
  color=(RdYlGn-10-5);
  color=(RdYlGn-10-6);
  color=(RdYlGn-10-7);
  color=(RdYlGn-10-8);
  color=(RdYlGn-10-9);
  color=(RdYlGn-10-10);
},
colormap={RdYlGn-11}{
  color=(RdYlGn-11-1);
  color=(RdYlGn-11-2);
  color=(RdYlGn-11-3);
  color=(RdYlGn-11-4);
  color=(RdYlGn-11-5);
  color=(RdYlGn-11-6);
  color=(RdYlGn-11-7);
  color=(RdYlGn-11-8);
  color=(RdYlGn-11-9);
  color=(RdYlGn-11-10);
  color=(RdYlGn-11-11);
},
colormap={Set3-3}{
  color=(Set3-3-1);
  color=(Set3-3-2);
  color=(Set3-3-3);
},
colormap={Set3-4}{
  color=(Set3-4-1);
  color=(Set3-4-2);
  color=(Set3-4-3);
  color=(Set3-4-4);
},
colormap={Set3-5}{
  color=(Set3-5-1);
  color=(Set3-5-2);
  color=(Set3-5-3);
  color=(Set3-5-4);
  color=(Set3-5-5);
},
colormap={Set3-6}{
  color=(Set3-6-1);
  color=(Set3-6-2);
  color=(Set3-6-3);
  color=(Set3-6-4);
  color=(Set3-6-5);
  color=(Set3-6-6);
},
colormap={Set3-7}{
  color=(Set3-7-1);
  color=(Set3-7-2);
  color=(Set3-7-3);
  color=(Set3-7-4);
  color=(Set3-7-5);
  color=(Set3-7-6);
  color=(Set3-7-7);
},
colormap={Set3-8}{
  color=(Set3-8-1);
  color=(Set3-8-2);
  color=(Set3-8-3);
  color=(Set3-8-4);
  color=(Set3-8-5);
  color=(Set3-8-6);
  color=(Set3-8-7);
  color=(Set3-8-8);
},
colormap={Set3-9}{
  color=(Set3-9-1);
  color=(Set3-9-2);
  color=(Set3-9-3);
  color=(Set3-9-4);
  color=(Set3-9-5);
  color=(Set3-9-6);
  color=(Set3-9-7);
  color=(Set3-9-8);
  color=(Set3-9-9);
},
colormap={Set3-10}{
  color=(Set3-10-1);
  color=(Set3-10-2);
  color=(Set3-10-3);
  color=(Set3-10-4);
  color=(Set3-10-5);
  color=(Set3-10-6);
  color=(Set3-10-7);
  color=(Set3-10-8);
  color=(Set3-10-9);
  color=(Set3-10-10);
},
colormap={Set3-11}{
  color=(Set3-11-1);
  color=(Set3-11-2);
  color=(Set3-11-3);
  color=(Set3-11-4);
  color=(Set3-11-5);
  color=(Set3-11-6);
  color=(Set3-11-7);
  color=(Set3-11-8);
  color=(Set3-11-9);
  color=(Set3-11-10);
  color=(Set3-11-11);
},
colormap={Set3-12}{
  color=(Set3-12-1);
  color=(Set3-12-2);
  color=(Set3-12-3);
  color=(Set3-12-4);
  color=(Set3-12-5);
  color=(Set3-12-6);
  color=(Set3-12-7);
  color=(Set3-12-8);
  color=(Set3-12-9);
  color=(Set3-12-10);
  color=(Set3-12-11);
  color=(Set3-12-12);
},
colormap={Pastel1-3}{
  color=(Pastel1-3-1);
  color=(Pastel1-3-2);
  color=(Pastel1-3-3);
},
colormap={Pastel1-4}{
  color=(Pastel1-4-1);
  color=(Pastel1-4-2);
  color=(Pastel1-4-3);
  color=(Pastel1-4-4);
},
colormap={Pastel1-5}{
  color=(Pastel1-5-1);
  color=(Pastel1-5-2);
  color=(Pastel1-5-3);
  color=(Pastel1-5-4);
  color=(Pastel1-5-5);
},
colormap={Pastel1-6}{
  color=(Pastel1-6-1);
  color=(Pastel1-6-2);
  color=(Pastel1-6-3);
  color=(Pastel1-6-4);
  color=(Pastel1-6-5);
  color=(Pastel1-6-6);
},
colormap={Pastel1-7}{
  color=(Pastel1-7-1);
  color=(Pastel1-7-2);
  color=(Pastel1-7-3);
  color=(Pastel1-7-4);
  color=(Pastel1-7-5);
  color=(Pastel1-7-6);
  color=(Pastel1-7-7);
},
colormap={Pastel1-8}{
  color=(Pastel1-8-1);
  color=(Pastel1-8-2);
  color=(Pastel1-8-3);
  color=(Pastel1-8-4);
  color=(Pastel1-8-5);
  color=(Pastel1-8-6);
  color=(Pastel1-8-7);
  color=(Pastel1-8-8);
},
colormap={Pastel1-9}{
  color=(Pastel1-9-1);
  color=(Pastel1-9-2);
  color=(Pastel1-9-3);
  color=(Pastel1-9-4);
  color=(Pastel1-9-5);
  color=(Pastel1-9-6);
  color=(Pastel1-9-7);
  color=(Pastel1-9-8);
  color=(Pastel1-9-9);
},
colormap={Set1-3}{
  color=(Set1-3-1);
  color=(Set1-3-2);
  color=(Set1-3-3);
},
colormap={Set1-4}{
  color=(Set1-4-1);
  color=(Set1-4-2);
  color=(Set1-4-3);
  color=(Set1-4-4);
},
colormap={Set1-5}{
  color=(Set1-5-1);
  color=(Set1-5-2);
  color=(Set1-5-3);
  color=(Set1-5-4);
  color=(Set1-5-5);
},
colormap={Set1-6}{
  color=(Set1-6-1);
  color=(Set1-6-2);
  color=(Set1-6-3);
  color=(Set1-6-4);
  color=(Set1-6-5);
  color=(Set1-6-6);
},
colormap={Set1-7}{
  color=(Set1-7-1);
  color=(Set1-7-2);
  color=(Set1-7-3);
  color=(Set1-7-4);
  color=(Set1-7-5);
  color=(Set1-7-6);
  color=(Set1-7-7);
},
colormap={Set1-8}{
  color=(Set1-8-1);
  color=(Set1-8-2);
  color=(Set1-8-3);
  color=(Set1-8-4);
  color=(Set1-8-5);
  color=(Set1-8-6);
  color=(Set1-8-7);
  color=(Set1-8-8);
},
colormap={Set1-9}{
  color=(Set1-9-1);
  color=(Set1-9-2);
  color=(Set1-9-3);
  color=(Set1-9-4);
  color=(Set1-9-5);
  color=(Set1-9-6);
  color=(Set1-9-7);
  color=(Set1-9-8);
  color=(Set1-9-9);
},
colormap={Pastel2-3}{
  color=(Pastel2-3-1);
  color=(Pastel2-3-2);
  color=(Pastel2-3-3);
},
colormap={Pastel2-4}{
  color=(Pastel2-4-1);
  color=(Pastel2-4-2);
  color=(Pastel2-4-3);
  color=(Pastel2-4-4);
},
colormap={Pastel2-5}{
  color=(Pastel2-5-1);
  color=(Pastel2-5-2);
  color=(Pastel2-5-3);
  color=(Pastel2-5-4);
  color=(Pastel2-5-5);
},
colormap={Pastel2-6}{
  color=(Pastel2-6-1);
  color=(Pastel2-6-2);
  color=(Pastel2-6-3);
  color=(Pastel2-6-4);
  color=(Pastel2-6-5);
  color=(Pastel2-6-6);
},
colormap={Pastel2-7}{
  color=(Pastel2-7-1);
  color=(Pastel2-7-2);
  color=(Pastel2-7-3);
  color=(Pastel2-7-4);
  color=(Pastel2-7-5);
  color=(Pastel2-7-6);
  color=(Pastel2-7-7);
},
colormap={Pastel2-8}{
  color=(Pastel2-8-1);
  color=(Pastel2-8-2);
  color=(Pastel2-8-3);
  color=(Pastel2-8-4);
  color=(Pastel2-8-5);
  color=(Pastel2-8-6);
  color=(Pastel2-8-7);
  color=(Pastel2-8-8);
},
colormap={Set2-3}{
  color=(Set2-3-1);
  color=(Set2-3-2);
  color=(Set2-3-3);
},
colormap={Set2-4}{
  color=(Set2-4-1);
  color=(Set2-4-2);
  color=(Set2-4-3);
  color=(Set2-4-4);
},
colormap={Set2-5}{
  color=(Set2-5-1);
  color=(Set2-5-2);
  color=(Set2-5-3);
  color=(Set2-5-4);
  color=(Set2-5-5);
},
colormap={Set2-6}{
  color=(Set2-6-1);
  color=(Set2-6-2);
  color=(Set2-6-3);
  color=(Set2-6-4);
  color=(Set2-6-5);
  color=(Set2-6-6);
},
colormap={Set2-7}{
  color=(Set2-7-1);
  color=(Set2-7-2);
  color=(Set2-7-3);
  color=(Set2-7-4);
  color=(Set2-7-5);
  color=(Set2-7-6);
  color=(Set2-7-7);
},
colormap={Set2-8}{
  color=(Set2-8-1);
  color=(Set2-8-2);
  color=(Set2-8-3);
  color=(Set2-8-4);
  color=(Set2-8-5);
  color=(Set2-8-6);
  color=(Set2-8-7);
  color=(Set2-8-8);
},
colormap={Dark2-3}{
  color=(Dark2-3-1);
  color=(Dark2-3-2);
  color=(Dark2-3-3);
},
colormap={Dark2-4}{
  color=(Dark2-4-1);
  color=(Dark2-4-2);
  color=(Dark2-4-3);
  color=(Dark2-4-4);
},
colormap={Dark2-5}{
  color=(Dark2-5-1);
  color=(Dark2-5-2);
  color=(Dark2-5-3);
  color=(Dark2-5-4);
  color=(Dark2-5-5);
},
colormap={Dark2-6}{
  color=(Dark2-6-1);
  color=(Dark2-6-2);
  color=(Dark2-6-3);
  color=(Dark2-6-4);
  color=(Dark2-6-5);
  color=(Dark2-6-6);
},
colormap={Dark2-7}{
  color=(Dark2-7-1);
  color=(Dark2-7-2);
  color=(Dark2-7-3);
  color=(Dark2-7-4);
  color=(Dark2-7-5);
  color=(Dark2-7-6);
  color=(Dark2-7-7);
},
colormap={Dark2-8}{
  color=(Dark2-8-1);
  color=(Dark2-8-2);
  color=(Dark2-8-3);
  color=(Dark2-8-4);
  color=(Dark2-8-5);
  color=(Dark2-8-6);
  color=(Dark2-8-7);
  color=(Dark2-8-8);
},
colormap={Paired-3}{
  color=(Paired-3-1);
  color=(Paired-3-2);
  color=(Paired-3-3);
},
colormap={Paired-4}{
  color=(Paired-4-1);
  color=(Paired-4-2);
  color=(Paired-4-3);
  color=(Paired-4-4);
},
colormap={Paired-5}{
  color=(Paired-5-1);
  color=(Paired-5-2);
  color=(Paired-5-3);
  color=(Paired-5-4);
  color=(Paired-5-5);
},
colormap={Paired-6}{
  color=(Paired-6-1);
  color=(Paired-6-2);
  color=(Paired-6-3);
  color=(Paired-6-4);
  color=(Paired-6-5);
  color=(Paired-6-6);
},
colormap={Paired-7}{
  color=(Paired-7-1);
  color=(Paired-7-2);
  color=(Paired-7-3);
  color=(Paired-7-4);
  color=(Paired-7-5);
  color=(Paired-7-6);
  color=(Paired-7-7);
},
colormap={Paired-8}{
  color=(Paired-8-1);
  color=(Paired-8-2);
  color=(Paired-8-3);
  color=(Paired-8-4);
  color=(Paired-8-5);
  color=(Paired-8-6);
  color=(Paired-8-7);
  color=(Paired-8-8);
},
colormap={Paired-9}{
  color=(Paired-9-1);
  color=(Paired-9-2);
  color=(Paired-9-3);
  color=(Paired-9-4);
  color=(Paired-9-5);
  color=(Paired-9-6);
  color=(Paired-9-7);
  color=(Paired-9-8);
  color=(Paired-9-9);
},
colormap={Paired-10}{
  color=(Paired-10-1);
  color=(Paired-10-2);
  color=(Paired-10-3);
  color=(Paired-10-4);
  color=(Paired-10-5);
  color=(Paired-10-6);
  color=(Paired-10-7);
  color=(Paired-10-8);
  color=(Paired-10-9);
  color=(Paired-10-10);
},
colormap={Paired-11}{
  color=(Paired-11-1);
  color=(Paired-11-2);
  color=(Paired-11-3);
  color=(Paired-11-4);
  color=(Paired-11-5);
  color=(Paired-11-6);
  color=(Paired-11-7);
  color=(Paired-11-8);
  color=(Paired-11-9);
  color=(Paired-11-10);
  color=(Paired-11-11);
},
colormap={Paired-12}{
  color=(Paired-12-1);
  color=(Paired-12-2);
  color=(Paired-12-3);
  color=(Paired-12-4);
  color=(Paired-12-5);
  color=(Paired-12-6);
  color=(Paired-12-7);
  color=(Paired-12-8);
  color=(Paired-12-9);
  color=(Paired-12-10);
  color=(Paired-12-11);
  color=(Paired-12-12);
},
colormap={Accent-3}{
  color=(Accent-3-1);
  color=(Accent-3-2);
  color=(Accent-3-3);
},
colormap={Accent-4}{
  color=(Accent-4-1);
  color=(Accent-4-2);
  color=(Accent-4-3);
  color=(Accent-4-4);
},
colormap={Accent-5}{
  color=(Accent-5-1);
  color=(Accent-5-2);
  color=(Accent-5-3);
  color=(Accent-5-4);
  color=(Accent-5-5);
},
colormap={Accent-6}{
  color=(Accent-6-1);
  color=(Accent-6-2);
  color=(Accent-6-3);
  color=(Accent-6-4);
  color=(Accent-6-5);
  color=(Accent-6-6);
},
colormap={Accent-7}{
  color=(Accent-7-1);
  color=(Accent-7-2);
  color=(Accent-7-3);
  color=(Accent-7-4);
  color=(Accent-7-5);
  color=(Accent-7-6);
  color=(Accent-7-7);
},
colormap={Accent-8}{
  color=(Accent-8-1);
  color=(Accent-8-2);
  color=(Accent-8-3);
  color=(Accent-8-4);
  color=(Accent-8-5);
  color=(Accent-8-6);
  color=(Accent-8-7);
  color=(Accent-8-8);
}
}


==> tikzlibrarycolorbrewer.code.tex <==
% Color schemes as obtained from http://colorbrewer2.org/
%
% Apache-Style Software License for ColorBrewer software and ColorBrewer Color
% Schemes
% 
% Copyright (c) 2002 Cynthia Brewer, Mark Harrower, and The Pennsylvania State
% University.
% 
% Licensed under the Apache License, Version 2.0 (the "License"); you may not
% use this file except in compliance with the License.  You may obtain a copy of
% the License at
% 
%        http://www.apache.org/licenses/LICENSE-2.0
% 
% Unless required by applicable law or agreed to in writing, software
% distributed under the License is distributed on an "AS IS" BASIS, WITHOUT
% WARRANTIES OR CONDITIONS OF ANY KIND, either express or implied.  See the
% License for the specific language governing permissions and limitations under
% the License.
% 
% Redistribution and use in source and binary forms, with or without
% modification, are permitted provided that the following conditions are met:
% 1. Redistributions as source code must retain the above copyright notice, this
%    list of conditions and the following disclaimer.
% 2. The end-user documentation included with the redistribution, if any, must
%    include the following acknowledgment: This product includes color
%    specifications and designs developed by Cynthia Brewer
%    (http://colorbrewer.org/).  Alternately, this acknowledgment may appear in the
%    software itself, if and wherever such third-party acknowledgments normally
%    appear.
% 3. The name "ColorBrewer" must not be used to endorse or promote products
%    derived from this software without prior written permission.  For written
%    permission, please contact Cynthia Brewer at cbrewer@psu.edu.
% 4. Products derived from this software may not be called "ColorBrewer", nor
%    may "ColorBrewer" appear in their name, without prior written permission of
%    Cynthia Brewer.
\definecolor{YlGn-3-1}{RGB}{247,252,185}
\definecolor{YlGn-3-C}{RGB}{247,252,185}
\definecolor{YlGn-3-2}{RGB}{173,221,142}
\definecolor{YlGn-3-F}{RGB}{173,221,142}
\definecolor{YlGn-3-3}{RGB}{49,163,84}
\definecolor{YlGn-3-I}{RGB}{49,163,84}
\definecolor{YlGn-4-1}{RGB}{255,255,204}
\definecolor{YlGn-4-B}{RGB}{255,255,204}
\definecolor{YlGn-4-2}{RGB}{194,230,153}
\definecolor{YlGn-4-E}{RGB}{194,230,153}
\definecolor{YlGn-4-3}{RGB}{120,198,121}
\definecolor{YlGn-4-G}{RGB}{120,198,121}
\definecolor{YlGn-4-4}{RGB}{35,132,67}
\definecolor{YlGn-4-J}{RGB}{35,132,67}
\definecolor{YlGn-5-1}{RGB}{255,255,204}
\definecolor{YlGn-5-B}{RGB}{255,255,204}
\definecolor{YlGn-5-2}{RGB}{194,230,153}
\definecolor{YlGn-5-E}{RGB}{194,230,153}
\definecolor{YlGn-5-3}{RGB}{120,198,121}
\definecolor{YlGn-5-G}{RGB}{120,198,121}
\definecolor{YlGn-5-4}{RGB}{49,163,84}
\definecolor{YlGn-5-I}{RGB}{49,163,84}
\definecolor{YlGn-5-5}{RGB}{0,104,55}
\definecolor{YlGn-5-K}{RGB}{0,104,55}
\definecolor{YlGn-6-1}{RGB}{255,255,204}
\definecolor{YlGn-6-B}{RGB}{255,255,204}
\definecolor{YlGn-6-2}{RGB}{217,240,163}
\definecolor{YlGn-6-D}{RGB}{217,240,163}
\definecolor{YlGn-6-3}{RGB}{173,221,142}
\definecolor{YlGn-6-F}{RGB}{173,221,142}
\definecolor{YlGn-6-4}{RGB}{120,198,121}
\definecolor{YlGn-6-G}{RGB}{120,198,121}
\definecolor{YlGn-6-5}{RGB}{49,163,84}
\definecolor{YlGn-6-I}{RGB}{49,163,84}
\definecolor{YlGn-6-6}{RGB}{0,104,55}
\definecolor{YlGn-6-K}{RGB}{0,104,55}
\definecolor{YlGn-7-1}{RGB}{255,255,204}
\definecolor{YlGn-7-B}{RGB}{255,255,204}
\definecolor{YlGn-7-2}{RGB}{217,240,163}
\definecolor{YlGn-7-D}{RGB}{217,240,163}
\definecolor{YlGn-7-3}{RGB}{173,221,142}
\definecolor{YlGn-7-F}{RGB}{173,221,142}
\definecolor{YlGn-7-4}{RGB}{120,198,121}
\definecolor{YlGn-7-G}{RGB}{120,198,121}
\definecolor{YlGn-7-5}{RGB}{65,171,93}
\definecolor{YlGn-7-H}{RGB}{65,171,93}
\definecolor{YlGn-7-6}{RGB}{35,132,67}
\definecolor{YlGn-7-J}{RGB}{35,132,67}
\definecolor{YlGn-7-7}{RGB}{0,90,50}
\definecolor{YlGn-7-L}{RGB}{0,90,50}
\definecolor{YlGn-8-1}{RGB}{255,255,229}
\definecolor{YlGn-8-A}{RGB}{255,255,229}
\definecolor{YlGn-8-2}{RGB}{247,252,185}
\definecolor{YlGn-8-C}{RGB}{247,252,185}
\definecolor{YlGn-8-3}{RGB}{217,240,163}
\definecolor{YlGn-8-D}{RGB}{217,240,163}
\definecolor{YlGn-8-4}{RGB}{173,221,142}
\definecolor{YlGn-8-F}{RGB}{173,221,142}
\definecolor{YlGn-8-5}{RGB}{120,198,121}
\definecolor{YlGn-8-G}{RGB}{120,198,121}
\definecolor{YlGn-8-6}{RGB}{65,171,93}
\definecolor{YlGn-8-H}{RGB}{65,171,93}
\definecolor{YlGn-8-7}{RGB}{35,132,67}
\definecolor{YlGn-8-J}{RGB}{35,132,67}
\definecolor{YlGn-8-8}{RGB}{0,90,50}
\definecolor{YlGn-8-L}{RGB}{0,90,50}
\definecolor{YlGn-9-1}{RGB}{255,255,229}
\definecolor{YlGn-9-A}{RGB}{255,255,229}
\definecolor{YlGn-9-2}{RGB}{247,252,185}
\definecolor{YlGn-9-C}{RGB}{247,252,185}
\definecolor{YlGn-9-3}{RGB}{217,240,163}
\definecolor{YlGn-9-D}{RGB}{217,240,163}
\definecolor{YlGn-9-4}{RGB}{173,221,142}
\definecolor{YlGn-9-F}{RGB}{173,221,142}
\definecolor{YlGn-9-5}{RGB}{120,198,121}
\definecolor{YlGn-9-G}{RGB}{120,198,121}
\definecolor{YlGn-9-6}{RGB}{65,171,93}
\definecolor{YlGn-9-H}{RGB}{65,171,93}
\definecolor{YlGn-9-7}{RGB}{35,132,67}
\definecolor{YlGn-9-J}{RGB}{35,132,67}
\definecolor{YlGn-9-8}{RGB}{0,104,55}
\definecolor{YlGn-9-K}{RGB}{0,104,55}
\definecolor{YlGn-9-9}{RGB}{0,69,41}
\definecolor{YlGn-9-M}{RGB}{0,69,41}
\definecolor{YlGnBu-3-1}{RGB}{237,248,177}
\definecolor{YlGnBu-3-C}{RGB}{237,248,177}
\definecolor{YlGnBu-3-2}{RGB}{127,205,187}
\definecolor{YlGnBu-3-F}{RGB}{127,205,187}
\definecolor{YlGnBu-3-3}{RGB}{44,127,184}
\definecolor{YlGnBu-3-I}{RGB}{44,127,184}
\definecolor{YlGnBu-4-1}{RGB}{255,255,204}
\definecolor{YlGnBu-4-B}{RGB}{255,255,204}
\definecolor{YlGnBu-4-2}{RGB}{161,218,180}
\definecolor{YlGnBu-4-E}{RGB}{161,218,180}
\definecolor{YlGnBu-4-3}{RGB}{65,182,196}
\definecolor{YlGnBu-4-G}{RGB}{65,182,196}
\definecolor{YlGnBu-4-4}{RGB}{34,94,168}
\definecolor{YlGnBu-4-J}{RGB}{34,94,168}
\definecolor{YlGnBu-5-1}{RGB}{255,255,204}
\definecolor{YlGnBu-5-B}{RGB}{255,255,204}
\definecolor{YlGnBu-5-2}{RGB}{161,218,180}
\definecolor{YlGnBu-5-E}{RGB}{161,218,180}
\definecolor{YlGnBu-5-3}{RGB}{65,182,196}
\definecolor{YlGnBu-5-G}{RGB}{65,182,196}
\definecolor{YlGnBu-5-4}{RGB}{44,127,184}
\definecolor{YlGnBu-5-I}{RGB}{44,127,184}
\definecolor{YlGnBu-5-5}{RGB}{37,52,148}
\definecolor{YlGnBu-5-K}{RGB}{37,52,148}
\definecolor{YlGnBu-6-1}{RGB}{255,255,204}
\definecolor{YlGnBu-6-B}{RGB}{255,255,204}
\definecolor{YlGnBu-6-2}{RGB}{199,233,180}
\definecolor{YlGnBu-6-D}{RGB}{199,233,180}
\definecolor{YlGnBu-6-3}{RGB}{127,205,187}
\definecolor{YlGnBu-6-F}{RGB}{127,205,187}
\definecolor{YlGnBu-6-4}{RGB}{65,182,196}
\definecolor{YlGnBu-6-G}{RGB}{65,182,196}
\definecolor{YlGnBu-6-5}{RGB}{44,127,184}
\definecolor{YlGnBu-6-I}{RGB}{44,127,184}
\definecolor{YlGnBu-6-6}{RGB}{37,52,148}
\definecolor{YlGnBu-6-K}{RGB}{37,52,148}
\definecolor{YlGnBu-7-1}{RGB}{255,255,204}
\definecolor{YlGnBu-7-B}{RGB}{255,255,204}
\definecolor{YlGnBu-7-2}{RGB}{199,233,180}
\definecolor{YlGnBu-7-D}{RGB}{199,233,180}
\definecolor{YlGnBu-7-3}{RGB}{127,205,187}
\definecolor{YlGnBu-7-F}{RGB}{127,205,187}
\definecolor{YlGnBu-7-4}{RGB}{65,182,196}
\definecolor{YlGnBu-7-G}{RGB}{65,182,196}
\definecolor{YlGnBu-7-5}{RGB}{29,145,192}
\definecolor{YlGnBu-7-H}{RGB}{29,145,192}
\definecolor{YlGnBu-7-6}{RGB}{34,94,168}
\definecolor{YlGnBu-7-J}{RGB}{34,94,168}
\definecolor{YlGnBu-7-7}{RGB}{12,44,132}
\definecolor{YlGnBu-7-L}{RGB}{12,44,132}
\definecolor{YlGnBu-8-1}{RGB}{255,255,217}
\definecolor{YlGnBu-8-A}{RGB}{255,255,217}
\definecolor{YlGnBu-8-2}{RGB}{237,248,177}
\definecolor{YlGnBu-8-C}{RGB}{237,248,177}
\definecolor{YlGnBu-8-3}{RGB}{199,233,180}
\definecolor{YlGnBu-8-D}{RGB}{199,233,180}
\definecolor{YlGnBu-8-4}{RGB}{127,205,187}
\definecolor{YlGnBu-8-F}{RGB}{127,205,187}
\definecolor{YlGnBu-8-5}{RGB}{65,182,196}
\definecolor{YlGnBu-8-G}{RGB}{65,182,196}
\definecolor{YlGnBu-8-6}{RGB}{29,145,192}
\definecolor{YlGnBu-8-H}{RGB}{29,145,192}
\definecolor{YlGnBu-8-7}{RGB}{34,94,168}
\definecolor{YlGnBu-8-J}{RGB}{34,94,168}
\definecolor{YlGnBu-8-8}{RGB}{12,44,132}
\definecolor{YlGnBu-8-L}{RGB}{12,44,132}
\definecolor{YlGnBu-9-1}{RGB}{255,255,217}
\definecolor{YlGnBu-9-A}{RGB}{255,255,217}
\definecolor{YlGnBu-9-2}{RGB}{237,248,177}
\definecolor{YlGnBu-9-C}{RGB}{237,248,177}
\definecolor{YlGnBu-9-3}{RGB}{199,233,180}
\definecolor{YlGnBu-9-D}{RGB}{199,233,180}
\definecolor{YlGnBu-9-4}{RGB}{127,205,187}
\definecolor{YlGnBu-9-F}{RGB}{127,205,187}
\definecolor{YlGnBu-9-5}{RGB}{65,182,196}
\definecolor{YlGnBu-9-G}{RGB}{65,182,196}
\definecolor{YlGnBu-9-6}{RGB}{29,145,192}
\definecolor{YlGnBu-9-H}{RGB}{29,145,192}
\definecolor{YlGnBu-9-7}{RGB}{34,94,168}
\definecolor{YlGnBu-9-J}{RGB}{34,94,168}
\definecolor{YlGnBu-9-8}{RGB}{37,52,148}
\definecolor{YlGnBu-9-K}{RGB}{37,52,148}
\definecolor{YlGnBu-9-9}{RGB}{8,29,88}
\definecolor{YlGnBu-9-M}{RGB}{8,29,88}
\definecolor{GnBu-3-1}{RGB}{224,243,219}
\definecolor{GnBu-3-C}{RGB}{224,243,219}
\definecolor{GnBu-3-2}{RGB}{168,221,181}
\definecolor{GnBu-3-F}{RGB}{168,221,181}
\definecolor{GnBu-3-3}{RGB}{67,162,202}
\definecolor{GnBu-3-I}{RGB}{67,162,202}
\definecolor{GnBu-4-1}{RGB}{240,249,232}
\definecolor{GnBu-4-B}{RGB}{240,249,232}
\definecolor{GnBu-4-2}{RGB}{186,228,188}
\definecolor{GnBu-4-E}{RGB}{186,228,188}
\definecolor{GnBu-4-3}{RGB}{123,204,196}
\definecolor{GnBu-4-G}{RGB}{123,204,196}
\definecolor{GnBu-4-4}{RGB}{43,140,190}
\definecolor{GnBu-4-J}{RGB}{43,140,190}
\definecolor{GnBu-5-1}{RGB}{240,249,232}
\definecolor{GnBu-5-B}{RGB}{240,249,232}
\definecolor{GnBu-5-2}{RGB}{186,228,188}
\definecolor{GnBu-5-E}{RGB}{186,228,188}
\definecolor{GnBu-5-3}{RGB}{123,204,196}
\definecolor{GnBu-5-G}{RGB}{123,204,196}
\definecolor{GnBu-5-4}{RGB}{67,162,202}
\definecolor{GnBu-5-I}{RGB}{67,162,202}
\definecolor{GnBu-5-5}{RGB}{8,104,172}
\definecolor{GnBu-5-K}{RGB}{8,104,172}
\definecolor{GnBu-6-1}{RGB}{240,249,232}
\definecolor{GnBu-6-B}{RGB}{240,249,232}
\definecolor{GnBu-6-2}{RGB}{204,235,197}
\definecolor{GnBu-6-D}{RGB}{204,235,197}
\definecolor{GnBu-6-3}{RGB}{168,221,181}
\definecolor{GnBu-6-F}{RGB}{168,221,181}
\definecolor{GnBu-6-4}{RGB}{123,204,196}
\definecolor{GnBu-6-G}{RGB}{123,204,196}
\definecolor{GnBu-6-5}{RGB}{67,162,202}
\definecolor{GnBu-6-I}{RGB}{67,162,202}
\definecolor{GnBu-6-6}{RGB}{8,104,172}
\definecolor{GnBu-6-K}{RGB}{8,104,172}
\definecolor{GnBu-7-1}{RGB}{240,249,232}
\definecolor{GnBu-7-B}{RGB}{240,249,232}
\definecolor{GnBu-7-2}{RGB}{204,235,197}
\definecolor{GnBu-7-D}{RGB}{204,235,197}
\definecolor{GnBu-7-3}{RGB}{168,221,181}
\definecolor{GnBu-7-F}{RGB}{168,221,181}
\definecolor{GnBu-7-4}{RGB}{123,204,196}
\definecolor{GnBu-7-G}{RGB}{123,204,196}
\definecolor{GnBu-7-5}{RGB}{78,179,211}
\definecolor{GnBu-7-H}{RGB}{78,179,211}
\definecolor{GnBu-7-6}{RGB}{43,140,190}
\definecolor{GnBu-7-J}{RGB}{43,140,190}
\definecolor{GnBu-7-7}{RGB}{8,88,158}
\definecolor{GnBu-7-L}{RGB}{8,88,158}
\definecolor{GnBu-8-1}{RGB}{247,252,240}
\definecolor{GnBu-8-A}{RGB}{247,252,240}
\definecolor{GnBu-8-2}{RGB}{224,243,219}
\definecolor{GnBu-8-C}{RGB}{224,243,219}
\definecolor{GnBu-8-3}{RGB}{204,235,197}
\definecolor{GnBu-8-D}{RGB}{204,235,197}
\definecolor{GnBu-8-4}{RGB}{168,221,181}
\definecolor{GnBu-8-F}{RGB}{168,221,181}
\definecolor{GnBu-8-5}{RGB}{123,204,196}
\definecolor{GnBu-8-G}{RGB}{123,204,196}
\definecolor{GnBu-8-6}{RGB}{78,179,211}
\definecolor{GnBu-8-H}{RGB}{78,179,211}
\definecolor{GnBu-8-7}{RGB}{43,140,190}
\definecolor{GnBu-8-J}{RGB}{43,140,190}
\definecolor{GnBu-8-8}{RGB}{8,88,158}
\definecolor{GnBu-8-L}{RGB}{8,88,158}
\definecolor{GnBu-9-1}{RGB}{247,252,240}
\definecolor{GnBu-9-A}{RGB}{247,252,240}
\definecolor{GnBu-9-2}{RGB}{224,243,219}
\definecolor{GnBu-9-C}{RGB}{224,243,219}
\definecolor{GnBu-9-3}{RGB}{204,235,197}
\definecolor{GnBu-9-D}{RGB}{204,235,197}
\definecolor{GnBu-9-4}{RGB}{168,221,181}
\definecolor{GnBu-9-F}{RGB}{168,221,181}
\definecolor{GnBu-9-5}{RGB}{123,204,196}
\definecolor{GnBu-9-G}{RGB}{123,204,196}
\definecolor{GnBu-9-6}{RGB}{78,179,211}
\definecolor{GnBu-9-H}{RGB}{78,179,211}
\definecolor{GnBu-9-7}{RGB}{43,140,190}
\definecolor{GnBu-9-J}{RGB}{43,140,190}
\definecolor{GnBu-9-8}{RGB}{8,104,172}
\definecolor{GnBu-9-K}{RGB}{8,104,172}
\definecolor{GnBu-9-9}{RGB}{8,64,129}
\definecolor{GnBu-9-M}{RGB}{8,64,129}
\definecolor{BuGn-3-1}{RGB}{229,245,249}
\definecolor{BuGn-3-C}{RGB}{229,245,249}
\definecolor{BuGn-3-2}{RGB}{153,216,201}
\definecolor{BuGn-3-F}{RGB}{153,216,201}
\definecolor{BuGn-3-3}{RGB}{44,162,95}
\definecolor{BuGn-3-I}{RGB}{44,162,95}
\definecolor{BuGn-4-1}{RGB}{237,248,251}
\definecolor{BuGn-4-B}{RGB}{237,248,251}
\definecolor{BuGn-4-2}{RGB}{178,226,226}
\definecolor{BuGn-4-E}{RGB}{178,226,226}
\definecolor{BuGn-4-3}{RGB}{102,194,164}
\definecolor{BuGn-4-G}{RGB}{102,194,164}
\definecolor{BuGn-4-4}{RGB}{35,139,69}
\definecolor{BuGn-4-J}{RGB}{35,139,69}
\definecolor{BuGn-5-1}{RGB}{237,248,251}
\definecolor{BuGn-5-B}{RGB}{237,248,251}
\definecolor{BuGn-5-2}{RGB}{178,226,226}
\definecolor{BuGn-5-E}{RGB}{178,226,226}
\definecolor{BuGn-5-3}{RGB}{102,194,164}
\definecolor{BuGn-5-G}{RGB}{102,194,164}
\definecolor{BuGn-5-4}{RGB}{44,162,95}
\definecolor{BuGn-5-I}{RGB}{44,162,95}
\definecolor{BuGn-5-5}{RGB}{0,109,44}
\definecolor{BuGn-5-K}{RGB}{0,109,44}
\definecolor{BuGn-6-1}{RGB}{237,248,251}
\definecolor{BuGn-6-B}{RGB}{237,248,251}
\definecolor{BuGn-6-2}{RGB}{204,236,230}
\definecolor{BuGn-6-D}{RGB}{204,236,230}
\definecolor{BuGn-6-3}{RGB}{153,216,201}
\definecolor{BuGn-6-F}{RGB}{153,216,201}
\definecolor{BuGn-6-4}{RGB}{102,194,164}
\definecolor{BuGn-6-G}{RGB}{102,194,164}
\definecolor{BuGn-6-5}{RGB}{44,162,95}
\definecolor{BuGn-6-I}{RGB}{44,162,95}
\definecolor{BuGn-6-6}{RGB}{0,109,44}
\definecolor{BuGn-6-K}{RGB}{0,109,44}
\definecolor{BuGn-7-1}{RGB}{237,248,251}
\definecolor{BuGn-7-B}{RGB}{237,248,251}
\definecolor{BuGn-7-2}{RGB}{204,236,230}
\definecolor{BuGn-7-D}{RGB}{204,236,230}
\definecolor{BuGn-7-3}{RGB}{153,216,201}
\definecolor{BuGn-7-F}{RGB}{153,216,201}
\definecolor{BuGn-7-4}{RGB}{102,194,164}
\definecolor{BuGn-7-G}{RGB}{102,194,164}
\definecolor{BuGn-7-5}{RGB}{65,174,118}
\definecolor{BuGn-7-H}{RGB}{65,174,118}
\definecolor{BuGn-7-6}{RGB}{35,139,69}
\definecolor{BuGn-7-J}{RGB}{35,139,69}
\definecolor{BuGn-7-7}{RGB}{0,88,36}
\definecolor{BuGn-7-L}{RGB}{0,88,36}
\definecolor{BuGn-8-1}{RGB}{247,252,253}
\definecolor{BuGn-8-A}{RGB}{247,252,253}
\definecolor{BuGn-8-2}{RGB}{229,245,249}
\definecolor{BuGn-8-C}{RGB}{229,245,249}
\definecolor{BuGn-8-3}{RGB}{204,236,230}
\definecolor{BuGn-8-D}{RGB}{204,236,230}
\definecolor{BuGn-8-4}{RGB}{153,216,201}
\definecolor{BuGn-8-F}{RGB}{153,216,201}
\definecolor{BuGn-8-5}{RGB}{102,194,164}
\definecolor{BuGn-8-G}{RGB}{102,194,164}
\definecolor{BuGn-8-6}{RGB}{65,174,118}
\definecolor{BuGn-8-H}{RGB}{65,174,118}
\definecolor{BuGn-8-7}{RGB}{35,139,69}
\definecolor{BuGn-8-J}{RGB}{35,139,69}
\definecolor{BuGn-8-8}{RGB}{0,88,36}
\definecolor{BuGn-8-L}{RGB}{0,88,36}
\definecolor{BuGn-9-1}{RGB}{247,252,253}
\definecolor{BuGn-9-A}{RGB}{247,252,253}
\definecolor{BuGn-9-2}{RGB}{229,245,249}
\definecolor{BuGn-9-C}{RGB}{229,245,249}
\definecolor{BuGn-9-3}{RGB}{204,236,230}
\definecolor{BuGn-9-D}{RGB}{204,236,230}
\definecolor{BuGn-9-4}{RGB}{153,216,201}
\definecolor{BuGn-9-F}{RGB}{153,216,201}
\definecolor{BuGn-9-5}{RGB}{102,194,164}
\definecolor{BuGn-9-G}{RGB}{102,194,164}
\definecolor{BuGn-9-6}{RGB}{65,174,118}
\definecolor{BuGn-9-H}{RGB}{65,174,118}
\definecolor{BuGn-9-7}{RGB}{35,139,69}
\definecolor{BuGn-9-J}{RGB}{35,139,69}
\definecolor{BuGn-9-8}{RGB}{0,109,44}
\definecolor{BuGn-9-K}{RGB}{0,109,44}
\definecolor{BuGn-9-9}{RGB}{0,68,27}
\definecolor{BuGn-9-M}{RGB}{0,68,27}
\definecolor{PuBuGn-3-1}{RGB}{236,226,240}
\definecolor{PuBuGn-3-C}{RGB}{236,226,240}
\definecolor{PuBuGn-3-2}{RGB}{166,189,219}
\definecolor{PuBuGn-3-F}{RGB}{166,189,219}
\definecolor{PuBuGn-3-3}{RGB}{28,144,153}
\definecolor{PuBuGn-3-I}{RGB}{28,144,153}
\definecolor{PuBuGn-4-1}{RGB}{246,239,247}
\definecolor{PuBuGn-4-B}{RGB}{246,239,247}
\definecolor{PuBuGn-4-2}{RGB}{189,201,225}
\definecolor{PuBuGn-4-E}{RGB}{189,201,225}
\definecolor{PuBuGn-4-3}{RGB}{103,169,207}
\definecolor{PuBuGn-4-G}{RGB}{103,169,207}
\definecolor{PuBuGn-4-4}{RGB}{2,129,138}
\definecolor{PuBuGn-4-J}{RGB}{2,129,138}
\definecolor{PuBuGn-5-1}{RGB}{246,239,247}
\definecolor{PuBuGn-5-B}{RGB}{246,239,247}
\definecolor{PuBuGn-5-2}{RGB}{189,201,225}
\definecolor{PuBuGn-5-E}{RGB}{189,201,225}
\definecolor{PuBuGn-5-3}{RGB}{103,169,207}
\definecolor{PuBuGn-5-G}{RGB}{103,169,207}
\definecolor{PuBuGn-5-4}{RGB}{28,144,153}
\definecolor{PuBuGn-5-I}{RGB}{28,144,153}
\definecolor{PuBuGn-5-5}{RGB}{1,108,89}
\definecolor{PuBuGn-5-K}{RGB}{1,108,89}
\definecolor{PuBuGn-6-1}{RGB}{246,239,247}
\definecolor{PuBuGn-6-B}{RGB}{246,239,247}
\definecolor{PuBuGn-6-2}{RGB}{208,209,230}
\definecolor{PuBuGn-6-D}{RGB}{208,209,230}
\definecolor{PuBuGn-6-3}{RGB}{166,189,219}
\definecolor{PuBuGn-6-F}{RGB}{166,189,219}
\definecolor{PuBuGn-6-4}{RGB}{103,169,207}
\definecolor{PuBuGn-6-G}{RGB}{103,169,207}
\definecolor{PuBuGn-6-5}{RGB}{28,144,153}
\definecolor{PuBuGn-6-I}{RGB}{28,144,153}
\definecolor{PuBuGn-6-6}{RGB}{1,108,89}
\definecolor{PuBuGn-6-K}{RGB}{1,108,89}
\definecolor{PuBuGn-7-1}{RGB}{246,239,247}
\definecolor{PuBuGn-7-B}{RGB}{246,239,247}
\definecolor{PuBuGn-7-2}{RGB}{208,209,230}
\definecolor{PuBuGn-7-D}{RGB}{208,209,230}
\definecolor{PuBuGn-7-3}{RGB}{166,189,219}
\definecolor{PuBuGn-7-F}{RGB}{166,189,219}
\definecolor{PuBuGn-7-4}{RGB}{103,169,207}
\definecolor{PuBuGn-7-G}{RGB}{103,169,207}
\definecolor{PuBuGn-7-5}{RGB}{54,144,192}
\definecolor{PuBuGn-7-H}{RGB}{54,144,192}
\definecolor{PuBuGn-7-6}{RGB}{2,129,138}
\definecolor{PuBuGn-7-J}{RGB}{2,129,138}
\definecolor{PuBuGn-7-7}{RGB}{1,100,80}
\definecolor{PuBuGn-7-L}{RGB}{1,100,80}
\definecolor{PuBuGn-8-1}{RGB}{255,247,251}
\definecolor{PuBuGn-8-A}{RGB}{255,247,251}
\definecolor{PuBuGn-8-2}{RGB}{236,226,240}
\definecolor{PuBuGn-8-C}{RGB}{236,226,240}
\definecolor{PuBuGn-8-3}{RGB}{208,209,230}
\definecolor{PuBuGn-8-D}{RGB}{208,209,230}
\definecolor{PuBuGn-8-4}{RGB}{166,189,219}
\definecolor{PuBuGn-8-F}{RGB}{166,189,219}
\definecolor{PuBuGn-8-5}{RGB}{103,169,207}
\definecolor{PuBuGn-8-G}{RGB}{103,169,207}
\definecolor{PuBuGn-8-6}{RGB}{54,144,192}
\definecolor{PuBuGn-8-H}{RGB}{54,144,192}
\definecolor{PuBuGn-8-7}{RGB}{2,129,138}
\definecolor{PuBuGn-8-J}{RGB}{2,129,138}
\definecolor{PuBuGn-8-8}{RGB}{1,100,80}
\definecolor{PuBuGn-8-L}{RGB}{1,100,80}
\definecolor{PuBuGn-9-1}{RGB}{255,247,251}
\definecolor{PuBuGn-9-A}{RGB}{255,247,251}
\definecolor{PuBuGn-9-2}{RGB}{236,226,240}
\definecolor{PuBuGn-9-C}{RGB}{236,226,240}
\definecolor{PuBuGn-9-3}{RGB}{208,209,230}
\definecolor{PuBuGn-9-D}{RGB}{208,209,230}
\definecolor{PuBuGn-9-4}{RGB}{166,189,219}
\definecolor{PuBuGn-9-F}{RGB}{166,189,219}
\definecolor{PuBuGn-9-5}{RGB}{103,169,207}
\definecolor{PuBuGn-9-G}{RGB}{103,169,207}
\definecolor{PuBuGn-9-6}{RGB}{54,144,192}
\definecolor{PuBuGn-9-H}{RGB}{54,144,192}
\definecolor{PuBuGn-9-7}{RGB}{2,129,138}
\definecolor{PuBuGn-9-J}{RGB}{2,129,138}
\definecolor{PuBuGn-9-8}{RGB}{1,108,89}
\definecolor{PuBuGn-9-K}{RGB}{1,108,89}
\definecolor{PuBuGn-9-9}{RGB}{1,70,54}
\definecolor{PuBuGn-9-M}{RGB}{1,70,54}
\definecolor{PuBu-3-1}{RGB}{236,231,242}
\definecolor{PuBu-3-C}{RGB}{236,231,242}
\definecolor{PuBu-3-2}{RGB}{166,189,219}
\definecolor{PuBu-3-F}{RGB}{166,189,219}
\definecolor{PuBu-3-3}{RGB}{43,140,190}
\definecolor{PuBu-3-I}{RGB}{43,140,190}
\definecolor{PuBu-4-1}{RGB}{241,238,246}
\definecolor{PuBu-4-B}{RGB}{241,238,246}
\definecolor{PuBu-4-2}{RGB}{189,201,225}
\definecolor{PuBu-4-E}{RGB}{189,201,225}
\definecolor{PuBu-4-3}{RGB}{116,169,207}
\definecolor{PuBu-4-G}{RGB}{116,169,207}
\definecolor{PuBu-4-4}{RGB}{5,112,176}
\definecolor{PuBu-4-J}{RGB}{5,112,176}
\definecolor{PuBu-5-1}{RGB}{241,238,246}
\definecolor{PuBu-5-B}{RGB}{241,238,246}
\definecolor{PuBu-5-2}{RGB}{189,201,225}
\definecolor{PuBu-5-E}{RGB}{189,201,225}
\definecolor{PuBu-5-3}{RGB}{116,169,207}
\definecolor{PuBu-5-G}{RGB}{116,169,207}
\definecolor{PuBu-5-4}{RGB}{43,140,190}
\definecolor{PuBu-5-I}{RGB}{43,140,190}
\definecolor{PuBu-5-5}{RGB}{4,90,141}
\definecolor{PuBu-5-K}{RGB}{4,90,141}
\definecolor{PuBu-6-1}{RGB}{241,238,246}
\definecolor{PuBu-6-B}{RGB}{241,238,246}
\definecolor{PuBu-6-2}{RGB}{208,209,230}
\definecolor{PuBu-6-D}{RGB}{208,209,230}
\definecolor{PuBu-6-3}{RGB}{166,189,219}
\definecolor{PuBu-6-F}{RGB}{166,189,219}
\definecolor{PuBu-6-4}{RGB}{116,169,207}
\definecolor{PuBu-6-G}{RGB}{116,169,207}
\definecolor{PuBu-6-5}{RGB}{43,140,190}
\definecolor{PuBu-6-I}{RGB}{43,140,190}
\definecolor{PuBu-6-6}{RGB}{4,90,141}
\definecolor{PuBu-6-K}{RGB}{4,90,141}
\definecolor{PuBu-7-1}{RGB}{241,238,246}
\definecolor{PuBu-7-B}{RGB}{241,238,246}
\definecolor{PuBu-7-2}{RGB}{208,209,230}
\definecolor{PuBu-7-D}{RGB}{208,209,230}
\definecolor{PuBu-7-3}{RGB}{166,189,219}
\definecolor{PuBu-7-F}{RGB}{166,189,219}
\definecolor{PuBu-7-4}{RGB}{116,169,207}
\definecolor{PuBu-7-G}{RGB}{116,169,207}
\definecolor{PuBu-7-5}{RGB}{54,144,192}
\definecolor{PuBu-7-H}{RGB}{54,144,192}
\definecolor{PuBu-7-6}{RGB}{5,112,176}
\definecolor{PuBu-7-J}{RGB}{5,112,176}
\definecolor{PuBu-7-7}{RGB}{3,78,123}
\definecolor{PuBu-7-L}{RGB}{3,78,123}
\definecolor{PuBu-8-1}{RGB}{255,247,251}
\definecolor{PuBu-8-A}{RGB}{255,247,251}
\definecolor{PuBu-8-2}{RGB}{236,231,242}
\definecolor{PuBu-8-C}{RGB}{236,231,242}
\definecolor{PuBu-8-3}{RGB}{208,209,230}
\definecolor{PuBu-8-D}{RGB}{208,209,230}
\definecolor{PuBu-8-4}{RGB}{166,189,219}
\definecolor{PuBu-8-F}{RGB}{166,189,219}
\definecolor{PuBu-8-5}{RGB}{116,169,207}
\definecolor{PuBu-8-G}{RGB}{116,169,207}
\definecolor{PuBu-8-6}{RGB}{54,144,192}
\definecolor{PuBu-8-H}{RGB}{54,144,192}
\definecolor{PuBu-8-7}{RGB}{5,112,176}
\definecolor{PuBu-8-J}{RGB}{5,112,176}
\definecolor{PuBu-8-8}{RGB}{3,78,123}
\definecolor{PuBu-8-L}{RGB}{3,78,123}
\definecolor{PuBu-9-1}{RGB}{255,247,251}
\definecolor{PuBu-9-A}{RGB}{255,247,251}
\definecolor{PuBu-9-2}{RGB}{236,231,242}
\definecolor{PuBu-9-C}{RGB}{236,231,242}
\definecolor{PuBu-9-3}{RGB}{208,209,230}
\definecolor{PuBu-9-D}{RGB}{208,209,230}
\definecolor{PuBu-9-4}{RGB}{166,189,219}
\definecolor{PuBu-9-F}{RGB}{166,189,219}
\definecolor{PuBu-9-5}{RGB}{116,169,207}
\definecolor{PuBu-9-G}{RGB}{116,169,207}
\definecolor{PuBu-9-6}{RGB}{54,144,192}
\definecolor{PuBu-9-H}{RGB}{54,144,192}
\definecolor{PuBu-9-7}{RGB}{5,112,176}
\definecolor{PuBu-9-J}{RGB}{5,112,176}
\definecolor{PuBu-9-8}{RGB}{4,90,141}
\definecolor{PuBu-9-K}{RGB}{4,90,141}
\definecolor{PuBu-9-9}{RGB}{2,56,88}
\definecolor{PuBu-9-M}{RGB}{2,56,88}
\definecolor{BuPu-3-1}{RGB}{224,236,244}
\definecolor{BuPu-3-C}{RGB}{224,236,244}
\definecolor{BuPu-3-2}{RGB}{158,188,218}
\definecolor{BuPu-3-F}{RGB}{158,188,218}
\definecolor{BuPu-3-3}{RGB}{136,86,167}
\definecolor{BuPu-3-I}{RGB}{136,86,167}
\definecolor{BuPu-4-1}{RGB}{237,248,251}
\definecolor{BuPu-4-B}{RGB}{237,248,251}
\definecolor{BuPu-4-2}{RGB}{179,205,227}
\definecolor{BuPu-4-E}{RGB}{179,205,227}
\definecolor{BuPu-4-3}{RGB}{140,150,198}
\definecolor{BuPu-4-G}{RGB}{140,150,198}
\definecolor{BuPu-4-4}{RGB}{136,65,157}
\definecolor{BuPu-4-J}{RGB}{136,65,157}
\definecolor{BuPu-5-1}{RGB}{237,248,251}
\definecolor{BuPu-5-B}{RGB}{237,248,251}
\definecolor{BuPu-5-2}{RGB}{179,205,227}
\definecolor{BuPu-5-E}{RGB}{179,205,227}
\definecolor{BuPu-5-3}{RGB}{140,150,198}
\definecolor{BuPu-5-G}{RGB}{140,150,198}
\definecolor{BuPu-5-4}{RGB}{136,86,167}
\definecolor{BuPu-5-I}{RGB}{136,86,167}
\definecolor{BuPu-5-5}{RGB}{129,15,124}
\definecolor{BuPu-5-K}{RGB}{129,15,124}
\definecolor{BuPu-6-1}{RGB}{237,248,251}
\definecolor{BuPu-6-B}{RGB}{237,248,251}
\definecolor{BuPu-6-2}{RGB}{191,211,230}
\definecolor{BuPu-6-D}{RGB}{191,211,230}
\definecolor{BuPu-6-3}{RGB}{158,188,218}
\definecolor{BuPu-6-F}{RGB}{158,188,218}
\definecolor{BuPu-6-4}{RGB}{140,150,198}
\definecolor{BuPu-6-G}{RGB}{140,150,198}
\definecolor{BuPu-6-5}{RGB}{136,86,167}
\definecolor{BuPu-6-I}{RGB}{136,86,167}
\definecolor{BuPu-6-6}{RGB}{129,15,124}
\definecolor{BuPu-6-K}{RGB}{129,15,124}
\definecolor{BuPu-7-1}{RGB}{237,248,251}
\definecolor{BuPu-7-B}{RGB}{237,248,251}
\definecolor{BuPu-7-2}{RGB}{191,211,230}
\definecolor{BuPu-7-D}{RGB}{191,211,230}
\definecolor{BuPu-7-3}{RGB}{158,188,218}
\definecolor{BuPu-7-F}{RGB}{158,188,218}
\definecolor{BuPu-7-4}{RGB}{140,150,198}
\definecolor{BuPu-7-G}{RGB}{140,150,198}
\definecolor{BuPu-7-5}{RGB}{140,107,177}
\definecolor{BuPu-7-H}{RGB}{140,107,177}
\definecolor{BuPu-7-6}{RGB}{136,65,157}
\definecolor{BuPu-7-J}{RGB}{136,65,157}
\definecolor{BuPu-7-7}{RGB}{110,1,107}
\definecolor{BuPu-7-L}{RGB}{110,1,107}
\definecolor{BuPu-8-1}{RGB}{247,252,253}
\definecolor{BuPu-8-A}{RGB}{247,252,253}
\definecolor{BuPu-8-2}{RGB}{224,236,244}
\definecolor{BuPu-8-C}{RGB}{224,236,244}
\definecolor{BuPu-8-3}{RGB}{191,211,230}
\definecolor{BuPu-8-D}{RGB}{191,211,230}
\definecolor{BuPu-8-4}{RGB}{158,188,218}
\definecolor{BuPu-8-F}{RGB}{158,188,218}
\definecolor{BuPu-8-5}{RGB}{140,150,198}
\definecolor{BuPu-8-G}{RGB}{140,150,198}
\definecolor{BuPu-8-6}{RGB}{140,107,177}
\definecolor{BuPu-8-H}{RGB}{140,107,177}
\definecolor{BuPu-8-7}{RGB}{136,65,157}
\definecolor{BuPu-8-J}{RGB}{136,65,157}
\definecolor{BuPu-8-8}{RGB}{110,1,107}
\definecolor{BuPu-8-L}{RGB}{110,1,107}
\definecolor{BuPu-9-1}{RGB}{247,252,253}
\definecolor{BuPu-9-A}{RGB}{247,252,253}
\definecolor{BuPu-9-2}{RGB}{224,236,244}
\definecolor{BuPu-9-C}{RGB}{224,236,244}
\definecolor{BuPu-9-3}{RGB}{191,211,230}
\definecolor{BuPu-9-D}{RGB}{191,211,230}
\definecolor{BuPu-9-4}{RGB}{158,188,218}
\definecolor{BuPu-9-F}{RGB}{158,188,218}
\definecolor{BuPu-9-5}{RGB}{140,150,198}
\definecolor{BuPu-9-G}{RGB}{140,150,198}
\definecolor{BuPu-9-6}{RGB}{140,107,177}
\definecolor{BuPu-9-H}{RGB}{140,107,177}
\definecolor{BuPu-9-7}{RGB}{136,65,157}
\definecolor{BuPu-9-J}{RGB}{136,65,157}
\definecolor{BuPu-9-8}{RGB}{129,15,124}
\definecolor{BuPu-9-K}{RGB}{129,15,124}
\definecolor{BuPu-9-9}{RGB}{77,0,75}
\definecolor{BuPu-9-M}{RGB}{77,0,75}
\definecolor{RdPu-3-1}{RGB}{253,224,221}
\definecolor{RdPu-3-C}{RGB}{253,224,221}
\definecolor{RdPu-3-2}{RGB}{250,159,181}
\definecolor{RdPu-3-F}{RGB}{250,159,181}
\definecolor{RdPu-3-3}{RGB}{197,27,138}
\definecolor{RdPu-3-I}{RGB}{197,27,138}
\definecolor{RdPu-4-1}{RGB}{254,235,226}
\definecolor{RdPu-4-B}{RGB}{254,235,226}
\definecolor{RdPu-4-2}{RGB}{251,180,185}
\definecolor{RdPu-4-E}{RGB}{251,180,185}
\definecolor{RdPu-4-3}{RGB}{247,104,161}
\definecolor{RdPu-4-G}{RGB}{247,104,161}
\definecolor{RdPu-4-4}{RGB}{174,1,126}
\definecolor{RdPu-4-J}{RGB}{174,1,126}
\definecolor{RdPu-5-1}{RGB}{254,235,226}
\definecolor{RdPu-5-B}{RGB}{254,235,226}
\definecolor{RdPu-5-2}{RGB}{251,180,185}
\definecolor{RdPu-5-E}{RGB}{251,180,185}
\definecolor{RdPu-5-3}{RGB}{247,104,161}
\definecolor{RdPu-5-G}{RGB}{247,104,161}
\definecolor{RdPu-5-4}{RGB}{197,27,138}
\definecolor{RdPu-5-I}{RGB}{197,27,138}
\definecolor{RdPu-5-5}{RGB}{122,1,119}
\definecolor{RdPu-5-K}{RGB}{122,1,119}
\definecolor{RdPu-6-1}{RGB}{254,235,226}
\definecolor{RdPu-6-B}{RGB}{254,235,226}
\definecolor{RdPu-6-2}{RGB}{252,197,192}
\definecolor{RdPu-6-D}{RGB}{252,197,192}
\definecolor{RdPu-6-3}{RGB}{250,159,181}
\definecolor{RdPu-6-F}{RGB}{250,159,181}
\definecolor{RdPu-6-4}{RGB}{247,104,161}
\definecolor{RdPu-6-G}{RGB}{247,104,161}
\definecolor{RdPu-6-5}{RGB}{197,27,138}
\definecolor{RdPu-6-I}{RGB}{197,27,138}
\definecolor{RdPu-6-6}{RGB}{122,1,119}
\definecolor{RdPu-6-K}{RGB}{122,1,119}
\definecolor{RdPu-7-1}{RGB}{254,235,226}
\definecolor{RdPu-7-B}{RGB}{254,235,226}
\definecolor{RdPu-7-2}{RGB}{252,197,192}
\definecolor{RdPu-7-D}{RGB}{252,197,192}
\definecolor{RdPu-7-3}{RGB}{250,159,181}
\definecolor{RdPu-7-F}{RGB}{250,159,181}
\definecolor{RdPu-7-4}{RGB}{247,104,161}
\definecolor{RdPu-7-G}{RGB}{247,104,161}
\definecolor{RdPu-7-5}{RGB}{221,52,151}
\definecolor{RdPu-7-H}{RGB}{221,52,151}
\definecolor{RdPu-7-6}{RGB}{174,1,126}
\definecolor{RdPu-7-J}{RGB}{174,1,126}
\definecolor{RdPu-7-7}{RGB}{122,1,119}
\definecolor{RdPu-7-L}{RGB}{122,1,119}
\definecolor{RdPu-8-1}{RGB}{255,247,243}
\definecolor{RdPu-8-A}{RGB}{255,247,243}
\definecolor{RdPu-8-2}{RGB}{253,224,221}
\definecolor{RdPu-8-C}{RGB}{253,224,221}
\definecolor{RdPu-8-3}{RGB}{252,197,192}
\definecolor{RdPu-8-D}{RGB}{252,197,192}
\definecolor{RdPu-8-4}{RGB}{250,159,181}
\definecolor{RdPu-8-F}{RGB}{250,159,181}
\definecolor{RdPu-8-5}{RGB}{247,104,161}
\definecolor{RdPu-8-G}{RGB}{247,104,161}
\definecolor{RdPu-8-6}{RGB}{221,52,151}
\definecolor{RdPu-8-H}{RGB}{221,52,151}
\definecolor{RdPu-8-7}{RGB}{174,1,126}
\definecolor{RdPu-8-J}{RGB}{174,1,126}
\definecolor{RdPu-8-8}{RGB}{122,1,119}
\definecolor{RdPu-8-L}{RGB}{122,1,119}
\definecolor{RdPu-9-1}{RGB}{255,247,243}
\definecolor{RdPu-9-A}{RGB}{255,247,243}
\definecolor{RdPu-9-2}{RGB}{253,224,221}
\definecolor{RdPu-9-C}{RGB}{253,224,221}
\definecolor{RdPu-9-3}{RGB}{252,197,192}
\definecolor{RdPu-9-D}{RGB}{252,197,192}
\definecolor{RdPu-9-4}{RGB}{250,159,181}
\definecolor{RdPu-9-F}{RGB}{250,159,181}
\definecolor{RdPu-9-5}{RGB}{247,104,161}
\definecolor{RdPu-9-G}{RGB}{247,104,161}
\definecolor{RdPu-9-6}{RGB}{221,52,151}
\definecolor{RdPu-9-H}{RGB}{221,52,151}
\definecolor{RdPu-9-7}{RGB}{174,1,126}
\definecolor{RdPu-9-J}{RGB}{174,1,126}
\definecolor{RdPu-9-8}{RGB}{122,1,119}
\definecolor{RdPu-9-K}{RGB}{122,1,119}
\definecolor{RdPu-9-9}{RGB}{73,0,106}
\definecolor{RdPu-9-M}{RGB}{73,0,106}
\definecolor{PuRd-3-1}{RGB}{231,225,239}
\definecolor{PuRd-3-C}{RGB}{231,225,239}
\definecolor{PuRd-3-2}{RGB}{201,148,199}
\definecolor{PuRd-3-F}{RGB}{201,148,199}
\definecolor{PuRd-3-3}{RGB}{221,28,119}
\definecolor{PuRd-3-I}{RGB}{221,28,119}
\definecolor{PuRd-4-1}{RGB}{241,238,246}
\definecolor{PuRd-4-B}{RGB}{241,238,246}
\definecolor{PuRd-4-2}{RGB}{215,181,216}
\definecolor{PuRd-4-E}{RGB}{215,181,216}
\definecolor{PuRd-4-3}{RGB}{223,101,176}
\definecolor{PuRd-4-G}{RGB}{223,101,176}
\definecolor{PuRd-4-4}{RGB}{206,18,86}
\definecolor{PuRd-4-J}{RGB}{206,18,86}
\definecolor{PuRd-5-1}{RGB}{241,238,246}
\definecolor{PuRd-5-B}{RGB}{241,238,246}
\definecolor{PuRd-5-2}{RGB}{215,181,216}
\definecolor{PuRd-5-E}{RGB}{215,181,216}
\definecolor{PuRd-5-3}{RGB}{223,101,176}
\definecolor{PuRd-5-G}{RGB}{223,101,176}
\definecolor{PuRd-5-4}{RGB}{221,28,119}
\definecolor{PuRd-5-I}{RGB}{221,28,119}
\definecolor{PuRd-5-5}{RGB}{152,0,67}
\definecolor{PuRd-5-K}{RGB}{152,0,67}
\definecolor{PuRd-6-1}{RGB}{241,238,246}
\definecolor{PuRd-6-B}{RGB}{241,238,246}
\definecolor{PuRd-6-2}{RGB}{212,185,218}
\definecolor{PuRd-6-D}{RGB}{212,185,218}
\definecolor{PuRd-6-3}{RGB}{201,148,199}
\definecolor{PuRd-6-F}{RGB}{201,148,199}
\definecolor{PuRd-6-4}{RGB}{223,101,176}
\definecolor{PuRd-6-G}{RGB}{223,101,176}
\definecolor{PuRd-6-5}{RGB}{221,28,119}
\definecolor{PuRd-6-I}{RGB}{221,28,119}
\definecolor{PuRd-6-6}{RGB}{152,0,67}
\definecolor{PuRd-6-K}{RGB}{152,0,67}
\definecolor{PuRd-7-1}{RGB}{241,238,246}
\definecolor{PuRd-7-B}{RGB}{241,238,246}
\definecolor{PuRd-7-2}{RGB}{212,185,218}
\definecolor{PuRd-7-D}{RGB}{212,185,218}
\definecolor{PuRd-7-3}{RGB}{201,148,199}
\definecolor{PuRd-7-F}{RGB}{201,148,199}
\definecolor{PuRd-7-4}{RGB}{223,101,176}
\definecolor{PuRd-7-G}{RGB}{223,101,176}
\definecolor{PuRd-7-5}{RGB}{231,41,138}
\definecolor{PuRd-7-H}{RGB}{231,41,138}
\definecolor{PuRd-7-6}{RGB}{206,18,86}
\definecolor{PuRd-7-J}{RGB}{206,18,86}
\definecolor{PuRd-7-7}{RGB}{145,0,63}
\definecolor{PuRd-7-L}{RGB}{145,0,63}
\definecolor{PuRd-8-1}{RGB}{247,244,249}
\definecolor{PuRd-8-A}{RGB}{247,244,249}
\definecolor{PuRd-8-2}{RGB}{231,225,239}
\definecolor{PuRd-8-C}{RGB}{231,225,239}
\definecolor{PuRd-8-3}{RGB}{212,185,218}
\definecolor{PuRd-8-D}{RGB}{212,185,218}
\definecolor{PuRd-8-4}{RGB}{201,148,199}
\definecolor{PuRd-8-F}{RGB}{201,148,199}
\definecolor{PuRd-8-5}{RGB}{223,101,176}
\definecolor{PuRd-8-G}{RGB}{223,101,176}
\definecolor{PuRd-8-6}{RGB}{231,41,138}
\definecolor{PuRd-8-H}{RGB}{231,41,138}
\definecolor{PuRd-8-7}{RGB}{206,18,86}
\definecolor{PuRd-8-J}{RGB}{206,18,86}
\definecolor{PuRd-8-8}{RGB}{145,0,63}
\definecolor{PuRd-8-L}{RGB}{145,0,63}
\definecolor{PuRd-9-1}{RGB}{247,244,249}
\definecolor{PuRd-9-A}{RGB}{247,244,249}
\definecolor{PuRd-9-2}{RGB}{231,225,239}
\definecolor{PuRd-9-C}{RGB}{231,225,239}
\definecolor{PuRd-9-3}{RGB}{212,185,218}
\definecolor{PuRd-9-D}{RGB}{212,185,218}
\definecolor{PuRd-9-4}{RGB}{201,148,199}
\definecolor{PuRd-9-F}{RGB}{201,148,199}
\definecolor{PuRd-9-5}{RGB}{223,101,176}
\definecolor{PuRd-9-G}{RGB}{223,101,176}
\definecolor{PuRd-9-6}{RGB}{231,41,138}
\definecolor{PuRd-9-H}{RGB}{231,41,138}
\definecolor{PuRd-9-7}{RGB}{206,18,86}
\definecolor{PuRd-9-J}{RGB}{206,18,86}
\definecolor{PuRd-9-8}{RGB}{152,0,67}
\definecolor{PuRd-9-K}{RGB}{152,0,67}
\definecolor{PuRd-9-9}{RGB}{103,0,31}
\definecolor{PuRd-9-M}{RGB}{103,0,31}
\definecolor{OrRd-3-1}{RGB}{254,232,200}
\definecolor{OrRd-3-C}{RGB}{254,232,200}
\definecolor{OrRd-3-2}{RGB}{253,187,132}
\definecolor{OrRd-3-F}{RGB}{253,187,132}
\definecolor{OrRd-3-3}{RGB}{227,74,51}
\definecolor{OrRd-3-I}{RGB}{227,74,51}
\definecolor{OrRd-4-1}{RGB}{254,240,217}
\definecolor{OrRd-4-B}{RGB}{254,240,217}
\definecolor{OrRd-4-2}{RGB}{253,204,138}
\definecolor{OrRd-4-E}{RGB}{253,204,138}
\definecolor{OrRd-4-3}{RGB}{252,141,89}
\definecolor{OrRd-4-G}{RGB}{252,141,89}
\definecolor{OrRd-4-4}{RGB}{215,48,31}
\definecolor{OrRd-4-J}{RGB}{215,48,31}
\definecolor{OrRd-5-1}{RGB}{254,240,217}
\definecolor{OrRd-5-B}{RGB}{254,240,217}
\definecolor{OrRd-5-2}{RGB}{253,204,138}
\definecolor{OrRd-5-E}{RGB}{253,204,138}
\definecolor{OrRd-5-3}{RGB}{252,141,89}
\definecolor{OrRd-5-G}{RGB}{252,141,89}
\definecolor{OrRd-5-4}{RGB}{227,74,51}
\definecolor{OrRd-5-I}{RGB}{227,74,51}
\definecolor{OrRd-5-5}{RGB}{179,0,0}
\definecolor{OrRd-5-K}{RGB}{179,0,0}
\definecolor{OrRd-6-1}{RGB}{254,240,217}
\definecolor{OrRd-6-B}{RGB}{254,240,217}
\definecolor{OrRd-6-2}{RGB}{253,212,158}
\definecolor{OrRd-6-D}{RGB}{253,212,158}
\definecolor{OrRd-6-3}{RGB}{253,187,132}
\definecolor{OrRd-6-F}{RGB}{253,187,132}
\definecolor{OrRd-6-4}{RGB}{252,141,89}
\definecolor{OrRd-6-G}{RGB}{252,141,89}
\definecolor{OrRd-6-5}{RGB}{227,74,51}
\definecolor{OrRd-6-I}{RGB}{227,74,51}
\definecolor{OrRd-6-6}{RGB}{179,0,0}
\definecolor{OrRd-6-K}{RGB}{179,0,0}
\definecolor{OrRd-7-1}{RGB}{254,240,217}
\definecolor{OrRd-7-B}{RGB}{254,240,217}
\definecolor{OrRd-7-2}{RGB}{253,212,158}
\definecolor{OrRd-7-D}{RGB}{253,212,158}
\definecolor{OrRd-7-3}{RGB}{253,187,132}
\definecolor{OrRd-7-F}{RGB}{253,187,132}
\definecolor{OrRd-7-4}{RGB}{252,141,89}
\definecolor{OrRd-7-G}{RGB}{252,141,89}
\definecolor{OrRd-7-5}{RGB}{239,101,72}
\definecolor{OrRd-7-H}{RGB}{239,101,72}
\definecolor{OrRd-7-6}{RGB}{215,48,31}
\definecolor{OrRd-7-J}{RGB}{215,48,31}
\definecolor{OrRd-7-7}{RGB}{153,0,0}
\definecolor{OrRd-7-L}{RGB}{153,0,0}
\definecolor{OrRd-8-1}{RGB}{255,247,236}
\definecolor{OrRd-8-A}{RGB}{255,247,236}
\definecolor{OrRd-8-2}{RGB}{254,232,200}
\definecolor{OrRd-8-C}{RGB}{254,232,200}
\definecolor{OrRd-8-3}{RGB}{253,212,158}
\definecolor{OrRd-8-D}{RGB}{253,212,158}
\definecolor{OrRd-8-4}{RGB}{253,187,132}
\definecolor{OrRd-8-F}{RGB}{253,187,132}
\definecolor{OrRd-8-5}{RGB}{252,141,89}
\definecolor{OrRd-8-G}{RGB}{252,141,89}
\definecolor{OrRd-8-6}{RGB}{239,101,72}
\definecolor{OrRd-8-H}{RGB}{239,101,72}
\definecolor{OrRd-8-7}{RGB}{215,48,31}
\definecolor{OrRd-8-J}{RGB}{215,48,31}
\definecolor{OrRd-8-8}{RGB}{153,0,0}
\definecolor{OrRd-8-L}{RGB}{153,0,0}
\definecolor{OrRd-9-1}{RGB}{255,247,236}
\definecolor{OrRd-9-A}{RGB}{255,247,236}
\definecolor{OrRd-9-2}{RGB}{254,232,200}
\definecolor{OrRd-9-C}{RGB}{254,232,200}
\definecolor{OrRd-9-3}{RGB}{253,212,158}
\definecolor{OrRd-9-D}{RGB}{253,212,158}
\definecolor{OrRd-9-4}{RGB}{253,187,132}
\definecolor{OrRd-9-F}{RGB}{253,187,132}
\definecolor{OrRd-9-5}{RGB}{252,141,89}
\definecolor{OrRd-9-G}{RGB}{252,141,89}
\definecolor{OrRd-9-6}{RGB}{239,101,72}
\definecolor{OrRd-9-H}{RGB}{239,101,72}
\definecolor{OrRd-9-7}{RGB}{215,48,31}
\definecolor{OrRd-9-J}{RGB}{215,48,31}
\definecolor{OrRd-9-8}{RGB}{179,0,0}
\definecolor{OrRd-9-K}{RGB}{179,0,0}
\definecolor{OrRd-9-9}{RGB}{127,0,0}
\definecolor{OrRd-9-M}{RGB}{127,0,0}
\definecolor{YlOrRd-3-1}{RGB}{255,237,160}
\definecolor{YlOrRd-3-C}{RGB}{255,237,160}
\definecolor{YlOrRd-3-2}{RGB}{254,178,76}
\definecolor{YlOrRd-3-F}{RGB}{254,178,76}
\definecolor{YlOrRd-3-3}{RGB}{240,59,32}
\definecolor{YlOrRd-3-I}{RGB}{240,59,32}
\definecolor{YlOrRd-4-1}{RGB}{255,255,178}
\definecolor{YlOrRd-4-B}{RGB}{255,255,178}
\definecolor{YlOrRd-4-2}{RGB}{254,204,92}
\definecolor{YlOrRd-4-E}{RGB}{254,204,92}
\definecolor{YlOrRd-4-3}{RGB}{253,141,60}
\definecolor{YlOrRd-4-G}{RGB}{253,141,60}
\definecolor{YlOrRd-4-4}{RGB}{227,26,28}
\definecolor{YlOrRd-4-J}{RGB}{227,26,28}
\definecolor{YlOrRd-5-1}{RGB}{255,255,178}
\definecolor{YlOrRd-5-B}{RGB}{255,255,178}
\definecolor{YlOrRd-5-2}{RGB}{254,204,92}
\definecolor{YlOrRd-5-E}{RGB}{254,204,92}
\definecolor{YlOrRd-5-3}{RGB}{253,141,60}
\definecolor{YlOrRd-5-G}{RGB}{253,141,60}
\definecolor{YlOrRd-5-4}{RGB}{240,59,32}
\definecolor{YlOrRd-5-I}{RGB}{240,59,32}
\definecolor{YlOrRd-5-5}{RGB}{189,0,38}
\definecolor{YlOrRd-5-K}{RGB}{189,0,38}
\definecolor{YlOrRd-6-1}{RGB}{255,255,178}
\definecolor{YlOrRd-6-B}{RGB}{255,255,178}
\definecolor{YlOrRd-6-2}{RGB}{254,217,118}
\definecolor{YlOrRd-6-D}{RGB}{254,217,118}
\definecolor{YlOrRd-6-3}{RGB}{254,178,76}
\definecolor{YlOrRd-6-F}{RGB}{254,178,76}
\definecolor{YlOrRd-6-4}{RGB}{253,141,60}
\definecolor{YlOrRd-6-G}{RGB}{253,141,60}
\definecolor{YlOrRd-6-5}{RGB}{240,59,32}
\definecolor{YlOrRd-6-I}{RGB}{240,59,32}
\definecolor{YlOrRd-6-6}{RGB}{189,0,38}
\definecolor{YlOrRd-6-K}{RGB}{189,0,38}
\definecolor{YlOrRd-7-1}{RGB}{255,255,178}
\definecolor{YlOrRd-7-B}{RGB}{255,255,178}
\definecolor{YlOrRd-7-2}{RGB}{254,217,118}
\definecolor{YlOrRd-7-D}{RGB}{254,217,118}
\definecolor{YlOrRd-7-3}{RGB}{254,178,76}
\definecolor{YlOrRd-7-F}{RGB}{254,178,76}
\definecolor{YlOrRd-7-4}{RGB}{253,141,60}
\definecolor{YlOrRd-7-G}{RGB}{253,141,60}
\definecolor{YlOrRd-7-5}{RGB}{252,78,42}
\definecolor{YlOrRd-7-H}{RGB}{252,78,42}
\definecolor{YlOrRd-7-6}{RGB}{227,26,28}
\definecolor{YlOrRd-7-J}{RGB}{227,26,28}
\definecolor{YlOrRd-7-7}{RGB}{177,0,38}
\definecolor{YlOrRd-7-L}{RGB}{177,0,38}
\definecolor{YlOrRd-8-1}{RGB}{255,255,204}
\definecolor{YlOrRd-8-A}{RGB}{255,255,204}
\definecolor{YlOrRd-8-2}{RGB}{255,237,160}
\definecolor{YlOrRd-8-C}{RGB}{255,237,160}
\definecolor{YlOrRd-8-3}{RGB}{254,217,118}
\definecolor{YlOrRd-8-D}{RGB}{254,217,118}
\definecolor{YlOrRd-8-4}{RGB}{254,178,76}
\definecolor{YlOrRd-8-F}{RGB}{254,178,76}
\definecolor{YlOrRd-8-5}{RGB}{253,141,60}
\definecolor{YlOrRd-8-G}{RGB}{253,141,60}
\definecolor{YlOrRd-8-6}{RGB}{252,78,42}
\definecolor{YlOrRd-8-H}{RGB}{252,78,42}
\definecolor{YlOrRd-8-7}{RGB}{227,26,28}
\definecolor{YlOrRd-8-J}{RGB}{227,26,28}
\definecolor{YlOrRd-8-8}{RGB}{177,0,38}
\definecolor{YlOrRd-8-L}{RGB}{177,0,38}
\definecolor{YlOrRd-9-1}{RGB}{255,255,204}
\definecolor{YlOrRd-9-A}{RGB}{255,255,204}
\definecolor{YlOrRd-9-2}{RGB}{255,237,160}
\definecolor{YlOrRd-9-C}{RGB}{255,237,160}
\definecolor{YlOrRd-9-3}{RGB}{254,217,118}
\definecolor{YlOrRd-9-D}{RGB}{254,217,118}
\definecolor{YlOrRd-9-4}{RGB}{254,178,76}
\definecolor{YlOrRd-9-F}{RGB}{254,178,76}
\definecolor{YlOrRd-9-5}{RGB}{253,141,60}
\definecolor{YlOrRd-9-G}{RGB}{253,141,60}
\definecolor{YlOrRd-9-6}{RGB}{252,78,42}
\definecolor{YlOrRd-9-H}{RGB}{252,78,42}
\definecolor{YlOrRd-9-7}{RGB}{227,26,28}
\definecolor{YlOrRd-9-J}{RGB}{227,26,28}
\definecolor{YlOrRd-9-8}{RGB}{189,0,38}
\definecolor{YlOrRd-9-K}{RGB}{189,0,38}
\definecolor{YlOrRd-9-9}{RGB}{128,0,38}
\definecolor{YlOrRd-9-M}{RGB}{128,0,38}
\definecolor{YlOrBr-3-1}{RGB}{255,247,188}
\definecolor{YlOrBr-3-C}{RGB}{255,247,188}
\definecolor{YlOrBr-3-2}{RGB}{254,196,79}
\definecolor{YlOrBr-3-F}{RGB}{254,196,79}
\definecolor{YlOrBr-3-3}{RGB}{217,95,14}
\definecolor{YlOrBr-3-I}{RGB}{217,95,14}
\definecolor{YlOrBr-4-1}{RGB}{255,255,212}
\definecolor{YlOrBr-4-B}{RGB}{255,255,212}
\definecolor{YlOrBr-4-2}{RGB}{254,217,142}
\definecolor{YlOrBr-4-E}{RGB}{254,217,142}
\definecolor{YlOrBr-4-3}{RGB}{254,153,41}
\definecolor{YlOrBr-4-G}{RGB}{254,153,41}
\definecolor{YlOrBr-4-4}{RGB}{204,76,2}
\definecolor{YlOrBr-4-J}{RGB}{204,76,2}
\definecolor{YlOrBr-5-1}{RGB}{255,255,212}
\definecolor{YlOrBr-5-B}{RGB}{255,255,212}
\definecolor{YlOrBr-5-2}{RGB}{254,217,142}
\definecolor{YlOrBr-5-E}{RGB}{254,217,142}
\definecolor{YlOrBr-5-3}{RGB}{254,153,41}
\definecolor{YlOrBr-5-G}{RGB}{254,153,41}
\definecolor{YlOrBr-5-4}{RGB}{217,95,14}
\definecolor{YlOrBr-5-I}{RGB}{217,95,14}
\definecolor{YlOrBr-5-5}{RGB}{153,52,4}
\definecolor{YlOrBr-5-K}{RGB}{153,52,4}
\definecolor{YlOrBr-6-1}{RGB}{255,255,212}
\definecolor{YlOrBr-6-B}{RGB}{255,255,212}
\definecolor{YlOrBr-6-2}{RGB}{254,227,145}
\definecolor{YlOrBr-6-D}{RGB}{254,227,145}
\definecolor{YlOrBr-6-3}{RGB}{254,196,79}
\definecolor{YlOrBr-6-F}{RGB}{254,196,79}
\definecolor{YlOrBr-6-4}{RGB}{254,153,41}
\definecolor{YlOrBr-6-G}{RGB}{254,153,41}
\definecolor{YlOrBr-6-5}{RGB}{217,95,14}
\definecolor{YlOrBr-6-I}{RGB}{217,95,14}
\definecolor{YlOrBr-6-6}{RGB}{153,52,4}
\definecolor{YlOrBr-6-K}{RGB}{153,52,4}
\definecolor{YlOrBr-7-1}{RGB}{255,255,212}
\definecolor{YlOrBr-7-B}{RGB}{255,255,212}
\definecolor{YlOrBr-7-2}{RGB}{254,227,145}
\definecolor{YlOrBr-7-D}{RGB}{254,227,145}
\definecolor{YlOrBr-7-3}{RGB}{254,196,79}
\definecolor{YlOrBr-7-F}{RGB}{254,196,79}
\definecolor{YlOrBr-7-4}{RGB}{254,153,41}
\definecolor{YlOrBr-7-G}{RGB}{254,153,41}
\definecolor{YlOrBr-7-5}{RGB}{236,112,20}
\definecolor{YlOrBr-7-H}{RGB}{236,112,20}
\definecolor{YlOrBr-7-6}{RGB}{204,76,2}
\definecolor{YlOrBr-7-J}{RGB}{204,76,2}
\definecolor{YlOrBr-7-7}{RGB}{140,45,4}
\definecolor{YlOrBr-7-L}{RGB}{140,45,4}
\definecolor{YlOrBr-8-1}{RGB}{255,255,229}
\definecolor{YlOrBr-8-A}{RGB}{255,255,229}
\definecolor{YlOrBr-8-2}{RGB}{255,247,188}
\definecolor{YlOrBr-8-C}{RGB}{255,247,188}
\definecolor{YlOrBr-8-3}{RGB}{254,227,145}
\definecolor{YlOrBr-8-D}{RGB}{254,227,145}
\definecolor{YlOrBr-8-4}{RGB}{254,196,79}
\definecolor{YlOrBr-8-F}{RGB}{254,196,79}
\definecolor{YlOrBr-8-5}{RGB}{254,153,41}
\definecolor{YlOrBr-8-G}{RGB}{254,153,41}
\definecolor{YlOrBr-8-6}{RGB}{236,112,20}
\definecolor{YlOrBr-8-H}{RGB}{236,112,20}
\definecolor{YlOrBr-8-7}{RGB}{204,76,2}
\definecolor{YlOrBr-8-J}{RGB}{204,76,2}
\definecolor{YlOrBr-8-8}{RGB}{140,45,4}
\definecolor{YlOrBr-8-L}{RGB}{140,45,4}
\definecolor{YlOrBr-9-1}{RGB}{255,255,229}
\definecolor{YlOrBr-9-A}{RGB}{255,255,229}
\definecolor{YlOrBr-9-2}{RGB}{255,247,188}
\definecolor{YlOrBr-9-C}{RGB}{255,247,188}
\definecolor{YlOrBr-9-3}{RGB}{254,227,145}
\definecolor{YlOrBr-9-D}{RGB}{254,227,145}
\definecolor{YlOrBr-9-4}{RGB}{254,196,79}
\definecolor{YlOrBr-9-F}{RGB}{254,196,79}
\definecolor{YlOrBr-9-5}{RGB}{254,153,41}
\definecolor{YlOrBr-9-G}{RGB}{254,153,41}
\definecolor{YlOrBr-9-6}{RGB}{236,112,20}
\definecolor{YlOrBr-9-H}{RGB}{236,112,20}
\definecolor{YlOrBr-9-7}{RGB}{204,76,2}
\definecolor{YlOrBr-9-J}{RGB}{204,76,2}
\definecolor{YlOrBr-9-8}{RGB}{153,52,4}
\definecolor{YlOrBr-9-K}{RGB}{153,52,4}
\definecolor{YlOrBr-9-9}{RGB}{102,37,6}
\definecolor{YlOrBr-9-M}{RGB}{102,37,6}
\definecolor{Purples-3-1}{RGB}{239,237,245}
\definecolor{Purples-3-C}{RGB}{239,237,245}
\definecolor{Purples-3-2}{RGB}{188,189,220}
\definecolor{Purples-3-F}{RGB}{188,189,220}
\definecolor{Purples-3-3}{RGB}{117,107,177}
\definecolor{Purples-3-I}{RGB}{117,107,177}
\definecolor{Purples-4-1}{RGB}{242,240,247}
\definecolor{Purples-4-B}{RGB}{242,240,247}
\definecolor{Purples-4-2}{RGB}{203,201,226}
\definecolor{Purples-4-E}{RGB}{203,201,226}
\definecolor{Purples-4-3}{RGB}{158,154,200}
\definecolor{Purples-4-G}{RGB}{158,154,200}
\definecolor{Purples-4-4}{RGB}{106,81,163}
\definecolor{Purples-4-J}{RGB}{106,81,163}
\definecolor{Purples-5-1}{RGB}{242,240,247}
\definecolor{Purples-5-B}{RGB}{242,240,247}
\definecolor{Purples-5-2}{RGB}{203,201,226}
\definecolor{Purples-5-E}{RGB}{203,201,226}
\definecolor{Purples-5-3}{RGB}{158,154,200}
\definecolor{Purples-5-G}{RGB}{158,154,200}
\definecolor{Purples-5-4}{RGB}{117,107,177}
\definecolor{Purples-5-I}{RGB}{117,107,177}
\definecolor{Purples-5-5}{RGB}{84,39,143}
\definecolor{Purples-5-K}{RGB}{84,39,143}
\definecolor{Purples-6-1}{RGB}{242,240,247}
\definecolor{Purples-6-B}{RGB}{242,240,247}
\definecolor{Purples-6-2}{RGB}{218,218,235}
\definecolor{Purples-6-D}{RGB}{218,218,235}
\definecolor{Purples-6-3}{RGB}{188,189,220}
\definecolor{Purples-6-F}{RGB}{188,189,220}
\definecolor{Purples-6-4}{RGB}{158,154,200}
\definecolor{Purples-6-G}{RGB}{158,154,200}
\definecolor{Purples-6-5}{RGB}{117,107,177}
\definecolor{Purples-6-I}{RGB}{117,107,177}
\definecolor{Purples-6-6}{RGB}{84,39,143}
\definecolor{Purples-6-K}{RGB}{84,39,143}
\definecolor{Purples-7-1}{RGB}{242,240,247}
\definecolor{Purples-7-B}{RGB}{242,240,247}
\definecolor{Purples-7-2}{RGB}{218,218,235}
\definecolor{Purples-7-D}{RGB}{218,218,235}
\definecolor{Purples-7-3}{RGB}{188,189,220}
\definecolor{Purples-7-F}{RGB}{188,189,220}
\definecolor{Purples-7-4}{RGB}{158,154,200}
\definecolor{Purples-7-G}{RGB}{158,154,200}
\definecolor{Purples-7-5}{RGB}{128,125,186}
\definecolor{Purples-7-H}{RGB}{128,125,186}
\definecolor{Purples-7-6}{RGB}{106,81,163}
\definecolor{Purples-7-J}{RGB}{106,81,163}
\definecolor{Purples-7-7}{RGB}{74,20,134}
\definecolor{Purples-7-L}{RGB}{74,20,134}
\definecolor{Purples-8-1}{RGB}{252,251,253}
\definecolor{Purples-8-A}{RGB}{252,251,253}
\definecolor{Purples-8-2}{RGB}{239,237,245}
\definecolor{Purples-8-C}{RGB}{239,237,245}
\definecolor{Purples-8-3}{RGB}{218,218,235}
\definecolor{Purples-8-D}{RGB}{218,218,235}
\definecolor{Purples-8-4}{RGB}{188,189,220}
\definecolor{Purples-8-F}{RGB}{188,189,220}
\definecolor{Purples-8-5}{RGB}{158,154,200}
\definecolor{Purples-8-G}{RGB}{158,154,200}
\definecolor{Purples-8-6}{RGB}{128,125,186}
\definecolor{Purples-8-H}{RGB}{128,125,186}
\definecolor{Purples-8-7}{RGB}{106,81,163}
\definecolor{Purples-8-J}{RGB}{106,81,163}
\definecolor{Purples-8-8}{RGB}{74,20,134}
\definecolor{Purples-8-L}{RGB}{74,20,134}
\definecolor{Purples-9-1}{RGB}{252,251,253}
\definecolor{Purples-9-A}{RGB}{252,251,253}
\definecolor{Purples-9-2}{RGB}{239,237,245}
\definecolor{Purples-9-C}{RGB}{239,237,245}
\definecolor{Purples-9-3}{RGB}{218,218,235}
\definecolor{Purples-9-D}{RGB}{218,218,235}
\definecolor{Purples-9-4}{RGB}{188,189,220}
\definecolor{Purples-9-F}{RGB}{188,189,220}
\definecolor{Purples-9-5}{RGB}{158,154,200}
\definecolor{Purples-9-G}{RGB}{158,154,200}
\definecolor{Purples-9-6}{RGB}{128,125,186}
\definecolor{Purples-9-H}{RGB}{128,125,186}
\definecolor{Purples-9-7}{RGB}{106,81,163}
\definecolor{Purples-9-J}{RGB}{106,81,163}
\definecolor{Purples-9-8}{RGB}{84,39,143}
\definecolor{Purples-9-K}{RGB}{84,39,143}
\definecolor{Purples-9-9}{RGB}{63,0,125}
\definecolor{Purples-9-M}{RGB}{63,0,125}
\definecolor{Blues-3-1}{RGB}{222,235,247}
\definecolor{Blues-3-C}{RGB}{222,235,247}
\definecolor{Blues-3-2}{RGB}{158,202,225}
\definecolor{Blues-3-F}{RGB}{158,202,225}
\definecolor{Blues-3-3}{RGB}{49,130,189}
\definecolor{Blues-3-I}{RGB}{49,130,189}
\definecolor{Blues-4-1}{RGB}{239,243,255}
\definecolor{Blues-4-B}{RGB}{239,243,255}
\definecolor{Blues-4-2}{RGB}{189,215,231}
\definecolor{Blues-4-E}{RGB}{189,215,231}
\definecolor{Blues-4-3}{RGB}{107,174,214}
\definecolor{Blues-4-G}{RGB}{107,174,214}
\definecolor{Blues-4-4}{RGB}{33,113,181}
\definecolor{Blues-4-J}{RGB}{33,113,181}
\definecolor{Blues-5-1}{RGB}{239,243,255}
\definecolor{Blues-5-B}{RGB}{239,243,255}
\definecolor{Blues-5-2}{RGB}{189,215,231}
\definecolor{Blues-5-E}{RGB}{189,215,231}
\definecolor{Blues-5-3}{RGB}{107,174,214}
\definecolor{Blues-5-G}{RGB}{107,174,214}
\definecolor{Blues-5-4}{RGB}{49,130,189}
\definecolor{Blues-5-I}{RGB}{49,130,189}
\definecolor{Blues-5-5}{RGB}{8,81,156}
\definecolor{Blues-5-K}{RGB}{8,81,156}
\definecolor{Blues-6-1}{RGB}{239,243,255}
\definecolor{Blues-6-B}{RGB}{239,243,255}
\definecolor{Blues-6-2}{RGB}{198,219,239}
\definecolor{Blues-6-D}{RGB}{198,219,239}
\definecolor{Blues-6-3}{RGB}{158,202,225}
\definecolor{Blues-6-F}{RGB}{158,202,225}
\definecolor{Blues-6-4}{RGB}{107,174,214}
\definecolor{Blues-6-G}{RGB}{107,174,214}
\definecolor{Blues-6-5}{RGB}{49,130,189}
\definecolor{Blues-6-I}{RGB}{49,130,189}
\definecolor{Blues-6-6}{RGB}{8,81,156}
\definecolor{Blues-6-K}{RGB}{8,81,156}
\definecolor{Blues-7-1}{RGB}{239,243,255}
\definecolor{Blues-7-B}{RGB}{239,243,255}
\definecolor{Blues-7-2}{RGB}{198,219,239}
\definecolor{Blues-7-D}{RGB}{198,219,239}
\definecolor{Blues-7-3}{RGB}{158,202,225}
\definecolor{Blues-7-F}{RGB}{158,202,225}
\definecolor{Blues-7-4}{RGB}{107,174,214}
\definecolor{Blues-7-G}{RGB}{107,174,214}
\definecolor{Blues-7-5}{RGB}{66,146,198}
\definecolor{Blues-7-H}{RGB}{66,146,198}
\definecolor{Blues-7-6}{RGB}{33,113,181}
\definecolor{Blues-7-J}{RGB}{33,113,181}
\definecolor{Blues-7-7}{RGB}{8,69,148}
\definecolor{Blues-7-L}{RGB}{8,69,148}
\definecolor{Blues-8-1}{RGB}{247,251,255}
\definecolor{Blues-8-A}{RGB}{247,251,255}
\definecolor{Blues-8-2}{RGB}{222,235,247}
\definecolor{Blues-8-C}{RGB}{222,235,247}
\definecolor{Blues-8-3}{RGB}{198,219,239}
\definecolor{Blues-8-D}{RGB}{198,219,239}
\definecolor{Blues-8-4}{RGB}{158,202,225}
\definecolor{Blues-8-F}{RGB}{158,202,225}
\definecolor{Blues-8-5}{RGB}{107,174,214}
\definecolor{Blues-8-G}{RGB}{107,174,214}
\definecolor{Blues-8-6}{RGB}{66,146,198}
\definecolor{Blues-8-H}{RGB}{66,146,198}
\definecolor{Blues-8-7}{RGB}{33,113,181}
\definecolor{Blues-8-J}{RGB}{33,113,181}
\definecolor{Blues-8-8}{RGB}{8,69,148}
\definecolor{Blues-8-L}{RGB}{8,69,148}
\definecolor{Blues-9-1}{RGB}{247,251,255}
\definecolor{Blues-9-A}{RGB}{247,251,255}
\definecolor{Blues-9-2}{RGB}{222,235,247}
\definecolor{Blues-9-C}{RGB}{222,235,247}
\definecolor{Blues-9-3}{RGB}{198,219,239}
\definecolor{Blues-9-D}{RGB}{198,219,239}
\definecolor{Blues-9-4}{RGB}{158,202,225}
\definecolor{Blues-9-F}{RGB}{158,202,225}
\definecolor{Blues-9-5}{RGB}{107,174,214}
\definecolor{Blues-9-G}{RGB}{107,174,214}
\definecolor{Blues-9-6}{RGB}{66,146,198}
\definecolor{Blues-9-H}{RGB}{66,146,198}
\definecolor{Blues-9-7}{RGB}{33,113,181}
\definecolor{Blues-9-J}{RGB}{33,113,181}
\definecolor{Blues-9-8}{RGB}{8,81,156}
\definecolor{Blues-9-K}{RGB}{8,81,156}
\definecolor{Blues-9-9}{RGB}{8,48,107}
\definecolor{Blues-9-M}{RGB}{8,48,107}
\definecolor{Greens-3-1}{RGB}{229,245,224}
\definecolor{Greens-3-C}{RGB}{229,245,224}
\definecolor{Greens-3-2}{RGB}{161,217,155}
\definecolor{Greens-3-F}{RGB}{161,217,155}
\definecolor{Greens-3-3}{RGB}{49,163,84}
\definecolor{Greens-3-I}{RGB}{49,163,84}
\definecolor{Greens-4-1}{RGB}{237,248,233}
\definecolor{Greens-4-B}{RGB}{237,248,233}
\definecolor{Greens-4-2}{RGB}{186,228,179}
\definecolor{Greens-4-E}{RGB}{186,228,179}
\definecolor{Greens-4-3}{RGB}{116,196,118}
\definecolor{Greens-4-G}{RGB}{116,196,118}
\definecolor{Greens-4-4}{RGB}{35,139,69}
\definecolor{Greens-4-J}{RGB}{35,139,69}
\definecolor{Greens-5-1}{RGB}{237,248,233}
\definecolor{Greens-5-B}{RGB}{237,248,233}
\definecolor{Greens-5-2}{RGB}{186,228,179}
\definecolor{Greens-5-E}{RGB}{186,228,179}
\definecolor{Greens-5-3}{RGB}{116,196,118}
\definecolor{Greens-5-G}{RGB}{116,196,118}
\definecolor{Greens-5-4}{RGB}{49,163,84}
\definecolor{Greens-5-I}{RGB}{49,163,84}
\definecolor{Greens-5-5}{RGB}{0,109,44}
\definecolor{Greens-5-K}{RGB}{0,109,44}
\definecolor{Greens-6-1}{RGB}{237,248,233}
\definecolor{Greens-6-B}{RGB}{237,248,233}
\definecolor{Greens-6-2}{RGB}{199,233,192}
\definecolor{Greens-6-D}{RGB}{199,233,192}
\definecolor{Greens-6-3}{RGB}{161,217,155}
\definecolor{Greens-6-F}{RGB}{161,217,155}
\definecolor{Greens-6-4}{RGB}{116,196,118}
\definecolor{Greens-6-G}{RGB}{116,196,118}
\definecolor{Greens-6-5}{RGB}{49,163,84}
\definecolor{Greens-6-I}{RGB}{49,163,84}
\definecolor{Greens-6-6}{RGB}{0,109,44}
\definecolor{Greens-6-K}{RGB}{0,109,44}
\definecolor{Greens-7-1}{RGB}{237,248,233}
\definecolor{Greens-7-B}{RGB}{237,248,233}
\definecolor{Greens-7-2}{RGB}{199,233,192}
\definecolor{Greens-7-D}{RGB}{199,233,192}
\definecolor{Greens-7-3}{RGB}{161,217,155}
\definecolor{Greens-7-F}{RGB}{161,217,155}
\definecolor{Greens-7-4}{RGB}{116,196,118}
\definecolor{Greens-7-G}{RGB}{116,196,118}
\definecolor{Greens-7-5}{RGB}{65,171,93}
\definecolor{Greens-7-H}{RGB}{65,171,93}
\definecolor{Greens-7-6}{RGB}{35,139,69}
\definecolor{Greens-7-J}{RGB}{35,139,69}
\definecolor{Greens-7-7}{RGB}{0,90,50}
\definecolor{Greens-7-L}{RGB}{0,90,50}
\definecolor{Greens-8-1}{RGB}{247,252,245}
\definecolor{Greens-8-A}{RGB}{247,252,245}
\definecolor{Greens-8-2}{RGB}{229,245,224}
\definecolor{Greens-8-C}{RGB}{229,245,224}
\definecolor{Greens-8-3}{RGB}{199,233,192}
\definecolor{Greens-8-D}{RGB}{199,233,192}
\definecolor{Greens-8-4}{RGB}{161,217,155}
\definecolor{Greens-8-F}{RGB}{161,217,155}
\definecolor{Greens-8-5}{RGB}{116,196,118}
\definecolor{Greens-8-G}{RGB}{116,196,118}
\definecolor{Greens-8-6}{RGB}{65,171,93}
\definecolor{Greens-8-H}{RGB}{65,171,93}
\definecolor{Greens-8-7}{RGB}{35,139,69}
\definecolor{Greens-8-J}{RGB}{35,139,69}
\definecolor{Greens-8-8}{RGB}{0,90,50}
\definecolor{Greens-8-L}{RGB}{0,90,50}
\definecolor{Greens-9-1}{RGB}{247,252,245}
\definecolor{Greens-9-A}{RGB}{247,252,245}
\definecolor{Greens-9-2}{RGB}{229,245,224}
\definecolor{Greens-9-C}{RGB}{229,245,224}
\definecolor{Greens-9-3}{RGB}{199,233,192}
\definecolor{Greens-9-D}{RGB}{199,233,192}
\definecolor{Greens-9-4}{RGB}{161,217,155}
\definecolor{Greens-9-F}{RGB}{161,217,155}
\definecolor{Greens-9-5}{RGB}{116,196,118}
\definecolor{Greens-9-G}{RGB}{116,196,118}
\definecolor{Greens-9-6}{RGB}{65,171,93}
\definecolor{Greens-9-H}{RGB}{65,171,93}
\definecolor{Greens-9-7}{RGB}{35,139,69}
\definecolor{Greens-9-J}{RGB}{35,139,69}
\definecolor{Greens-9-8}{RGB}{0,109,44}
\definecolor{Greens-9-K}{RGB}{0,109,44}
\definecolor{Greens-9-9}{RGB}{0,68,27}
\definecolor{Greens-9-M}{RGB}{0,68,27}
\definecolor{Oranges-3-1}{RGB}{254,230,206}
\definecolor{Oranges-3-C}{RGB}{254,230,206}
\definecolor{Oranges-3-2}{RGB}{253,174,107}
\definecolor{Oranges-3-F}{RGB}{253,174,107}
\definecolor{Oranges-3-3}{RGB}{230,85,13}
\definecolor{Oranges-3-I}{RGB}{230,85,13}
\definecolor{Oranges-4-1}{RGB}{254,237,222}
\definecolor{Oranges-4-B}{RGB}{254,237,222}
\definecolor{Oranges-4-2}{RGB}{253,190,133}
\definecolor{Oranges-4-E}{RGB}{253,190,133}
\definecolor{Oranges-4-3}{RGB}{253,141,60}
\definecolor{Oranges-4-G}{RGB}{253,141,60}
\definecolor{Oranges-4-4}{RGB}{217,71,1}
\definecolor{Oranges-4-J}{RGB}{217,71,1}
\definecolor{Oranges-5-1}{RGB}{254,237,222}
\definecolor{Oranges-5-B}{RGB}{254,237,222}
\definecolor{Oranges-5-2}{RGB}{253,190,133}
\definecolor{Oranges-5-E}{RGB}{253,190,133}
\definecolor{Oranges-5-3}{RGB}{253,141,60}
\definecolor{Oranges-5-G}{RGB}{253,141,60}
\definecolor{Oranges-5-4}{RGB}{230,85,13}
\definecolor{Oranges-5-I}{RGB}{230,85,13}
\definecolor{Oranges-5-5}{RGB}{166,54,3}
\definecolor{Oranges-5-K}{RGB}{166,54,3}
\definecolor{Oranges-6-1}{RGB}{254,237,222}
\definecolor{Oranges-6-B}{RGB}{254,237,222}
\definecolor{Oranges-6-2}{RGB}{253,208,162}
\definecolor{Oranges-6-D}{RGB}{253,208,162}
\definecolor{Oranges-6-3}{RGB}{253,174,107}
\definecolor{Oranges-6-F}{RGB}{253,174,107}
\definecolor{Oranges-6-4}{RGB}{253,141,60}
\definecolor{Oranges-6-G}{RGB}{253,141,60}
\definecolor{Oranges-6-5}{RGB}{230,85,13}
\definecolor{Oranges-6-I}{RGB}{230,85,13}
\definecolor{Oranges-6-6}{RGB}{166,54,3}
\definecolor{Oranges-6-K}{RGB}{166,54,3}
\definecolor{Oranges-7-1}{RGB}{254,237,222}
\definecolor{Oranges-7-B}{RGB}{254,237,222}
\definecolor{Oranges-7-2}{RGB}{253,208,162}
\definecolor{Oranges-7-D}{RGB}{253,208,162}
\definecolor{Oranges-7-3}{RGB}{253,174,107}
\definecolor{Oranges-7-F}{RGB}{253,174,107}
\definecolor{Oranges-7-4}{RGB}{253,141,60}
\definecolor{Oranges-7-G}{RGB}{253,141,60}
\definecolor{Oranges-7-5}{RGB}{241,105,19}
\definecolor{Oranges-7-H}{RGB}{241,105,19}
\definecolor{Oranges-7-6}{RGB}{217,72,1}
\definecolor{Oranges-7-J}{RGB}{217,72,1}
\definecolor{Oranges-7-7}{RGB}{140,45,4}
\definecolor{Oranges-7-L}{RGB}{140,45,4}
\definecolor{Oranges-8-1}{RGB}{255,245,235}
\definecolor{Oranges-8-A}{RGB}{255,245,235}
\definecolor{Oranges-8-2}{RGB}{254,230,206}
\definecolor{Oranges-8-C}{RGB}{254,230,206}
\definecolor{Oranges-8-3}{RGB}{253,208,162}
\definecolor{Oranges-8-D}{RGB}{253,208,162}
\definecolor{Oranges-8-4}{RGB}{253,174,107}
\definecolor{Oranges-8-F}{RGB}{253,174,107}
\definecolor{Oranges-8-5}{RGB}{253,141,60}
\definecolor{Oranges-8-G}{RGB}{253,141,60}
\definecolor{Oranges-8-6}{RGB}{241,105,19}
\definecolor{Oranges-8-H}{RGB}{241,105,19}
\definecolor{Oranges-8-7}{RGB}{217,72,1}
\definecolor{Oranges-8-J}{RGB}{217,72,1}
\definecolor{Oranges-8-8}{RGB}{140,45,4}
\definecolor{Oranges-8-L}{RGB}{140,45,4}
\definecolor{Oranges-9-1}{RGB}{255,245,235}
\definecolor{Oranges-9-A}{RGB}{255,245,235}
\definecolor{Oranges-9-2}{RGB}{254,230,206}
\definecolor{Oranges-9-C}{RGB}{254,230,206}
\definecolor{Oranges-9-3}{RGB}{253,208,162}
\definecolor{Oranges-9-D}{RGB}{253,208,162}
\definecolor{Oranges-9-4}{RGB}{253,174,107}
\definecolor{Oranges-9-F}{RGB}{253,174,107}
\definecolor{Oranges-9-5}{RGB}{253,141,60}
\definecolor{Oranges-9-G}{RGB}{253,141,60}
\definecolor{Oranges-9-6}{RGB}{241,105,19}
\definecolor{Oranges-9-H}{RGB}{241,105,19}
\definecolor{Oranges-9-7}{RGB}{217,72,1}
\definecolor{Oranges-9-J}{RGB}{217,72,1}
\definecolor{Oranges-9-8}{RGB}{166,54,3}
\definecolor{Oranges-9-K}{RGB}{166,54,3}
\definecolor{Oranges-9-9}{RGB}{127,39,4}
\definecolor{Oranges-9-M}{RGB}{127,39,4}
\definecolor{Reds-3-1}{RGB}{254,224,210}
\definecolor{Reds-3-C}{RGB}{254,224,210}
\definecolor{Reds-3-2}{RGB}{252,146,114}
\definecolor{Reds-3-F}{RGB}{252,146,114}
\definecolor{Reds-3-3}{RGB}{222,45,38}
\definecolor{Reds-3-I}{RGB}{222,45,38}
\definecolor{Reds-4-1}{RGB}{254,229,217}
\definecolor{Reds-4-B}{RGB}{254,229,217}
\definecolor{Reds-4-2}{RGB}{252,174,145}
\definecolor{Reds-4-E}{RGB}{252,174,145}
\definecolor{Reds-4-3}{RGB}{251,106,74}
\definecolor{Reds-4-G}{RGB}{251,106,74}
\definecolor{Reds-4-4}{RGB}{203,24,29}
\definecolor{Reds-4-J}{RGB}{203,24,29}
\definecolor{Reds-5-1}{RGB}{254,229,217}
\definecolor{Reds-5-B}{RGB}{254,229,217}
\definecolor{Reds-5-2}{RGB}{252,174,145}
\definecolor{Reds-5-E}{RGB}{252,174,145}
\definecolor{Reds-5-3}{RGB}{251,106,74}
\definecolor{Reds-5-G}{RGB}{251,106,74}
\definecolor{Reds-5-4}{RGB}{222,45,38}
\definecolor{Reds-5-I}{RGB}{222,45,38}
\definecolor{Reds-5-5}{RGB}{165,15,21}
\definecolor{Reds-5-K}{RGB}{165,15,21}
\definecolor{Reds-6-1}{RGB}{254,229,217}
\definecolor{Reds-6-B}{RGB}{254,229,217}
\definecolor{Reds-6-2}{RGB}{252,187,161}
\definecolor{Reds-6-D}{RGB}{252,187,161}
\definecolor{Reds-6-3}{RGB}{252,146,114}
\definecolor{Reds-6-F}{RGB}{252,146,114}
\definecolor{Reds-6-4}{RGB}{251,106,74}
\definecolor{Reds-6-G}{RGB}{251,106,74}
\definecolor{Reds-6-5}{RGB}{222,45,38}
\definecolor{Reds-6-I}{RGB}{222,45,38}
\definecolor{Reds-6-6}{RGB}{165,15,21}
\definecolor{Reds-6-K}{RGB}{165,15,21}
\definecolor{Reds-7-1}{RGB}{254,229,217}
\definecolor{Reds-7-B}{RGB}{254,229,217}
\definecolor{Reds-7-2}{RGB}{252,187,161}
\definecolor{Reds-7-D}{RGB}{252,187,161}
\definecolor{Reds-7-3}{RGB}{252,146,114}
\definecolor{Reds-7-F}{RGB}{252,146,114}
\definecolor{Reds-7-4}{RGB}{251,106,74}
\definecolor{Reds-7-G}{RGB}{251,106,74}
\definecolor{Reds-7-5}{RGB}{239,59,44}
\definecolor{Reds-7-H}{RGB}{239,59,44}
\definecolor{Reds-7-6}{RGB}{203,24,29}
\definecolor{Reds-7-J}{RGB}{203,24,29}
\definecolor{Reds-7-7}{RGB}{153,0,13}
\definecolor{Reds-7-L}{RGB}{153,0,13}
\definecolor{Reds-8-1}{RGB}{255,245,240}
\definecolor{Reds-8-A}{RGB}{255,245,240}
\definecolor{Reds-8-2}{RGB}{254,224,210}
\definecolor{Reds-8-C}{RGB}{254,224,210}
\definecolor{Reds-8-3}{RGB}{252,187,161}
\definecolor{Reds-8-D}{RGB}{252,187,161}
\definecolor{Reds-8-4}{RGB}{252,146,114}
\definecolor{Reds-8-F}{RGB}{252,146,114}
\definecolor{Reds-8-5}{RGB}{251,106,74}
\definecolor{Reds-8-G}{RGB}{251,106,74}
\definecolor{Reds-8-6}{RGB}{239,59,44}
\definecolor{Reds-8-H}{RGB}{239,59,44}
\definecolor{Reds-8-7}{RGB}{203,24,29}
\definecolor{Reds-8-J}{RGB}{203,24,29}
\definecolor{Reds-8-8}{RGB}{153,0,13}
\definecolor{Reds-8-L}{RGB}{153,0,13}
\definecolor{Reds-9-1}{RGB}{255,245,240}
\definecolor{Reds-9-A}{RGB}{255,245,240}
\definecolor{Reds-9-2}{RGB}{254,224,210}
\definecolor{Reds-9-C}{RGB}{254,224,210}
\definecolor{Reds-9-3}{RGB}{252,187,161}
\definecolor{Reds-9-D}{RGB}{252,187,161}
\definecolor{Reds-9-4}{RGB}{252,146,114}
\definecolor{Reds-9-F}{RGB}{252,146,114}
\definecolor{Reds-9-5}{RGB}{251,106,74}
\definecolor{Reds-9-G}{RGB}{251,106,74}
\definecolor{Reds-9-6}{RGB}{239,59,44}
\definecolor{Reds-9-H}{RGB}{239,59,44}
\definecolor{Reds-9-7}{RGB}{203,24,29}
\definecolor{Reds-9-J}{RGB}{203,24,29}
\definecolor{Reds-9-8}{RGB}{165,15,21}
\definecolor{Reds-9-K}{RGB}{165,15,21}
\definecolor{Reds-9-9}{RGB}{103,0,13}
\definecolor{Reds-9-M}{RGB}{103,0,13}
\definecolor{Greys-3-1}{RGB}{240,240,240}
\definecolor{Greys-3-C}{RGB}{240,240,240}
\definecolor{Greys-3-2}{RGB}{189,189,189}
\definecolor{Greys-3-F}{RGB}{189,189,189}
\definecolor{Greys-3-3}{RGB}{99,99,99}
\definecolor{Greys-3-I}{RGB}{99,99,99}
\definecolor{Greys-4-1}{RGB}{247,247,247}
\definecolor{Greys-4-B}{RGB}{247,247,247}
\definecolor{Greys-4-2}{RGB}{204,204,204}
\definecolor{Greys-4-E}{RGB}{204,204,204}
\definecolor{Greys-4-3}{RGB}{150,150,150}
\definecolor{Greys-4-G}{RGB}{150,150,150}
\definecolor{Greys-4-4}{RGB}{82,82,82}
\definecolor{Greys-4-J}{RGB}{82,82,82}
\definecolor{Greys-5-1}{RGB}{247,247,247}
\definecolor{Greys-5-B}{RGB}{247,247,247}
\definecolor{Greys-5-2}{RGB}{204,204,204}
\definecolor{Greys-5-E}{RGB}{204,204,204}
\definecolor{Greys-5-3}{RGB}{150,150,150}
\definecolor{Greys-5-G}{RGB}{150,150,150}
\definecolor{Greys-5-4}{RGB}{99,99,99}
\definecolor{Greys-5-I}{RGB}{99,99,99}
\definecolor{Greys-5-5}{RGB}{37,37,37}
\definecolor{Greys-5-K}{RGB}{37,37,37}
\definecolor{Greys-6-1}{RGB}{247,247,247}
\definecolor{Greys-6-B}{RGB}{247,247,247}
\definecolor{Greys-6-2}{RGB}{217,217,217}
\definecolor{Greys-6-D}{RGB}{217,217,217}
\definecolor{Greys-6-3}{RGB}{189,189,189}
\definecolor{Greys-6-F}{RGB}{189,189,189}
\definecolor{Greys-6-4}{RGB}{150,150,150}
\definecolor{Greys-6-G}{RGB}{150,150,150}
\definecolor{Greys-6-5}{RGB}{99,99,99}
\definecolor{Greys-6-I}{RGB}{99,99,99}
\definecolor{Greys-6-6}{RGB}{37,37,37}
\definecolor{Greys-6-K}{RGB}{37,37,37}
\definecolor{Greys-7-1}{RGB}{247,247,247}
\definecolor{Greys-7-B}{RGB}{247,247,247}
\definecolor{Greys-7-2}{RGB}{217,217,217}
\definecolor{Greys-7-D}{RGB}{217,217,217}
\definecolor{Greys-7-3}{RGB}{189,189,189}
\definecolor{Greys-7-F}{RGB}{189,189,189}
\definecolor{Greys-7-4}{RGB}{150,150,150}
\definecolor{Greys-7-G}{RGB}{150,150,150}
\definecolor{Greys-7-5}{RGB}{115,115,115}
\definecolor{Greys-7-H}{RGB}{115,115,115}
\definecolor{Greys-7-6}{RGB}{82,82,82}
\definecolor{Greys-7-J}{RGB}{82,82,82}
\definecolor{Greys-7-7}{RGB}{37,37,37}
\definecolor{Greys-7-L}{RGB}{37,37,37}
\definecolor{Greys-8-1}{RGB}{255,255,255}
\definecolor{Greys-8-A}{RGB}{255,255,255}
\definecolor{Greys-8-2}{RGB}{240,240,240}
\definecolor{Greys-8-C}{RGB}{240,240,240}
\definecolor{Greys-8-3}{RGB}{217,217,217}
\definecolor{Greys-8-D}{RGB}{217,217,217}
\definecolor{Greys-8-4}{RGB}{189,189,189}
\definecolor{Greys-8-F}{RGB}{189,189,189}
\definecolor{Greys-8-5}{RGB}{150,150,150}
\definecolor{Greys-8-G}{RGB}{150,150,150}
\definecolor{Greys-8-6}{RGB}{115,115,115}
\definecolor{Greys-8-H}{RGB}{115,115,115}
\definecolor{Greys-8-7}{RGB}{82,82,82}
\definecolor{Greys-8-J}{RGB}{82,82,82}
\definecolor{Greys-8-8}{RGB}{37,37,37}
\definecolor{Greys-8-L}{RGB}{37,37,37}
\definecolor{Greys-9-1}{RGB}{255,255,255}
\definecolor{Greys-9-A}{RGB}{255,255,255}
\definecolor{Greys-9-2}{RGB}{240,240,240}
\definecolor{Greys-9-C}{RGB}{240,240,240}
\definecolor{Greys-9-3}{RGB}{217,217,217}
\definecolor{Greys-9-D}{RGB}{217,217,217}
\definecolor{Greys-9-4}{RGB}{189,189,189}
\definecolor{Greys-9-F}{RGB}{189,189,189}
\definecolor{Greys-9-5}{RGB}{150,150,150}
\definecolor{Greys-9-G}{RGB}{150,150,150}
\definecolor{Greys-9-6}{RGB}{115,115,115}
\definecolor{Greys-9-H}{RGB}{115,115,115}
\definecolor{Greys-9-7}{RGB}{82,82,82}
\definecolor{Greys-9-J}{RGB}{82,82,82}
\definecolor{Greys-9-8}{RGB}{37,37,37}
\definecolor{Greys-9-K}{RGB}{37,37,37}
\definecolor{Greys-9-9}{RGB}{0,0,0}
\definecolor{Greys-9-M}{RGB}{0,0,0}
\definecolor{PuOr-3-1}{RGB}{241,163,64}
\definecolor{PuOr-3-E}{RGB}{241,163,64}
\definecolor{PuOr-3-2}{RGB}{247,247,247}
\definecolor{PuOr-3-H}{RGB}{247,247,247}
\definecolor{PuOr-3-3}{RGB}{153,142,195}
\definecolor{PuOr-3-K}{RGB}{153,142,195}
\definecolor{PuOr-4-1}{RGB}{230,97,1}
\definecolor{PuOr-4-C}{RGB}{230,97,1}
\definecolor{PuOr-4-2}{RGB}{253,184,99}
\definecolor{PuOr-4-F}{RGB}{253,184,99}
\definecolor{PuOr-4-3}{RGB}{178,171,210}
\definecolor{PuOr-4-J}{RGB}{178,171,210}
\definecolor{PuOr-4-4}{RGB}{94,60,153}
\definecolor{PuOr-4-M}{RGB}{94,60,153}
\definecolor{PuOr-5-1}{RGB}{230,97,1}
\definecolor{PuOr-5-C}{RGB}{230,97,1}
\definecolor{PuOr-5-2}{RGB}{253,184,99}
\definecolor{PuOr-5-F}{RGB}{253,184,99}
\definecolor{PuOr-5-3}{RGB}{247,247,247}
\definecolor{PuOr-5-H}{RGB}{247,247,247}
\definecolor{PuOr-5-4}{RGB}{178,171,210}
\definecolor{PuOr-5-J}{RGB}{178,171,210}
\definecolor{PuOr-5-5}{RGB}{94,60,153}
\definecolor{PuOr-5-M}{RGB}{94,60,153}
\definecolor{PuOr-6-1}{RGB}{179,88,6}
\definecolor{PuOr-6-B}{RGB}{179,88,6}
\definecolor{PuOr-6-2}{RGB}{241,163,64}
\definecolor{PuOr-6-E}{RGB}{241,163,64}
\definecolor{PuOr-6-3}{RGB}{254,224,182}
\definecolor{PuOr-6-G}{RGB}{254,224,182}
\definecolor{PuOr-6-4}{RGB}{216,218,235}
\definecolor{PuOr-6-I}{RGB}{216,218,235}
\definecolor{PuOr-6-5}{RGB}{153,142,195}
\definecolor{PuOr-6-K}{RGB}{153,142,195}
\definecolor{PuOr-6-6}{RGB}{84,39,136}
\definecolor{PuOr-6-N}{RGB}{84,39,136}
\definecolor{PuOr-7-1}{RGB}{179,88,6}
\definecolor{PuOr-7-B}{RGB}{179,88,6}
\definecolor{PuOr-7-2}{RGB}{241,163,64}
\definecolor{PuOr-7-E}{RGB}{241,163,64}
\definecolor{PuOr-7-3}{RGB}{254,224,182}
\definecolor{PuOr-7-G}{RGB}{254,224,182}
\definecolor{PuOr-7-4}{RGB}{247,247,247}
\definecolor{PuOr-7-H}{RGB}{247,247,247}
\definecolor{PuOr-7-5}{RGB}{216,218,235}
\definecolor{PuOr-7-I}{RGB}{216,218,235}
\definecolor{PuOr-7-6}{RGB}{153,142,195}
\definecolor{PuOr-7-K}{RGB}{153,142,195}
\definecolor{PuOr-7-7}{RGB}{84,39,136}
\definecolor{PuOr-7-N}{RGB}{84,39,136}
\definecolor{PuOr-8-1}{RGB}{179,88,6}
\definecolor{PuOr-8-B}{RGB}{179,88,6}
\definecolor{PuOr-8-2}{RGB}{224,130,20}
\definecolor{PuOr-8-D}{RGB}{224,130,20}
\definecolor{PuOr-8-3}{RGB}{253,184,99}
\definecolor{PuOr-8-F}{RGB}{253,184,99}
\definecolor{PuOr-8-4}{RGB}{254,224,182}
\definecolor{PuOr-8-G}{RGB}{254,224,182}
\definecolor{PuOr-8-5}{RGB}{216,218,235}
\definecolor{PuOr-8-I}{RGB}{216,218,235}
\definecolor{PuOr-8-6}{RGB}{178,171,210}
\definecolor{PuOr-8-J}{RGB}{178,171,210}
\definecolor{PuOr-8-7}{RGB}{128,115,172}
\definecolor{PuOr-8-L}{RGB}{128,115,172}
\definecolor{PuOr-8-8}{RGB}{84,39,136}
\definecolor{PuOr-8-N}{RGB}{84,39,136}
\definecolor{PuOr-9-1}{RGB}{179,88,6}
\definecolor{PuOr-9-B}{RGB}{179,88,6}
\definecolor{PuOr-9-2}{RGB}{224,130,20}
\definecolor{PuOr-9-D}{RGB}{224,130,20}
\definecolor{PuOr-9-3}{RGB}{253,184,99}
\definecolor{PuOr-9-F}{RGB}{253,184,99}
\definecolor{PuOr-9-4}{RGB}{254,224,182}
\definecolor{PuOr-9-G}{RGB}{254,224,182}
\definecolor{PuOr-9-5}{RGB}{247,247,247}
\definecolor{PuOr-9-H}{RGB}{247,247,247}
\definecolor{PuOr-9-6}{RGB}{216,218,235}
\definecolor{PuOr-9-I}{RGB}{216,218,235}
\definecolor{PuOr-9-7}{RGB}{178,171,210}
\definecolor{PuOr-9-J}{RGB}{178,171,210}
\definecolor{PuOr-9-8}{RGB}{128,115,172}
\definecolor{PuOr-9-L}{RGB}{128,115,172}
\definecolor{PuOr-9-9}{RGB}{84,39,136}
\definecolor{PuOr-9-N}{RGB}{84,39,136}
\definecolor{PuOr-10-1}{RGB}{127,59,8}
\definecolor{PuOr-10-A}{RGB}{127,59,8}
\definecolor{PuOr-10-2}{RGB}{179,88,6}
\definecolor{PuOr-10-B}{RGB}{179,88,6}
\definecolor{PuOr-10-3}{RGB}{224,130,20}
\definecolor{PuOr-10-D}{RGB}{224,130,20}
\definecolor{PuOr-10-4}{RGB}{253,184,99}
\definecolor{PuOr-10-F}{RGB}{253,184,99}
\definecolor{PuOr-10-5}{RGB}{254,224,182}
\definecolor{PuOr-10-G}{RGB}{254,224,182}
\definecolor{PuOr-10-6}{RGB}{216,218,235}
\definecolor{PuOr-10-I}{RGB}{216,218,235}
\definecolor{PuOr-10-7}{RGB}{178,171,210}
\definecolor{PuOr-10-J}{RGB}{178,171,210}
\definecolor{PuOr-10-8}{RGB}{128,115,172}
\definecolor{PuOr-10-L}{RGB}{128,115,172}
\definecolor{PuOr-10-9}{RGB}{84,39,136}
\definecolor{PuOr-10-N}{RGB}{84,39,136}
\definecolor{PuOr-10-10}{RGB}{45,0,75}
\definecolor{PuOr-10-O}{RGB}{45,0,75}
\definecolor{PuOr-11-1}{RGB}{127,59,8}
\definecolor{PuOr-11-A}{RGB}{127,59,8}
\definecolor{PuOr-11-2}{RGB}{179,88,6}
\definecolor{PuOr-11-B}{RGB}{179,88,6}
\definecolor{PuOr-11-3}{RGB}{224,130,20}
\definecolor{PuOr-11-D}{RGB}{224,130,20}
\definecolor{PuOr-11-4}{RGB}{253,184,99}
\definecolor{PuOr-11-F}{RGB}{253,184,99}
\definecolor{PuOr-11-5}{RGB}{254,224,182}
\definecolor{PuOr-11-G}{RGB}{254,224,182}
\definecolor{PuOr-11-6}{RGB}{247,247,247}
\definecolor{PuOr-11-H}{RGB}{247,247,247}
\definecolor{PuOr-11-7}{RGB}{216,218,235}
\definecolor{PuOr-11-I}{RGB}{216,218,235}
\definecolor{PuOr-11-8}{RGB}{178,171,210}
\definecolor{PuOr-11-J}{RGB}{178,171,210}
\definecolor{PuOr-11-9}{RGB}{128,115,172}
\definecolor{PuOr-11-L}{RGB}{128,115,172}
\definecolor{PuOr-11-10}{RGB}{84,39,136}
\definecolor{PuOr-11-N}{RGB}{84,39,136}
\definecolor{PuOr-11-11}{RGB}{45,0,75}
\definecolor{PuOr-11-O}{RGB}{45,0,75}
\definecolor{BrBG-3-1}{RGB}{216,179,101}
\definecolor{BrBG-3-E}{RGB}{216,179,101}
\definecolor{BrBG-3-2}{RGB}{245,245,245}
\definecolor{BrBG-3-H}{RGB}{245,245,245}
\definecolor{BrBG-3-3}{RGB}{90,180,172}
\definecolor{BrBG-3-K}{RGB}{90,180,172}
\definecolor{BrBG-4-1}{RGB}{166,97,26}
\definecolor{BrBG-4-C}{RGB}{166,97,26}
\definecolor{BrBG-4-2}{RGB}{223,194,125}
\definecolor{BrBG-4-F}{RGB}{223,194,125}
\definecolor{BrBG-4-3}{RGB}{128,205,193}
\definecolor{BrBG-4-J}{RGB}{128,205,193}
\definecolor{BrBG-4-4}{RGB}{1,133,113}
\definecolor{BrBG-4-M}{RGB}{1,133,113}
\definecolor{BrBG-5-1}{RGB}{166,97,26}
\definecolor{BrBG-5-C}{RGB}{166,97,26}
\definecolor{BrBG-5-2}{RGB}{223,194,125}
\definecolor{BrBG-5-F}{RGB}{223,194,125}
\definecolor{BrBG-5-3}{RGB}{245,245,245}
\definecolor{BrBG-5-H}{RGB}{245,245,245}
\definecolor{BrBG-5-4}{RGB}{128,205,193}
\definecolor{BrBG-5-J}{RGB}{128,205,193}
\definecolor{BrBG-5-5}{RGB}{1,133,113}
\definecolor{BrBG-5-M}{RGB}{1,133,113}
\definecolor{BrBG-6-1}{RGB}{140,81,10}
\definecolor{BrBG-6-B}{RGB}{140,81,10}
\definecolor{BrBG-6-2}{RGB}{216,179,101}
\definecolor{BrBG-6-E}{RGB}{216,179,101}
\definecolor{BrBG-6-3}{RGB}{246,232,195}
\definecolor{BrBG-6-G}{RGB}{246,232,195}
\definecolor{BrBG-6-4}{RGB}{199,234,229}
\definecolor{BrBG-6-I}{RGB}{199,234,229}
\definecolor{BrBG-6-5}{RGB}{90,180,172}
\definecolor{BrBG-6-K}{RGB}{90,180,172}
\definecolor{BrBG-6-6}{RGB}{1,102,94}
\definecolor{BrBG-6-N}{RGB}{1,102,94}
\definecolor{BrBG-7-1}{RGB}{140,81,10}
\definecolor{BrBG-7-B}{RGB}{140,81,10}
\definecolor{BrBG-7-2}{RGB}{216,179,101}
\definecolor{BrBG-7-E}{RGB}{216,179,101}
\definecolor{BrBG-7-3}{RGB}{246,232,195}
\definecolor{BrBG-7-G}{RGB}{246,232,195}
\definecolor{BrBG-7-4}{RGB}{245,245,245}
\definecolor{BrBG-7-H}{RGB}{245,245,245}
\definecolor{BrBG-7-5}{RGB}{199,234,229}
\definecolor{BrBG-7-I}{RGB}{199,234,229}
\definecolor{BrBG-7-6}{RGB}{90,180,172}
\definecolor{BrBG-7-K}{RGB}{90,180,172}
\definecolor{BrBG-7-7}{RGB}{1,102,94}
\definecolor{BrBG-7-N}{RGB}{1,102,94}
\definecolor{BrBG-8-1}{RGB}{140,81,10}
\definecolor{BrBG-8-B}{RGB}{140,81,10}
\definecolor{BrBG-8-2}{RGB}{191,129,45}
\definecolor{BrBG-8-D}{RGB}{191,129,45}
\definecolor{BrBG-8-3}{RGB}{223,194,125}
\definecolor{BrBG-8-F}{RGB}{223,194,125}
\definecolor{BrBG-8-4}{RGB}{246,232,195}
\definecolor{BrBG-8-G}{RGB}{246,232,195}
\definecolor{BrBG-8-5}{RGB}{199,234,229}
\definecolor{BrBG-8-I}{RGB}{199,234,229}
\definecolor{BrBG-8-6}{RGB}{128,205,193}
\definecolor{BrBG-8-J}{RGB}{128,205,193}
\definecolor{BrBG-8-7}{RGB}{53,151,143}
\definecolor{BrBG-8-L}{RGB}{53,151,143}
\definecolor{BrBG-8-8}{RGB}{1,102,94}
\definecolor{BrBG-8-N}{RGB}{1,102,94}
\definecolor{BrBG-9-1}{RGB}{140,81,10}
\definecolor{BrBG-9-B}{RGB}{140,81,10}
\definecolor{BrBG-9-2}{RGB}{191,129,45}
\definecolor{BrBG-9-D}{RGB}{191,129,45}
\definecolor{BrBG-9-3}{RGB}{223,194,125}
\definecolor{BrBG-9-F}{RGB}{223,194,125}
\definecolor{BrBG-9-4}{RGB}{246,232,195}
\definecolor{BrBG-9-G}{RGB}{246,232,195}
\definecolor{BrBG-9-5}{RGB}{245,245,245}
\definecolor{BrBG-9-H}{RGB}{245,245,245}
\definecolor{BrBG-9-6}{RGB}{199,234,229}
\definecolor{BrBG-9-I}{RGB}{199,234,229}
\definecolor{BrBG-9-7}{RGB}{128,205,193}
\definecolor{BrBG-9-J}{RGB}{128,205,193}
\definecolor{BrBG-9-8}{RGB}{53,151,143}
\definecolor{BrBG-9-L}{RGB}{53,151,143}
\definecolor{BrBG-9-9}{RGB}{1,102,94}
\definecolor{BrBG-9-N}{RGB}{1,102,94}
\definecolor{BrBG-10-1}{RGB}{84,48,5}
\definecolor{BrBG-10-A}{RGB}{84,48,5}
\definecolor{BrBG-10-2}{RGB}{140,81,10}
\definecolor{BrBG-10-B}{RGB}{140,81,10}
\definecolor{BrBG-10-3}{RGB}{191,129,45}
\definecolor{BrBG-10-D}{RGB}{191,129,45}
\definecolor{BrBG-10-4}{RGB}{223,194,125}
\definecolor{BrBG-10-F}{RGB}{223,194,125}
\definecolor{BrBG-10-5}{RGB}{246,232,195}
\definecolor{BrBG-10-G}{RGB}{246,232,195}
\definecolor{BrBG-10-6}{RGB}{199,234,229}
\definecolor{BrBG-10-I}{RGB}{199,234,229}
\definecolor{BrBG-10-7}{RGB}{128,205,193}
\definecolor{BrBG-10-J}{RGB}{128,205,193}
\definecolor{BrBG-10-8}{RGB}{53,151,143}
\definecolor{BrBG-10-L}{RGB}{53,151,143}
\definecolor{BrBG-10-9}{RGB}{1,102,94}
\definecolor{BrBG-10-N}{RGB}{1,102,94}
\definecolor{BrBG-10-10}{RGB}{0,60,48}
\definecolor{BrBG-10-O}{RGB}{0,60,48}
\definecolor{BrBG-11-1}{RGB}{84,48,5}
\definecolor{BrBG-11-A}{RGB}{84,48,5}
\definecolor{BrBG-11-2}{RGB}{140,81,10}
\definecolor{BrBG-11-B}{RGB}{140,81,10}
\definecolor{BrBG-11-3}{RGB}{191,129,45}
\definecolor{BrBG-11-D}{RGB}{191,129,45}
\definecolor{BrBG-11-4}{RGB}{223,194,125}
\definecolor{BrBG-11-F}{RGB}{223,194,125}
\definecolor{BrBG-11-5}{RGB}{246,232,195}
\definecolor{BrBG-11-G}{RGB}{246,232,195}
\definecolor{BrBG-11-6}{RGB}{245,245,245}
\definecolor{BrBG-11-H}{RGB}{245,245,245}
\definecolor{BrBG-11-7}{RGB}{199,234,229}
\definecolor{BrBG-11-I}{RGB}{199,234,229}
\definecolor{BrBG-11-8}{RGB}{128,205,193}
\definecolor{BrBG-11-J}{RGB}{128,205,193}
\definecolor{BrBG-11-9}{RGB}{53,151,143}
\definecolor{BrBG-11-L}{RGB}{53,151,143}
\definecolor{BrBG-11-10}{RGB}{1,102,94}
\definecolor{BrBG-11-N}{RGB}{1,102,94}
\definecolor{BrBG-11-11}{RGB}{0,60,48}
\definecolor{BrBG-11-O}{RGB}{0,60,48}
\definecolor{PRGn-3-1}{RGB}{175,141,195}
\definecolor{PRGn-3-E}{RGB}{175,141,195}
\definecolor{PRGn-3-2}{RGB}{247,247,247}
\definecolor{PRGn-3-H}{RGB}{247,247,247}
\definecolor{PRGn-3-3}{RGB}{127,191,123}
\definecolor{PRGn-3-K}{RGB}{127,191,123}
\definecolor{PRGn-4-1}{RGB}{123,50,148}
\definecolor{PRGn-4-C}{RGB}{123,50,148}
\definecolor{PRGn-4-2}{RGB}{194,165,207}
\definecolor{PRGn-4-F}{RGB}{194,165,207}
\definecolor{PRGn-4-3}{RGB}{166,219,160}
\definecolor{PRGn-4-J}{RGB}{166,219,160}
\definecolor{PRGn-4-4}{RGB}{0,136,55}
\definecolor{PRGn-4-M}{RGB}{0,136,55}
\definecolor{PRGn-5-1}{RGB}{123,50,148}
\definecolor{PRGn-5-C}{RGB}{123,50,148}
\definecolor{PRGn-5-2}{RGB}{194,165,207}
\definecolor{PRGn-5-F}{RGB}{194,165,207}
\definecolor{PRGn-5-3}{RGB}{247,247,247}
\definecolor{PRGn-5-H}{RGB}{247,247,247}
\definecolor{PRGn-5-4}{RGB}{166,219,160}
\definecolor{PRGn-5-J}{RGB}{166,219,160}
\definecolor{PRGn-5-5}{RGB}{0,136,55}
\definecolor{PRGn-5-M}{RGB}{0,136,55}
\definecolor{PRGn-6-1}{RGB}{118,42,131}
\definecolor{PRGn-6-B}{RGB}{118,42,131}
\definecolor{PRGn-6-2}{RGB}{175,141,195}
\definecolor{PRGn-6-E}{RGB}{175,141,195}
\definecolor{PRGn-6-3}{RGB}{231,212,232}
\definecolor{PRGn-6-G}{RGB}{231,212,232}
\definecolor{PRGn-6-4}{RGB}{217,240,211}
\definecolor{PRGn-6-I}{RGB}{217,240,211}
\definecolor{PRGn-6-5}{RGB}{127,191,123}
\definecolor{PRGn-6-K}{RGB}{127,191,123}
\definecolor{PRGn-6-6}{RGB}{27,120,55}
\definecolor{PRGn-6-N}{RGB}{27,120,55}
\definecolor{PRGn-7-1}{RGB}{118,42,131}
\definecolor{PRGn-7-B}{RGB}{118,42,131}
\definecolor{PRGn-7-2}{RGB}{175,141,195}
\definecolor{PRGn-7-E}{RGB}{175,141,195}
\definecolor{PRGn-7-3}{RGB}{231,212,232}
\definecolor{PRGn-7-G}{RGB}{231,212,232}
\definecolor{PRGn-7-4}{RGB}{247,247,247}
\definecolor{PRGn-7-H}{RGB}{247,247,247}
\definecolor{PRGn-7-5}{RGB}{217,240,211}
\definecolor{PRGn-7-I}{RGB}{217,240,211}
\definecolor{PRGn-7-6}{RGB}{127,191,123}
\definecolor{PRGn-7-K}{RGB}{127,191,123}
\definecolor{PRGn-7-7}{RGB}{27,120,55}
\definecolor{PRGn-7-N}{RGB}{27,120,55}
\definecolor{PRGn-8-1}{RGB}{118,42,131}
\definecolor{PRGn-8-B}{RGB}{118,42,131}
\definecolor{PRGn-8-2}{RGB}{153,112,171}
\definecolor{PRGn-8-D}{RGB}{153,112,171}
\definecolor{PRGn-8-3}{RGB}{194,165,207}
\definecolor{PRGn-8-F}{RGB}{194,165,207}
\definecolor{PRGn-8-4}{RGB}{231,212,232}
\definecolor{PRGn-8-G}{RGB}{231,212,232}
\definecolor{PRGn-8-5}{RGB}{217,240,211}
\definecolor{PRGn-8-I}{RGB}{217,240,211}
\definecolor{PRGn-8-6}{RGB}{166,219,160}
\definecolor{PRGn-8-J}{RGB}{166,219,160}
\definecolor{PRGn-8-7}{RGB}{90,174,97}
\definecolor{PRGn-8-L}{RGB}{90,174,97}
\definecolor{PRGn-8-8}{RGB}{27,120,55}
\definecolor{PRGn-8-N}{RGB}{27,120,55}
\definecolor{PRGn-9-1}{RGB}{118,42,131}
\definecolor{PRGn-9-B}{RGB}{118,42,131}
\definecolor{PRGn-9-2}{RGB}{153,112,171}
\definecolor{PRGn-9-D}{RGB}{153,112,171}
\definecolor{PRGn-9-3}{RGB}{194,165,207}
\definecolor{PRGn-9-F}{RGB}{194,165,207}
\definecolor{PRGn-9-4}{RGB}{231,212,232}
\definecolor{PRGn-9-G}{RGB}{231,212,232}
\definecolor{PRGn-9-5}{RGB}{247,247,247}
\definecolor{PRGn-9-H}{RGB}{247,247,247}
\definecolor{PRGn-9-6}{RGB}{217,240,211}
\definecolor{PRGn-9-I}{RGB}{217,240,211}
\definecolor{PRGn-9-7}{RGB}{166,219,160}
\definecolor{PRGn-9-J}{RGB}{166,219,160}
\definecolor{PRGn-9-8}{RGB}{90,174,97}
\definecolor{PRGn-9-L}{RGB}{90,174,97}
\definecolor{PRGn-9-9}{RGB}{27,120,55}
\definecolor{PRGn-9-N}{RGB}{27,120,55}
\definecolor{PRGn-10-1}{RGB}{64,0,75}
\definecolor{PRGn-10-A}{RGB}{64,0,75}
\definecolor{PRGn-10-2}{RGB}{118,42,131}
\definecolor{PRGn-10-B}{RGB}{118,42,131}
\definecolor{PRGn-10-3}{RGB}{153,112,171}
\definecolor{PRGn-10-D}{RGB}{153,112,171}
\definecolor{PRGn-10-4}{RGB}{194,165,207}
\definecolor{PRGn-10-F}{RGB}{194,165,207}
\definecolor{PRGn-10-5}{RGB}{231,212,232}
\definecolor{PRGn-10-G}{RGB}{231,212,232}
\definecolor{PRGn-10-6}{RGB}{217,240,211}
\definecolor{PRGn-10-I}{RGB}{217,240,211}
\definecolor{PRGn-10-7}{RGB}{166,219,160}
\definecolor{PRGn-10-J}{RGB}{166,219,160}
\definecolor{PRGn-10-8}{RGB}{90,174,97}
\definecolor{PRGn-10-L}{RGB}{90,174,97}
\definecolor{PRGn-10-9}{RGB}{27,120,55}
\definecolor{PRGn-10-N}{RGB}{27,120,55}
\definecolor{PRGn-10-10}{RGB}{0,68,27}
\definecolor{PRGn-10-O}{RGB}{0,68,27}
\definecolor{PRGn-11-1}{RGB}{64,0,75}
\definecolor{PRGn-11-A}{RGB}{64,0,75}
\definecolor{PRGn-11-2}{RGB}{118,42,131}
\definecolor{PRGn-11-B}{RGB}{118,42,131}
\definecolor{PRGn-11-3}{RGB}{153,112,171}
\definecolor{PRGn-11-D}{RGB}{153,112,171}
\definecolor{PRGn-11-4}{RGB}{194,165,207}
\definecolor{PRGn-11-F}{RGB}{194,165,207}
\definecolor{PRGn-11-5}{RGB}{231,212,232}
\definecolor{PRGn-11-G}{RGB}{231,212,232}
\definecolor{PRGn-11-6}{RGB}{247,247,247}
\definecolor{PRGn-11-H}{RGB}{247,247,247}
\definecolor{PRGn-11-7}{RGB}{217,240,211}
\definecolor{PRGn-11-I}{RGB}{217,240,211}
\definecolor{PRGn-11-8}{RGB}{166,219,160}
\definecolor{PRGn-11-J}{RGB}{166,219,160}
\definecolor{PRGn-11-9}{RGB}{90,174,97}
\definecolor{PRGn-11-L}{RGB}{90,174,97}
\definecolor{PRGn-11-10}{RGB}{27,120,55}
\definecolor{PRGn-11-N}{RGB}{27,120,55}
\definecolor{PRGn-11-11}{RGB}{0,68,27}
\definecolor{PRGn-11-O}{RGB}{0,68,27}
\definecolor{PiYG-3-1}{RGB}{233,163,201}
\definecolor{PiYG-3-E}{RGB}{233,163,201}
\definecolor{PiYG-3-2}{RGB}{247,247,247}
\definecolor{PiYG-3-H}{RGB}{247,247,247}
\definecolor{PiYG-3-3}{RGB}{161,215,106}
\definecolor{PiYG-3-K}{RGB}{161,215,106}
\definecolor{PiYG-4-1}{RGB}{208,28,139}
\definecolor{PiYG-4-C}{RGB}{208,28,139}
\definecolor{PiYG-4-2}{RGB}{241,182,218}
\definecolor{PiYG-4-F}{RGB}{241,182,218}
\definecolor{PiYG-4-3}{RGB}{184,225,134}
\definecolor{PiYG-4-J}{RGB}{184,225,134}
\definecolor{PiYG-4-4}{RGB}{77,172,38}
\definecolor{PiYG-4-M}{RGB}{77,172,38}
\definecolor{PiYG-5-1}{RGB}{208,28,139}
\definecolor{PiYG-5-C}{RGB}{208,28,139}
\definecolor{PiYG-5-2}{RGB}{241,182,218}
\definecolor{PiYG-5-F}{RGB}{241,182,218}
\definecolor{PiYG-5-3}{RGB}{247,247,247}
\definecolor{PiYG-5-H}{RGB}{247,247,247}
\definecolor{PiYG-5-4}{RGB}{184,225,134}
\definecolor{PiYG-5-J}{RGB}{184,225,134}
\definecolor{PiYG-5-5}{RGB}{77,172,38}
\definecolor{PiYG-5-M}{RGB}{77,172,38}
\definecolor{PiYG-6-1}{RGB}{197,27,125}
\definecolor{PiYG-6-B}{RGB}{197,27,125}
\definecolor{PiYG-6-2}{RGB}{233,163,201}
\definecolor{PiYG-6-E}{RGB}{233,163,201}
\definecolor{PiYG-6-3}{RGB}{253,224,239}
\definecolor{PiYG-6-G}{RGB}{253,224,239}
\definecolor{PiYG-6-4}{RGB}{230,245,208}
\definecolor{PiYG-6-I}{RGB}{230,245,208}
\definecolor{PiYG-6-5}{RGB}{161,215,106}
\definecolor{PiYG-6-K}{RGB}{161,215,106}
\definecolor{PiYG-6-6}{RGB}{77,146,33}
\definecolor{PiYG-6-N}{RGB}{77,146,33}
\definecolor{PiYG-7-1}{RGB}{197,27,125}
\definecolor{PiYG-7-B}{RGB}{197,27,125}
\definecolor{PiYG-7-2}{RGB}{233,163,201}
\definecolor{PiYG-7-E}{RGB}{233,163,201}
\definecolor{PiYG-7-3}{RGB}{253,224,239}
\definecolor{PiYG-7-G}{RGB}{253,224,239}
\definecolor{PiYG-7-4}{RGB}{247,247,247}
\definecolor{PiYG-7-H}{RGB}{247,247,247}
\definecolor{PiYG-7-5}{RGB}{230,245,208}
\definecolor{PiYG-7-I}{RGB}{230,245,208}
\definecolor{PiYG-7-6}{RGB}{161,215,106}
\definecolor{PiYG-7-K}{RGB}{161,215,106}
\definecolor{PiYG-7-7}{RGB}{77,146,33}
\definecolor{PiYG-7-N}{RGB}{77,146,33}
\definecolor{PiYG-8-1}{RGB}{197,27,125}
\definecolor{PiYG-8-B}{RGB}{197,27,125}
\definecolor{PiYG-8-2}{RGB}{222,119,174}
\definecolor{PiYG-8-D}{RGB}{222,119,174}
\definecolor{PiYG-8-3}{RGB}{241,182,218}
\definecolor{PiYG-8-F}{RGB}{241,182,218}
\definecolor{PiYG-8-4}{RGB}{253,224,239}
\definecolor{PiYG-8-G}{RGB}{253,224,239}
\definecolor{PiYG-8-5}{RGB}{230,245,208}
\definecolor{PiYG-8-I}{RGB}{230,245,208}
\definecolor{PiYG-8-6}{RGB}{184,225,134}
\definecolor{PiYG-8-J}{RGB}{184,225,134}
\definecolor{PiYG-8-7}{RGB}{127,188,65}
\definecolor{PiYG-8-L}{RGB}{127,188,65}
\definecolor{PiYG-8-8}{RGB}{77,146,33}
\definecolor{PiYG-8-N}{RGB}{77,146,33}
\definecolor{PiYG-9-1}{RGB}{197,27,125}
\definecolor{PiYG-9-B}{RGB}{197,27,125}
\definecolor{PiYG-9-2}{RGB}{222,119,174}
\definecolor{PiYG-9-D}{RGB}{222,119,174}
\definecolor{PiYG-9-3}{RGB}{241,182,218}
\definecolor{PiYG-9-F}{RGB}{241,182,218}
\definecolor{PiYG-9-4}{RGB}{253,224,239}
\definecolor{PiYG-9-G}{RGB}{253,224,239}
\definecolor{PiYG-9-5}{RGB}{247,247,247}
\definecolor{PiYG-9-H}{RGB}{247,247,247}
\definecolor{PiYG-9-6}{RGB}{230,245,208}
\definecolor{PiYG-9-I}{RGB}{230,245,208}
\definecolor{PiYG-9-7}{RGB}{184,225,134}
\definecolor{PiYG-9-J}{RGB}{184,225,134}
\definecolor{PiYG-9-8}{RGB}{127,188,65}
\definecolor{PiYG-9-L}{RGB}{127,188,65}
\definecolor{PiYG-9-9}{RGB}{77,146,33}
\definecolor{PiYG-9-N}{RGB}{77,146,33}
\definecolor{PiYG-10-1}{RGB}{142,1,82}
\definecolor{PiYG-10-A}{RGB}{142,1,82}
\definecolor{PiYG-10-2}{RGB}{197,27,125}
\definecolor{PiYG-10-B}{RGB}{197,27,125}
\definecolor{PiYG-10-3}{RGB}{222,119,174}
\definecolor{PiYG-10-D}{RGB}{222,119,174}
\definecolor{PiYG-10-4}{RGB}{241,182,218}
\definecolor{PiYG-10-F}{RGB}{241,182,218}
\definecolor{PiYG-10-5}{RGB}{253,224,239}
\definecolor{PiYG-10-G}{RGB}{253,224,239}
\definecolor{PiYG-10-6}{RGB}{230,245,208}
\definecolor{PiYG-10-I}{RGB}{230,245,208}
\definecolor{PiYG-10-7}{RGB}{184,225,134}
\definecolor{PiYG-10-J}{RGB}{184,225,134}
\definecolor{PiYG-10-8}{RGB}{127,188,65}
\definecolor{PiYG-10-L}{RGB}{127,188,65}
\definecolor{PiYG-10-9}{RGB}{77,146,33}
\definecolor{PiYG-10-N}{RGB}{77,146,33}
\definecolor{PiYG-10-10}{RGB}{39,100,25}
\definecolor{PiYG-10-O}{RGB}{39,100,25}
\definecolor{PiYG-11-1}{RGB}{142,1,82}
\definecolor{PiYG-11-A}{RGB}{142,1,82}
\definecolor{PiYG-11-2}{RGB}{197,27,125}
\definecolor{PiYG-11-B}{RGB}{197,27,125}
\definecolor{PiYG-11-3}{RGB}{222,119,174}
\definecolor{PiYG-11-D}{RGB}{222,119,174}
\definecolor{PiYG-11-4}{RGB}{241,182,218}
\definecolor{PiYG-11-F}{RGB}{241,182,218}
\definecolor{PiYG-11-5}{RGB}{253,224,239}
\definecolor{PiYG-11-G}{RGB}{253,224,239}
\definecolor{PiYG-11-6}{RGB}{247,247,247}
\definecolor{PiYG-11-H}{RGB}{247,247,247}
\definecolor{PiYG-11-7}{RGB}{230,245,208}
\definecolor{PiYG-11-I}{RGB}{230,245,208}
\definecolor{PiYG-11-8}{RGB}{184,225,134}
\definecolor{PiYG-11-J}{RGB}{184,225,134}
\definecolor{PiYG-11-9}{RGB}{127,188,65}
\definecolor{PiYG-11-L}{RGB}{127,188,65}
\definecolor{PiYG-11-10}{RGB}{77,146,33}
\definecolor{PiYG-11-N}{RGB}{77,146,33}
\definecolor{PiYG-11-11}{RGB}{39,100,25}
\definecolor{PiYG-11-O}{RGB}{39,100,25}
\definecolor{RdBu-3-1}{RGB}{239,138,98}
\definecolor{RdBu-3-E}{RGB}{239,138,98}
\definecolor{RdBu-3-2}{RGB}{247,247,247}
\definecolor{RdBu-3-H}{RGB}{247,247,247}
\definecolor{RdBu-3-3}{RGB}{103,169,207}
\definecolor{RdBu-3-K}{RGB}{103,169,207}
\definecolor{RdBu-4-1}{RGB}{202,0,32}
\definecolor{RdBu-4-C}{RGB}{202,0,32}
\definecolor{RdBu-4-2}{RGB}{244,165,130}
\definecolor{RdBu-4-F}{RGB}{244,165,130}
\definecolor{RdBu-4-3}{RGB}{146,197,222}
\definecolor{RdBu-4-J}{RGB}{146,197,222}
\definecolor{RdBu-4-4}{RGB}{5,113,176}
\definecolor{RdBu-4-M}{RGB}{5,113,176}
\definecolor{RdBu-5-1}{RGB}{202,0,32}
\definecolor{RdBu-5-C}{RGB}{202,0,32}
\definecolor{RdBu-5-2}{RGB}{244,165,130}
\definecolor{RdBu-5-F}{RGB}{244,165,130}
\definecolor{RdBu-5-3}{RGB}{247,247,247}
\definecolor{RdBu-5-H}{RGB}{247,247,247}
\definecolor{RdBu-5-4}{RGB}{146,197,222}
\definecolor{RdBu-5-J}{RGB}{146,197,222}
\definecolor{RdBu-5-5}{RGB}{5,113,176}
\definecolor{RdBu-5-M}{RGB}{5,113,176}
\definecolor{RdBu-6-1}{RGB}{178,24,43}
\definecolor{RdBu-6-B}{RGB}{178,24,43}
\definecolor{RdBu-6-2}{RGB}{239,138,98}
\definecolor{RdBu-6-E}{RGB}{239,138,98}
\definecolor{RdBu-6-3}{RGB}{253,219,199}
\definecolor{RdBu-6-G}{RGB}{253,219,199}
\definecolor{RdBu-6-4}{RGB}{209,229,240}
\definecolor{RdBu-6-I}{RGB}{209,229,240}
\definecolor{RdBu-6-5}{RGB}{103,169,207}
\definecolor{RdBu-6-K}{RGB}{103,169,207}
\definecolor{RdBu-6-6}{RGB}{33,102,172}
\definecolor{RdBu-6-N}{RGB}{33,102,172}
\definecolor{RdBu-7-1}{RGB}{178,24,43}
\definecolor{RdBu-7-B}{RGB}{178,24,43}
\definecolor{RdBu-7-2}{RGB}{239,138,98}
\definecolor{RdBu-7-E}{RGB}{239,138,98}
\definecolor{RdBu-7-3}{RGB}{253,219,199}
\definecolor{RdBu-7-G}{RGB}{253,219,199}
\definecolor{RdBu-7-4}{RGB}{247,247,247}
\definecolor{RdBu-7-H}{RGB}{247,247,247}
\definecolor{RdBu-7-5}{RGB}{209,229,240}
\definecolor{RdBu-7-I}{RGB}{209,229,240}
\definecolor{RdBu-7-6}{RGB}{103,169,207}
\definecolor{RdBu-7-K}{RGB}{103,169,207}
\definecolor{RdBu-7-7}{RGB}{33,102,172}
\definecolor{RdBu-7-N}{RGB}{33,102,172}
\definecolor{RdBu-8-1}{RGB}{178,24,43}
\definecolor{RdBu-8-B}{RGB}{178,24,43}
\definecolor{RdBu-8-2}{RGB}{214,96,77}
\definecolor{RdBu-8-D}{RGB}{214,96,77}
\definecolor{RdBu-8-3}{RGB}{244,165,130}
\definecolor{RdBu-8-F}{RGB}{244,165,130}
\definecolor{RdBu-8-4}{RGB}{253,219,199}
\definecolor{RdBu-8-G}{RGB}{253,219,199}
\definecolor{RdBu-8-5}{RGB}{209,229,240}
\definecolor{RdBu-8-I}{RGB}{209,229,240}
\definecolor{RdBu-8-6}{RGB}{146,197,222}
\definecolor{RdBu-8-J}{RGB}{146,197,222}
\definecolor{RdBu-8-7}{RGB}{67,147,195}
\definecolor{RdBu-8-L}{RGB}{67,147,195}
\definecolor{RdBu-8-8}{RGB}{33,102,172}
\definecolor{RdBu-8-N}{RGB}{33,102,172}
\definecolor{RdBu-9-1}{RGB}{178,24,43}
\definecolor{RdBu-9-B}{RGB}{178,24,43}
\definecolor{RdBu-9-2}{RGB}{214,96,77}
\definecolor{RdBu-9-D}{RGB}{214,96,77}
\definecolor{RdBu-9-3}{RGB}{244,165,130}
\definecolor{RdBu-9-F}{RGB}{244,165,130}
\definecolor{RdBu-9-4}{RGB}{253,219,199}
\definecolor{RdBu-9-G}{RGB}{253,219,199}
\definecolor{RdBu-9-5}{RGB}{247,247,247}
\definecolor{RdBu-9-H}{RGB}{247,247,247}
\definecolor{RdBu-9-6}{RGB}{209,229,240}
\definecolor{RdBu-9-I}{RGB}{209,229,240}
\definecolor{RdBu-9-7}{RGB}{146,197,222}
\definecolor{RdBu-9-J}{RGB}{146,197,222}
\definecolor{RdBu-9-8}{RGB}{67,147,195}
\definecolor{RdBu-9-L}{RGB}{67,147,195}
\definecolor{RdBu-9-9}{RGB}{33,102,172}
\definecolor{RdBu-9-N}{RGB}{33,102,172}
\definecolor{RdBu-10-1}{RGB}{103,0,31}
\definecolor{RdBu-10-A}{RGB}{103,0,31}
\definecolor{RdBu-10-2}{RGB}{178,24,43}
\definecolor{RdBu-10-B}{RGB}{178,24,43}
\definecolor{RdBu-10-3}{RGB}{214,96,77}
\definecolor{RdBu-10-D}{RGB}{214,96,77}
\definecolor{RdBu-10-4}{RGB}{244,165,130}
\definecolor{RdBu-10-F}{RGB}{244,165,130}
\definecolor{RdBu-10-5}{RGB}{253,219,199}
\definecolor{RdBu-10-G}{RGB}{253,219,199}
\definecolor{RdBu-10-6}{RGB}{209,229,240}
\definecolor{RdBu-10-I}{RGB}{209,229,240}
\definecolor{RdBu-10-7}{RGB}{146,197,222}
\definecolor{RdBu-10-J}{RGB}{146,197,222}
\definecolor{RdBu-10-8}{RGB}{67,147,195}
\definecolor{RdBu-10-L}{RGB}{67,147,195}
\definecolor{RdBu-10-9}{RGB}{33,102,172}
\definecolor{RdBu-10-N}{RGB}{33,102,172}
\definecolor{RdBu-10-10}{RGB}{5,48,97}
\definecolor{RdBu-10-O}{RGB}{5,48,97}
\definecolor{RdBu-11-1}{RGB}{103,0,31}
\definecolor{RdBu-11-A}{RGB}{103,0,31}
\definecolor{RdBu-11-2}{RGB}{178,24,43}
\definecolor{RdBu-11-B}{RGB}{178,24,43}
\definecolor{RdBu-11-3}{RGB}{214,96,77}
\definecolor{RdBu-11-D}{RGB}{214,96,77}
\definecolor{RdBu-11-4}{RGB}{244,165,130}
\definecolor{RdBu-11-F}{RGB}{244,165,130}
\definecolor{RdBu-11-5}{RGB}{253,219,199}
\definecolor{RdBu-11-G}{RGB}{253,219,199}
\definecolor{RdBu-11-6}{RGB}{247,247,247}
\definecolor{RdBu-11-H}{RGB}{247,247,247}
\definecolor{RdBu-11-7}{RGB}{209,229,240}
\definecolor{RdBu-11-I}{RGB}{209,229,240}
\definecolor{RdBu-11-8}{RGB}{146,197,222}
\definecolor{RdBu-11-J}{RGB}{146,197,222}
\definecolor{RdBu-11-9}{RGB}{67,147,195}
\definecolor{RdBu-11-L}{RGB}{67,147,195}
\definecolor{RdBu-11-10}{RGB}{33,102,172}
\definecolor{RdBu-11-N}{RGB}{33,102,172}
\definecolor{RdBu-11-11}{RGB}{5,48,97}
\definecolor{RdBu-11-O}{RGB}{5,48,97}
\definecolor{RdGy-3-1}{RGB}{239,138,98}
\definecolor{RdGy-3-E}{RGB}{239,138,98}
\definecolor{RdGy-3-2}{RGB}{255,255,255}
\definecolor{RdGy-3-H}{RGB}{255,255,255}
\definecolor{RdGy-3-3}{RGB}{153,153,153}
\definecolor{RdGy-3-K}{RGB}{153,153,153}
\definecolor{RdGy-4-1}{RGB}{202,0,32}
\definecolor{RdGy-4-C}{RGB}{202,0,32}
\definecolor{RdGy-4-2}{RGB}{244,165,130}
\definecolor{RdGy-4-F}{RGB}{244,165,130}
\definecolor{RdGy-4-3}{RGB}{186,186,186}
\definecolor{RdGy-4-J}{RGB}{186,186,186}
\definecolor{RdGy-4-4}{RGB}{64,64,64}
\definecolor{RdGy-4-M}{RGB}{64,64,64}
\definecolor{RdGy-5-1}{RGB}{202,0,32}
\definecolor{RdGy-5-C}{RGB}{202,0,32}
\definecolor{RdGy-5-2}{RGB}{244,165,130}
\definecolor{RdGy-5-F}{RGB}{244,165,130}
\definecolor{RdGy-5-3}{RGB}{255,255,255}
\definecolor{RdGy-5-H}{RGB}{255,255,255}
\definecolor{RdGy-5-4}{RGB}{186,186,186}
\definecolor{RdGy-5-J}{RGB}{186,186,186}
\definecolor{RdGy-5-5}{RGB}{64,64,64}
\definecolor{RdGy-5-M}{RGB}{64,64,64}
\definecolor{RdGy-6-1}{RGB}{178,24,43}
\definecolor{RdGy-6-B}{RGB}{178,24,43}
\definecolor{RdGy-6-2}{RGB}{239,138,98}
\definecolor{RdGy-6-E}{RGB}{239,138,98}
\definecolor{RdGy-6-3}{RGB}{253,219,199}
\definecolor{RdGy-6-G}{RGB}{253,219,199}
\definecolor{RdGy-6-4}{RGB}{224,224,224}
\definecolor{RdGy-6-I}{RGB}{224,224,224}
\definecolor{RdGy-6-5}{RGB}{153,153,153}
\definecolor{RdGy-6-K}{RGB}{153,153,153}
\definecolor{RdGy-6-6}{RGB}{77,77,77}
\definecolor{RdGy-6-N}{RGB}{77,77,77}
\definecolor{RdGy-7-1}{RGB}{178,24,43}
\definecolor{RdGy-7-B}{RGB}{178,24,43}
\definecolor{RdGy-7-2}{RGB}{239,138,98}
\definecolor{RdGy-7-E}{RGB}{239,138,98}
\definecolor{RdGy-7-3}{RGB}{253,219,199}
\definecolor{RdGy-7-G}{RGB}{253,219,199}
\definecolor{RdGy-7-4}{RGB}{255,255,255}
\definecolor{RdGy-7-H}{RGB}{255,255,255}
\definecolor{RdGy-7-5}{RGB}{224,224,224}
\definecolor{RdGy-7-I}{RGB}{224,224,224}
\definecolor{RdGy-7-6}{RGB}{153,153,153}
\definecolor{RdGy-7-K}{RGB}{153,153,153}
\definecolor{RdGy-7-7}{RGB}{77,77,77}
\definecolor{RdGy-7-N}{RGB}{77,77,77}
\definecolor{RdGy-8-1}{RGB}{178,24,43}
\definecolor{RdGy-8-B}{RGB}{178,24,43}
\definecolor{RdGy-8-2}{RGB}{214,96,77}
\definecolor{RdGy-8-D}{RGB}{214,96,77}
\definecolor{RdGy-8-3}{RGB}{244,165,130}
\definecolor{RdGy-8-F}{RGB}{244,165,130}
\definecolor{RdGy-8-4}{RGB}{253,219,199}
\definecolor{RdGy-8-G}{RGB}{253,219,199}
\definecolor{RdGy-8-5}{RGB}{224,224,224}
\definecolor{RdGy-8-I}{RGB}{224,224,224}
\definecolor{RdGy-8-6}{RGB}{186,186,186}
\definecolor{RdGy-8-J}{RGB}{186,186,186}
\definecolor{RdGy-8-7}{RGB}{135,135,135}
\definecolor{RdGy-8-L}{RGB}{135,135,135}
\definecolor{RdGy-8-8}{RGB}{77,77,77}
\definecolor{RdGy-8-N}{RGB}{77,77,77}
\definecolor{RdGy-9-1}{RGB}{178,24,43}
\definecolor{RdGy-9-B}{RGB}{178,24,43}
\definecolor{RdGy-9-2}{RGB}{214,96,77}
\definecolor{RdGy-9-D}{RGB}{214,96,77}
\definecolor{RdGy-9-3}{RGB}{244,165,130}
\definecolor{RdGy-9-F}{RGB}{244,165,130}
\definecolor{RdGy-9-4}{RGB}{253,219,199}
\definecolor{RdGy-9-G}{RGB}{253,219,199}
\definecolor{RdGy-9-5}{RGB}{255,255,255}
\definecolor{RdGy-9-H}{RGB}{255,255,255}
\definecolor{RdGy-9-6}{RGB}{224,224,224}
\definecolor{RdGy-9-I}{RGB}{224,224,224}
\definecolor{RdGy-9-7}{RGB}{186,186,186}
\definecolor{RdGy-9-J}{RGB}{186,186,186}
\definecolor{RdGy-9-8}{RGB}{135,135,135}
\definecolor{RdGy-9-L}{RGB}{135,135,135}
\definecolor{RdGy-9-9}{RGB}{77,77,77}
\definecolor{RdGy-9-N}{RGB}{77,77,77}
\definecolor{RdGy-10-1}{RGB}{103,0,31}
\definecolor{RdGy-10-A}{RGB}{103,0,31}
\definecolor{RdGy-10-2}{RGB}{178,24,43}
\definecolor{RdGy-10-B}{RGB}{178,24,43}
\definecolor{RdGy-10-3}{RGB}{214,96,77}
\definecolor{RdGy-10-D}{RGB}{214,96,77}
\definecolor{RdGy-10-4}{RGB}{244,165,130}
\definecolor{RdGy-10-F}{RGB}{244,165,130}
\definecolor{RdGy-10-5}{RGB}{253,219,199}
\definecolor{RdGy-10-G}{RGB}{253,219,199}
\definecolor{RdGy-10-6}{RGB}{224,224,224}
\definecolor{RdGy-10-I}{RGB}{224,224,224}
\definecolor{RdGy-10-7}{RGB}{186,186,186}
\definecolor{RdGy-10-J}{RGB}{186,186,186}
\definecolor{RdGy-10-8}{RGB}{135,135,135}
\definecolor{RdGy-10-L}{RGB}{135,135,135}
\definecolor{RdGy-10-9}{RGB}{77,77,77}
\definecolor{RdGy-10-N}{RGB}{77,77,77}
\definecolor{RdGy-10-10}{RGB}{26,26,26}
\definecolor{RdGy-10-O}{RGB}{26,26,26}
\definecolor{RdGy-11-1}{RGB}{103,0,31}
\definecolor{RdGy-11-A}{RGB}{103,0,31}
\definecolor{RdGy-11-2}{RGB}{178,24,43}
\definecolor{RdGy-11-B}{RGB}{178,24,43}
\definecolor{RdGy-11-3}{RGB}{214,96,77}
\definecolor{RdGy-11-D}{RGB}{214,96,77}
\definecolor{RdGy-11-4}{RGB}{244,165,130}
\definecolor{RdGy-11-F}{RGB}{244,165,130}
\definecolor{RdGy-11-5}{RGB}{253,219,199}
\definecolor{RdGy-11-G}{RGB}{253,219,199}
\definecolor{RdGy-11-6}{RGB}{255,255,255}
\definecolor{RdGy-11-H}{RGB}{255,255,255}
\definecolor{RdGy-11-7}{RGB}{224,224,224}
\definecolor{RdGy-11-I}{RGB}{224,224,224}
\definecolor{RdGy-11-8}{RGB}{186,186,186}
\definecolor{RdGy-11-J}{RGB}{186,186,186}
\definecolor{RdGy-11-9}{RGB}{135,135,135}
\definecolor{RdGy-11-L}{RGB}{135,135,135}
\definecolor{RdGy-11-10}{RGB}{77,77,77}
\definecolor{RdGy-11-N}{RGB}{77,77,77}
\definecolor{RdGy-11-11}{RGB}{26,26,26}
\definecolor{RdGy-11-O}{RGB}{26,26,26}
\definecolor{RdYlBu-3-1}{RGB}{252,141,89}
\definecolor{RdYlBu-3-E}{RGB}{252,141,89}
\definecolor{RdYlBu-3-2}{RGB}{255,255,191}
\definecolor{RdYlBu-3-H}{RGB}{255,255,191}
\definecolor{RdYlBu-3-3}{RGB}{145,191,219}
\definecolor{RdYlBu-3-K}{RGB}{145,191,219}
\definecolor{RdYlBu-4-1}{RGB}{215,25,28}
\definecolor{RdYlBu-4-C}{RGB}{215,25,28}
\definecolor{RdYlBu-4-2}{RGB}{253,174,97}
\definecolor{RdYlBu-4-F}{RGB}{253,174,97}
\definecolor{RdYlBu-4-3}{RGB}{171,217,233}
\definecolor{RdYlBu-4-J}{RGB}{171,217,233}
\definecolor{RdYlBu-4-4}{RGB}{44,123,182}
\definecolor{RdYlBu-4-M}{RGB}{44,123,182}
\definecolor{RdYlBu-5-1}{RGB}{215,25,28}
\definecolor{RdYlBu-5-C}{RGB}{215,25,28}
\definecolor{RdYlBu-5-2}{RGB}{253,174,97}
\definecolor{RdYlBu-5-F}{RGB}{253,174,97}
\definecolor{RdYlBu-5-3}{RGB}{255,255,191}
\definecolor{RdYlBu-5-H}{RGB}{255,255,191}
\definecolor{RdYlBu-5-4}{RGB}{171,217,233}
\definecolor{RdYlBu-5-J}{RGB}{171,217,233}
\definecolor{RdYlBu-5-5}{RGB}{44,123,182}
\definecolor{RdYlBu-5-M}{RGB}{44,123,182}
\definecolor{RdYlBu-6-1}{RGB}{215,48,39}
\definecolor{RdYlBu-6-B}{RGB}{215,48,39}
\definecolor{RdYlBu-6-2}{RGB}{252,141,89}
\definecolor{RdYlBu-6-E}{RGB}{252,141,89}
\definecolor{RdYlBu-6-3}{RGB}{254,224,144}
\definecolor{RdYlBu-6-G}{RGB}{254,224,144}
\definecolor{RdYlBu-6-4}{RGB}{224,243,248}
\definecolor{RdYlBu-6-I}{RGB}{224,243,248}
\definecolor{RdYlBu-6-5}{RGB}{145,191,219}
\definecolor{RdYlBu-6-K}{RGB}{145,191,219}
\definecolor{RdYlBu-6-6}{RGB}{69,117,180}
\definecolor{RdYlBu-6-N}{RGB}{69,117,180}
\definecolor{RdYlBu-7-1}{RGB}{215,48,39}
\definecolor{RdYlBu-7-B}{RGB}{215,48,39}
\definecolor{RdYlBu-7-2}{RGB}{252,141,89}
\definecolor{RdYlBu-7-E}{RGB}{252,141,89}
\definecolor{RdYlBu-7-3}{RGB}{254,224,144}
\definecolor{RdYlBu-7-G}{RGB}{254,224,144}
\definecolor{RdYlBu-7-4}{RGB}{255,255,191}
\definecolor{RdYlBu-7-H}{RGB}{255,255,191}
\definecolor{RdYlBu-7-5}{RGB}{224,243,248}
\definecolor{RdYlBu-7-I}{RGB}{224,243,248}
\definecolor{RdYlBu-7-6}{RGB}{145,191,219}
\definecolor{RdYlBu-7-K}{RGB}{145,191,219}
\definecolor{RdYlBu-7-7}{RGB}{69,117,180}
\definecolor{RdYlBu-7-N}{RGB}{69,117,180}
\definecolor{RdYlBu-8-1}{RGB}{215,48,39}
\definecolor{RdYlBu-8-B}{RGB}{215,48,39}
\definecolor{RdYlBu-8-2}{RGB}{244,109,67}
\definecolor{RdYlBu-8-D}{RGB}{244,109,67}
\definecolor{RdYlBu-8-3}{RGB}{253,174,97}
\definecolor{RdYlBu-8-F}{RGB}{253,174,97}
\definecolor{RdYlBu-8-4}{RGB}{254,224,144}
\definecolor{RdYlBu-8-G}{RGB}{254,224,144}
\definecolor{RdYlBu-8-5}{RGB}{224,243,248}
\definecolor{RdYlBu-8-I}{RGB}{224,243,248}
\definecolor{RdYlBu-8-6}{RGB}{171,217,233}
\definecolor{RdYlBu-8-J}{RGB}{171,217,233}
\definecolor{RdYlBu-8-7}{RGB}{116,173,209}
\definecolor{RdYlBu-8-L}{RGB}{116,173,209}
\definecolor{RdYlBu-8-8}{RGB}{69,117,180}
\definecolor{RdYlBu-8-N}{RGB}{69,117,180}
\definecolor{RdYlBu-9-1}{RGB}{215,48,39}
\definecolor{RdYlBu-9-B}{RGB}{215,48,39}
\definecolor{RdYlBu-9-2}{RGB}{244,109,67}
\definecolor{RdYlBu-9-D}{RGB}{244,109,67}
\definecolor{RdYlBu-9-3}{RGB}{253,174,97}
\definecolor{RdYlBu-9-F}{RGB}{253,174,97}
\definecolor{RdYlBu-9-4}{RGB}{254,224,144}
\definecolor{RdYlBu-9-G}{RGB}{254,224,144}
\definecolor{RdYlBu-9-5}{RGB}{255,255,191}
\definecolor{RdYlBu-9-H}{RGB}{255,255,191}
\definecolor{RdYlBu-9-6}{RGB}{224,243,248}
\definecolor{RdYlBu-9-I}{RGB}{224,243,248}
\definecolor{RdYlBu-9-7}{RGB}{171,217,233}
\definecolor{RdYlBu-9-J}{RGB}{171,217,233}
\definecolor{RdYlBu-9-8}{RGB}{116,173,209}
\definecolor{RdYlBu-9-L}{RGB}{116,173,209}
\definecolor{RdYlBu-9-9}{RGB}{69,117,180}
\definecolor{RdYlBu-9-N}{RGB}{69,117,180}
\definecolor{RdYlBu-10-1}{RGB}{165,0,38}
\definecolor{RdYlBu-10-A}{RGB}{165,0,38}
\definecolor{RdYlBu-10-2}{RGB}{215,48,39}
\definecolor{RdYlBu-10-B}{RGB}{215,48,39}
\definecolor{RdYlBu-10-3}{RGB}{244,109,67}
\definecolor{RdYlBu-10-D}{RGB}{244,109,67}
\definecolor{RdYlBu-10-4}{RGB}{253,174,97}
\definecolor{RdYlBu-10-F}{RGB}{253,174,97}
\definecolor{RdYlBu-10-5}{RGB}{254,224,144}
\definecolor{RdYlBu-10-G}{RGB}{254,224,144}
\definecolor{RdYlBu-10-6}{RGB}{224,243,248}
\definecolor{RdYlBu-10-I}{RGB}{224,243,248}
\definecolor{RdYlBu-10-7}{RGB}{171,217,233}
\definecolor{RdYlBu-10-J}{RGB}{171,217,233}
\definecolor{RdYlBu-10-8}{RGB}{116,173,209}
\definecolor{RdYlBu-10-L}{RGB}{116,173,209}
\definecolor{RdYlBu-10-9}{RGB}{69,117,180}
\definecolor{RdYlBu-10-N}{RGB}{69,117,180}
\definecolor{RdYlBu-10-10}{RGB}{49,54,149}
\definecolor{RdYlBu-10-O}{RGB}{49,54,149}
\definecolor{RdYlBu-11-1}{RGB}{165,0,38}
\definecolor{RdYlBu-11-A}{RGB}{165,0,38}
\definecolor{RdYlBu-11-2}{RGB}{215,48,39}
\definecolor{RdYlBu-11-B}{RGB}{215,48,39}
\definecolor{RdYlBu-11-3}{RGB}{244,109,67}
\definecolor{RdYlBu-11-D}{RGB}{244,109,67}
\definecolor{RdYlBu-11-4}{RGB}{253,174,97}
\definecolor{RdYlBu-11-F}{RGB}{253,174,97}
\definecolor{RdYlBu-11-5}{RGB}{254,224,144}
\definecolor{RdYlBu-11-G}{RGB}{254,224,144}
\definecolor{RdYlBu-11-6}{RGB}{255,255,191}
\definecolor{RdYlBu-11-H}{RGB}{255,255,191}
\definecolor{RdYlBu-11-7}{RGB}{224,243,248}
\definecolor{RdYlBu-11-I}{RGB}{224,243,248}
\definecolor{RdYlBu-11-8}{RGB}{171,217,233}
\definecolor{RdYlBu-11-J}{RGB}{171,217,233}
\definecolor{RdYlBu-11-9}{RGB}{116,173,209}
\definecolor{RdYlBu-11-L}{RGB}{116,173,209}
\definecolor{RdYlBu-11-10}{RGB}{69,117,180}
\definecolor{RdYlBu-11-N}{RGB}{69,117,180}
\definecolor{RdYlBu-11-11}{RGB}{49,54,149}
\definecolor{RdYlBu-11-O}{RGB}{49,54,149}
\definecolor{Spectral-3-1}{RGB}{252,141,89}
\definecolor{Spectral-3-E}{RGB}{252,141,89}
\definecolor{Spectral-3-2}{RGB}{255,255,191}
\definecolor{Spectral-3-H}{RGB}{255,255,191}
\definecolor{Spectral-3-3}{RGB}{153,213,148}
\definecolor{Spectral-3-K}{RGB}{153,213,148}
\definecolor{Spectral-4-1}{RGB}{215,25,28}
\definecolor{Spectral-4-C}{RGB}{215,25,28}
\definecolor{Spectral-4-2}{RGB}{253,174,97}
\definecolor{Spectral-4-F}{RGB}{253,174,97}
\definecolor{Spectral-4-3}{RGB}{171,221,164}
\definecolor{Spectral-4-J}{RGB}{171,221,164}
\definecolor{Spectral-4-4}{RGB}{43,131,186}
\definecolor{Spectral-4-M}{RGB}{43,131,186}
\definecolor{Spectral-5-1}{RGB}{215,25,28}
\definecolor{Spectral-5-C}{RGB}{215,25,28}
\definecolor{Spectral-5-2}{RGB}{253,174,97}
\definecolor{Spectral-5-F}{RGB}{253,174,97}
\definecolor{Spectral-5-3}{RGB}{255,255,191}
\definecolor{Spectral-5-H}{RGB}{255,255,191}
\definecolor{Spectral-5-4}{RGB}{171,221,164}
\definecolor{Spectral-5-J}{RGB}{171,221,164}
\definecolor{Spectral-5-5}{RGB}{43,131,186}
\definecolor{Spectral-5-M}{RGB}{43,131,186}
\definecolor{Spectral-6-1}{RGB}{213,62,79}
\definecolor{Spectral-6-B}{RGB}{213,62,79}
\definecolor{Spectral-6-2}{RGB}{252,141,89}
\definecolor{Spectral-6-E}{RGB}{252,141,89}
\definecolor{Spectral-6-3}{RGB}{254,224,139}
\definecolor{Spectral-6-G}{RGB}{254,224,139}
\definecolor{Spectral-6-4}{RGB}{230,245,152}
\definecolor{Spectral-6-I}{RGB}{230,245,152}
\definecolor{Spectral-6-5}{RGB}{153,213,148}
\definecolor{Spectral-6-K}{RGB}{153,213,148}
\definecolor{Spectral-6-6}{RGB}{50,136,189}
\definecolor{Spectral-6-N}{RGB}{50,136,189}
\definecolor{Spectral-7-1}{RGB}{213,62,79}
\definecolor{Spectral-7-B}{RGB}{213,62,79}
\definecolor{Spectral-7-2}{RGB}{252,141,89}
\definecolor{Spectral-7-E}{RGB}{252,141,89}
\definecolor{Spectral-7-3}{RGB}{254,224,139}
\definecolor{Spectral-7-G}{RGB}{254,224,139}
\definecolor{Spectral-7-4}{RGB}{255,255,191}
\definecolor{Spectral-7-H}{RGB}{255,255,191}
\definecolor{Spectral-7-5}{RGB}{230,245,152}
\definecolor{Spectral-7-I}{RGB}{230,245,152}
\definecolor{Spectral-7-6}{RGB}{153,213,148}
\definecolor{Spectral-7-K}{RGB}{153,213,148}
\definecolor{Spectral-7-7}{RGB}{50,136,189}
\definecolor{Spectral-7-N}{RGB}{50,136,189}
\definecolor{Spectral-8-1}{RGB}{213,62,79}
\definecolor{Spectral-8-B}{RGB}{213,62,79}
\definecolor{Spectral-8-2}{RGB}{244,109,67}
\definecolor{Spectral-8-D}{RGB}{244,109,67}
\definecolor{Spectral-8-3}{RGB}{253,174,97}
\definecolor{Spectral-8-F}{RGB}{253,174,97}
\definecolor{Spectral-8-4}{RGB}{254,224,139}
\definecolor{Spectral-8-G}{RGB}{254,224,139}
\definecolor{Spectral-8-5}{RGB}{230,245,152}
\definecolor{Spectral-8-I}{RGB}{230,245,152}
\definecolor{Spectral-8-6}{RGB}{171,221,164}
\definecolor{Spectral-8-J}{RGB}{171,221,164}
\definecolor{Spectral-8-7}{RGB}{102,194,165}
\definecolor{Spectral-8-L}{RGB}{102,194,165}
\definecolor{Spectral-8-8}{RGB}{50,136,189}
\definecolor{Spectral-8-N}{RGB}{50,136,189}
\definecolor{Spectral-9-1}{RGB}{213,62,79}
\definecolor{Spectral-9-B}{RGB}{213,62,79}
\definecolor{Spectral-9-2}{RGB}{244,109,67}
\definecolor{Spectral-9-D}{RGB}{244,109,67}
\definecolor{Spectral-9-3}{RGB}{253,174,97}
\definecolor{Spectral-9-F}{RGB}{253,174,97}
\definecolor{Spectral-9-4}{RGB}{254,224,139}
\definecolor{Spectral-9-G}{RGB}{254,224,139}
\definecolor{Spectral-9-5}{RGB}{255,255,191}
\definecolor{Spectral-9-H}{RGB}{255,255,191}
\definecolor{Spectral-9-6}{RGB}{230,245,152}
\definecolor{Spectral-9-I}{RGB}{230,245,152}
\definecolor{Spectral-9-7}{RGB}{171,221,164}
\definecolor{Spectral-9-J}{RGB}{171,221,164}
\definecolor{Spectral-9-8}{RGB}{102,194,165}
\definecolor{Spectral-9-L}{RGB}{102,194,165}
\definecolor{Spectral-9-9}{RGB}{50,136,189}
\definecolor{Spectral-9-N}{RGB}{50,136,189}
\definecolor{Spectral-10-1}{RGB}{158,1,66}
\definecolor{Spectral-10-A}{RGB}{158,1,66}
\definecolor{Spectral-10-2}{RGB}{213,62,79}
\definecolor{Spectral-10-B}{RGB}{213,62,79}
\definecolor{Spectral-10-3}{RGB}{244,109,67}
\definecolor{Spectral-10-D}{RGB}{244,109,67}
\definecolor{Spectral-10-4}{RGB}{253,174,97}
\definecolor{Spectral-10-F}{RGB}{253,174,97}
\definecolor{Spectral-10-5}{RGB}{254,224,139}
\definecolor{Spectral-10-G}{RGB}{254,224,139}
\definecolor{Spectral-10-6}{RGB}{230,245,152}
\definecolor{Spectral-10-I}{RGB}{230,245,152}
\definecolor{Spectral-10-7}{RGB}{171,221,164}
\definecolor{Spectral-10-J}{RGB}{171,221,164}
\definecolor{Spectral-10-8}{RGB}{102,194,165}
\definecolor{Spectral-10-L}{RGB}{102,194,165}
\definecolor{Spectral-10-9}{RGB}{50,136,189}
\definecolor{Spectral-10-N}{RGB}{50,136,189}
\definecolor{Spectral-10-10}{RGB}{94,79,162}
\definecolor{Spectral-10-O}{RGB}{94,79,162}
\definecolor{Spectral-11-1}{RGB}{158,1,66}
\definecolor{Spectral-11-A}{RGB}{158,1,66}
\definecolor{Spectral-11-2}{RGB}{213,62,79}
\definecolor{Spectral-11-B}{RGB}{213,62,79}
\definecolor{Spectral-11-3}{RGB}{244,109,67}
\definecolor{Spectral-11-D}{RGB}{244,109,67}
\definecolor{Spectral-11-4}{RGB}{253,174,97}
\definecolor{Spectral-11-F}{RGB}{253,174,97}
\definecolor{Spectral-11-5}{RGB}{254,224,139}
\definecolor{Spectral-11-G}{RGB}{254,224,139}
\definecolor{Spectral-11-6}{RGB}{255,255,191}
\definecolor{Spectral-11-H}{RGB}{255,255,191}
\definecolor{Spectral-11-7}{RGB}{230,245,152}
\definecolor{Spectral-11-I}{RGB}{230,245,152}
\definecolor{Spectral-11-8}{RGB}{171,221,164}
\definecolor{Spectral-11-J}{RGB}{171,221,164}
\definecolor{Spectral-11-9}{RGB}{102,194,165}
\definecolor{Spectral-11-L}{RGB}{102,194,165}
\definecolor{Spectral-11-10}{RGB}{50,136,189}
\definecolor{Spectral-11-N}{RGB}{50,136,189}
\definecolor{Spectral-11-11}{RGB}{94,79,162}
\definecolor{Spectral-11-O}{RGB}{94,79,162}
\definecolor{RdYlGn-3-1}{RGB}{252,141,89}
\definecolor{RdYlGn-3-E}{RGB}{252,141,89}
\definecolor{RdYlGn-3-2}{RGB}{255,255,191}
\definecolor{RdYlGn-3-H}{RGB}{255,255,191}
\definecolor{RdYlGn-3-3}{RGB}{145,207,96}
\definecolor{RdYlGn-3-K}{RGB}{145,207,96}
\definecolor{RdYlGn-4-1}{RGB}{215,25,28}
\definecolor{RdYlGn-4-C}{RGB}{215,25,28}
\definecolor{RdYlGn-4-2}{RGB}{253,174,97}
\definecolor{RdYlGn-4-F}{RGB}{253,174,97}
\definecolor{RdYlGn-4-3}{RGB}{166,217,106}
\definecolor{RdYlGn-4-J}{RGB}{166,217,106}
\definecolor{RdYlGn-4-4}{RGB}{26,150,65}
\definecolor{RdYlGn-4-M}{RGB}{26,150,65}
\definecolor{RdYlGn-5-1}{RGB}{215,25,28}
\definecolor{RdYlGn-5-C}{RGB}{215,25,28}
\definecolor{RdYlGn-5-2}{RGB}{253,174,97}
\definecolor{RdYlGn-5-F}{RGB}{253,174,97}
\definecolor{RdYlGn-5-3}{RGB}{255,255,191}
\definecolor{RdYlGn-5-H}{RGB}{255,255,191}
\definecolor{RdYlGn-5-4}{RGB}{166,217,106}
\definecolor{RdYlGn-5-J}{RGB}{166,217,106}
\definecolor{RdYlGn-5-5}{RGB}{26,150,65}
\definecolor{RdYlGn-5-M}{RGB}{26,150,65}
\definecolor{RdYlGn-6-1}{RGB}{215,48,39}
\definecolor{RdYlGn-6-B}{RGB}{215,48,39}
\definecolor{RdYlGn-6-2}{RGB}{252,141,89}
\definecolor{RdYlGn-6-E}{RGB}{252,141,89}
\definecolor{RdYlGn-6-3}{RGB}{254,224,139}
\definecolor{RdYlGn-6-G}{RGB}{254,224,139}
\definecolor{RdYlGn-6-4}{RGB}{217,239,139}
\definecolor{RdYlGn-6-I}{RGB}{217,239,139}
\definecolor{RdYlGn-6-5}{RGB}{145,207,96}
\definecolor{RdYlGn-6-K}{RGB}{145,207,96}
\definecolor{RdYlGn-6-6}{RGB}{26,152,80}
\definecolor{RdYlGn-6-N}{RGB}{26,152,80}
\definecolor{RdYlGn-7-1}{RGB}{215,48,39}
\definecolor{RdYlGn-7-B}{RGB}{215,48,39}
\definecolor{RdYlGn-7-2}{RGB}{252,141,89}
\definecolor{RdYlGn-7-E}{RGB}{252,141,89}
\definecolor{RdYlGn-7-3}{RGB}{254,224,139}
\definecolor{RdYlGn-7-G}{RGB}{254,224,139}
\definecolor{RdYlGn-7-4}{RGB}{255,255,191}
\definecolor{RdYlGn-7-H}{RGB}{255,255,191}
\definecolor{RdYlGn-7-5}{RGB}{217,239,139}
\definecolor{RdYlGn-7-I}{RGB}{217,239,139}
\definecolor{RdYlGn-7-6}{RGB}{145,207,96}
\definecolor{RdYlGn-7-K}{RGB}{145,207,96}
\definecolor{RdYlGn-7-7}{RGB}{26,152,80}
\definecolor{RdYlGn-7-N}{RGB}{26,152,80}
\definecolor{RdYlGn-8-1}{RGB}{215,48,39}
\definecolor{RdYlGn-8-B}{RGB}{215,48,39}
\definecolor{RdYlGn-8-2}{RGB}{244,109,67}
\definecolor{RdYlGn-8-D}{RGB}{244,109,67}
\definecolor{RdYlGn-8-3}{RGB}{253,174,97}
\definecolor{RdYlGn-8-F}{RGB}{253,174,97}
\definecolor{RdYlGn-8-4}{RGB}{254,224,139}
\definecolor{RdYlGn-8-G}{RGB}{254,224,139}
\definecolor{RdYlGn-8-5}{RGB}{217,239,139}
\definecolor{RdYlGn-8-I}{RGB}{217,239,139}
\definecolor{RdYlGn-8-6}{RGB}{166,217,106}
\definecolor{RdYlGn-8-J}{RGB}{166,217,106}
\definecolor{RdYlGn-8-7}{RGB}{102,189,99}
\definecolor{RdYlGn-8-L}{RGB}{102,189,99}
\definecolor{RdYlGn-8-8}{RGB}{26,152,80}
\definecolor{RdYlGn-8-N}{RGB}{26,152,80}
\definecolor{RdYlGn-9-1}{RGB}{215,48,39}
\definecolor{RdYlGn-9-B}{RGB}{215,48,39}
\definecolor{RdYlGn-9-2}{RGB}{244,109,67}
\definecolor{RdYlGn-9-D}{RGB}{244,109,67}
\definecolor{RdYlGn-9-3}{RGB}{253,174,97}
\definecolor{RdYlGn-9-F}{RGB}{253,174,97}
\definecolor{RdYlGn-9-4}{RGB}{254,224,139}
\definecolor{RdYlGn-9-G}{RGB}{254,224,139}
\definecolor{RdYlGn-9-5}{RGB}{255,255,191}
\definecolor{RdYlGn-9-H}{RGB}{255,255,191}
\definecolor{RdYlGn-9-6}{RGB}{217,239,139}
\definecolor{RdYlGn-9-I}{RGB}{217,239,139}
\definecolor{RdYlGn-9-7}{RGB}{166,217,106}
\definecolor{RdYlGn-9-J}{RGB}{166,217,106}
\definecolor{RdYlGn-9-8}{RGB}{102,189,99}
\definecolor{RdYlGn-9-L}{RGB}{102,189,99}
\definecolor{RdYlGn-9-9}{RGB}{26,152,80}
\definecolor{RdYlGn-9-N}{RGB}{26,152,80}
\definecolor{RdYlGn-10-1}{RGB}{165,0,38}
\definecolor{RdYlGn-10-A}{RGB}{165,0,38}
\definecolor{RdYlGn-10-2}{RGB}{215,48,39}
\definecolor{RdYlGn-10-B}{RGB}{215,48,39}
\definecolor{RdYlGn-10-3}{RGB}{244,109,67}
\definecolor{RdYlGn-10-D}{RGB}{244,109,67}
\definecolor{RdYlGn-10-4}{RGB}{253,174,97}
\definecolor{RdYlGn-10-F}{RGB}{253,174,97}
\definecolor{RdYlGn-10-5}{RGB}{254,224,139}
\definecolor{RdYlGn-10-G}{RGB}{254,224,139}
\definecolor{RdYlGn-10-6}{RGB}{217,239,139}
\definecolor{RdYlGn-10-I}{RGB}{217,239,139}
\definecolor{RdYlGn-10-7}{RGB}{166,217,106}
\definecolor{RdYlGn-10-J}{RGB}{166,217,106}
\definecolor{RdYlGn-10-8}{RGB}{102,189,99}
\definecolor{RdYlGn-10-L}{RGB}{102,189,99}
\definecolor{RdYlGn-10-9}{RGB}{26,152,80}
\definecolor{RdYlGn-10-N}{RGB}{26,152,80}
\definecolor{RdYlGn-10-10}{RGB}{0,104,55}
\definecolor{RdYlGn-10-O}{RGB}{0,104,55}
\definecolor{RdYlGn-11-1}{RGB}{165,0,38}
\definecolor{RdYlGn-11-A}{RGB}{165,0,38}
\definecolor{RdYlGn-11-2}{RGB}{215,48,39}
\definecolor{RdYlGn-11-B}{RGB}{215,48,39}
\definecolor{RdYlGn-11-3}{RGB}{244,109,67}
\definecolor{RdYlGn-11-D}{RGB}{244,109,67}
\definecolor{RdYlGn-11-4}{RGB}{253,174,97}
\definecolor{RdYlGn-11-F}{RGB}{253,174,97}
\definecolor{RdYlGn-11-5}{RGB}{254,224,139}
\definecolor{RdYlGn-11-G}{RGB}{254,224,139}
\definecolor{RdYlGn-11-6}{RGB}{255,255,191}
\definecolor{RdYlGn-11-H}{RGB}{255,255,191}
\definecolor{RdYlGn-11-7}{RGB}{217,239,139}
\definecolor{RdYlGn-11-I}{RGB}{217,239,139}
\definecolor{RdYlGn-11-8}{RGB}{166,217,106}
\definecolor{RdYlGn-11-J}{RGB}{166,217,106}
\definecolor{RdYlGn-11-9}{RGB}{102,189,99}
\definecolor{RdYlGn-11-L}{RGB}{102,189,99}
\definecolor{RdYlGn-11-10}{RGB}{26,152,80}
\definecolor{RdYlGn-11-N}{RGB}{26,152,80}
\definecolor{RdYlGn-11-11}{RGB}{0,104,55}
\definecolor{RdYlGn-11-O}{RGB}{0,104,55}
\definecolor{Set3-3-1}{RGB}{141,211,199}
\definecolor{Set3-3-A}{RGB}{141,211,199}
\definecolor{Set3-3-2}{RGB}{255,255,179}
\definecolor{Set3-3-B}{RGB}{255,255,179}
\definecolor{Set3-3-3}{RGB}{190,186,218}
\definecolor{Set3-3-C}{RGB}{190,186,218}
\definecolor{Set3-4-1}{RGB}{141,211,199}
\definecolor{Set3-4-A}{RGB}{141,211,199}
\definecolor{Set3-4-2}{RGB}{255,255,179}
\definecolor{Set3-4-B}{RGB}{255,255,179}
\definecolor{Set3-4-3}{RGB}{190,186,218}
\definecolor{Set3-4-C}{RGB}{190,186,218}
\definecolor{Set3-4-4}{RGB}{251,128,114}
\definecolor{Set3-4-D}{RGB}{251,128,114}
\definecolor{Set3-5-1}{RGB}{141,211,199}
\definecolor{Set3-5-A}{RGB}{141,211,199}
\definecolor{Set3-5-2}{RGB}{255,255,179}
\definecolor{Set3-5-B}{RGB}{255,255,179}
\definecolor{Set3-5-3}{RGB}{190,186,218}
\definecolor{Set3-5-C}{RGB}{190,186,218}
\definecolor{Set3-5-4}{RGB}{251,128,114}
\definecolor{Set3-5-D}{RGB}{251,128,114}
\definecolor{Set3-5-5}{RGB}{128,177,211}
\definecolor{Set3-5-E}{RGB}{128,177,211}
\definecolor{Set3-6-1}{RGB}{141,211,199}
\definecolor{Set3-6-A}{RGB}{141,211,199}
\definecolor{Set3-6-2}{RGB}{255,255,179}
\definecolor{Set3-6-B}{RGB}{255,255,179}
\definecolor{Set3-6-3}{RGB}{190,186,218}
\definecolor{Set3-6-C}{RGB}{190,186,218}
\definecolor{Set3-6-4}{RGB}{251,128,114}
\definecolor{Set3-6-D}{RGB}{251,128,114}
\definecolor{Set3-6-5}{RGB}{128,177,211}
\definecolor{Set3-6-E}{RGB}{128,177,211}
\definecolor{Set3-6-6}{RGB}{253,180,98}
\definecolor{Set3-6-F}{RGB}{253,180,98}
\definecolor{Set3-7-1}{RGB}{141,211,199}
\definecolor{Set3-7-A}{RGB}{141,211,199}
\definecolor{Set3-7-2}{RGB}{255,255,179}
\definecolor{Set3-7-B}{RGB}{255,255,179}
\definecolor{Set3-7-3}{RGB}{190,186,218}
\definecolor{Set3-7-C}{RGB}{190,186,218}
\definecolor{Set3-7-4}{RGB}{251,128,114}
\definecolor{Set3-7-D}{RGB}{251,128,114}
\definecolor{Set3-7-5}{RGB}{128,177,211}
\definecolor{Set3-7-E}{RGB}{128,177,211}
\definecolor{Set3-7-6}{RGB}{253,180,98}
\definecolor{Set3-7-F}{RGB}{253,180,98}
\definecolor{Set3-7-7}{RGB}{179,222,105}
\definecolor{Set3-7-G}{RGB}{179,222,105}
\definecolor{Set3-8-1}{RGB}{141,211,199}
\definecolor{Set3-8-A}{RGB}{141,211,199}
\definecolor{Set3-8-2}{RGB}{255,255,179}
\definecolor{Set3-8-B}{RGB}{255,255,179}
\definecolor{Set3-8-3}{RGB}{190,186,218}
\definecolor{Set3-8-C}{RGB}{190,186,218}
\definecolor{Set3-8-4}{RGB}{251,128,114}
\definecolor{Set3-8-D}{RGB}{251,128,114}
\definecolor{Set3-8-5}{RGB}{128,177,211}
\definecolor{Set3-8-E}{RGB}{128,177,211}
\definecolor{Set3-8-6}{RGB}{253,180,98}
\definecolor{Set3-8-F}{RGB}{253,180,98}
\definecolor{Set3-8-7}{RGB}{179,222,105}
\definecolor{Set3-8-G}{RGB}{179,222,105}
\definecolor{Set3-8-8}{RGB}{252,205,229}
\definecolor{Set3-8-H}{RGB}{252,205,229}
\definecolor{Set3-9-1}{RGB}{141,211,199}
\definecolor{Set3-9-A}{RGB}{141,211,199}
\definecolor{Set3-9-2}{RGB}{255,255,179}
\definecolor{Set3-9-B}{RGB}{255,255,179}
\definecolor{Set3-9-3}{RGB}{190,186,218}
\definecolor{Set3-9-C}{RGB}{190,186,218}
\definecolor{Set3-9-4}{RGB}{251,128,114}
\definecolor{Set3-9-D}{RGB}{251,128,114}
\definecolor{Set3-9-5}{RGB}{128,177,211}
\definecolor{Set3-9-E}{RGB}{128,177,211}
\definecolor{Set3-9-6}{RGB}{253,180,98}
\definecolor{Set3-9-F}{RGB}{253,180,98}
\definecolor{Set3-9-7}{RGB}{179,222,105}
\definecolor{Set3-9-G}{RGB}{179,222,105}
\definecolor{Set3-9-8}{RGB}{252,205,229}
\definecolor{Set3-9-H}{RGB}{252,205,229}
\definecolor{Set3-9-9}{RGB}{217,217,217}
\definecolor{Set3-9-I}{RGB}{217,217,217}
\definecolor{Set3-10-1}{RGB}{141,211,199}
\definecolor{Set3-10-A}{RGB}{141,211,199}
\definecolor{Set3-10-2}{RGB}{255,255,179}
\definecolor{Set3-10-B}{RGB}{255,255,179}
\definecolor{Set3-10-3}{RGB}{190,186,218}
\definecolor{Set3-10-C}{RGB}{190,186,218}
\definecolor{Set3-10-4}{RGB}{251,128,114}
\definecolor{Set3-10-D}{RGB}{251,128,114}
\definecolor{Set3-10-5}{RGB}{128,177,211}
\definecolor{Set3-10-E}{RGB}{128,177,211}
\definecolor{Set3-10-6}{RGB}{253,180,98}
\definecolor{Set3-10-F}{RGB}{253,180,98}
\definecolor{Set3-10-7}{RGB}{179,222,105}
\definecolor{Set3-10-G}{RGB}{179,222,105}
\definecolor{Set3-10-8}{RGB}{252,205,229}
\definecolor{Set3-10-H}{RGB}{252,205,229}
\definecolor{Set3-10-9}{RGB}{217,217,217}
\definecolor{Set3-10-I}{RGB}{217,217,217}
\definecolor{Set3-10-10}{RGB}{188,128,189}
\definecolor{Set3-10-J}{RGB}{188,128,189}
\definecolor{Set3-11-1}{RGB}{141,211,199}
\definecolor{Set3-11-A}{RGB}{141,211,199}
\definecolor{Set3-11-2}{RGB}{255,255,179}
\definecolor{Set3-11-B}{RGB}{255,255,179}
\definecolor{Set3-11-3}{RGB}{190,186,218}
\definecolor{Set3-11-C}{RGB}{190,186,218}
\definecolor{Set3-11-4}{RGB}{251,128,114}
\definecolor{Set3-11-D}{RGB}{251,128,114}
\definecolor{Set3-11-5}{RGB}{128,177,211}
\definecolor{Set3-11-E}{RGB}{128,177,211}
\definecolor{Set3-11-6}{RGB}{253,180,98}
\definecolor{Set3-11-F}{RGB}{253,180,98}
\definecolor{Set3-11-7}{RGB}{179,222,105}
\definecolor{Set3-11-G}{RGB}{179,222,105}
\definecolor{Set3-11-8}{RGB}{252,205,229}
\definecolor{Set3-11-H}{RGB}{252,205,229}
\definecolor{Set3-11-9}{RGB}{217,217,217}
\definecolor{Set3-11-I}{RGB}{217,217,217}
\definecolor{Set3-11-10}{RGB}{188,128,189}
\definecolor{Set3-11-J}{RGB}{188,128,189}
\definecolor{Set3-11-11}{RGB}{204,235,197}
\definecolor{Set3-11-K}{RGB}{204,235,197}
\definecolor{Set3-12-1}{RGB}{141,211,199}
\definecolor{Set3-12-A}{RGB}{141,211,199}
\definecolor{Set3-12-2}{RGB}{255,255,179}
\definecolor{Set3-12-B}{RGB}{255,255,179}
\definecolor{Set3-12-3}{RGB}{190,186,218}
\definecolor{Set3-12-C}{RGB}{190,186,218}
\definecolor{Set3-12-4}{RGB}{251,128,114}
\definecolor{Set3-12-D}{RGB}{251,128,114}
\definecolor{Set3-12-5}{RGB}{128,177,211}
\definecolor{Set3-12-E}{RGB}{128,177,211}
\definecolor{Set3-12-6}{RGB}{253,180,98}
\definecolor{Set3-12-F}{RGB}{253,180,98}
\definecolor{Set3-12-7}{RGB}{179,222,105}
\definecolor{Set3-12-G}{RGB}{179,222,105}
\definecolor{Set3-12-8}{RGB}{252,205,229}
\definecolor{Set3-12-H}{RGB}{252,205,229}
\definecolor{Set3-12-9}{RGB}{217,217,217}
\definecolor{Set3-12-I}{RGB}{217,217,217}
\definecolor{Set3-12-10}{RGB}{188,128,189}
\definecolor{Set3-12-J}{RGB}{188,128,189}
\definecolor{Set3-12-11}{RGB}{204,235,197}
\definecolor{Set3-12-K}{RGB}{204,235,197}
\definecolor{Set3-12-12}{RGB}{255,237,111}
\definecolor{Set3-12-L}{RGB}{255,237,111}
\definecolor{Pastel1-3-1}{RGB}{251,180,174}
\definecolor{Pastel1-3-A}{RGB}{251,180,174}
\definecolor{Pastel1-3-2}{RGB}{179,205,227}
\definecolor{Pastel1-3-B}{RGB}{179,205,227}
\definecolor{Pastel1-3-3}{RGB}{204,235,197}
\definecolor{Pastel1-3-C}{RGB}{204,235,197}
\definecolor{Pastel1-4-1}{RGB}{251,180,174}
\definecolor{Pastel1-4-A}{RGB}{251,180,174}
\definecolor{Pastel1-4-2}{RGB}{179,205,227}
\definecolor{Pastel1-4-B}{RGB}{179,205,227}
\definecolor{Pastel1-4-3}{RGB}{204,235,197}
\definecolor{Pastel1-4-C}{RGB}{204,235,197}
\definecolor{Pastel1-4-4}{RGB}{222,203,228}
\definecolor{Pastel1-4-D}{RGB}{222,203,228}
\definecolor{Pastel1-5-1}{RGB}{251,180,174}
\definecolor{Pastel1-5-A}{RGB}{251,180,174}
\definecolor{Pastel1-5-2}{RGB}{179,205,227}
\definecolor{Pastel1-5-B}{RGB}{179,205,227}
\definecolor{Pastel1-5-3}{RGB}{204,235,197}
\definecolor{Pastel1-5-C}{RGB}{204,235,197}
\definecolor{Pastel1-5-4}{RGB}{222,203,228}
\definecolor{Pastel1-5-D}{RGB}{222,203,228}
\definecolor{Pastel1-5-5}{RGB}{254,217,166}
\definecolor{Pastel1-5-E}{RGB}{254,217,166}
\definecolor{Pastel1-6-1}{RGB}{251,180,174}
\definecolor{Pastel1-6-A}{RGB}{251,180,174}
\definecolor{Pastel1-6-2}{RGB}{179,205,227}
\definecolor{Pastel1-6-B}{RGB}{179,205,227}
\definecolor{Pastel1-6-3}{RGB}{204,235,197}
\definecolor{Pastel1-6-C}{RGB}{204,235,197}
\definecolor{Pastel1-6-4}{RGB}{222,203,228}
\definecolor{Pastel1-6-D}{RGB}{222,203,228}
\definecolor{Pastel1-6-5}{RGB}{254,217,166}
\definecolor{Pastel1-6-E}{RGB}{254,217,166}
\definecolor{Pastel1-6-6}{RGB}{255,255,204}
\definecolor{Pastel1-6-F}{RGB}{255,255,204}
\definecolor{Pastel1-7-1}{RGB}{251,180,174}
\definecolor{Pastel1-7-A}{RGB}{251,180,174}
\definecolor{Pastel1-7-2}{RGB}{179,205,227}
\definecolor{Pastel1-7-B}{RGB}{179,205,227}
\definecolor{Pastel1-7-3}{RGB}{204,235,197}
\definecolor{Pastel1-7-C}{RGB}{204,235,197}
\definecolor{Pastel1-7-4}{RGB}{222,203,228}
\definecolor{Pastel1-7-D}{RGB}{222,203,228}
\definecolor{Pastel1-7-5}{RGB}{254,217,166}
\definecolor{Pastel1-7-E}{RGB}{254,217,166}
\definecolor{Pastel1-7-6}{RGB}{255,255,204}
\definecolor{Pastel1-7-F}{RGB}{255,255,204}
\definecolor{Pastel1-7-7}{RGB}{229,216,189}
\definecolor{Pastel1-7-G}{RGB}{229,216,189}
\definecolor{Pastel1-8-1}{RGB}{251,180,174}
\definecolor{Pastel1-8-A}{RGB}{251,180,174}
\definecolor{Pastel1-8-2}{RGB}{179,205,227}
\definecolor{Pastel1-8-B}{RGB}{179,205,227}
\definecolor{Pastel1-8-3}{RGB}{204,235,197}
\definecolor{Pastel1-8-C}{RGB}{204,235,197}
\definecolor{Pastel1-8-4}{RGB}{222,203,228}
\definecolor{Pastel1-8-D}{RGB}{222,203,228}
\definecolor{Pastel1-8-5}{RGB}{254,217,166}
\definecolor{Pastel1-8-E}{RGB}{254,217,166}
\definecolor{Pastel1-8-6}{RGB}{255,255,204}
\definecolor{Pastel1-8-F}{RGB}{255,255,204}
\definecolor{Pastel1-8-7}{RGB}{229,216,189}
\definecolor{Pastel1-8-G}{RGB}{229,216,189}
\definecolor{Pastel1-8-8}{RGB}{253,218,236}
\definecolor{Pastel1-8-H}{RGB}{253,218,236}
\definecolor{Pastel1-9-1}{RGB}{251,180,174}
\definecolor{Pastel1-9-A}{RGB}{251,180,174}
\definecolor{Pastel1-9-2}{RGB}{179,205,227}
\definecolor{Pastel1-9-B}{RGB}{179,205,227}
\definecolor{Pastel1-9-3}{RGB}{204,235,197}
\definecolor{Pastel1-9-C}{RGB}{204,235,197}
\definecolor{Pastel1-9-4}{RGB}{222,203,228}
\definecolor{Pastel1-9-D}{RGB}{222,203,228}
\definecolor{Pastel1-9-5}{RGB}{254,217,166}
\definecolor{Pastel1-9-E}{RGB}{254,217,166}
\definecolor{Pastel1-9-6}{RGB}{255,255,204}
\definecolor{Pastel1-9-F}{RGB}{255,255,204}
\definecolor{Pastel1-9-7}{RGB}{229,216,189}
\definecolor{Pastel1-9-G}{RGB}{229,216,189}
\definecolor{Pastel1-9-8}{RGB}{253,218,236}
\definecolor{Pastel1-9-H}{RGB}{253,218,236}
\definecolor{Pastel1-9-9}{RGB}{242,242,242}
\definecolor{Pastel1-9-I}{RGB}{242,242,242}
\definecolor{Set1-3-1}{RGB}{228,26,28}
\definecolor{Set1-3-A}{RGB}{228,26,28}
\definecolor{Set1-3-2}{RGB}{55,126,184}
\definecolor{Set1-3-B}{RGB}{55,126,184}
\definecolor{Set1-3-3}{RGB}{77,175,74}
\definecolor{Set1-3-C}{RGB}{77,175,74}
\definecolor{Set1-4-1}{RGB}{228,26,28}
\definecolor{Set1-4-A}{RGB}{228,26,28}
\definecolor{Set1-4-2}{RGB}{55,126,184}
\definecolor{Set1-4-B}{RGB}{55,126,184}
\definecolor{Set1-4-3}{RGB}{77,175,74}
\definecolor{Set1-4-C}{RGB}{77,175,74}
\definecolor{Set1-4-4}{RGB}{152,78,163}
\definecolor{Set1-4-D}{RGB}{152,78,163}
\definecolor{Set1-5-1}{RGB}{228,26,28}
\definecolor{Set1-5-A}{RGB}{228,26,28}
\definecolor{Set1-5-2}{RGB}{55,126,184}
\definecolor{Set1-5-B}{RGB}{55,126,184}
\definecolor{Set1-5-3}{RGB}{77,175,74}
\definecolor{Set1-5-C}{RGB}{77,175,74}
\definecolor{Set1-5-4}{RGB}{152,78,163}
\definecolor{Set1-5-D}{RGB}{152,78,163}
\definecolor{Set1-5-5}{RGB}{255,127,0}
\definecolor{Set1-5-E}{RGB}{255,127,0}
\definecolor{Set1-6-1}{RGB}{228,26,28}
\definecolor{Set1-6-A}{RGB}{228,26,28}
\definecolor{Set1-6-2}{RGB}{55,126,184}
\definecolor{Set1-6-B}{RGB}{55,126,184}
\definecolor{Set1-6-3}{RGB}{77,175,74}
\definecolor{Set1-6-C}{RGB}{77,175,74}
\definecolor{Set1-6-4}{RGB}{152,78,163}
\definecolor{Set1-6-D}{RGB}{152,78,163}
\definecolor{Set1-6-5}{RGB}{255,127,0}
\definecolor{Set1-6-E}{RGB}{255,127,0}
\definecolor{Set1-6-6}{RGB}{255,255,51}
\definecolor{Set1-6-F}{RGB}{255,255,51}
\definecolor{Set1-7-1}{RGB}{228,26,28}
\definecolor{Set1-7-A}{RGB}{228,26,28}
\definecolor{Set1-7-2}{RGB}{55,126,184}
\definecolor{Set1-7-B}{RGB}{55,126,184}
\definecolor{Set1-7-3}{RGB}{77,175,74}
\definecolor{Set1-7-C}{RGB}{77,175,74}
\definecolor{Set1-7-4}{RGB}{152,78,163}
\definecolor{Set1-7-D}{RGB}{152,78,163}
\definecolor{Set1-7-5}{RGB}{255,127,0}
\definecolor{Set1-7-E}{RGB}{255,127,0}
\definecolor{Set1-7-6}{RGB}{255,255,51}
\definecolor{Set1-7-F}{RGB}{255,255,51}
\definecolor{Set1-7-7}{RGB}{166,86,40}
\definecolor{Set1-7-G}{RGB}{166,86,40}
\definecolor{Set1-8-1}{RGB}{228,26,28}
\definecolor{Set1-8-A}{RGB}{228,26,28}
\definecolor{Set1-8-2}{RGB}{55,126,184}
\definecolor{Set1-8-B}{RGB}{55,126,184}
\definecolor{Set1-8-3}{RGB}{77,175,74}
\definecolor{Set1-8-C}{RGB}{77,175,74}
\definecolor{Set1-8-4}{RGB}{152,78,163}
\definecolor{Set1-8-D}{RGB}{152,78,163}
\definecolor{Set1-8-5}{RGB}{255,127,0}
\definecolor{Set1-8-E}{RGB}{255,127,0}
\definecolor{Set1-8-6}{RGB}{255,255,51}
\definecolor{Set1-8-F}{RGB}{255,255,51}
\definecolor{Set1-8-7}{RGB}{166,86,40}
\definecolor{Set1-8-G}{RGB}{166,86,40}
\definecolor{Set1-8-8}{RGB}{247,129,191}
\definecolor{Set1-8-H}{RGB}{247,129,191}
\definecolor{Set1-9-1}{RGB}{228,26,28}
\definecolor{Set1-9-A}{RGB}{228,26,28}
\definecolor{Set1-9-2}{RGB}{55,126,184}
\definecolor{Set1-9-B}{RGB}{55,126,184}
\definecolor{Set1-9-3}{RGB}{77,175,74}
\definecolor{Set1-9-C}{RGB}{77,175,74}
\definecolor{Set1-9-4}{RGB}{152,78,163}
\definecolor{Set1-9-D}{RGB}{152,78,163}
\definecolor{Set1-9-5}{RGB}{255,127,0}
\definecolor{Set1-9-E}{RGB}{255,127,0}
\definecolor{Set1-9-6}{RGB}{255,255,51}
\definecolor{Set1-9-F}{RGB}{255,255,51}
\definecolor{Set1-9-7}{RGB}{166,86,40}
\definecolor{Set1-9-G}{RGB}{166,86,40}
\definecolor{Set1-9-8}{RGB}{247,129,191}
\definecolor{Set1-9-H}{RGB}{247,129,191}
\definecolor{Set1-9-9}{RGB}{153,153,153}
\definecolor{Set1-9-I}{RGB}{153,153,153}
\definecolor{Pastel2-3-1}{RGB}{179,226,205}
\definecolor{Pastel2-3-A}{RGB}{179,226,205}
\definecolor{Pastel2-3-2}{RGB}{253,205,172}
\definecolor{Pastel2-3-B}{RGB}{253,205,172}
\definecolor{Pastel2-3-3}{RGB}{203,213,232}
\definecolor{Pastel2-3-C}{RGB}{203,213,232}
\definecolor{Pastel2-4-1}{RGB}{179,226,205}
\definecolor{Pastel2-4-A}{RGB}{179,226,205}
\definecolor{Pastel2-4-2}{RGB}{253,205,172}
\definecolor{Pastel2-4-B}{RGB}{253,205,172}
\definecolor{Pastel2-4-3}{RGB}{203,213,232}
\definecolor{Pastel2-4-C}{RGB}{203,213,232}
\definecolor{Pastel2-4-4}{RGB}{244,202,228}
\definecolor{Pastel2-4-D}{RGB}{244,202,228}
\definecolor{Pastel2-5-1}{RGB}{179,226,205}
\definecolor{Pastel2-5-A}{RGB}{179,226,205}
\definecolor{Pastel2-5-2}{RGB}{253,205,172}
\definecolor{Pastel2-5-B}{RGB}{253,205,172}
\definecolor{Pastel2-5-3}{RGB}{203,213,232}
\definecolor{Pastel2-5-C}{RGB}{203,213,232}
\definecolor{Pastel2-5-4}{RGB}{244,202,228}
\definecolor{Pastel2-5-D}{RGB}{244,202,228}
\definecolor{Pastel2-5-5}{RGB}{230,245,201}
\definecolor{Pastel2-5-E}{RGB}{230,245,201}
\definecolor{Pastel2-6-1}{RGB}{179,226,205}
\definecolor{Pastel2-6-A}{RGB}{179,226,205}
\definecolor{Pastel2-6-2}{RGB}{253,205,172}
\definecolor{Pastel2-6-B}{RGB}{253,205,172}
\definecolor{Pastel2-6-3}{RGB}{203,213,232}
\definecolor{Pastel2-6-C}{RGB}{203,213,232}
\definecolor{Pastel2-6-4}{RGB}{244,202,228}
\definecolor{Pastel2-6-D}{RGB}{244,202,228}
\definecolor{Pastel2-6-5}{RGB}{230,245,201}
\definecolor{Pastel2-6-E}{RGB}{230,245,201}
\definecolor{Pastel2-6-6}{RGB}{255,242,174}
\definecolor{Pastel2-6-F}{RGB}{255,242,174}
\definecolor{Pastel2-7-1}{RGB}{179,226,205}
\definecolor{Pastel2-7-A}{RGB}{179,226,205}
\definecolor{Pastel2-7-2}{RGB}{253,205,172}
\definecolor{Pastel2-7-B}{RGB}{253,205,172}
\definecolor{Pastel2-7-3}{RGB}{203,213,232}
\definecolor{Pastel2-7-C}{RGB}{203,213,232}
\definecolor{Pastel2-7-4}{RGB}{244,202,228}
\definecolor{Pastel2-7-D}{RGB}{244,202,228}
\definecolor{Pastel2-7-5}{RGB}{230,245,201}
\definecolor{Pastel2-7-E}{RGB}{230,245,201}
\definecolor{Pastel2-7-6}{RGB}{255,242,174}
\definecolor{Pastel2-7-F}{RGB}{255,242,174}
\definecolor{Pastel2-7-7}{RGB}{241,226,204}
\definecolor{Pastel2-7-G}{RGB}{241,226,204}
\definecolor{Pastel2-8-1}{RGB}{179,226,205}
\definecolor{Pastel2-8-A}{RGB}{179,226,205}
\definecolor{Pastel2-8-2}{RGB}{253,205,172}
\definecolor{Pastel2-8-B}{RGB}{253,205,172}
\definecolor{Pastel2-8-3}{RGB}{203,213,232}
\definecolor{Pastel2-8-C}{RGB}{203,213,232}
\definecolor{Pastel2-8-4}{RGB}{244,202,228}
\definecolor{Pastel2-8-D}{RGB}{244,202,228}
\definecolor{Pastel2-8-5}{RGB}{230,245,201}
\definecolor{Pastel2-8-E}{RGB}{230,245,201}
\definecolor{Pastel2-8-6}{RGB}{255,242,174}
\definecolor{Pastel2-8-F}{RGB}{255,242,174}
\definecolor{Pastel2-8-7}{RGB}{241,226,204}
\definecolor{Pastel2-8-G}{RGB}{241,226,204}
\definecolor{Pastel2-8-8}{RGB}{204,204,204}
\definecolor{Pastel2-8-H}{RGB}{204,204,204}
\definecolor{Set2-3-1}{RGB}{102,194,165}
\definecolor{Set2-3-A}{RGB}{102,194,165}
\definecolor{Set2-3-2}{RGB}{252,141,98}
\definecolor{Set2-3-B}{RGB}{252,141,98}
\definecolor{Set2-3-3}{RGB}{141,160,203}
\definecolor{Set2-3-C}{RGB}{141,160,203}
\definecolor{Set2-4-1}{RGB}{102,194,165}
\definecolor{Set2-4-A}{RGB}{102,194,165}
\definecolor{Set2-4-2}{RGB}{252,141,98}
\definecolor{Set2-4-B}{RGB}{252,141,98}
\definecolor{Set2-4-3}{RGB}{141,160,203}
\definecolor{Set2-4-C}{RGB}{141,160,203}
\definecolor{Set2-4-4}{RGB}{231,138,195}
\definecolor{Set2-4-D}{RGB}{231,138,195}
\definecolor{Set2-5-1}{RGB}{102,194,165}
\definecolor{Set2-5-A}{RGB}{102,194,165}
\definecolor{Set2-5-2}{RGB}{252,141,98}
\definecolor{Set2-5-B}{RGB}{252,141,98}
\definecolor{Set2-5-3}{RGB}{141,160,203}
\definecolor{Set2-5-C}{RGB}{141,160,203}
\definecolor{Set2-5-4}{RGB}{231,138,195}
\definecolor{Set2-5-D}{RGB}{231,138,195}
\definecolor{Set2-5-5}{RGB}{166,216,84}
\definecolor{Set2-5-E}{RGB}{166,216,84}
\definecolor{Set2-6-1}{RGB}{102,194,165}
\definecolor{Set2-6-A}{RGB}{102,194,165}
\definecolor{Set2-6-2}{RGB}{252,141,98}
\definecolor{Set2-6-B}{RGB}{252,141,98}
\definecolor{Set2-6-3}{RGB}{141,160,203}
\definecolor{Set2-6-C}{RGB}{141,160,203}
\definecolor{Set2-6-4}{RGB}{231,138,195}
\definecolor{Set2-6-D}{RGB}{231,138,195}
\definecolor{Set2-6-5}{RGB}{166,216,84}
\definecolor{Set2-6-E}{RGB}{166,216,84}
\definecolor{Set2-6-6}{RGB}{255,217,47}
\definecolor{Set2-6-F}{RGB}{255,217,47}
\definecolor{Set2-7-1}{RGB}{102,194,165}
\definecolor{Set2-7-A}{RGB}{102,194,165}
\definecolor{Set2-7-2}{RGB}{252,141,98}
\definecolor{Set2-7-B}{RGB}{252,141,98}
\definecolor{Set2-7-3}{RGB}{141,160,203}
\definecolor{Set2-7-C}{RGB}{141,160,203}
\definecolor{Set2-7-4}{RGB}{231,138,195}
\definecolor{Set2-7-D}{RGB}{231,138,195}
\definecolor{Set2-7-5}{RGB}{166,216,84}
\definecolor{Set2-7-E}{RGB}{166,216,84}
\definecolor{Set2-7-6}{RGB}{255,217,47}
\definecolor{Set2-7-F}{RGB}{255,217,47}
\definecolor{Set2-7-7}{RGB}{229,196,148}
\definecolor{Set2-7-G}{RGB}{229,196,148}
\definecolor{Set2-8-1}{RGB}{102,194,165}
\definecolor{Set2-8-A}{RGB}{102,194,165}
\definecolor{Set2-8-2}{RGB}{252,141,98}
\definecolor{Set2-8-B}{RGB}{252,141,98}
\definecolor{Set2-8-3}{RGB}{141,160,203}
\definecolor{Set2-8-C}{RGB}{141,160,203}
\definecolor{Set2-8-4}{RGB}{231,138,195}
\definecolor{Set2-8-D}{RGB}{231,138,195}
\definecolor{Set2-8-5}{RGB}{166,216,84}
\definecolor{Set2-8-E}{RGB}{166,216,84}
\definecolor{Set2-8-6}{RGB}{255,217,47}
\definecolor{Set2-8-F}{RGB}{255,217,47}
\definecolor{Set2-8-7}{RGB}{229,196,148}
\definecolor{Set2-8-G}{RGB}{229,196,148}
\definecolor{Set2-8-8}{RGB}{179,179,179}
\definecolor{Set2-8-H}{RGB}{179,179,179}
\definecolor{Dark2-3-1}{RGB}{27,158,119}
\definecolor{Dark2-3-A}{RGB}{27,158,119}
\definecolor{Dark2-3-2}{RGB}{217,95,2}
\definecolor{Dark2-3-B}{RGB}{217,95,2}
\definecolor{Dark2-3-3}{RGB}{117,112,179}
\definecolor{Dark2-3-C}{RGB}{117,112,179}
\definecolor{Dark2-4-1}{RGB}{27,158,119}
\definecolor{Dark2-4-A}{RGB}{27,158,119}
\definecolor{Dark2-4-2}{RGB}{217,95,2}
\definecolor{Dark2-4-B}{RGB}{217,95,2}
\definecolor{Dark2-4-3}{RGB}{117,112,179}
\definecolor{Dark2-4-C}{RGB}{117,112,179}
\definecolor{Dark2-4-4}{RGB}{231,41,138}
\definecolor{Dark2-4-D}{RGB}{231,41,138}
\definecolor{Dark2-5-1}{RGB}{27,158,119}
\definecolor{Dark2-5-A}{RGB}{27,158,119}
\definecolor{Dark2-5-2}{RGB}{217,95,2}
\definecolor{Dark2-5-B}{RGB}{217,95,2}
\definecolor{Dark2-5-3}{RGB}{117,112,179}
\definecolor{Dark2-5-C}{RGB}{117,112,179}
\definecolor{Dark2-5-4}{RGB}{231,41,138}
\definecolor{Dark2-5-D}{RGB}{231,41,138}
\definecolor{Dark2-5-5}{RGB}{102,166,30}
\definecolor{Dark2-5-E}{RGB}{102,166,30}
\definecolor{Dark2-6-1}{RGB}{27,158,119}
\definecolor{Dark2-6-A}{RGB}{27,158,119}
\definecolor{Dark2-6-2}{RGB}{217,95,2}
\definecolor{Dark2-6-B}{RGB}{217,95,2}
\definecolor{Dark2-6-3}{RGB}{117,112,179}
\definecolor{Dark2-6-C}{RGB}{117,112,179}
\definecolor{Dark2-6-4}{RGB}{231,41,138}
\definecolor{Dark2-6-D}{RGB}{231,41,138}
\definecolor{Dark2-6-5}{RGB}{102,166,30}
\definecolor{Dark2-6-E}{RGB}{102,166,30}
\definecolor{Dark2-6-6}{RGB}{230,171,2}
\definecolor{Dark2-6-F}{RGB}{230,171,2}
\definecolor{Dark2-7-1}{RGB}{27,158,119}
\definecolor{Dark2-7-A}{RGB}{27,158,119}
\definecolor{Dark2-7-2}{RGB}{217,95,2}
\definecolor{Dark2-7-B}{RGB}{217,95,2}
\definecolor{Dark2-7-3}{RGB}{117,112,179}
\definecolor{Dark2-7-C}{RGB}{117,112,179}
\definecolor{Dark2-7-4}{RGB}{231,41,138}
\definecolor{Dark2-7-D}{RGB}{231,41,138}
\definecolor{Dark2-7-5}{RGB}{102,166,30}
\definecolor{Dark2-7-E}{RGB}{102,166,30}
\definecolor{Dark2-7-6}{RGB}{230,171,2}
\definecolor{Dark2-7-F}{RGB}{230,171,2}
\definecolor{Dark2-7-7}{RGB}{166,118,29}
\definecolor{Dark2-7-G}{RGB}{166,118,29}
\definecolor{Dark2-8-1}{RGB}{27,158,119}
\definecolor{Dark2-8-A}{RGB}{27,158,119}
\definecolor{Dark2-8-2}{RGB}{217,95,2}
\definecolor{Dark2-8-B}{RGB}{217,95,2}
\definecolor{Dark2-8-3}{RGB}{117,112,179}
\definecolor{Dark2-8-C}{RGB}{117,112,179}
\definecolor{Dark2-8-4}{RGB}{231,41,138}
\definecolor{Dark2-8-D}{RGB}{231,41,138}
\definecolor{Dark2-8-5}{RGB}{102,166,30}
\definecolor{Dark2-8-E}{RGB}{102,166,30}
\definecolor{Dark2-8-6}{RGB}{230,171,2}
\definecolor{Dark2-8-F}{RGB}{230,171,2}
\definecolor{Dark2-8-7}{RGB}{166,118,29}
\definecolor{Dark2-8-G}{RGB}{166,118,29}
\definecolor{Dark2-8-8}{RGB}{102,102,102}
\definecolor{Dark2-8-H}{RGB}{102,102,102}
\definecolor{Paired-3-1}{RGB}{166,206,227}
\definecolor{Paired-3-A}{RGB}{166,206,227}
\definecolor{Paired-3-2}{RGB}{31,120,180}
\definecolor{Paired-3-B}{RGB}{31,120,180}
\definecolor{Paired-3-3}{RGB}{178,223,138}
\definecolor{Paired-3-C}{RGB}{178,223,138}
\definecolor{Paired-4-1}{RGB}{166,206,227}
\definecolor{Paired-4-A}{RGB}{166,206,227}
\definecolor{Paired-4-2}{RGB}{31,120,180}
\definecolor{Paired-4-B}{RGB}{31,120,180}
\definecolor{Paired-4-3}{RGB}{178,223,138}
\definecolor{Paired-4-C}{RGB}{178,223,138}
\definecolor{Paired-4-4}{RGB}{51,160,44}
\definecolor{Paired-4-D}{RGB}{51,160,44}
\definecolor{Paired-5-1}{RGB}{166,206,227}
\definecolor{Paired-5-A}{RGB}{166,206,227}
\definecolor{Paired-5-2}{RGB}{31,120,180}
\definecolor{Paired-5-B}{RGB}{31,120,180}
\definecolor{Paired-5-3}{RGB}{178,223,138}
\definecolor{Paired-5-C}{RGB}{178,223,138}
\definecolor{Paired-5-4}{RGB}{51,160,44}
\definecolor{Paired-5-D}{RGB}{51,160,44}
\definecolor{Paired-5-5}{RGB}{251,154,153}
\definecolor{Paired-5-E}{RGB}{251,154,153}
\definecolor{Paired-6-1}{RGB}{166,206,227}
\definecolor{Paired-6-A}{RGB}{166,206,227}
\definecolor{Paired-6-2}{RGB}{31,120,180}
\definecolor{Paired-6-B}{RGB}{31,120,180}
\definecolor{Paired-6-3}{RGB}{178,223,138}
\definecolor{Paired-6-C}{RGB}{178,223,138}
\definecolor{Paired-6-4}{RGB}{51,160,44}
\definecolor{Paired-6-D}{RGB}{51,160,44}
\definecolor{Paired-6-5}{RGB}{251,154,153}
\definecolor{Paired-6-E}{RGB}{251,154,153}
\definecolor{Paired-6-6}{RGB}{227,26,28}
\definecolor{Paired-6-F}{RGB}{227,26,28}
\definecolor{Paired-7-1}{RGB}{166,206,227}
\definecolor{Paired-7-A}{RGB}{166,206,227}
\definecolor{Paired-7-2}{RGB}{31,120,180}
\definecolor{Paired-7-B}{RGB}{31,120,180}
\definecolor{Paired-7-3}{RGB}{178,223,138}
\definecolor{Paired-7-C}{RGB}{178,223,138}
\definecolor{Paired-7-4}{RGB}{51,160,44}
\definecolor{Paired-7-D}{RGB}{51,160,44}
\definecolor{Paired-7-5}{RGB}{251,154,153}
\definecolor{Paired-7-E}{RGB}{251,154,153}
\definecolor{Paired-7-6}{RGB}{227,26,28}
\definecolor{Paired-7-F}{RGB}{227,26,28}
\definecolor{Paired-7-7}{RGB}{253,191,111}
\definecolor{Paired-7-G}{RGB}{253,191,111}
\definecolor{Paired-8-1}{RGB}{166,206,227}
\definecolor{Paired-8-A}{RGB}{166,206,227}
\definecolor{Paired-8-2}{RGB}{31,120,180}
\definecolor{Paired-8-B}{RGB}{31,120,180}
\definecolor{Paired-8-3}{RGB}{178,223,138}
\definecolor{Paired-8-C}{RGB}{178,223,138}
\definecolor{Paired-8-4}{RGB}{51,160,44}
\definecolor{Paired-8-D}{RGB}{51,160,44}
\definecolor{Paired-8-5}{RGB}{251,154,153}
\definecolor{Paired-8-E}{RGB}{251,154,153}
\definecolor{Paired-8-6}{RGB}{227,26,28}
\definecolor{Paired-8-F}{RGB}{227,26,28}
\definecolor{Paired-8-7}{RGB}{253,191,111}
\definecolor{Paired-8-G}{RGB}{253,191,111}
\definecolor{Paired-8-8}{RGB}{255,127,0}
\definecolor{Paired-8-H}{RGB}{255,127,0}
\definecolor{Paired-9-1}{RGB}{166,206,227}
\definecolor{Paired-9-A}{RGB}{166,206,227}
\definecolor{Paired-9-2}{RGB}{31,120,180}
\definecolor{Paired-9-B}{RGB}{31,120,180}
\definecolor{Paired-9-3}{RGB}{178,223,138}
\definecolor{Paired-9-C}{RGB}{178,223,138}
\definecolor{Paired-9-4}{RGB}{51,160,44}
\definecolor{Paired-9-D}{RGB}{51,160,44}
\definecolor{Paired-9-5}{RGB}{251,154,153}
\definecolor{Paired-9-E}{RGB}{251,154,153}
\definecolor{Paired-9-6}{RGB}{227,26,28}
\definecolor{Paired-9-F}{RGB}{227,26,28}
\definecolor{Paired-9-7}{RGB}{253,191,111}
\definecolor{Paired-9-G}{RGB}{253,191,111}
\definecolor{Paired-9-8}{RGB}{255,127,0}
\definecolor{Paired-9-H}{RGB}{255,127,0}
\definecolor{Paired-9-9}{RGB}{202,178,214}
\definecolor{Paired-9-I}{RGB}{202,178,214}
\definecolor{Paired-10-1}{RGB}{166,206,227}
\definecolor{Paired-10-A}{RGB}{166,206,227}
\definecolor{Paired-10-2}{RGB}{31,120,180}
\definecolor{Paired-10-B}{RGB}{31,120,180}
\definecolor{Paired-10-3}{RGB}{178,223,138}
\definecolor{Paired-10-C}{RGB}{178,223,138}
\definecolor{Paired-10-4}{RGB}{51,160,44}
\definecolor{Paired-10-D}{RGB}{51,160,44}
\definecolor{Paired-10-5}{RGB}{251,154,153}
\definecolor{Paired-10-E}{RGB}{251,154,153}
\definecolor{Paired-10-6}{RGB}{227,26,28}
\definecolor{Paired-10-F}{RGB}{227,26,28}
\definecolor{Paired-10-7}{RGB}{253,191,111}
\definecolor{Paired-10-G}{RGB}{253,191,111}
\definecolor{Paired-10-8}{RGB}{255,127,0}
\definecolor{Paired-10-H}{RGB}{255,127,0}
\definecolor{Paired-10-9}{RGB}{202,178,214}
\definecolor{Paired-10-I}{RGB}{202,178,214}
\definecolor{Paired-10-10}{RGB}{106,61,154}
\definecolor{Paired-10-J}{RGB}{106,61,154}
\definecolor{Paired-11-1}{RGB}{166,206,227}
\definecolor{Paired-11-A}{RGB}{166,206,227}
\definecolor{Paired-11-2}{RGB}{31,120,180}
\definecolor{Paired-11-B}{RGB}{31,120,180}
\definecolor{Paired-11-3}{RGB}{178,223,138}
\definecolor{Paired-11-C}{RGB}{178,223,138}
\definecolor{Paired-11-4}{RGB}{51,160,44}
\definecolor{Paired-11-D}{RGB}{51,160,44}
\definecolor{Paired-11-5}{RGB}{251,154,153}
\definecolor{Paired-11-E}{RGB}{251,154,153}
\definecolor{Paired-11-6}{RGB}{227,26,28}
\definecolor{Paired-11-F}{RGB}{227,26,28}
\definecolor{Paired-11-7}{RGB}{253,191,111}
\definecolor{Paired-11-G}{RGB}{253,191,111}
\definecolor{Paired-11-8}{RGB}{255,127,0}
\definecolor{Paired-11-H}{RGB}{255,127,0}
\definecolor{Paired-11-9}{RGB}{202,178,214}
\definecolor{Paired-11-I}{RGB}{202,178,214}
\definecolor{Paired-11-10}{RGB}{106,61,154}
\definecolor{Paired-11-J}{RGB}{106,61,154}
\definecolor{Paired-11-11}{RGB}{255,255,153}
\definecolor{Paired-11-K}{RGB}{255,255,153}
\definecolor{Paired-12-1}{RGB}{166,206,227}
\definecolor{Paired-12-A}{RGB}{166,206,227}
\definecolor{Paired-12-2}{RGB}{31,120,180}
\definecolor{Paired-12-B}{RGB}{31,120,180}
\definecolor{Paired-12-3}{RGB}{178,223,138}
\definecolor{Paired-12-C}{RGB}{178,223,138}
\definecolor{Paired-12-4}{RGB}{51,160,44}
\definecolor{Paired-12-D}{RGB}{51,160,44}
\definecolor{Paired-12-5}{RGB}{251,154,153}
\definecolor{Paired-12-E}{RGB}{251,154,153}
\definecolor{Paired-12-6}{RGB}{227,26,28}
\definecolor{Paired-12-F}{RGB}{227,26,28}
\definecolor{Paired-12-7}{RGB}{253,191,111}
\definecolor{Paired-12-G}{RGB}{253,191,111}
\definecolor{Paired-12-8}{RGB}{255,127,0}
\definecolor{Paired-12-H}{RGB}{255,127,0}
\definecolor{Paired-12-9}{RGB}{202,178,214}
\definecolor{Paired-12-I}{RGB}{202,178,214}
\definecolor{Paired-12-10}{RGB}{106,61,154}
\definecolor{Paired-12-J}{RGB}{106,61,154}
\definecolor{Paired-12-11}{RGB}{255,255,153}
\definecolor{Paired-12-K}{RGB}{255,255,153}
\definecolor{Paired-12-12}{RGB}{177,89,40}
\definecolor{Paired-12-L}{RGB}{177,89,40}
\definecolor{Accent-3-1}{RGB}{127,201,127}
\definecolor{Accent-3-A}{RGB}{127,201,127}
\definecolor{Accent-3-2}{RGB}{190,174,212}
\definecolor{Accent-3-B}{RGB}{190,174,212}
\definecolor{Accent-3-3}{RGB}{253,192,134}
\definecolor{Accent-3-C}{RGB}{253,192,134}
\definecolor{Accent-4-1}{RGB}{127,201,127}
\definecolor{Accent-4-A}{RGB}{127,201,127}
\definecolor{Accent-4-2}{RGB}{190,174,212}
\definecolor{Accent-4-B}{RGB}{190,174,212}
\definecolor{Accent-4-3}{RGB}{253,192,134}
\definecolor{Accent-4-C}{RGB}{253,192,134}
\definecolor{Accent-4-4}{RGB}{255,255,153}
\definecolor{Accent-4-D}{RGB}{255,255,153}
\definecolor{Accent-5-1}{RGB}{127,201,127}
\definecolor{Accent-5-A}{RGB}{127,201,127}
\definecolor{Accent-5-2}{RGB}{190,174,212}
\definecolor{Accent-5-B}{RGB}{190,174,212}
\definecolor{Accent-5-3}{RGB}{253,192,134}
\definecolor{Accent-5-C}{RGB}{253,192,134}
\definecolor{Accent-5-4}{RGB}{255,255,153}
\definecolor{Accent-5-D}{RGB}{255,255,153}
\definecolor{Accent-5-5}{RGB}{56,108,176}
\definecolor{Accent-5-E}{RGB}{56,108,176}
\definecolor{Accent-6-1}{RGB}{127,201,127}
\definecolor{Accent-6-A}{RGB}{127,201,127}
\definecolor{Accent-6-2}{RGB}{190,174,212}
\definecolor{Accent-6-B}{RGB}{190,174,212}
\definecolor{Accent-6-3}{RGB}{253,192,134}
\definecolor{Accent-6-C}{RGB}{253,192,134}
\definecolor{Accent-6-4}{RGB}{255,255,153}
\definecolor{Accent-6-D}{RGB}{255,255,153}
\definecolor{Accent-6-5}{RGB}{56,108,176}
\definecolor{Accent-6-E}{RGB}{56,108,176}
\definecolor{Accent-6-6}{RGB}{240,2,127}
\definecolor{Accent-6-F}{RGB}{240,2,127}
\definecolor{Accent-7-1}{RGB}{127,201,127}
\definecolor{Accent-7-A}{RGB}{127,201,127}
\definecolor{Accent-7-2}{RGB}{190,174,212}
\definecolor{Accent-7-B}{RGB}{190,174,212}
\definecolor{Accent-7-3}{RGB}{253,192,134}
\definecolor{Accent-7-C}{RGB}{253,192,134}
\definecolor{Accent-7-4}{RGB}{255,255,153}
\definecolor{Accent-7-D}{RGB}{255,255,153}
\definecolor{Accent-7-5}{RGB}{56,108,176}
\definecolor{Accent-7-E}{RGB}{56,108,176}
\definecolor{Accent-7-6}{RGB}{240,2,127}
\definecolor{Accent-7-F}{RGB}{240,2,127}
\definecolor{Accent-7-7}{RGB}{191,91,23}
\definecolor{Accent-7-G}{RGB}{191,91,23}
\definecolor{Accent-8-1}{RGB}{127,201,127}
\definecolor{Accent-8-A}{RGB}{127,201,127}
\definecolor{Accent-8-2}{RGB}{190,174,212}
\definecolor{Accent-8-B}{RGB}{190,174,212}
\definecolor{Accent-8-3}{RGB}{253,192,134}
\definecolor{Accent-8-C}{RGB}{253,192,134}
\definecolor{Accent-8-4}{RGB}{255,255,153}
\definecolor{Accent-8-D}{RGB}{255,255,153}
\definecolor{Accent-8-5}{RGB}{56,108,176}
\definecolor{Accent-8-E}{RGB}{56,108,176}
\definecolor{Accent-8-6}{RGB}{240,2,127}
\definecolor{Accent-8-F}{RGB}{240,2,127}
\definecolor{Accent-8-7}{RGB}{191,91,23}
\definecolor{Accent-8-G}{RGB}{191,91,23}
\definecolor{Accent-8-8}{RGB}{102,102,102}
\definecolor{Accent-8-H}{RGB}{102,102,102}

